Transformers Can Solve Non-Linear and Non-Markovian Filtering Problems in Continuous Time For Conditionally Gaussian Signals

The use of attention-based deep learning models in stochastic filtering, e.g. transformers and deep Kalman filters, has recently come into focus; however, the potential for these models to solve stochastic filtering problems remains largely unknown. The paper provides an affirmative answer to this open problem in the theoretical foundations of machine learning by showing that a class of continuous-time transformer models, called \textit{filterformers}, can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-time (possibly non-Gaussian) measurements. Our approximation guarantees hold uniformly over sufficiently regular compact subsets of continuous-time paths, where the worst-case 2-Wasserstein distance between the true optimal filter and our deep learning model quantifies the approximation error. Our construction relies on two new customizations of the standard attention mechanism: The first can losslessly adapt to the characteristics of a broad range of paths since we show that the attention mechanism implements bi-Lipschitz embeddings of sufficiently regular sets of paths into low-dimensional Euclidean spaces; thus, it incurs no ``dimension reduction error''. The latter attention mechanism is tailored to the geometry of Gaussian measures in the $2$-Wasserstein space. Our analysis relies on new stability estimates of robust optimal filters in the conditionally Gaussian setting.

==> OLD/Cover_Letter/AAP_Submission__Version.tex <==
% % https://mcmaster.zoom.us/j/2601491351
% \documentclass[aap]{imsart}

% %% Packages
% \RequirePackage{amsthm,amsmath,amsfonts,amssymb}
% \RequirePackage[numbers,sort&compress]{natbib}
% %\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
% \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
% \RequirePackage{graphicx}

% \startlocaldefs

% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% % \documentclass[preprint,12pt,authoryear]{elsarticle}
% % \usepackage{amssymb}
% % \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}



% \begin{document}



% % AAP
% \begin{frontmatter}
% \title{Deep Kalman Filters Can Filter}

% \begin{aug}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Only one address is permitted per author. %%
% %% Only division, organization and e-mail is %%
% %% included in the address.                  %%
% %% Additional information can be included in %%
% %% the Acknowledgments section if necessary. %%
% %% ORCID can be inserted by command:         %%
% %% \orcid{0000-0000-0000-0000}               %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % \author[inst1]{Matheus Grasselli}
% \author[A,D]{\fnms{Blanka}~\snm{Hovarth}\ead[label=e1]{horvath@maths.ox.ac.uk}},
% \author[B,C]{\fnms{Anastasis}~\snm{Kratsios}\ead[label=e2]{kratsioa@mcmaster.ca}},%\orcid{0000-0000-0000-0000}}
% \author[A,D]{\fnms{Yannick}~\snm{Limmer}\ead[label=e3]{limmery@maths.ox.ac.uk}},
% \author[B]{\fnms{Xuwei}~\snm{Yang}\ead[label=e4]{yangx212@mcmaster.ca}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Addresses                                %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \address[A]{Department of Mathematics,
% University of Oxford \printead[presep={,\ }]{e1}\printead[presep={,\ }]{e3}}
% \address[D]{Oxford Man Institute for Quantitative Finance, University of Oxford}
% \address[B]{Department of Mathematics,
% McMaster University\printead[presep={,\ }]{e2}\printead[presep={,\ }]{e4}}
% \address[C]{Vector Institute}
% % Elseview
% % \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
% %             % addressline={Hamilton, Ontario}, 
% %             city={Hamilton},
% %             % postcode={00000}, 
% %             % state={Ontario},
% %             country={Canada}}

% % \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
% %             % addressline={Address Two}, 
% %             city={Oxford},
% %             % postcode={22222}, 
% %             % state={Oxfordshire},
% %             country={United Kingdom}}

% % \affiliation[inst3]{organization={Oxford-MAN Instute for Quantitative Finance, University of Oxford},
% %             % addressline={Address Two}, 
% %             city={Oxford},
% %             % postcode={22222}, 
% %             % state={Oxfordshire},
% %             country={United Kingdom}}
            
% % \affiliation[inst4]{organization={Vector Institute},
% %             % addressline={Address Two}, 
% %             city={Toronto},
% %             % postcode={22222}, 
% %             % state={Ontario},
% %             country={Canada}}
% \end{aug}

% \begin{abstract}
% Deep Kalman filters (DKFs) are a class of neural network models that generate Gaussian probability measures from sequential data.  Though DKFs are inspired by the Kalman filter, they lack concrete theoretical ties to the stochastic filtering problem, thus limiting their applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-times measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  
% \end{abstract}


% % \begin{keyword}
% % %% keywords here, in the form: keyword \sep keyword
% % Stochastic Filtering \sep Conditionally Gaussian Processes \sep Geometric Deep Learning
% % %% PACS codes here, in the form: \PACS code \sep code
% % % \PACS 0000 \sep 1111
% % %% MSC codes here, in the form: \MSC code \sep code
% % %% or \MSC[2008] code \sep code (2000 is the default)
% % \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% % \end{keyword}

% \begin{keyword}[class=MSC]
% \kwd[Primary ]{62M20}
% \kwd{62M45}
% \kwd[; secondary ]{93E11}
% \end{keyword}

% \begin{keyword}
% \kwd{Robust Filtering}
% \kwd{Deep Kalman Filtering}
% \kwd{Partial Information}
% \end{keyword}

% \end{frontmatter}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Please use \tableofcontents for articles %%
% %% with 50 pages and more                   %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\tableofcontents
% % \end{frontmatter}


% \section{Introduction}
% \label{s:Introduction_Deep_Filtering}

% % \byyan{Opening.}\hfill\\
% In several scientific problems, e.g. in mathematical finance, one is interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$. Here both of the processes are often assumed to have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0:T]},\mathbb{P})$.  For example, market sentiment(signal) impacts market prices(observations), however, only the latter of these two can be directly measured.  The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is to identify a continuous function $f_t:C([0:t],\mathbb{R}^{d_Y})\rightarrow \mathcal{P}(\mathbb{R}^{d_X})$, with $d_X, d_Y \in \N$ for $t>0$, satisfying 
% \begin{align}
%     \label{goal:Robust_Filtering}
%         f_t(Y_{[0:t]})
%     =
%         \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)
%     ,
% \end{align}
% where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $d_X$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0:t]}$. The key innovation in \eqref{goal:Robust_Filtering} is the continuity, and the uniqueness, of $f_t$.  In contrast, a Borel $f_t$ satisfying \eqref{goal:Robust_Filtering} exists by elementary measure-theoretic \citep[Theorem 6.3]{Kallenberg_2021__FoundationsOfModernProbability}. 
% The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^{d_X}$, denoted by $\mathcal{P}(\mathbb{R}^{d_X})$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^{d_Y}$, denoted by $C([0:t],\mathbb{R}^{d_Y})$, with the uniform norm.

% % \byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
% When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^{d_Y})$.  These robust representations are particularly invaluable in mathematical finance, where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

% % \byyan{Do Optimal Filters Exist?.}\hfill\\
% In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued path-dependent processes, make the problem computationally intractable. 

% % \byyan{Computational Challenges}\hfill\\
% The exception to this rule is so-called finite-dimensional filters. These encapsulate rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

% % \byyan{Numerical Approaches.}\hfill\\
% The computational intractability of the general filtering problem leads to the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} where it can be tracked using finitely parameterized representations.  The latter two approaches work well if the coupled system $(X_{\cdot},Y_{\cdot})$ follows the postulated affine dynamics, and the former particle-filtering approach is well-suited to low-dimensional settings. Nevertheless, one would like to have access to (approximate) optimal finite dimensionaly filters for a broader range of situations.    

% % \byyan{Why Deep Learning?.}\hfill\\
% One possibility could be via deep learning, since deep neural networks have demonstrated that they can efficiently solve a variety of previously intractable numerical problems. The expressivity of neural networks on classical learning problems has inspired the use of deep learning approaches to the numerical stochastic filtering problems; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering}, and the development of measure-valued deep learning models; e.g.~\cite{Acciaio2022_GHT}.  At the forefront of these methods, are the class of deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, these are the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered models are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem \eqref{goal:Robust_Filtering}. 

% This paper constructs a DKF model which can uniformly approximate the map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering}, to arbitrary precision, for any pair of non-Markovian $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0:T]}$-adapted \textit{conditionally Gaussian} stochastic processes studied by \cite{LipShiryaev_II_2001}.  
% %%%%
% %%%%
% %%%%
% \begin{InformalTheorem}[The DKF is a Universal Conditionally-Gaussian Robust Filter]
% \label{Informal_Theorem_Main:Informal_Theorem}
% Let $(X_{\cdot},Y_{\cdot})$ be the partially-observed system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} below, subject to mild regularity conditions.  For any suitable compact subset $K\subseteq C([0:T],\mathbb{R}^{d_Y})$, every $T>0$, and any approximation error $\varepsilon>0$ there exists a DKF model $\hat{F}:[0:T]\times C([0:T]\times\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ satisfying the uniform estimate
% \[
%     \max_{0\le t\le T,\,y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})
%             ,
%                 \hat{F}(t,y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.
% \end{InformalTheorem}
% %%%%
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=.4\linewidth]{Graphics/Mask.pdf}
%     \caption{The DKF model in Informal Theorem~\ref{Informal_Theorem_Main:Informal_Theorem} has two inputs: a time $t$ and a continuous path $y_{\cdot}$ defined up to some time $T\ge t$.  The first parameter $t$ acts as a mask hiding the future evolution of the observation (input) path $y_{\cdot}$ beyond the current time $t$.  We note that there is no loss of generality in assuming that the path $y_{\cdot}$ is defined up to time $T$, since any path can be trivially extended beyond the current time $t$ by setting $y_{s}=y_t$ for all $s\in [t,T]$; e.g.\ as in the Functional It\^{o} Calculus \cite{MR3939653,MR2782350,MR3059194}.
%     \\
%     The mask, i.e.\ the parameter $t$, fills the same analogous role to recursions in classical stochastic filters.  That is, by varying the time parameter $t$, the prediction of the DKFs evolves into the future without having to retrain the DKF model.}
%     \label{fig:Mask}
% \end{figure}
% %%%%
% Our uniform estimates hold for coupled stochastic differential equations governed by
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% % \tag{Sig}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% % \tag{Obs}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $\smash{([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})}$, and where $\smash{\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))}$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
% We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $\smash{W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}}$ and $\smash{W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}}$, of respective dimensions $d_X$ and $d_Y$, for positive integers $d_X$ and $d_Y$. The requirements for the dynamics \labelcref{eq:filtering_dynamics__signal,eq:filtering_dynamics__observation} are detailed in \Cref{ass:technical_evolution_conditions} below.

% \subsection{The Deep Kalman Filter Model}
% \label{s:Introduction_Deep_Filtering__ss:ModelDetails}
% The proposed deep Kalman filter (DKF), illustrated in \Cref{fig:DKFModel}, generates predictions on the finite-dimensional metric space $(\mathcal{N}_{d_X},\mathcal{W}_2)$ whose points are non-singular Gaussian measures, and whose distance between points is quantified by the $2$-Wasserstein distance.  These predictions are generated from the continuous input paths via the following three-phase process.  
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
%     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
%     \label{fig:DKFModel}
% \end{figure}

% \begin{enumerate}[label=\emph{Phase \arabic*}.]
%     \item The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly, our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^{d_Y})$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifold.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is is devoid of any projection onto a finite-dimensional (Schauder) basis, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.
    
%     \item In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
    
%     \item In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_{d_X}$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{goal:Robust_Filtering}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.
% \end{enumerate}


% \subsection{Organization of Paper}
% \Cref{s:Setting} formalizes the basic required regularity conditions on the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} and it overviews any background material.  \Cref{s:Model} rigorously introduces the relevant DKF model.  \Cref{s:Main_Results} contains the paper's main theoretical results, as well as an overview of the proof methodology.  Several results of independent interest, both concerning the approximation capacity of the DKF model and the local Lipschitz regularity of the robust filtering map~\eqref{goal:Robust_Filtering} are discussed.  Detailed proofs of our results are relegated to \Cref{s:Proof}. 

% \section*{Notation}
% % \label{s:Notation}
% \noindent This section serves as a reference, which records the notation used throughout our manuscript.  In what follows, $N,I,J\in \mathbb{N}_+$, $A$ is an arbitrary $I\times J$ matrix, $x,x_1,\dots,x_J\in \mathbb{R}^N$, $f$ is an arbitrary real-valued function on $\mathbb{R}$, and $t\in \mathbb{R}$.
% \begin{enumerate}[itemsep=3pt]
%     \item \textit{Componentwise Composition:} $\smash{f\bullet x\eqdef (f(x_n))_{n=1}^N}$ for any $N\in \mathbb{N}_+$.%, $x\in \mathbb{R}^N$, and $f:\mathbb{R}\rightarrow \mathbb{R}$.
%     \item \textit{Rectified Linear Unit (ReLU):} $\operatorname{ReLU}:\mathbb{R}\rightarrow\mathbb{R}$ given by $\smash{\operatorname{ReLU}(t)\eqdef \max\{0,t\}}$.
%     \item \textit{Rowwise Product:} $\smash{v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}}$.% for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
%     \item \textit{Softmax Function:} $\smash{\operatorname{Softmax}(x)\eqdef (e^{x_n}/\sum_{i=1}^N\,e^{x_i})_{n=1}^N}$.% for any $N\in \mathbb{N}_+$ and any $x\in \mathbb{R}^N$.
%     \item \textit{Sparsity:} $\smash{\|(A_{i,j})_{i,j=1}^{I,J}\|_0\eqdef \#\{A_{i,j}\neq 0:\,i,j=1,\dots,I\}}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
%     \item \textit{Vector Concatenation:} $\smash{\oplus_{j=1}^N x_j\eqdef (x_1,\dots,x_J)^{\top}}$ is the $J\times N$-matrix whose $j^{th}$ row is $x_j$.%, for $j=1,\dots,N$.
%     \item \textit{Vectorization:} $\smash{\operatorname{vec}((A_{i,j})_{i,j=1}^{I,J})\eqdef (A_{1,1},\dots,,A_{I,1},\dots,A_{1, J}, \dots, A_{I,J})}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$. 
%     \item \textit{Euclidean Norm:} 
%     $\smash{\|A\| = (\sum_{i,j=1}^{I,J} |A_{i,j}|^2 )^{1/2}}$. 
%     \item \textit{Supremum Norm:} 
%     $\smash{\|A\|_\infty=\sup \{ A_{i,j} : \, i=1,..., I, j=1, ..., J \}}$. 
% \end{enumerate}

% \section{The Setting}
% \label{s:Setting}
% This section formalizes the setting in which our analysis takes place.  We begin by specifying the dynamics of the stochastic processes in the filtering problem.  Next, the source space of paths considered is introduced.  Subsequently, we formulate the target space of probability measures wherein the optimal filter lies.

% \subsection{Regularity Conditions on the Partially-Observed System}
% % \label{s:Preliminaries__ss:Dynamics}
% % This section formulates the theoretical problem which this paper addresses.
% % % Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% % % Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  
% % These processes evolve according to the coupled dynamics
% % \begin{align}
% % \label{eq:filtering_dynamics__signal}
% % dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% % \label{eq:filtering_dynamics__observation}
% % dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% % \end{align}
% % where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.
% % 
% % 
% % Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% % \begin{align}
% % \label{id:ConditionalDistribution}
% %     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) 
% % \end{align}
% % where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of the theoretical foundations of DKFs.
% % \begin{question}
% % \label{question:main}
% % Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$?
% % \end{question}
% We henceforth maintain the following basic regularity assumptions on the dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
% %%
% \begin{assumption}[Regularity Conditions: Dynamics]
% \label{ass:technical_evolution_conditions}
% We will assume the following uniform bounds:
% \begin{align*}
%     \vert \process{a_1}{t, y}{i, j}\vert \le L
%     \mbox{ and }
%     \vert \process{A_1}{t, y}{k, j}\vert \le L
% \end{align*}
% for $y \in C([0:t], \R^{d_Y})$, $t \in [0:T]$, $i,j=1,\dots,d_X$, and $k=1,\dots,d_Y$.  
% Further, we require the following integrability conditions:\footnote{In particular, the integrability conditions imply that $\bE\big[\sum_{j = 1}^{d_X}(X_0)_j^4\big] < \infty$.}
% \begin{enumerate}[label=(\roman*)]
%     \item $\int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item $\int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     % \item $\int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt < \infty$, \yannick{Follows from Lip-cont.}
%     % \item $\int_0^T (\process{b_2}{t, y_{[0:t]}}{i, k})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{k, i})^2 dt < \infty$, \yannick{Follows f. Lip-cont.}
%     % \item $\int_0^T (\process{A_0}{t, y_{[0:t]}}{k})^2 + (\process{B_2}{t, y_{[0:t]}}{k, l})^2 dt < \infty$, \yannick{Follows from Lip-cont.}
% \end{enumerate}
% hold for $i,j=1,\dots,d_X$, and $k,l=1,\dots,d_Y$ and all paths $y_{[0:T]} \in C([0:T], \R^{d_Y})$. We define 
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\top + B_2B_2^\top, \quad 
%     b \circ B \eqdef b_1B_1^\top + b_2B_2^\top, \quad 
%     b \circ b \eqdef b_1b_1^\top + b_2b_2^\top.
% \end{align*}
% and require that the matrix $B \circ B$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% \begin{enumerate}[label=(\roman*), resume]
%     \item $\vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%         \le
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2$,
%     \item $(B_k)_{i,j}(t, x)^2  
%         \le 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2)$,
%     \item $\int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt < \infty$,
%     \item $\bE[\vert (X_t)_j \vert] < \infty, \quad \forall t \in [0:T]$,
%     \item $\bP\big( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \big) = 1$,
% \end{enumerate}
% for indices $i=1,\dots,d_Y$ and $j=1,\dots,d_X$, where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$.  

%     We further impose the following assumptions on the dynamics \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}:
%     \begin{enumerate}[label=(\roman*), resume]
%         \item Local Lipschitz continuity in the path component uniformly in time\footnote{
%             By \emph{local Lipschitz continuity uniformly in time} we mean that there exists a constant that is a local Lipschitz-constant for the path at all times $t \in [0,T]$.
%         }, as well as global Lipschitz continuity in the time component of $a_0$, $a_1$, $b \circ b$, $b \circ B$, $ A_0$, $A_1$, $(b \circ B)$, $(B \circ B)^{-1}$ with respect to the $l^2$-norm, or Frobenius norm if matrix-valued. \label{asm:Regulartiy__1}
%         \item Positive semi-definiteness of $(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ for all times $t \in [0:T]$ and paths $y_{[0:T]} \in C^1([0:T], \R^{d_X})$. \label{asm:Regulartiy__2}
%         \item \label{asm:Regularity__3} Let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$ for any path $y_{[0:T]} \in C^1([0:T], \R^{d_X})$, where 
%         \begin{align*}
%             \Tilde{a}_1^\top(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%         \end{align*}
%         There exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$ as well as $K_3 > 0$ s.t. $\tr(A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$. 
%     \end{enumerate}

%     Eventually we require for the initial conditions that 
%     \begin{enumerate}[label=(\roman*), resume]
%         \item the conditional distribution of $X_0$ given $Y_0$ is normal,
%         \item the covariance matrix $\Sigma_0 := \mathbb{E}[(X_0 - \mu_0)(X_0 - \mu_0)^\intercal \vert Y_0]$ is positive definite, where $\mu_0 := \mathbb{E}[X_0 \vert Y_0]$, and that
%         \item \label{asm:Regularity__LipInit} Lipschitz continuity of $\mu_0, \Sigma_0$ in $Y_0$ w.r.t. the $\Vert \cdot \Vert_2$-norm holds. 
%     \end{enumerate}
% \end{assumption}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Setting__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^{d_Y})$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^{d_Y}$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^{d_Y})$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^{d_Y}$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically embed any path $y\in C([0:t],\mathbb{R}^{d_Y})$ into a path $\bar{y} \in C([0:T],\mathbb{R}^{d_Y})$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     \bar{y}(s)\eqdef \begin{cases}
%         y(s) &: \mbox{ if } 0\le s \le t\\
%         y(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $\bar{\cdot}: C([0:t],\mathbb{R}^{d_Y}) \to C([0:T],\mathbb{R}^{d_Y})$ is a linear isometric embedding of the Banach spaces, since
% \[
% \|\bar{y}\|_T = \max_{0\le s\le T}\, \|y(s)\|_2
% = \max_{0\le s\le t}\, \|y(s)\|_2 = \|y\|_t, 
% \]
% since $y(s)=y(t)$ for all $t<s\le T$.  Conversely, the restriction $\bar{y}_{[0:t]}$ of a path $\bar{y}\in C([0:T],\mathbb{R}^{d_Y})$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^{d_Y})$ to $C([0:t],\mathbb{R}^{d_Y})$ since
% \[
%         \|\bar{y}_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|\bar{y}_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|\bar{y}_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|\bar{y}(s)\|_2 
%     =
%         \|\bar{y}\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^{d_Y})$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot be approximated by standard deep neural networks parameterized determined by a number of trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing}.   

% The curse of dimensionality cannot be broken, but can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space -- as is the case in our results -- show that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}. However, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are either isometric to some compact Riemannian manifold or they are comprised of piecewise linear paths with finitely many pieces.  In particular, we exclude fractal-like subsets of the path space $C([0:T],\mathbb{R}^{d_Y})$ which need not be compressible into finitely many dimensions without ``loosing information'' (i.e.\ for which there is no bi-Lipschitz embedding into a finite-dimensional normed space).  

% In what follows, we denote the Riemannian volume of a connected $(C^2)$ Riemannian manifold $(\mathcal{M},g)$ by $\operatorname{Vol}(\mathcal{M},g)$.  We denote its geodesic distance function by $d_g$.
% \begin{assumption}[Domain Regularity]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ and a ``latent dimension $\ldim\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}[label=(\roman*)]
%     \item  \label{ass:reg_compact_finite}\emph{Finite Domains:} $K$ is finite.
%     \item \label{ass:reg_compact_linear} \emph{Piecewise Linear Domains:} There are $\pldim \in \mathbb{N}_+$, $0=t_0<\dots<t_\pldim=T$, and $C_K>0$ such that $y_{\cdot}\in K$ if and only if:
%         \begin{enumerate}[label=(\alph*)]
%             \item For $i=0,\dots,\pldim-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^{d_Y}$ satisfying
%             \[
%             \begin{aligned}
%                 & y(t)=A^{(i)}\,t+b^{(i)}
%                 \,
%                 &
%                 \,
%                 \mbox{ for all } t\in (t_i,t_{i+1})
%             ,
%             \end{aligned}
%             \]
%             \item $y_0=0$,
%             \item $\max_{i=1,\dots,\pldim}\,|y(t_i)|\le C_K$.
%         \end{enumerate}
%     \item \label{ass:reg_compact_riemann}\emph{Smooth Domains:} There exists a compact and connected $\ldim$-dimensional Riemannian manifold $(\mathcal{M},g)$ for which $(\mathcal{M},d_g)$ is isometric to $(K,\|\cdot\|_T)$.
%     %\anastasis{I think, I can do a bit better here, and get a compact subset of ...}
% \end{enumerate}
% \end{assumption}
% Evidently, their domains $K$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_finite} are easily exhibited, and they correspond to any \textit{training set}.  One can interpret results in this case as paralleling interpolation results for deep learning, e.g.\ \cite{CristaJosefMartin_2020_UnivInterpol,vershynin2020memory,KratsiosDevarnotDokmanic_SmallTransformers_JMLR2023}, but allowing for some arbitrarily small error as in \cite{park2021provable}.

% Compact subsets of the path-space $C([0:T],\mathbb{R}^{d_Y})$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann} are also plentiful.  The following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}, and related results such as~\cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}, illustrate this by guaranteeing that $C([0:T],\mathbb{R}^{d_Y})$ contains isometric copies of any compact metric space.  Consequentially, $C([0:T],\mathbb{R}^{d_Y})$ contains isometric copies of any compact and connected Riemannian manifold.
% \begin{proposition}[Isometric Copies of Every Compact Riemannian Manifold in the Path Space]
% \label{prop:Non_Vaccousness}
% Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}

% We obtain explicit estimates for the case where $(K,d_{\cdot})$ satisfies \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann}, if the ``model'' smooth manifold $\mathcal{M}$ is topologically regular, in that sense that it is \textit{aspherical}.
% This means that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$, what is for instance the case if $\mathcal{M}$ is a Torus. See e.g. \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups.  

% Domains $K$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_linear} include any piecewise linear interpolation of real-world financial time-series data, or simulated data.  This is because only a finite number of inflection points can be observed, and prices are not unbounded.  

% In this way, \Cref{ass:reg_compact} summarizes a rich family of compact subsets of the path-space $C([0:T],\mathbb{R}^{d_Y})$ which possess a sufficient degree of structure to be losslessly encoded into finitely many dimensions by our model's encoding layer, called its \textit{pathwise attention mechanism}.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Setting__ss:OutputSpace}

% Fix $1 \leq p \leq 2$. The $p$-Wasserstein space $\mathcal{P}_p(\mathbb{R}^{d_X})$ consists of all probability measures on $\mathbb{R}^{d_X}$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_p(\mathbb{R}^{d_X})$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^p]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_p$ on $\mathbb{P}_p(\mathbb{R}^{d_X})$ is given by minimizing the optimal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_p(\mathbb{P}, \mathbb{Q})^p
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^p]
%     .
% \]
% Generally, the $p$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, the $2$-Wasserstein distance is not always computationally intractable as for instance in the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^{d_X}$, \cite{dowson1982frechet} showed that it admits the following closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^{d_X})$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^{d_X})$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^{d_X}$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% %\yannick{Until here $d_X, d_Y$ is fixed, needs to be done in what follows.}

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% % This section introduces our attention-based model, our deep Kalman filter (DKF) model, illustrated in \Cref{fig:DKFModel}.  The proposed DKF generates a prediction on the space $(\mathcal{N}_{d_X},\mathcal{W}_2)$ from any observed continuous path in $C([0:T],\mathbb{R}^{d_Y})$, via a three-phase process.  

% % \begin{figure}[hpt!]%[H]%
% %     \centering
% %         \centering
% %         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
% %     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
% %     \label{fig:DKFModel}
% % \end{figure}

% % \subsubsection{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^{d_Y})$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ including classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geometry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% % \subsubsection{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner by adapting to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% % \subsubsection{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_{d_X}$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.


% \subsection{Phase 1 - Encoding via Pathwise Attention}
% \label{s:Model__ss:PathwiseAttention}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and the graph attention mechanism of \cite{velivckovic2017graph} to the context of continuous-time path sources/inputs.  Our attention mechanism, called \textit{pathwise attention}, encodes key information about a novel path $y_{\cdot}$ and, like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``known/previously generated paths''.  

% \begin{figure}[hpt!]%[H]%
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.8\linewidth]{Graphics/Similarity_Score.pdf}
%         \caption{\label{fig:Similarity_Score} The \textit{similarity score} component $\operatorname{sim}_T^{\theta_0}$ encodes a path into finite-dimensional vectorial data, by relating its similarity to a dictionary of previously observed ``contextual paths''.}  
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.8\linewidth]{Graphics/Positional_Emcoding.pdf}
%         \caption{\label{fig:PositionalEncoding} The \textit{positional encoding} component $\operatorname{post}_T^{\theta_0}$ of the attention mechanism allows the similarity scores to further adapt to any novel path by extracting sample-positions on the novel paths.}
%     \end{subfigure}
%     \caption[1]{Our \textit{pathwise attention mechanism} $\operatorname{attn}_t^{\theta}$, in \Cref{defn:PathAttention}, relies on two methods for adaptive feature extraction.  The first component of the mechanism, in~\ref{fig:Similarity_Score}, in is a similarity score which ranks the similarity of any novel path $x_{\cdot}$ to a dictionary of ``recognized/saved'' reference paths.  The second component of the mechanism, in~\ref{fig:PositionalEncoding}, samples points on the novel path $x_{\cdot}$ and perturbs the similarity scores by them.  The adeptness of the pathwise attention mechanism, unlike basis-based methods, is rooted in the fact that nearly all of its parameters are trainable, which allows it to be tasks-specific (similarly to the advantage of deep MLPs have over regression via basis-functions).}
%     \label{fig:Attention_Is_All_You_Need}
% \end{figure}


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $\rdim$, $\sdim$, $d_Y$, and a ``time horizon'' $T> 0$.  
% Given a set of $\rdim$ distinct paths $\{y^{(n)}\}_{n=1}^\rdim$ in $C([0,1],\mathbb{R}^{d_Y})$, an $\sdim \times \rdim$-matrix  $B$, $b\in \mathbb{R}^{\sdim}$, an $\sdim \times \sdim$-matrix $A$, and $a\in \mathbb{R}^{\sdim}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^\rdim)$.

% The \textit{similarity score}, is a map $\operatorname{sim}_T^{\theta_0}:C([0,1],\mathbb{R}^{d_Y})\rightarrow\mathbb{R}^\sdim$, mapping any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$ to
% \begin{equation}
% \label{eq:sim_score}
%     \operatorname{sim}_T^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%         \operatorname{Softmax}
%             \biggl(
%                     A\operatorname{ReLU}\bullet 
%                 \Big(
%                         B
%                         \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^\rdim
%                     +
%                         b
%                 \Big)
%                     +
%                         a
%             \biggr)
%     .
% \end{equation}
% % where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$. 
% % \yannick{The definition of $\bullet, \operatorname{Softmax}, \operatorname{ReLU}$ is also in the Notation section.}
% \end{definition}

% Illustrated in \Cref{fig:Attention_Is_All_You_Need}, our pathwise attention mechanism extracts features by reinterpreting two of the key features of attention mechanisms from natural language processing (NLP).  First, it utilizes \textit{similarity scores} which rank the likeness of any novel path against a dictionary of references paths.  These reference paths can either arise from real/stress historical (market) scenarios, they can be generated synthetically, or a combination of either.  These similarity scores are illustrated in \Cref{fig:Similarity_Score}, and they serve as pathwise analogues of contextual keys and queries in attention mechanisms in NLP.

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of \Cref{defn:Sim_Score}, fix a positive integer $\pdim$, and set of query times $0\le t_1<\dots< t_\tdim\le T$, an $\pdim\times {d_Y}$ matrix $V$, and an $\pdim\times \tdim$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^\tdim)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{post}_T^{\theta_0}:C([0,1],\mathbb{R}^{d_Y})\rightarrow\mathbb{R}^{\pdim \times d_Y}$, defined by 
% \begin{equation}
% \label{eq:pos_encoding}
%     \operatorname{post}_T^{\theta_1}
%         (y_{\cdot} )
%     \eqdef 
%         U \,
%         (\oplus_{j=1}^\tdim \, y_{t_j})
%         + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$.
% \end{definition}

% Next, the \textit{positional encoding} of any novel path, illustrated in \Cref{fig:PositionalEncoding}, encodes snapshots of this path at various times.  These indicate changes in any sample path, and they fully determined piecewise linear paths with finitely many pieces (as are generated in simulation studies).  This data then combines with the weights of the similarity scores to produce the features encodings of our pathwise attention mechanism. 


% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of \Cref{defn:Sim_Score,defn:PositionalEncoding}, set $\sdim=\pdim$.  A \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1,C)$, is the map $\operatorname{attn}_T^{\theta}:[0,T]\times C([0,T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim + 1}$ with representation
% \begin{align}
%     \label{eq:featuremap}
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot})
%     \eqdef 
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
% \end{align}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$ and $0\le t\le T$, where $C$ is an $\edim \times (\sdim d_Y)$-dimensional matrix.
% \end{definition}


% \begin{proposition}[Pathwise Attention Losslessly Encodes Regular Domains]
% \label{prop:Lossless_Encoding}
% Let $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact}.  Then, there exists an $\edim \in \mathbb{N}_+$ and a parameter $\theta$ as in \Cref{defn:PathAttention} such that, $\operatorname{attn}_T^{\theta}$ restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim+1},\|\cdot\|_2)$.

% Estimates for the encoding dimension $\edim$ are recorded in \Cref{tab:ATTENTION_Rates} on a case-by-base basis.
% \end{proposition}



% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for Lossless Pathwise Attention Encoding of Regular Compact Domains.}}
%     \label{tab:ATTENTION_Rates}
%     \begin{tabular}{lllll}
%     \toprule
%         Type of Compact Domain %& Complexity ($\|\theta\|_0$) 
%         & Encoding Dimension ($\edim$) & Ass.~\ref{ass:reg_compact} \\
%     \midrule
%         Finite%& $\mathcal{O}(\cdot)$ 
%         & $\mathcal{O}(\log(\# K))$ 
%         & \ref{ass:reg_compact_finite}
%         \\
%         P.W. Lin. ($\pldim$ Pieces) %& - 
%         & $\mathcal{O}(\pldim d)$
%         & \ref{ass:reg_compact_linear}
%         \\
%         Iso. Comp. Riemann.%& -- 
%         & Finite
%         & \ref{ass:reg_compact_riemann}
%         \\
%         Iso. Comp. Riemann $\&$ Aspherical %& -- 
%         & $\smash{\mathcal{O}\big(\mathfrak{N}_{d_g}(\mathcal{M},\operatorname{Vol}(\mathcal{M},g)^{1/\ldim} )\big)}$
%         & \ref{ass:reg_compact_riemann}
%         \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Fix an $A\subset \mathcal{M}$ and $\delta>0$.  The quantity $\mathfrak{N}_{d_g}(A,\delta)$ denotes the minimum number, $I$, of points $\{x_i\}_{i=1}^I \subseteq A$ for which every $x\in A$ is contained in a geodesic ball of radius $\delta$ about some $x_i$, for $i\in \{1,\dots,I\}$.}
% \end{table}

% \subsection{Phase 2 - Multi-Layered Perceptrons (MLPs) Transformation}
% \label{s:Model__ss:Review__MLPs}
% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an encoding dimension $\edim$ and a target dimension $\ddim$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^\edim$ to $\mathbb{R}^\ddim$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^\edim\rightarrow\mathbb{R}^\ddim$ with iterative representation: for each $x\in \mathbb{R}^\edim$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=\edim$ and $d_{J+1}=\ddim$.

% \subsection{Phase 3 - Decoding via Geometric Attention Mechanism}
% \label{s:Model__ss:GeometricAttentionMechanism}

% Fix $\ddim \in \mathbb{N}_+$.  In what follows, we denote the orthogonal projection of $\mathbb{R}^\ddim$ onto the $\ddim$-simplex 
% \[
%         \Delta_\ddim
%     \eqdef 
%     \Big\{
%         w \in [0,1]^\ddim:\,
%         \sum_{n=1}^\ddim\,w_n = 1
%     \Big\} 
% \]
% by $P_{\Delta_\ddim}$.  We note that the closedness and convexity of $\Delta_\ddim$ implies that $P_{\Delta_\ddim}$ is a well-defined $1$-Lipschitz map, see \citep[Proposition 4.8]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017}.  

% \begin{definition}[Geometric Attention Mechanism]
% \label{defn:GeometricAttentionMechanism}
% Let $\ddim,d_X \in \mathbb{N}_+$.  A geometric attention mechanism is a map $\operatorname{g-attn}_\ddim: \mathbb{R}^\ddim \rightarrow \mathcal{N}_{d_X}$ with representation
% \[
%         \operatorname{g-attn}_\ddim^{\vartheta}(v)
%     =
%         \mathcal{N}_{d_X}\Biggl(
%                 \sum_{n=1}^\ddim\,
%                     P_{\Delta_\ddim}(v)_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^\ddim\,
%                     P_{\Delta_\ddim}(v)_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)}
%         \Biggr)
% \]
% where $m^{(1)},\dots,m^{(\ddim)}\in \mathbb{R}^{d_X}$, $A^{(1)},\dots,A^{(\ddim)} \in \R^{d_X\times d_X}$; and $\vartheta\eqdef (m^{(n)},A^{(n)})_{n=1}^\ddim$.
% \end{definition}

% \subsection{The DKF Model}
% \label{s:Model__ss:DKFModel}
% We may now formalize the discrete Kalman filter model of \Cref{fig:DKFModel}.  
% \begin{definition}[Deep Kalman Filter]
% Let $d_X, d_Y \in\mathbb{N}_+$, $T>0$, and an activation function $\sigma:\mathbb{R}\rightarrow \mathbb{R}$.  
% A function $\hat{F}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathcal{N}_{d_X}$ is called a discrete Kalman Filter if it admits the representation
% \begin{equation}
% \label{eq:DKF_formalization}
%         \hat{F}
%     =
%             \operatorname{g-attn}_\ddim^{\vartheta}
%         \circ 
%             \hat{f}
%         \circ 
%             \operatorname{attn}_T^{\theta}
% \end{equation}
% where $\operatorname{g-attn}_\ddim^{\vartheta}$ is as in \Cref{defn:GeometricAttentionMechanism}, $\operatorname{attn}_T^{\theta}$ is as in \Cref{defn:PathAttention}, and $\hat{f}$ is an MLP as in~\eqref{eq:MLP}; such that the composition~\eqref{eq:DKF_formalization} is well-defined.
% \end{definition}



% \section{Main Result}
% \label{s:Main_Results}

% We are now ready to state our main theorem, which shows that the DKF~\eqref{eq:DKF_formalization} is indeed capable of asymptotically optimally filtering the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.  Our guarantees are of a non-asymptotic form; in that they depend on the complexity of the network.
% \begin{theorem}[The DKF Can Approximate the Optimal Filter]
% \label{thrm:MAIN}
% Let $d_X, d_Y \in \mathbb{N}_+$ and $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact}.  Suppose that the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies \Cref{ass:technical_evolution_conditions}.  % and let $f^{\star}$ denote its associated optimal filter~\eqref{id:ConditionalDistribution}.  
% For every $T>0$ there exists a DKF $\hat{F}:[0:T]\times C([0:T]\times\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ satisfying the uniform estimate
% \[
%     \max_{0\le t\le T,\,y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:T]})
%             ,
%                 \hat{F}(t,y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, \Cref{tab:ComplexityMain} records the complexity estimates of $\hat{F}$.
% \end{theorem}

% \begin{table}[H]%[ht!]
%     \centering
%     \caption{{Complexity Estimates for the DKF model $\hat{F}$ in~\Cref{thrm:MAIN}.}}
%     \label{tab:ComplexityMain}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 \varepsilon^{-\ddim}
%             \big)
%         }
%     	$
%         & 
%         $        
%         \smash{
%             \mathcal{O}\big(
%                 \varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          \smash{
%          \mathcal{O}\big(
%             \varepsilon^{-4\ddim-1}
%          \big)
%     	 }
%          $
%          &
%          $ \ddim + \edim +3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%          \smash{
%          \mathcal{O}\big(
%             \varepsilon^{-8\ddim-6}
%          \big)
%     	 }
%          $
%          & 
%          $\ddim+\edim+4$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%          \\
%          Non-Smooth $\&$ Non-poly.
%             &
%         Finite
%         &
%         $\ddim+\edim+3$
%          & $\mathcal{O}(1)$ & $\smash{\mathcal{O}\big(\varepsilon^{-1}\big)}$
%          \\
%     \bottomrule
%     \end{tabular}
% \end{table}



% \subsection{Proof Overview}
% \label{s:Theoretical_Analysis}
% This section overviews the derivation of our main result, namely, \Cref{thrm:MAIN}.

% %\subsubsection{Summary of What is Known}
% % \label{s:Theoretical_Analysis__ss:LipsterShiryaevSummary}
% Results in \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, they denote an explicit formulation of the resulting distribution which can then analyze directly. 
% In particular, \Cref{ass:technical_evolution_conditions} allows the application of \citep[Theorem 12.6]{LipShiryaev_II_2001} and we obtain that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.


% A function is uniformly approximable by a deep learning model if it is continuous.  If there is no clear favourable structure in the function being approximated, e.g.\ smoothness \cite{yarotsky2020phase,gonon2023approximation} or neural network-like structure \cite{cheridito2021efficient,mhaskar2016deep}, then the best available approximation rates are those corresponding to those where the target function is Lipschitz; see \cite{DaubechiesDeVoreFoucartHaninPetrova_CA_KnotFreeReLU_2022}. %devore1993constructive,
% Thus, the first step to obtaining approximability guarantees for the optimal filter by deep neural networks, which depend on relatively few trainable parameters, is to show that the optimal filter is a locally-Lipschitz function of observed paths.

% \begin{proposition}[Local Lipschitz-Continuity of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter}
%     Under \Cref{ass:technical_evolution_conditions}, $f_t$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous. In particular, for every time $t \in [0:T]$, path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$ there exists constant $C \ge 0$ such that for all times $s \in [0:T]$ and paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\vert t -s \vert < \epsilon$, $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]}))
%         \leq C 
%             \big(
%                 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T 
%             + 
%                 \vert t - s \vert
%             \big).
%     \end{align*}
% \end{proposition}

% Having established the regularity of the optimal filter for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, we need to verify that maps sharing the same domain (input space), codomain (output space), and regularity as the optimal filter are approximable by the proposed DKF model.  This is the content of the next proposition, which acts as its standalone approximation theorem for the DKF.


% \begin{table}[H]%[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{F}$ in \Cref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \begin{tabular}{@{}lllll@{}}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$) \\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 (LV( L))^{-\ddim}\,\varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 (LV(L))^{-\ddim}\,\varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          \smash{
%         \mathcal{O}\big(
%             L^{4\ddim+1}\, \varepsilon^{-4\ddim-1}
%         \big)
%     	}
%          $
%          &
%          $ \ddim + \edim +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%          \smash{
%         \mathcal{O}\big(
%             L^{8\ddim+6}\, \varepsilon^{-8\ddim-6}
%         \big)
%     	}
%          $
%          & 
%          $\ddim+\edim+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Non-Sm. $\&$ Non-poly.
%             &
%         Finite
%         &
%         $\ddim+\edim+2$
%          & $\mathcal{O}(1)$ & $\smash{\mathcal{O}\big(L\varepsilon^{-1}\big)}$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}

% \begin{proposition}[Approximation Capacity of DKFs]
% \label{prop:Universal_Approximation_Theorem__PathToNd}
% Let $d_X, d_Y \in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfying \Cref{ass:reg_compact}.  
% For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:([0,T]\times K,|\cdot| \times \|\cdot\|_{\infty})\rightarrow (\mathcal{N}_{d_X},\mathcal{W}_2)$ there exists a DKF $\smash{\hat{F}}$ 
% % \[
% %         \hat{t}(x)
% %     \eqdef
% %         \mathcal{N}_{d_X}\Biggl(
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     m^{(n)}
% %             ,
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     (A^{(n)})^{\top}A^{(n)})
% %         \Biggr)
% % \]
% % \anastasis{Update representation/simplify ofc + explain notation} 
% satisfying the uniform estimate 
% \[
%     \sup_{t, x\in [0:T]\times K}\,
%         \mathcal{W}_p\big(
%         f(t, x_\cdot) ,
%         \hat{F}(t,x_\cdot) 
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(\edim)$ and Decoding dimension $(\ddim)$ are all recorded in \Cref{tab:approximationrates__nonFlatVersion} depending on the activation function $\sigma$.
% \end{proposition}


% We now have at our disposal, the tools to prove our main result.  
% \begin{proof}[{Proof of \Cref{thrm:MAIN}}]
% Since the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies \Cref{ass:technical_evolution_conditions}, \Cref{prop:LocLipReg_OptimFilter} implies that the optimal filter $f_T$ in \eqref{goal:Robust_Filtering} 
% is a locally-Lipschitz map from $([0:T],  C([0:T],\mathbb{R}^{d_Y}),\vert \cdot \vert \times \|\cdot\|_T)$ to $(\mathcal{N}_{d_X},\mathcal{W}_2)$.  Since $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ is compact then, $f|_K$ is Lipschitz.  

% Since $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfies \Cref{ass:reg_compact} and $0<\varepsilon<1/2$ then, \Cref{prop:Universal_Approximation_Theorem__PathToNd} implies that there is a DKF $\hat{F}:C([0:T],\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ with representation~\eqref{eq:DKF_formalization} and complexity recorded in \Cref{tab:approximationrates__nonFlatVersion} satisfying
% \[
% 	\sup_{t, y\in [0:T]\times K}\,
% 		\mathcal{W}_p\big(
% 			f(t,y)
% 		,
% 			\hat{F}(t,y)
% 		\big)
% 	< 
% 		\varepsilon
% 	.
% \]
% This completes the proof of \Cref{thrm:MAIN}.
% \end{proof}

% \section{Discussion and Future Work}
% \label{s:Discussion}
% Our main result, namely Theorem~\ref{thrm:MAIN}, showed that there are deep Kalman filters which can solve the approximately stochastic filtering problem in continuous time for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, to arbitrary accuracy.  This complements the experimental work of \cite{KrishnanShalitSontag15,KrishnanShalitSontag17}, which shows that deep Kalman filters can be trained to offer state-of-the-art empirical performance.  

% From the theory perspective, it would be interesting to analyze the statistical learning theoretic properties of DKFs.  One would expect that elementary generalization bounds could be derived by using the bounds on VC-dimension derived in \cite{MR3960917} and a version of the results of \cite{MR1984026} or by directly modifying the transport theoretic arguments of \cite{hou2022instance}, to incorporate the effects of the pathwise and geometric attention layers in~\eqref{eq:DKF_formalization}.  Nevertheless, for problems in mathematical finance where one only observes a single training path (one-shot learning), the most interesting question in that direction is: \textit{How to train the DKFs in a way such that they have robust statistical guarantees when only a single training path is observed}.

% \section{Proofs}
% \label{s:Proof}
% This section contains the derivations of our paper's results.

% \subsection{Isometric Copies of Every Compact Riemannian Manifold in the Path Space -- Proof of \texorpdfstring{\Cref{prop:Non_Vaccousness}}{Proposition 1}}
% \label{s:Proof__ss:AuxResults}
% \begin{proof}[{Proof of \Cref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^{d_Y})$, given by $f\mapsto (f(\cdot /T),0,\dots,0)$, is an isometric embedding; then $\smash{\phi\eqdef \phi_3\circ\phi_2\circ \phi_1}$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^{d_Y})$.
% \end{proof}

% \subsection{Stability of the Optimal Filter - Proof of \texorpdfstring{\Cref{prop:LocLipReg_OptimFilter}}{Lipschitz Continuity}}
% We now prove the local Lipschitz stability of the optimal filter~\eqref{goal:Robust_Filtering}, for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, as a function of its observed/input path.  The proof builds on a series of Lemmata, which demonstrate the local Lipschitz continuity of the parameters defining the optimal filter.  

% We first observe that, \Cref{ass:technical_evolution_conditions} grants us access to \citep[Theorem 12.7]{LipShiryaev_II_2001}, which implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
%     d\mu_t 
%         &=[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\top}(t,y_{[0:t]})]\label{id:ClosedFormMu}
%         \\
%         & \pushright{
%              \times (B\circ B)^{-1}(t,y_{[0:t]}) [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt]  \notag
%         }
%         \\
%     \partial_t\Sigma_t
%         & = a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\top}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]})
%         \label{id:ClosedFormSigma} \\
%         & \pushright{
%               - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\top}(t,y_{[0:t]}) ]
%               (B\circ B)^{-1} (t,y_{[0:t]})} \notag \\
%         & \pushright{\times [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\top}(t,y_{[0:t]})]^{\top} }
%          \notag
% \end{align}
% with initial conditions $\mu_0\eqdef\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\top}|Y_0]$; where
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\top + B_2B_2^\top, \quad 
%     b \circ B \eqdef b_1B_1^\top + b_2B_2^\top, \quad 
%     b \circ b \eqdef b_1b_1^\top + b_2b_2^\top.
% \end{align*}
% Furthermore, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\Sigma_t$ is positive definite for all $t \in [0:T]$ since we have assume that $\Sigma_0$ in \Cref{ass:technical_evolution_conditions}.

% To clarify the argument's direction, we first record the proof of \Cref{prop:LocLipReg_OptimFilter}.  We subsequently derive the lemmata on which it relies.

% \begin{proof}[{Proof of \Cref{prop:LocLipReg_OptimFilter}}]
%     Fix $t \in [0:T]$, a path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$.
%     By \Cref{prop:LocLipReg_OptimFilter_Time} we can fix a $K_1 > 0$ such that for every time $0 < s < T$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})) \leq K_1 \vert t-s \vert_t.
%     \end{align*}
%     By \Cref{prop:LocLipReg_OptimFilter_Path} we can fix a $K_2 > 0$ such that for every path $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$ holds
%     \begin{align*}
%             \mathcal{W}_2(
%                 \mathbb{P}(X_u \in \cdot \vert y^{(1)}_{[0:u]})
%             ,
%                 \mathbb{P}(X_u \in \cdot \vert y^{(2)}_{[0:u]})
%             )
%         \leq
%             K_2 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T.
%     \end{align*}
    
%     We see by the triangular inequality of the $\mathcal{W}_2$-distance (that holds as we handle normal distributions, see \eqref{id:LipsterShiryaevRepresentation}),
%     \begin{align*}
%         &
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]})) \\
%         & \quad \leq 
%                 \mathcal{W}_2(
%                     \mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]})
%                 ,
%                     \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})
%                 )
%             + 
%                 \mathcal{W}_2(
%                     \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})
%                 ,
%                     \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]})
%                 )
%             \\
%         & \quad \leq \max\{ K_1, K_2 \} 
%             \big(
%                 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T 
%             + 
%                 \vert t - s \vert
%             \big)
%     \end{align*}
%     what concludes the proof.
% \end{proof}

% \subsubsection{Lipschitz-Continuity in the Path-Component of the Optimal Filter}

% \begin{lemma}[Local Lipschitz-Continuity in the Path-Component of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter_Path}
%     Under \Cref{ass:technical_evolution_conditions}, $f$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous uniformly in time. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$ there exists constant $C \ge 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq C \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T, \quad \forall t \in [0:T].
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a non-negative constant $\bar{K} < \infty$ satisfying the following for every pair of paths $y^{(1)}_{\cdot},y^{(2)}_{\cdot} \in C([0:T],\|\cdot\|_2)$ and all time $t \in [0:T]$
%     \begin{multline*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%     \\
%         \leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{multline*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma} that there exists a non-negative constant $K < \infty$, satisfying
%     \begin{align*}
%         \begin{split}
%                 \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%             & \leq
%                 K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \\ 
%                 \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%             & \leq
%                 K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%         \end{split}
%         \qquad \forall t \in [0:T]
%     \end{align*}
%     Therefore, for each $y_{\cdot}^{(1)},y^{(2)}_{\cdot}\in C([0:T],\mathbb{R}^{d_Y})$ we have  
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t,
%         \qquad \forall t \in [0:T]
%     \end{align*}
%     and the statement follows. 
% \end{proof}


% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]
% \label{lem:LipschitzMu}
%     Under \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous uniformly in time. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}  
%             \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%         \leq
%             K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t,
%         \qquad \forall t \in [0:T].
%     \end{align*} 
% \end{lemma}
% \begin{proof}
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) 
%    - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\top}}(s, y_{[0:s]}) ] \label{id:Phi1} \\ 
%  & \hspace{3cm} \times  (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \notag \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\top}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu} and for $t \in [0,T]$, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0:s]}) d y_{[0:s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align*}
%     \mu^{(1)}_t - \mu^{(2)}_t 
% & =   
%         \mu_0^{(1)} - \mu_0^{(2)} 
%     + 
%         \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \\
%     & \quad +   
%         \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0:s]}
%     - 
%         \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \\
%     & \quad +
%         \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds
%     +
%         \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\, (\mu^{(1)}_s - \mu^{(2)}_s ) ds .
% \end{align*} 
% By the triangle inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0:s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} \\ 
%   & + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwall's inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz with constant $K_1 < \infty$,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K_1 \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K_1 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K_2^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$ uniformly in time with constant $K_2 < \infty$, given by \Cref{lem:LipschitzPhi2}. Next, let $\lbrace [s_{i-1}:s_{i}] \vert i \in \myset{1}{I}\rbrace$, $I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K_2^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K_2^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K_2\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Integrating by parts, we find that
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         \notag \\
%     & \pushright{- \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2} \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         \notag \\
%     & \pushright{+ \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2} \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq T} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% \Cref{lem:LipschitzPhi2} yields (time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:T]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 =: K_3 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ uniformly in time with constant $K_4 < \infty$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 \\
%     & \leq \epsilon_I + K_4 t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that 
% \begin{align*}
% \eqref{t:gammaB} \leq \left(K_2 \sqrt{T} + K_3 + K_4 T\right) \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t.
% \end{align*}
% Next, we consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K_5 t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to (path-)Lipschitz continuity of $\Phi_1$ uniformly in time with constant $K_5$ which is obtained by \Cref{lem:LipschitzPhi1}. We conclude, since $\max_{s \in [0:T]} \|\mu^{(2)}_s \|_2 := K_6 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\gamma(t) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ with $K := K_1 + K_2 \sqrt{T} + K_3 + K_4 T + K_5 K_6 T$.

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \notag \\
%         & \pushright{\left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)}
%      \notag  
% \end{align} 
% Note that $\Phi_1$ is (time-)Lipschitz continuous, as shown in \Cref{lem:LipschitzPhi1}, therefore implying that $\max_{s \in [0:T]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$. As constants $K_1$, $K_2$, $K_3$, $K_3$, $K_4$, $K_5$, and $K_6$ were chosen independently of $t \in [0:T]$ and \Cref{ass:technical_evolution_conditions} \ref{asm:Regularity__LipInit} holds, we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}


% \begin{lemma}\label{lem:LipschitzPhi1}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists a constant $C\ge 0$ such that for all $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$, and times $t \in [0:T]$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq C \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
% \begin{enumerate}
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component uniformly in time. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) uniformly in time, this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $C\ge 0$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq C \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $C\ge 0$, such that for all $\epsilon > 0$,  paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $t \in [0:T]$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq C \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%     Under \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous uniformly in time. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $C \in \R$ such that for all $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $t \in [0:T]$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq C \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left-hand side refers to the Frobenius norm.
% \end{lemma} 
% \begin{proof} 
% From \eqref{id:ClosedFormSigma} and for $t \in [0:T]$, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
%         \Sigma_t
%     =
%         & \Sigma_0 + \int_0^t
%                 a_1(t,y_{[0:s]}) \Sigma_s
%             +
%                 \Sigma_s a_1^{\top}(s,y_{[0:s]})
%             +
%                 (b\circ b)(s,y_{[0:s]}) \hspace{3cm}
%             \notag\\
%                 &\pushright{- [
%                     (b\circ B)(s,y_{[0:s]})
%                 +
%                     \Sigma_s A_1^{\top}(s,y_{[0:s]})
%                 ]
%                 (B\circ B)^{-1} (s,y_{[0:s]}) } \hspace{1cm} \notag \\
%                 &\pushright{\times[
%                     (b\circ B)(s,y_{[0:s]}) 
%                 +
%                     \Sigma_s A_1^{\top}(s,y_{[0:s]})
%                 ]^{\top}
%         ds.} \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{multline*} 
% \Sigma^{(1)}_t - \Sigma^{(2)}_t
%  = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
%  + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \\
%  + 
% \Xi_2^\top (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{multline*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\top(s, y^{(1)}_{[0:s]}) - a_1^\top(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\top (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\top (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\top (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\top (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\top(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\top(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{multline} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef  a_1^\top(s, y^{(2)}_s) 
%  + A_1^\top(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]})  \\ 
%  \times(b\circ B) (s, y^{(1)}_{[0:s]})  
%  + A_1^\top(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
%  .   \label{Xi2} 
% \end{multline} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{multline} 
%     \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%     \leq  
%     \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%      \\ 
%   + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot  \\ 
%  \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \cdot \\ \cdot \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{multline}  
% From \Cref{lem:LipschitzA1}, we know that there exists a constant $K \in \R$ such that
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{multline}
%         \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
%     \leq  
%         \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big)  \cdot 
%         \\ 
%         \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 \cdot 
%         \\
%         \cdot \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{multline} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$ and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is uniformly bounded, according to \eqref{Xi2}. Therefore, from \eqref{Sigma1-2bddXi2} we obtain a constant $C \in \R$ such that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% C ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}
% We conclude the proof due to \Cref{ass:technical_evolution_conditions} \ref{asm:Regularity__LipInit}.
% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $K \in \R$, such that for all  $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $s \in [0:T]$ holds
% \begin{align*} 
%          \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%      \leq
%          K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component uniformly over all times, we conclude that $a_1$, $b \circ b$, $A_1^\top(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\top (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\top$ have the same property. By this, together with the triangular inequality, there exists a constant $K_1 \in \R$
%     \begin{align*}
%     &
%             \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  
%     \\& \quad
%         \leq  
%                 2K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) 
%             +
%                 K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2
%     \\ &
%             \pushright{
%             +
%                 K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s 
%             }
%     \\& \quad  
%         =
%             K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s
%             \Big(
%                     1
%                 +
%                     2 \Vert\Sigma^{(1)}_s \big\Vert_2
%                 +
%                     2 \Vert\Sigma^{(2)}_s \big\Vert_2 
%                 + 
%                     \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2
%             \Big).
%     \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < {K}_2$ for some $K_2 \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in the path-component and the closure of the set 
% \begin{align*}
%     \{y \in C^{1}([0:T]) \,:\, \Vert y_{[0:t]} - y^{(1)}_{[0:t]} \Vert_2 < \epsilon \}
% \end{align*}
% is compact, we know $\Vert\Sigma^{(2)}_s \Vert_2$ is bounded.
% \end{proof}

% \subsubsection{Lipschitz-Continuity in the Time-Component of the Optimal Filter}

% \begin{lemma}[Global Lipschitz-Continuity in the Time-Component of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter_Time}
%     Under \Cref{ass:technical_evolution_conditions}, $f_t$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous in the time-component. In particular, for every path $y_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$, $t \in [0:T]$, and  $\epsilon > 0$ there exists constant $C \ge 0$ such that for all times $s \in [0:T]$ with $\| t - s \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]})) \leq C \vert t - s \vert.
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     As in the proof of \Cref{prop:LocLipReg_OptimFilter_Path}, we argue that by \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a non-negative constant $\bar{K} < \infty$ satisfying the following for every path $y_{\cdot} \in C([0:T],\|\cdot\|_2)$ and all times $t, s \in [0:T]$
%     \begin{multline*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]}))
%     \\
%         \leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}) - \mu(y_{[0:s]}) \|_2^2 + \|\Sigma(y_{[0:t]})-\Sigma(y_{[0:s]} \|_2^2}.
%     \end{multline*}
%     We see from \Cref{lem:TimeLipschitzMu} and \Cref{lem:TimeLipschitzSigma} that there exists a non-negative Lipschitz-constant $K < \infty$ for both $\mu$ and $\Sigma$ such that
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]})) \leq \sqrt{2}\bar{K}K \vert t - s \vert,
%     \end{align*}
%     and the statement follows. 
% \end{proof}


% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{multline*}
%             \| \mu_t - \mu_s \|_2 
%         \\ \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0:u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0:u]})dy_{[0:u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0:u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{multline*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 \\
%         & \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwall's inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \le &
%             \overbrace{\Big\Vert \int_0^t a_0(u, y_{[0:u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0:u]})dy_{[0:u]} \Big\Vert_2}^{ \eqdef  \alpha(t)} \\
%           & + \int_0^t \big\Vert \Phi_1(u, y_{[0:u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0:s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0:u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0:u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}


% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\top}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\top}(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\top}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\top}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\top}(u,y_{[0:u]})^{\top} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \subsubsection{Lower Loewner order bound}

% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma} and \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__2}, \ref{asm:Regularity__3}, hold. Then there exists an $r > 0$, s.t. for all times $t \in [0:T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ holds that 
%     $\Sigma_t \preccurlyeq r I_d$. 
%     %$\Sigma_t - r \cdot I_{d_X}$ 
%     %is positive semi-definite.
% \end{lemma}
% \begin{proof}
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\top(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\top(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to $(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ being positive semi-definite at 
%     \begin{multline*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top ) \\
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\top
%                     \right)
%                 ds.
%     \end{multline*}
%     As $G_t(y_{[0:t]})$ is positive definite, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top
%                 (G_t(y_{[0:t]})^{-1})^\top
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top
%             )
%     \end{align*}
%     and 
%     \begin{multline*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\top
%             \right)
%         \\ \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{multline*}
%     As we assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$ as well as $K_3 > 0$ s.t. $\tr(A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$ we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\top(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]




% \subsection{Stable and Lossless Encoding by Pathwise Attention - Proof of \texorpdfstring{\Cref{prop:Lossless_Encoding}}{Proposition 2}}
% \label{s:Proof__ss:Encoding}



% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(\rdim)}$ in $C([0:T],\mathbb{R}^{d_Y})$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[Pathwise Attention Implements Stable Lossless Feature Maps -- Riemannian Case]
% \label{lem:Good_Feature_Map}
% Under \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann}, there exists a constant $C_{\ldim}>0$, depending only on $\ldim$, and a $\delta>0$ depending only on $(M,g)$ such that any $\delta$-packing $\{y^{(n)}\}_{n=1}^\ldim$ of $K$, there are matrices $A,B,b,V,U,C$ and vectors $a,b$ for which the parameter $\theta$, as in \Cref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim+1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0 \in \mathcal{O}(\edim^2)$.

% \noindent Moreover, if $(\mathcal{M},g)$ is aspherical then:
% \begin{enumerate}
%     \item[(i)] $\delta \in \mathcal{O}( \operatorname{Vol}(\mathcal{M},g)^{1/\ldim} )$
%     \item[(ii)] $\|\theta\|_0 \in \mathcal{O}(\edim^2)$,
%     \item[(iii)] $C_{\ldim}\in \mathcal{O}(\ldim^{3(\ldim+1)/2})$
%     % $0<C_{\ldim}< (3/5)\, (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}$.
%     % \item[(i)] $\|A\|_0=2N$, 
%     % \item[(ii)] $\|B\|_0=2N$, 
%     % \item[(iii)] $\|a\|_0=1$, 
%     % \item[(iv)] $\|b\|_0=0$, 
%     % \item[(v)] $\|C\|_0= N_1$, 
%     % \item[(vii)] $\|U\|_0=0$, 
%     % \item[(viii)] $\|V\|_0= N^2_1$,
%     % \item[(ix)] $0<C_{\ldim}< (3/5)\, (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}$.
% \end{enumerate}
% % \anastasis{perhaps I tally into a single parameter estimate} like $\|\theta\| \in \mathcal{O}(N^2)$.

% In particular, the attention mechanism $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{\mathrm{in}}$ on $K$.
% \end{lemma}

% \begin{proof}[{Proof of \Cref{lem:Good_Feature_Map}}]\hfill
% \begin{enumerate}[label=\emph{Step \arabic*:}, ref=\arabic*]
%     \item \label{step:GFM_1}\emph{Estimating $\rdim$ on the Riemannian Manifold $(\mathcal{M},g)$.}
% Since $(K,\|\cdot\|_T)$ be isometric to $(\mathcal{M},d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $\ldim$-dimensional Riemannian manifold $(\mathcal{M},g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $\mathcal{M}$ denoted by $\operatorname{sys}(\mathcal{M})$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(\mathcal{M}) 
%     \le
%     \,\tilde{C}_{\ldim}
%     \,
%         \operatorname{Vol}(\mathcal{M},g)^{1/\operatorname{dim}(\mathcal{M})}
%     ,
% \end{equation}
% where $\operatorname{Vol}(\mathcal{M},g)$ denotes the Riemannian volume of $(\mathcal{M},g)$ and $\tilde{C}_{\ldim}>0$ is a universal constant only depending on $\ldim$ satisfying
% \begin{align*}
%         0
%     <
%         \Tilde{C}_{\ldim}
%     <
%         6 (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}
% \,
% .
% \end{align*}
% By Stirling's approximation, $\sqrt{(\ldim+1)!} \in \mathcal{O}(\ldim^{(\ldim+1)/2})$; whence it follows that $\tilde{C}_{\ldim}\in 
% % \mathcal{O}(\ldim^{\ldim+1}\, \ldim^{(\ldim+1)/2})$
% \mathcal{O}(\ldim^{3(\ldim+1)/2})$.

% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(\mathcal{M})/10$ then given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(\mathcal{M},g)$, the map $\varphi_2:(\mathcal{M},d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{\ldim}\eqdef \tilde{C}_{\ldim}/10$ and $\rdim\eqdef \#\widetilde{\mathbb{X}}$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{\ldim}
%         \,
%         \operatorname{Vol}(\mathcal{M},g)^{1/\ldim}
%     .
% \]
% Enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^\rdim$.
% We note that if $K$ is not aspherical but if it is only isometric to a closed Riemannian manifold, then the conclusion still holds, however, without this explicit upper bound on $\delta$.
% \item \label{step:GFM_2} \emph{Building the Feature Map with Well-posed Inverse.}
% Let $\varphi_1:(\mathcal{M},d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have postulated to exist.  Set $\smash{\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^\rdim}$ where, for $n=1,\dots,\rdim$ we define $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\smash{\varphi: C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^\rdim}$ by $\smash{y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^\rdim}$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^\rdim
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\varphi_1(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^\rdim
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^\rdim
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^\rdim
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $\mathcal{M}$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $\rdim$-dimensional Euclidean space.

% \item \label{step:GFM_3} \emph{Aligning to a Hyperplane in $\mathbb{R}^{\sdim}$ with a Shallow ReLU Neural Network.}
% Set $\sdim \eqdef \rdim+1$.  Let $b$ be the zero vector in $\mathbb{R}^{2\rdim}$.
% We now consider a variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $\rdim \times 2\rdim$ and $2\rdim\times \rdim$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_\rdim & ~ -I_\rdim
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_\rdim \\
%             -I_\rdim
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^\rdim\rightarrow \mathbb{R}^\rdim$, with $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^\rdim$.  Consider the $\sdim\times \rdim$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{\sdim}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_\rdim \\
%             0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,\rdim\\
%             1 & \mbox{ if } i=\sdim
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2\rdim$, $\|B\|_0=2\rdim$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \item \label{step:GFM_4} \emph{Injectivity of Softmax Function on Hyperplane.}
% Note that, for each $u\in \mathbb{R}^\rdim$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^\rdim$ onto the $\rdim$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^\rdim\}$ in $\mathbb{R}^{\sdim}$.  Observe that the Softmax function, given for any $u\in \mathbb{R}^{\sdim}$ by $\smash{\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^\rdim\,e^{u_k})_{j=1}^\sdim}$, maps $H$ surjectively and continuously onto the image set 
% \begin{align*}
%     \operatorname{Softmax}(\mathbb{R}^{\sdim})\subseteq \operatorname{int}(\Delta_\sdim)\eqdef \Big\{v\in [0,1]^{\sdim}:\,\sum_{i=1}^{\sdim}\,v_i=1\Big\}; 
% \end{align*}
% i.e.\ of the interior of the $\sdim$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{\sdim}) + 1\big)_{i=1}^{\sdim}
% \end{equation}
% consitutes a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{\sdim})$ then, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{\sdim})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$. 
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_\sdim)$ of the $\sdim$-simplex, then, 
% \begin{align*}
% 	 C^{\star}\eqdef \max_{u\in \Phi(K)}~\min_{v\in \Delta_{\sdim}\setminus \operatorname{int}(\Delta_{\sdim})}\,\|u-v\|>0.
% \end{align*}
%   Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{\sdim}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{\sdim})
%             +
%             \bar{\Delta}_{\sdim}
%         \}
% \]
% where $\bar{\Delta}_{\sdim}\eqdef (1/\sdim,\dots,1/\sdim)$ is the barycenter of the $\sdim$-simplex $\Delta_{\sdim}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{\sdim}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is locally Lipschitz on $\operatorname{int}(\Delta_\sdim)$, it is Lipschitz on the compact set $\Delta_{\sdim}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image since it is the composition of Lipschitz functions with Lipschitz inverses.  
% \item \label{step:GFM_5} \emph{Representation as an Attention Mechanism.}
% Set $\theta_0 = (A,B,a,b, \{y^{(n)}_{\cdot}\}_{n=1}^\rdim)$ and observe that the map $\Psi$ is of the form~\eqref{eq:sim_score}.  
% We continue by choosing a map of the form \eqref{eq:pos_encoding}. For this, let $\tdim \in \N$, set $\pdim \eqdef \sdim$ and let $U$ be the $\pdim \times \tdim$-dimensional zero matrix, and let $V$ be the $\pdim \times d_Y$-dimensional matrix whose entries are all equal to $1$.  Set $\theta_1\eqdef (U,V,\{n/{\pdim}\}_{n=1}^{\tdim})$.  Define the encoding dimension $\edim \eqdef \sdim$ and let $C$ be the $\edim \times \edim\cdot  d_Y$-dimensional matrix given by $Cx = (x_{n \cdot d_Y})_{n=1}^{\edim}$ for every $x\in \mathbb{R}^{\edim d_Y}$.  Set $\theta\eqdef (\theta_0,\theta_1,C)$ and observe that 
% \[
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot}) 
%     \eqdef
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
%     = 
%         \big(1_{[0:T]}\times \Psi\big)
%             (t,y_{\cdot})
% \]
% for each $y_{\cdot}\in K.$ and every $y\in [0:T]$. 
% Consequentially, $\operatorname{attn}_T^{\theta_{\cdot}}$ is a bi-Lipschitz embedding of $[0:T]\times K$ to $\mathbb{R}^{1 + \edim}$.  Note that $\|C\|_0= \pdim$, $\|U\|_0=0$, and $\|V\|_0= \pdim d_Y$.  Thus, $\|\theta\|_0\in \mathcal{O}(\pdim \cdot d_Y + \rdim)$.
% \end{enumerate}
% This concludes the proof.
% \end{proof}

% \begin{lemma}[Pathwise Attention Implements Stable Lossless Feature Maps -- Finite Case]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under \Cref{ass:reg_compact} \ref{ass:reg_compact_finite} and let $\rdim \eqdef \#K$.  
% Set $\edim=192\lceil\log(\rdim)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There is a parameter $\theta$ as in \Cref{defn:PathAttention} defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim}$ which restricts to a $(2^{-1/2},(3\rdim/6)^{1/2})$-bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{1+\edim},\|\cdot\|_2)$.

% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer}. 
% \end{lemma}
% \begin{proof}
% We argue similarly to the proof of \Cref{lem:Good_Feature_Map}, with only Steps \ref{step:GFM_1} and \ref{step:GFM_2} of its proof being replaced with the following argument.  
% \begin{enumerate}[label=\emph{Step \arabic*:}, ref=\arabic*]
% \item[\emph{Steps 1 and 2 (Modified): Building the Feature Map.}] 
% Enumerate $\smash{K=\{x_n\}_{n=1}^\rdim}$.  The map $\smash{\phi_1:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^\rdim,\|\cdot\|_{\infty})}$ given by $\smash{x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^\rdim}$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le \rdim^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^\rdim$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^\rdim,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^\rdim,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% Define $\sdim \eqdef \lceil48\,\ln(\rdim)\rceil$.
% By the Johnson-Lindenstrauss Lemma, with ``small'' constant given in the derivation of \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $4*48$ as opposed to $4*200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , exists a linear map $\phi_3:(\mathbb{R}^\rdim,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\sdim},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $\sdim \times \rdim$-matrix $A_0$, satisfying: For every $u,v\in \mathbb{R}^\rdim$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, the map $\varphi:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^{\sdim},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3\rdim/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_T
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         \rdim^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3\rdim/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_T 
% .
% \end{align*}
% \item[\emph{Remaining Steps.}]
% The rest of the proof is identical to Steps \labelcref{step:GFM_3,step:GFM_4,step:GFM_5}\footnote{Here $\sdim$ corresponds to $\sdim - 1$ in Step \ref{step:GFM_3}.} of the proof of \Cref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_\sdim\, \,I_\sdim)^{\top}$.
% \end{enumerate}
% This concludes the proof.
% \end{proof}


% \begin{lemma}[Pathwise Attention Implements Stable Lossless Feature Maps -- Linear Case]
% \label{lem:biLip_pw_lin}
% Fix $\pldim \in \mathbb{N}_+$, $0=t_0<\dots<t_\pldim=T$, and a constant $C_K>0$.
% Let $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact} \ref{ass:reg_compact_linear}. 
% Then, there is a parameter $\theta$, as in \Cref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim + 1}$, with $\edim \eqdef \pldim \cdot d_Y$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim + 1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0\in \mathcal{O}(\pldim \cdot d_Y)$.

% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[{Proof of \Cref{lem:biLip_pw_lin}}]
% Let $\rdim \in \N_+$, set $\sdim \eqdef \pldim$, and define $A, B$ as zero-matrices as well as $a, b$ as zero-vectors according to the dimensions in \Cref{defn:Sim_Score}.
% By fixing $\theta_0=(A,B,a,b)$, we observe that 
% \begin{align}
% \label{eq:bijection_samplingA}
%     \operatorname{sim}_T^{\theta_0}(y_{\cdot}) = 1 \in \R^{\pldim}
% \end{align}
% for all $y\in C([0:T],\mathbb{R}^{d_Y})$.  

% Set $\tdim \eqdef \pdim \eqdef \pldim$. Then, let $V$ be the zero matrix and $U$ the identity matrix according to the dimensions in \Cref{defn:PositionalEncoding}\footnote{The point $t_0$ is not sampled since every path $y_{\cdot}$ in $K$ satisfies $y_0=0$ and, thus, there is no need to sample it at time $0$.}. Set $\theta_1=(U,V,\{t_n\}_{n=1}^\pldim)$ and with that, 
% \begin{equation}
% \label{eq:bijection_samplingB}
%         \operatorname{pos}_T^{\theta_1}(y_{\cdot})
%     =
%         (y_1,\dots,y_\pldim).
% \end{equation}
% In particular, the map $\operatorname{pos}_T^{\theta_1}$ in \eqref{eq:bijection_samplingB} defines a linear bijection between $K$ and the set $B_{C_K}(0)^\pldim$, where $B_{C_K}(0) := \lbrace z \in \R^{d_Y} : \vert z \vert \leq C_K\rbrace$.  Since $B_{C_K}(0)^\pldim$ is a subset of the finite-dimensional Banach space $(\mathbb{R}^{\pldim \times d_Y},\|\cdot\|_2)$ and all norms on a finite-dimensional normed are equivalent, then, $\operatorname{pos}_T^{\theta_1}$ is a bi-Lipschitz embedding of $K$ into $(\mathbb{R}^{\pldim \times d_Y},\|\cdot\|_2)$.  

% Fix $\edim \eqdef \pldim \cdot d_Y$ and let $C$ be the $\edim \times \edim$-dimensional matrix with $C_{i,j}=1$ for $i,j=1,\dots,\edim$.  Set $\theta=(\theta_0,\theta_1,C)$.  By construction $\|\theta\|_0\in \mathcal{O}(\pldim \cdot d_Y)$.  
% Then, 
% \begin{equation}
% \label{eq:bijection_sampling__RelabelingStuff}
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot})
%     \eqdef 
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
%     =
%         \big(t,(y_1,\dots,y_\pldim)\big)
%     .
% \end{equation}
% Together, \labelcref{eq:bijection_samplingA,eq:bijection_samplingB} imply that $\operatorname{attn}_T^{\theta}$ defines a bi-Lipschitz embedding of $K$ into the $\edim+1$-dimensional Euclidean space.
% \end{proof}

% \begin{proof}[{Proof of \Cref{prop:Lossless_Encoding}}]
% Follows directly from \Cref{lem:Good_Feature_Map,lem:Good_Feature_Map__FiniteVariant,lem:biLip_pw_lin}.
% \end{proof}

% \subsection{Approximability of Locally Lipschitz Maps By DKFs - Proof of \texorpdfstring{\Cref{prop:Universal_Approximation_Theorem__PathToNd}}{Proposition 4}}
% We now prove our main universal approximation theorem, \Cref{prop:Universal_Approximation_Theorem__PathToNd}.  We show that the target space/codomain of any considered DKF is geometrically regular, in the sense of \cite{Acciaio2022_GHT,kratsios2023transfer}.  Using this fact, we then combine and apply the results of \cite{kratsios2021universal,kratsios2023transfer} to deduce the result.

% \subsubsection{Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}

% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d_X \in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d_X}$ denote the set of $d_X\times d_X$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d_X\times d_X$ matrices.\footnote{The $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d_X}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.}  Consider the $2$-product metric on $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ given for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d_X+d_X^2}\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ by sending any $(m,A)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ quantizes $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})^{N} \rightarrow 
% \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d_X^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is a barycentric QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[Proof of \Cref{lem:QAS_Space_Sym0d}]  
% We begin by showing that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% \begin{itemize}
%     \item[\emph{QAS Space Structure.}]
% Since $\operatorname{Sym}_{0,d_X}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ is a closed and convex subset of the normed linear space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ as sending any $(m,A)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         & d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big) \\
%     \notag
%     & \quad = 
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     & \quad = 
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     & \quad \le
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     & \quad \le
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     & \quad = 
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $\smash{(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F},\mathcal{Q},\eta)}$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \item[\emph{Barycentricity.}]
% Since $(\mathbb{R}^{d_X}\times \operatorname{Sym}_d,d_{2,F})$ is a normed linear space then \cite{BruHeinicheLootgieter1993} shows that the only contracting barycenter map is given by $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{d},d_{2,F})\ni \mathbb{P}\rightarrow \mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{d}$. 
% Since $\operatorname{Sym}_{0,d_X}$ is a closed convex subset of the normed linear space $\operatorname{Sym}_d$ then Jensen's inequality, as formulated in \citep[Theorem 10.2.6]{DudleyRealAnalysisandPRobabilityBook1989Revised2002}, implies that for each $\mathbb{P}\in \mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ we have $\mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$; where $\mathbb{E}_{X\sim \mathbb{P}}[X]$ denote the Bochner integral of a random variable with law $\mathbb{P}$.  Consequentially, 
% $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})\ni \mathbb{P}\rightarrow \mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ is a contracting barycenter map.  Thus, $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is barycentric metric space.

% \begin{comment}
% % Consider the map $\sigma:(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})^2\times [0,1]$ given for any $(m,A),(\tilde{m},B)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ and $t\in [0,1]$ by
% % \[
% %         \sigma\big(
% %             (m,A),(\tilde{m},B),t
% %         \big)
% %     \eqdef 
% %         \eta\big(
% %             (m,A),(\tilde{m},B),(t,1-t)
% %         \big)
% %     .
% % \]
% % Since geodesics in $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ are line segments, since $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ is a closed and convex subset of the inner-product space $(\mathbb{R}^{d_X}\times \operatorname{Sym}_d)$, with inner-product given by the product of the Euclidean and Frobenius inner-products, then clearly for each $(m,A),(\tilde{m},B)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ the map $t\mapsto \sigma\big((m,A),(\tilde{m},B),t\big)$ is a geodesic in the global NPC space, as defined in \citep[Definition 2.1]{Sturm_2003}, $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$.  Thus, $\sigma$ is a \textit{geodesic bicombing} in the sense of \citep[page 1]{basso2018fixed}.  Since 
% % \[
% %         \sigma\big(
% %             (m,A),(\tilde{m},B),1/2
% %         \big)
% %     =
% %         \sigma\big(
% %             (m,A),(\tilde{m},B),1/2
% %         \big)
% % \]
% % then \citep[Theorem 3.4]{basso2018fixed} applies; whence $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is barycentric with $1$-Lipschitz barycenter map explicitly given therein.  
% \end{comment}
% Since is a barycentric QAS space then, \citep[Setting 3.6 (iii)]{kratsios2023transfer} is satisfied.
% \end{itemize}
% \end{proof}

% We are now ready to prove the following result, as we have established the barycentricity and the QAS space structure of $(\mathbb{R}^{d_X}\times\operatorname{Sym}_{0,d_X}, d_{2,F},\eta,\mathcal{Q}_{\cdot})$, 
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying \Cref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^{d_X})$ satisfying \Cref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:[0:T]\times K \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ there is a map $\hat{g}: [0:T]\times C([0:T],\mathbb{R}^{d_Y}) \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ satisfying the uniform estimate
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K}\,
%         d_{2,F}(\hat{g}(t,y_{\cdot}),f(t, y_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{g}(t, y_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^\ddim\,
%                 P_{\Delta_\ddim}(\hat{f}\circ \operatorname{attn}^\theta(t, y_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $\ddim \in \mathbb{N}_+$, $m^{(1)},\dots,m^{(\ddim)}\in \mathbb{R}^{d_X}$, $A^{(1)},\dots,A^{(\ddim)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_\ddim}:\mathbb{R}^\ddim\rightarrow\Delta_\ddim$ is the Euclidean (orthogonal) projection onto the $\ddim$-simplex, and an MLP $\hat{f}:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with activation function $\sigma$.  The depth, width, encoding dimension ($\edim$), and decoding dimension ($\ddim$) are recorded in \Cref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{\ldim}\operatorname{Vol}(M,g)^{1/\ldim})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \scriptsize
%     \caption{{Complexity Estimates for transformer-type model $\hat{g}$ in \Cref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-\edim-1}\,\varepsilon^{-\edim-1}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-\edim-1}\,\varepsilon^{-\edim-1}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4\edim+5}\, \varepsilon^{-4\edim-5}
%         \right)
%          $
%          &
%          $ \mathcal{O}(L\epsilon^{-1} + \edim +3)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8\edim+14}\, \varepsilon^{-8m-14} %m=(\edim-1)
%         \big)
%          $
%          & 
%          $\mathcal{O}(L\epsilon^{-1} + \edim +4)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $\mathcal{O}(L\epsilon^{-1} + \edim +3)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of \Cref{lem:approximation_Sym}}]
% %\anastasis{Relabel $N$ (index) as $M$}
% %\hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% Our objective is to apply \citep[Theorem 3.7]{kratsios2023transfer} by verifying each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \begin{enumerate}[label=\emph{Step \arabic*:}]
%     \item \emph{Implementing a Bi-Lipschitz Feature Map with the Attention Layer.}
%         \begin{remark}
%             We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap}  can be chosen such that $\operatorname{attn}^\theta$ is a suitable feature map.  
%         \end{remark}

%         When convenient, let $\operatorname{attn}^{\theta}$ be as in either of \Cref{lem:Good_Feature_Map,lem:Good_Feature_Map__FiniteVariant,lem:biLip_pw_lin} depending on which assumption of Assumptions~\ref{ass:reg_compact} (i), (ii), or (iii) holds.  For convenience, we denote the map $\operatorname{attn}$ by $\varphi$.  These lemmata show that the map $\varphi$ is a bi-Lipschitz embedding of $([0:T]\times K,\|\cdot\|\times \|\cdot\|_T)$ into a Euclidean space $(\mathbb{R}^N,\|\cdot\|_2)$.
    
%         We also observe that every bi-Lipschitz map is a quasi-symmetric map\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.  Thus, \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(\mathcal{M},d_g)$ is a doubling metric space, as defined on \citep[page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  Thus, $([0:T]\times K,\|\cdot\|\times \|\cdot\|_T)$ is a doubling metric space.  We have thus verified \citep[Setting 3.6 (i)]{kratsios2023transfer}.
%     \item \emph{Feature Space Geometry.}
%         Since the codomain of $\phi$ is simply a Euclidean space, then, the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^{\edim+1}}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^{\edim+1}$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^{\edim+1}$, 
%         \[
%             \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
%         \]
%         and the operator norm $\|1_{\mathbb{R}^{\edim+1}}\|_{\mathrm{op}}=1$. Thus, $(T^i)_{i\in \mathbb{N}}$ implements the $1$-BAP ($1$-bounded approximation property) on $\mathbb{R}^{\edim+1}$ for every $i$.  Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} holds.

% \item \emph{Geometry of $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$.}
% \Cref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is barycentric and it is a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $\ddim \in\mathbb{N}_+$, $u\in \mathbb{R}^\ddim$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(\ddim)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d_X^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^\ddim
%     \big)
%         \eqdef 
%             \sum_{n=1}^\ddim\,
%                 P_{\Delta_\ddim}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \item \emph{Determining The Euclidean Universal Approximator.}
% \begin{remark}
%     We now verify that the class of all MLPs with activation function $\sigma$ satisfying \Cref{ass:KLCondition}, thus assumption \citep[Setting 3.6 (iv)]{kratsios2023transfer} holds.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.
% \end{remark}
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $\edim,\ddim,c\in \mathbb{N}_+$ let $\mathcal{F}_{\edim, \ddim, c}$ denote the family of maps $f:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le \edim+\ddim+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy \Cref{ass:KLCondition} then by \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $\edim,\ddim,c\in \mathbb{N}_+$ let $\mathcal{F}_{\edim,\ddim,c}$ denote the family of maps $f:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \item \emph{Applying \citep[Theorem 3.7]{kratsios2023transfer}.}
% Steps $1$ though $5$ verify that the conditions of \citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the feature decomposition $\{([0,T]\times K,\varphi)\}$ of $([0,T]\times K,\|\cdot\|_T)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, by~\citep[Lemma 5.10]{kratsios2023transfer} for every $\varepsilon>0$ there is a map $\hat{F}:[0,T]\times K\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{F}(y_{\cdot})
%     = &
%         \beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot}),(Z_n)_{n=1}^\edim)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot}),(Z_n)_{n=1}^\edim)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^\ddim
%             \,
%                 \big(
%                     P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $y_{\cdot}\in K$ satisfying 
% \[
%     \sup_{y_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{F}(y_{\cdot})
%         ,
%             f(y_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\smash{\beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ (which exists by \Cref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}$ is a right-inverse of the map $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})$, where $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially, \labelcref{eq:transformer_pre_mapped_BEGIN,eq:transformer_barycentercancellation,eq:transformer_pre_mapped_END} reduces to \eqref{lem:approximation_Sym__approximation___representation}.  


% \item \emph{Tallying Parameters.}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $\edim=\mathcal{N}_{\operatorname{pack}}\big(K,C_{\ldim}\,\operatorname{Vol}(\mathcal{M},g)^{1/\ldim}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in \Cref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $\ddim$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             \ddim
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{enumerate}
% This concludes the proof.
% \end{proof}

% \subsubsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool, namely, \Cref{prop:Universal_Approximation_Theorem__PathToNd}.   
% %\begin{figure}[H]
% %    \centering
% %    \begin{tikzcd}
% %\big(C([0:T],\mathbb{R}^d), %\|\cdot\|_{\infty}\big) & %(\mathcal{P}_2(\mathbb{R}^d),
% %\mathcal{W}_2) \\
% %    (K,\|\cdot\|_{\infty}) 
% % \arrow[hookrightarrow{u}
% %{\iota} 
% %    \arrow{r}{f, \hat{t}} 
%     % \arrow[swap]{d}{\varphi} 
% %    \arrow{dr}{\varrho\circ f}
% % & ({\mathcal{N}}_d,
% %\mathcal{W}_2) 
% %   \arrow[hookrightarrow]{u}{i}
% %    \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
% %    & (\mathbb{R}^d\times \operatorname{Sym}_{0,d_X},\|\cdot\|\times \|\cdot\|_F)
% %    \end{tikzcd}
% %    \caption{Visual summary of the relationship between the spaces appearing in the proof of Proposition 4.}
% %\label{fig:Approximation_Theorem}
% %\end{figure}


% \begin{proof}[{Proof of \Cref{prop:Universal_Approximation_Theorem__PathToNd}}] \hfill
% \begin{enumerate}[label=\emph{Step \arabic*:}]
% \item \emph{Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$.}
% By \Cref{lem:LipschitzManifold_Nd}, the map $\varrho:(\mathcal{N}_{d_X},\mathcal{W}_2)\rightarrow (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^{d_X},\operatorname{Sym}_{0,d_X},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d_X},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous, then the map
% \[
%     g: ([0,T]\times K, 
%     | \cdot | \times \|\cdot\|_T)\ni (t,y_{\cdot}) \mapsto 
%     \pi\circ \varrho\circ f(t,y_{\cdot})
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d_X},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d_X \times d_X$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; by which we mean that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_{d_X}$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% By \Cref{lem:LoewnerBound}, we have that there is an $r>0$ such that $r=\lambda_{\operatorname{min}}(\Sigma_t)$ for all $0\le t\le T$. 
% Consequentially, \Cref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_{d_X},\mathcal{W}_2)\rightarrow (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \item \emph{Approximating $\varrho \circ f$ on $K$.}
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%     \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
%                     }}
%         \biggr\}
% .
% \end{equation}

% We apply \Cref{lem:approximation_Sym} to deduce that there exists a map $\hat{F}: [0:T]\times K \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K }\,
%         d_{2,F}(\hat{F}(t, y_\cdot),\varrho\circ f(t,y_\cdot))
%     <
%         \delta
% .
% \end{equation}
% Since \Cref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  
% Consider the $1$-thickening of $\varrho\circ f(K)$ defined by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}:\,(\exists (t,y_{\cdot} )\in [0:T]\times K )\, d_{2,F}(f(t, y_\cdot),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{F}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate} and \Cref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         \mathcal{W}_2\big(
%                 \rho^{-1}\circ F(t,y_{\cdot})
%             ,
%                 f(t,y_{\cdot})
%         \big)
% = & 
%     \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{F}(t,y_{\cdot})
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(t,y_{\cdot})
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         d_{2,F}\big(
%                 \hat{F}(t,y_{\cdot})
%             ,
%                 \varrho\circ f(t,y_{\cdot})
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
% \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
%     }
%     }
% \\
% % \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% % \le &
% %     \sqrt{d}2\sqrt{
% %             L
% %     \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
% %         }
% %     \,
% %     \varepsilon
% %     \,
% %     \frac1{
% %     \sqrt{d}2\sqrt{
% %         L
% % \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
% %     }
% %     }
% % \\
% \label{eq:Approxim_LEMMA__END}
% \le & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from \Cref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:Approxim_LEMMA__END} followed from the estimate~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho} for $\operatorname{Lip}( \varrho^{-1}  | \bar{B}_1 )$.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009} then, the estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% %\label{eq:Approxim_LEMMA__BEGIN}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K}\,
%         \mathcal{W}_p\big(
%                 \hat{F}(t,y), f(y)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \item \emph{Counting Parameters.}
% Using $\delta$, as defined in~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in \Cref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \end{enumerate}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_{d_X}}$ denote the set of Gaussian measure on $\mathbb{R}^{d_X}$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_{d_X}}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_{d_X}}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_{d_X}},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_{d_X}}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of \Cref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_{d_X}}$ sending any $(m,A)\in \mathbb{R}^{d_X}\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_{d_X}}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_{d_X}}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_{d_X}}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_{d_X}}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_{d_X}}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_{d_X}},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_{d_X}}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_{d_X}}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}


% \appendix
% \section{An Auxiliary Lemma - I.\ Pinelis}
% \label{s:AuxLemmata}
% This section records an auxiliary lemma due to Iosif Pinelis, \cite{LocalLipschitz_Pinelis}.  We include the result and its proof here for self-contentedness.  
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% then the following lower-bound holds
% \begin{align*}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     .
% \end{align*}
% Moreover, the following upper-bound also holds
% \begin{align*}
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{align*}
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}[{Proof of \Cref{lem:LipschitzManifold_Nd}}]
% By \citep[Proposition 7]{GivensShortt_ClassofWassersteinMetricforProbDists_1984} the $2$-Wasserstein distance between $\mathcal{N}(m^{(1)},A)$ and $\mathcal{N}(m^{(2)},B)$ satisfies
% \begin{equation*}
% 	\mathcal{W}_2(\mathcal{N}(m^{(1)},A),N(m^{(2)},B))=\sqrt{\|m^{(1)}-m^{(2)}\|^2+W_2(\mathcal{N}(0,A),N(0,B))^2}.
%  \label{10}
% \end{equation*}
% Thus, $\|m^{(1)}-m^{(2)}\|\le \mathcal{W}_2(N(m^{(1)},A),N(m^{(2)},B))$.  Moreover, for any unit vector $u\in\R^n=\R^{n\times1}$ we have
% \begin{align*}
% 	\mathbb{E}_{X\sim \mathcal{N}(0,A),\,Y\sim \mathcal{N}(0,B)}\|X-Y\|^2
%     \ge &
%         \mathbb{E}_{X\sim \mathcal{N}(0,A),\,Y\sim \mathcal{N}(0,B)}(u^\top X-u^\top Y)^2
%     \\
%     \ge& 
%         (\sqrt{u^\top A u}-\sqrt{u^\top B u})^2,
% \end{align*}
% where the last inequality holds (say, by mentioned \citep[Proposition 7]{GivensShortt_ClassofWassersteinMetricforProbDists_1984}) because $u^\top X$ and $u^\top Y$ are real-valued Gaussian zero-mean random variables respectively, if $X\sim Y\sim \mathcal{N}(0,A)$ and $Y\sim \mathcal{N}(0,B)$, with variances $u^\top A u$ and $u^\top B u$. 
% By \eqref{10}, for any unit vector $u\in\R^n=\R^{n\times1}$, we have
% \begin{equation*}
% \begin{aligned}
% 	\mathcal{W}_2(\mathcal{N}(a,A),\mathcal{N}(b,B))&\ge \mathcal{W}_2(N(0,A),N(0,B)) \\ 
% 	&\ge|\sqrt{u^\top A u}-\sqrt{u^\top B u}| \\ 
% 	&=\frac{|u^\top A u-u^\top B u|}{\sqrt{u^\top A u}+\sqrt{u^\top B u}} \\ 
% 	&\ge\frac{|u^\top(A-B)u|}{\sqrt{\|A\|}+\sqrt{\|B\|}} \\  
% 	&=\frac{\|A-B\|}{\sqrt{\|A\|}+\sqrt{\|B\|}} 
% \end{aligned}
% \end{equation*}
% for some unit vector $u\in\R^n=\R^{n\times1}$, where $\|M\|$ is the spectral norm of a matrix $M$. 
% So, 
% \begin{equation*}
% 	\|A-B\|\le(\sqrt{\|A\|}+\sqrt{\|B\|\,})\, \mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B)). \label{30}
% \end{equation*}
% The conclusion now follows from $\|m^{(1)}-m^{(2)}\|\le \mathcal{W}_2(N(m^{(1)},A),N(m^{(2)},B))$,~\eqref{30}, and the observation that $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$ where 
% \[
% \|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})
% \]
% denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}


% \bibliographystyle{imsart-number} 
% \bibliography{Bookkeaping/2_References}


% \end{document}




==> OLD/Historical_Versions/2023_09_15.tex <==
% % https://mcmaster.zoom.us/j/2601491351


% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% \documentclass[preprint,12pt,authoryear]{elsarticle}
% \usepackage{amssymb}

% \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}



% \begin{document}

% \begin{frontmatter}
% \title{Deep Kalman Filters Can Filter}
% % \title{Deep Kalman Filters Are Approximately-Optimal Stochastic Filters}

% % \author[inst1]{Matheus Grasselli}
% \author[inst2,inst3]{Blanka Horvath}
% \author[inst1,inst4]{Anastasis Kratsios}
% \author[inst2,inst3]{Yannick Limmer}
% \author[inst1]{Xuwei Yang}


% \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
%             % addressline={Hamilton, Ontario}, 
%             city={Hamilton},
%             % postcode={00000}, 
%             % state={Ontario},
%             country={Canada}}

% \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             % state={Oxfordshire},
%             country={United Kingdom}}

% \affiliation[inst3]{organization={Oxford-MAN Instute for Quantitative Finance, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             % state={Oxfordshire},
%             country={United Kingdom}}
            
% \affiliation[inst4]{organization={Vector Institute},
%             % addressline={Address Two}, 
%             city={Toronto},
%             % postcode={22222}, 
%             % state={Ontario},
%             country={Canada}}
            

% \begin{abstract}
% Deep Kalman filters (DKFs) are a class of neural network models that generate Gaussian probability measures from sequential data.  Though DKFs are inspired by the Kalman filter, they lack concrete theoretical ties to the stochastic filtering problem, thus limiting their applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-times measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  
% \end{abstract}


% \begin{keyword}
% %% keywords here, in the form: keyword \sep keyword
% Stochastic Filtering \sep Conditionally Gaussian Processes \sep Geometric Deep Learning
% %% PACS codes here, in the form: \PACS code \sep code
% % \PACS 0000 \sep 1111
% %% MSC codes here, in the form: \MSC code \sep code
% %% or \MSC[2008] code \sep code (2000 is the default)
% \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% \end{keyword}

% \end{frontmatter}


% \section{Introduction}
% \label{s:Introduction_Deep_Filtering}

% % \byyan{Opening.}\hfill\\
% In several scientific problems, especially in mathematical finance, one is typically interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$; both of which have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0,T]},\mathbb{P})$.  For example, market sentiment impacts market prices, however, only the latter of these two can be reliably measured.  The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is for any time $t>0$ to identify a continuous function $f_t:C([0,t],\mathbb{R}^d)\rightarrow \mathcal{P}(\mathbb{R}^D)$ satisfying 
% \begin{align}
%     \label{goal:Robust_Filtering}
%         f_t(y_{[0:t]})
%     =
%         \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)
%     ,
% \end{align}
% conditioned on any continuous path $y_{[0:t]}$ realized the $d$-dimensional observable process $Y_{\cdot}$ up time $t>0$; where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $D$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0,t]}$.  The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^D$, denoted by $\mathcal{P}(\mathbb{R}^D)$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^d$, denoted by $C([0,t],\mathbb{R}^d)$, with the uniform norm. 

% % \byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
% When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^d)$.  These robust representations are particularly invaluable in mathematical finance where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

% % \byyan{Do Optimal Filters Exist?.}\hfill\\
% In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,Sirjaev1965Filtering,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued processes, make the problem computationally intractable.  

% % \byyan{Computational Challenges}\hfill\\
% The exception to this rule is so-called finite-dimensional filters, which are rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

% % \byyan{Numerical Approaches.}\hfill\\
% The intractability of the computational general filtering problem has the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} when it admits a square-integrable density.  The latter two approaches work well if the coupled system $(X_{\cdot},Y_{\cdot})$ follows the postulated dynamics, and the former particle-filtering approach is well-suited to low-dimensional settings.  

% % \byyan{Why Deep Learning?.}\hfill\\
% The ability of deep neural networks to efficiently solve a variety of problems has inspired the use of deep learning approaches to the numerical stochastic filtering problems; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering}, and the development of measure-valued deep learning models; e.g.~\cite{Acciaio2022_GHT}.  In particular, the need for a more generic approximate stochastic filtering toolbox has motivated the deep learning community to introduce deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, which is the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered model, are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem.  

% This paper constructs a DKF model which can uniformly approximate the map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering}, to arbitrary precision, for any pair of non-Markovian $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0,T]}$-adapted \textit{conditionally Gaussian} stochastic processes studied by \cite{LipShiryaev_II_2001}.  
% %%%%
% %%%%
% %%%%
% \begin{InformalTheorem}[The DKF is a Universal Conditionally-Gaussian Robust Filter]
% \label{Informal_Theorem_Main:Informal_Theorem}
% Fix $t>0$ and let $(X_{\cdot},Y_{\cdot})$ be the partially-observed system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} below, subject to mild regularity conditions.  For any suitable compact subset $K\subseteq C([0:t],\mathbb{R}^d)$, and any approximation error $\varepsilon>0$ there exists a DKF model $\hat{f}:C([0:t],\mathbb{R}^d)\rightarrow \mathcal{N}_d$ satisfying
% \[
%         \sup_{y_{[0:t]}\in K}\,
%             \mathcal{W}_2\big(
%                 f(y_{[0:t]})
%             ,
%                 \hat{f}(y_{[0:t]})
%             \big)
%     <
%         \varepsilon
%     .
% \]
% \end{InformalTheorem}
% %%%%
% %%%%
% %%%%
% Our uniform estimates hold for coupled stochastic differential equations governed by
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% % \tag{Sig}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% % \tag{Obs}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
% We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$, of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% \subsection{The Deep Kalman Filter Model}
% \label{s:Introduction_Deep_Filtering__ss:ModelDetails}
% The proposed deep Kalman filter (DKF), illustrated in Figure~\ref{fig:DKFModel}, generates predictions on the finite-dimensional metric space $(\mathcal{N}_d,\mathcal{W}_2)$ whose points are non-singular Gaussian measures, and whose distance between points is quantified by the $2$-Wasserstein distance.  These predictions are generated from the continuous input paths via the following three-phase process.  
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
%     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
%     \label{fig:DKFModel}
% \end{figure}
% \paragraph{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^d)$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% \paragraph{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% \paragraph{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_d$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.

% \paragraph{Organization of Paper}
% Section~\eqref{s:Setting} formalizes the basic required regularity conditions on the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} and it overviews the required background in optimal transport.  Section~\ref{s:Model} rigersouly introduces the relevant DKF model.  Section~\ref{s:Main_Results} contains the paper's main theoretical results, as well as an overview of the proof methodology.  Several results of independant interest, both concerning the approximation capacity of the DKF model and the local Lipschitz regularity of the robust filtering map~\eqref{goal:Robust_Filtering} are discussed.  Detailed proofs of our results are relegated to Section~\ref{s:Proof}. 

% \section*{Notation}
% % \label{s:Notation}
% \noindent This section serves as a reference, which records the notation used throughout our manuscript.  In what follows, $N,I,J\in \mathbb{N}_+$, $A$ is an arbitrary $I\times J$ matrix, $x,x_1,\dots,x_J\in \mathbb{R}^N$, $f$ is an arbitrary real-valued function on $\mathbb{R}$, and $t\in \mathbb{R}$.
% \begin{enumerate}
%     \item \textbf{Componentwise Composition:} $f\bullet x\eqdef (f(x_n))_{n=1}^N$ for any $N\in \mathbb{N}_+$.%, $x\in \mathbb{R}^N$, and $f:\mathbb{R}\rightarrow \mathbb{R}$.
%     \item \textbf{Rectified Linear Unit (ReLU):} $\operatorname{ReLU}:\mathbb{R}\rightarrow\mathbb{R}$ given by $\operatorname{ReLU}(t)\eqdef \max\{0,t\}$.
%     \item \textbf{Rowwise Product:} $v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}$.% for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
%     \item \textbf{Softmax Function:} $\operatorname{Softmax}(x)\eqdef \big(e^{x_n}/\sum_{i=1}^N\,e^{x_i}\big)_{n=1}^N$.% for any $N\in \mathbb{N}_+$ and any $x\in \mathbb{R}^N$.
%     \item \textbf{Sparsity:} $\|(A_{i,j})_{i,j=1}^{I,J}\|_0\eqdef \#\{A_{i,j}\neq 0:\,i,j=1,\dots,I\}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
%     \item \textbf{Vector Concatenation:} $\oplus_{j=1}^N x_j\eqdef (x_1,\dots,x_J)^{\top}$ is the $J\times N$-matrix whose $j^{th}$ row is $x_j$.%, for $j=1,\dots,N$.
%     \item \textbf{Vectorization:} $\operatorname{vec}((A_{i,j})_{i,j=1}^{I,J})\eqdef (A_{1,1},\dots,A_{I,J})$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
% \end{enumerate}

% \section{The Setting}
% \label{s:Setting}
% This section formalizes the setting in which our analysis takes place.  We begin by specifying the dynamics of the stochastic processes in the filtering problem.  Next, the source space of paths considered is introduced.  Subsequently, we formulate the target space of probability measures wherein the optimal filter lies.

% \subsection{Regularity Conditions on the Partially-Observed System}
% % \label{s:Preliminaries__ss:Dynamics}
% % This section formulates the theoretical problem which this paper addresses.
% % % Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% % % Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  
% % These processes evolve according to the coupled dynamics
% % \begin{align}
% % \label{eq:filtering_dynamics__signal}
% % dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% % \label{eq:filtering_dynamics__observation}
% % dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% % \end{align}
% % where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.
% % 
% % 
% % Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% % \begin{align}
% % \label{id:ConditionalDistribution}
% %     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) 
% % \end{align}
% % where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of the theoretical foundations of DKFs.
% % \begin{question}
% % \label{question:main}
% % Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$?
% % \end{question}
% During our analysis, we maintain the following basic regularity assumptions on the dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
% %%
% \begin{assumption}[Regularity Conditions: Dynamics]
% \label{ass:technical_evolution_conditions}
% We will assume the following uniform bounds:
% \begin{align*}
%     \vert \process{a_1}{t, x}{i, j}\vert \le L
%     \mbox{ and }
%     \vert \process{A_1}{t, x}{k, j}\vert \le L
% \end{align*}
% for $x \in C([0:t], \R^{d_Y})$, $t \in [0:T]$, $i,j=1,\dots,d_X$, and $k=1,\dots,d_Y$.  
% Further, we require the following integrability conditions:\footnote{In particular, the integrability conditions imply that $\bE\bigg[\sum_{j = 1}^{d_X}(X_0)_j^4\bigg] < \infty$.}
% \begin{enumerate}
%     \item[(i)] $\int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item[(ii)] $\int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item[(iii)] $\int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt < \infty$,
%     \item[(iv)] $\int_0^T (\process{b_2}{t, y_{[0:t]}}{i, k})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{k, i})^2 dt < \infty$
%     \item[(v)] $\int_0^T (\process{A_0}{t, y_{[0:t]}}{k})^2 + (\process{B_2}{t, y_{[0:t]}}{k, l})^2 dt < \infty$
% \end{enumerate}
% hold for $i,j=1,\dots,d_X$, and $k,l=1,\dots,d_Y$ and all paths $y_{[0:T]} \in C([0:T], \R^{d_Y})$.  We require that the matrix $B \circ \process{B}{t,x}{}  \eqdef  \process{B_1}{t,x}{} \process{B_1}{t,x}{}^\intercal + \process{B_2}{t,x}{} \process{B_2}{t,x}{}^\intercal$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% \begin{enumerate}
%     \item[(vi)] $\vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%         \le
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2$,
%     \item[(vii)] $(B_k)_{i,j}(t, x)^2  
%         \le 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2)$,
%     \item[(viii)] $\int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt < \infty$,
%     \item[(ix)] $\bE[\vert (X_t)_j \vert] < \infty, \quad \forall t \in [0:T]$,
%     \item[(x)] $\bP\left( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \right) = 1$
% \end{enumerate}
% for indices $i=1,\dots,d_Y$ and $j=1,\dots,d_X$, where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$.  Lastly, we require that the covariance matrix $\Sigma_0$ is positive definite.\anastasis{where is $\Sigma_0$ defined?}
% \end{assumption}
% \begin{comment}
% Moreover, under mild regularity conditions ensuring that $f$ is sufficiently continuous the geometric deep learning results of \cite{kratsios2021universal} and \cite{Acciaio2022_GHT} guarantee that it can be approximated with a class of transformer models.  However, their analysis equally reveals that the required number of parameters to approximate each $f_t$ can depend highly non-favourably on the dimensions $d_X$ and $d_Y$, as a function of the local uniform approximation error, if nothing is assumed of $f_t$.  In these results, the \textit{uniform} (on compact sets) approximation of the probability measure-valued functions $f_{t}$ by a sequential learning model $\hat{f}_t$ \anastasis{dets later} is quantified by
% \[
%     \sup_{y_{[0:T]}\in K}\, \sup_{0\le t\le T}\,
%         \mathcal{W}_2\big(f_t(y_{[0:t]},\hat{f}_t(y_{[0:t]})\big)
%     ,
% \]
% where $K$ is a (non-empty) compact subset of the path-space $\dots$.  \anastasis{Make comment about adapted Wasserstein when predicting multiple steps forward it time.}
% \end{comment}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Setting__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^d)$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^d$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^d$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically\footnote{dets later; obvious.} embed any path $f\in C([0:t],\mathbb{R}^d)$ into a path $F\in C([0:T],\mathbb{R}^d)$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     F(s)\eqdef \begin{cases}
%         f(s) &: \mbox{ if } 0\le s \le t\\
%         f(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $f\mapsto F$ is a linear isometric embedding of the Banach space $C([0:t],\mathbb{R}^d)$ into $C([0:T],\mathbb{R}^d)$ since
% \[
% \|F\|_T = \max_{0\le s\le T}\, \|f(s)\|_2
% = \max_{0\le s\le t}\, \|f(s)\|_2 = \|f\|_t, 
% \]
% since $f(s)=f(t)$ for all $t<s\le T$.  Conversely, the restriction $F_{[0:t]}$ of a path $F\in C([0:T],\mathbb{R}^d)$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^d)$ to $C([0:t],\mathbb{R}^d)$ since
% \[
%         \|F_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|F_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|F_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|F(s)\|_2 
%     =
%         \|F\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^d)$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot by approximated by standard deep neural networks parameterized determined by a number trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing} for general rates.   

% The curse of dimensionality cannot be broken, by can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space, as is the case in our results, shows that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}, however, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are either isometric to some compact Riemannian manifold or they are comprised of piecewise linear paths with finitely many pieces.  In particular, we exclude fractal-like subsets of the path space $C([0:T],\mathbb{R}^d)$ which needn't be compressible into finitely many dimensions without ``loosing information'' (i.e.\ for which there is no bi-Lipschitz embedding into a finite-dimensional normed space).  

% In what follows, we denote the Riemannian volume of a connected $(C^2)$ Riemannian manifold $(M,g)$ by $\operatorname{Vol}(M,g)$.  We denote its geodesic distance function by $d_g$.
% \begin{assumption}[Domain Regularity]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^d)$ and a ``latent dimension $D_K\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}
%     \item[(i)] \textbf{Finite Domains:} $K$ is finite,
%     \item[(ii)] \textbf{Smooth Domains:} There exists a compact and connected $D_K$-dimensional Riemannian manifold $(M,g)$ for which $(M,d_g)$ is isometric to $(K,\|\cdot\|_T)$,
%     \anastasis{I think, I can do a bit better here, and get a compact subset of ...}
%     \item[(iii)] \textbf{Piecewise Linear Domains:} There are $N\in \mathbb{N}_+$, $0=t_0<\dots<t_N=T$, and $C_K>0$ such that $y_{\cdot}\in K$ if and only if:
%         \begin{enumerate}
%             \item[(a)] For $i=0,\dots,N-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^d$ satisfying
%             \[
%             \begin{aligned}
%                 & y(t)=A^{(i)}\,t+b^{(i)}
%                 \,
%                 &
%                 \,
%                 \mbox{ for all } t\in (t_i,t_{i+1})
%             ,
%             \end{aligned}
%             \]
%             \item[(b)] $y_0=0$,
%             \item[(c)] $\max_{i=1,\dots,N}\,|y(t_i)|\le C_K$.
%         \end{enumerate}
% \end{enumerate}
% \end{assumption}
% Evidently, their domains $K$ satisfying Assumption~\ref{ass:reg_compact} (i) are easily exhibited, and they correspond to any \textit{training set}.  One can interpret results in this case as paralleling interpolation results for deep learning, e.g.\ \cite{CristaJosefMartin_2020_UnivInterpol,vershynin2020memory,KratsiosDevarnotDokmanic_SmallTransformers_JMLR2023}, but allowing for some arbitrarily small error as in \cite{park2021provable}.

% Compact subsets of the path-space $C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact} (ii) are also plentiful.  The following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}, and related results such as~\cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}, illustrate this by guaranteeing that $C([0:T],\mathbb{R}^d)$ contains isometric copies of any compact metric space.  Consequentially, $C([0:T],\mathbb{R}^d)$ contains isometric copies of any compact and connected Riemannian manifold.
% \begin{proposition}[Isometric Copies of Every Compact Riemannian Manifold in The Path Space]
% \label{prop:Non_Vaccousness}
% Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^d)$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}

% We obtain explicit estimates for the case where $(K,d_{\cdot})$ satisfies Assumption~\ref{ass:reg_compact} (ii), if the ``model'' smooth manifold $M$ is topologically regular, in that sense that it is \textit{aspherical}.
% This means that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$ (see \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups).  E.g.\ $M$ can be a Torus.

% Domains $K$ satisfying Assumption~\ref{ass:reg_compact} include any piecewise linear interpolation of real-world financial time-series data, or simulated data.  This is because only a finite number of inflection points can be observed, and prices are not unbounded.  

% In this way, Assumption~\ref{ass:reg_compact} summarizes a rich family of compact subsets of the path-space $C([0:T],\mathbb{R}^d)$ which possess a sufficient degree of structure to be losslessly encoded into finitely many dimensions by our model's encoding layer, called its \textit{pathwise attention mechanism}.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Setting__ss:OutputSpace}

% The $2$-Wasserstein space $\mathcal{P}_2(\mathbb{R}^d)$ consists of all probability measures on $\mathbb{R}^d$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_2(\mathbb{R}^d)$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^2]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_2$ on $\mathbb{P}_2(\mathbb{R}^d)$ is given by minimizing the opimtal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_2(\mathbb{P}, \mathbb{Q})^2
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
%     .
% \]
% Generally, the $2$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, the $2$-Wasserstein distance is not always computationally in tractable and in the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite{dowson1982frechet} showed that it admits the following closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^d)$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^d)$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% % This section introduces our attention-based model, our deep Kalman filter (DKF) model, illustrated in Figure~\ref{fig:DKFModel}.  The proposed DKF generates a prediction on the space $(\mathcal{N}_d,\mathcal{W}_2)$ from any observed continuous path in $C([0:T],\mathbb{R}^d)$, via a three-phase process.  

% % \begin{figure}[hpt!]%[H]%
% %     \centering
% %         \centering
% %         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
% %     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
% %     \label{fig:DKFModel}
% % \end{figure}

% % \paragraph{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^d)$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% % \paragraph{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% % \paragraph{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_d$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.


% \subsection{Phase 1 - Encoding via Pathwise Attention}
% \label{s:Model__ss:PathwiseAttention}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and the graph attention mechanism of \cite{velivckovic2017graph} to the context of continuous-time path sources/inputs.  Our attention mechanism, called \textit{pathwise attention}, encodes key information about a novel path $y_{\cdot}$ and like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``know/previously generated paths''.  

% \begin{figure}[hpt!]%[H]%
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.9\linewidth]{Graphics/Similarity_Score.pdf}
%         \caption{\label{fig:Similarity_Score} The \textit{similarity score} component $\operatorname{sim}_t^{\theta_0}$ encodes a path into finite-dimensional vectorial data, by relating its similarity to a dictionary of previously observed ``contextual paths''.}  
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.9\linewidth]{Graphics/Positional_Emcoding.pdf}
%         \caption{\label{fig:PositionalEncoding} The \textit{positional encoding} component $\operatorname{pos}_t^{\theta_0}$ of the attention mechanism allows the similarity scores to further adapt to any novel path by extracting sample-positions on the novel paths.}
%     \end{subfigure}
%     \caption[1]{Our \textit{pathwise attention mechanism} $\operatorname{attn}_t^{\theta}$, in Definition~\ref{defn:PathAttention}, relies on two methods for adaptive feature extraction.  The first component of the mechanism, in~\ref{fig:Similarity_Score}, in is a similarity score which ranks the similarity of any novel path $x_{\cdot}$ to a dictionary of ``recognized/saved'' reference paths.  The second component of the mechanism, in~\ref{fig:PositionalEncoding}, samples points on the novel path $x_{\cdot}$ and perturbs the similarity scores by them.  The adeptness of the pathwise attention mechanism, unlike basis-based methods, is rooted in the fact that nearly all of its the parameters are trainable, which allows it to be tasks-specific (similarly to the advantage of deep MLPs have over regression via basis-functions).}
%     \label{fig:Attention_Is_All_You_Need}
% \end{figure}


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $N$, $N_1$, $d$, and a ``time horizon'' $t> 0$.  
% Given a set of $N$ distinct paths $\{y^{(n)}\}_{n=1}^N$ in $C([0,1],\mathbb{R}^d)$, a $B$ is an $N_1\times N$-matrix, $b\in \mathbb{R}^{N_1}$, $A$ is an $N_1\times N_1$-matrix, and $a\in \mathbb{R}^{N_1}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^N)$.\\
% \noindent The \textit{similarity score}, is a map $\operatorname{sim}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$ by
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{sim}_t^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%             \operatorname{Softmax}
%         \circ
%             \biggl(
%                 A\operatorname{ReLU}\bullet 
%             \Big(
%                     B
%                     \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^N
%                 +
%                     b
%             \Big)
%                 +
%                     a
%         \biggr)
%     ,
% \end{equation}
% where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$.
% \end{definition}

% Illustrated in Figure~\ref{fig:Attention_Is_All_You_Need}, our pathwise attention mechanism extracts features by reinterpreting two of the key features of attention mechanisms from natural language processing (NLP).  First, it utilizes \textit{similarity scores} which rank the likeness of any novel path against a dictionary of references paths.  These reference paths can either arise from real/stress historical (market) scenarios, they can be generated synthetically, or a combination of either.  These similarity scores are illustrated in Figure~\ref{fig:Similarity_Score}, and they serve as pathwise analogues of contextual keys and queries in attention mechanisms in NLP.

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of Definition~\ref{defn:Sim_Score}, fix a positive integer $N_2$, and set of query times $0\le t_1<\dots< t_N\le t$, an $N_2\times d$ matrix $V$, and a $N_2\times N$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^N)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{pos}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined by 
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{pos}_t^{\theta_1}
%         (y_{\cdot} )
%     \eqdef 
%         U \,
%         (\oplus_{j=1}^N \, y_{t_j})
%         + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$.
% \end{definition}

% Next, the \textit{positional encoding} of any novel path, illustrated in Figure~\ref{fig:PositionalEncoding}, encodes samples from the novel path.  These indicates changes in any sample path and they fully determined piecewise linear paths with finitely many pieces (as are generated in simulation studies).  This data is then combines with the weights of the similarity scores to produce the features encodings of our pathwise attention mechanism. 


% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of Definitions~\ref{defn:Sim_Score} and~\ref{defn:PositionalEncoding}, set $N_1=N_2$.  A \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1,C)$, is the map $\operatorname{attn}_t^{\theta}:C([0,1],\mathbb{R}^d)\rightarrow \mathbb{R}^{d\times N}$ with representation
% \[
%         \operatorname{attn}_t^{\theta}(y_{\cdot})
%     \eqdef 
%             C\,
%             \operatorname{vec}\big(
%                     \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%                 \odot
%                     \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%             \big)
% \]
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$, where $C$ is an $M\times (N_1 d)$-dimensional matrix.
% \end{definition}


% \begin{proposition}[Pathwise Attention Losslessly Encodes Regular Domains]
% \label{prop:Lossless_Encoding}
% \hfill\\
% Let $K\subseteq C([0:T],\mathbb{R}^d)$ satisfy Assumption~\ref{ass:reg_compact}.  Then, there exists an $N\in \mathbb{N}_+$ and a parameter $\theta$ as in Definition~\ref{defn:PathAttention} such that, $\operatorname{attn}_T^{\theta}$ restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^N,\|\cdot\|_2)$.
% \hfill\\
% Estimates for the encoding dimension $M$ are recorded in Table~\ref{tab:ATTENTION_Rates} on a case-by-base basis.
% \end{proposition}



% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for Lossless Pathwise Attention Encoding of Regular Compact Domains.}}
%     \label{tab:ATTENTION_Rates}
%     \begin{tabular}{lllll}
%     \toprule
%         Type of Compact Domain %& Complexity ($\|\theta\|_0$) 
%         & Encoding Dimension $(M)$ & Ass.~\ref{ass:reg_compact} \\
%     \midrule
%         Finite%& $\mathcal{O}(\cdot)$ 
%         & $\mathcal{O}(\log(\# K))$ 
%         & (i)
%         \\
%         Iso. Comp. Riemann.%& -- 
%         & Finite
%         & (ii)
%         \\
%         Iso. Comp. Riemann. + Aspherical %& -- 
%         & $\mathcal{O}\big(\mathcal{N}_{d_g}(M,\operatorname{Vol}(M,g)^{1/D_K} )\big)$
%         & (ii)
%         \\
%         P.W. Lin. (N. Pieces) %& - 
%         & $\mathcal{O}(Nd)$
%         & (iii)
%         \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Fix an $A\subset M$ and $\delta>0$.  The quantity $\mathcal{N}_{d_g}(A,\delta)$ denotes the minimum number, $I$, of points $\{x_i\}_{i=1}^I$ in $M$ for which every $x\in M$ is contained in a geodesic ball of radius $\delta$ about some $x_i$, for $i\in \{1,\dots,I\}$.}
% \end{table}

% \subsection{Phase 2 - Multi-Layered Perceptrons (MLPs) Transformation}
% \label{s:Model__ss:Review__MLPs}
% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an source dimension $d$ and a target dimension $D$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^d$ to $\mathbb{R}^D$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^d\rightarrow\mathbb{R}^D$ with iterative representation: for each $x\in \mathbb{R}^d$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=d$ and $d_{J+1}=D$.

% \subsection{Bloack 3 - Decoding via Geometric Attention Mechanism}
% \label{s:Model__ss:GeometricAttentionMechanism}

% Fix $N\in \mathbb{N}_+$.  In what follows, we denote the orthogonal projection of $\mathbb{R}^N$ onto the $N$-simplex 
% \[
%         \Delta_N
%     \eqdef 
%     \{
%         w \in [0,1]^N:\,
%         \sum_{n=1}^N\,w_n = 1
%     \}
% \]
% by $P_{\Delta_N}$.  We note that the closedness and convexity of $\Delta_N$ implies that $P_{\Delta_N}$ is a well-defined $1$-Lipschitz map, see \citep[Proposition 4.8]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017}.  

% \begin{definition}[Geometric Attention Mechanism]
% \label{defn:GeometricAttentionMechanism}
% Let $N,d\in \mathbb{N}_+$.  A geometric attention mechanism is a map $\operatorname{g-attn}_N:\mathbb{R}^N\rightarrow \mathcal{N}_d$ with representation
% \[
%         \operatorname{g-attn}_N^{\vartheta}(v)
%     =
%         \mathcal{N}_d\Biggl(
%                 \sum_{n=1}^N\,
%                     P_{\Delta_N}(v)_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^N\,
%                     P_{\Delta_N}(v)_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)})
%         \Biggr)
% \]
% where $m^{(1)},\dots,m^{(N)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(N)}$ are $d\times d$-matrices; and $\vartheta\eqdef (m^{(n)},A^{(n)})_{n=1}^N$.
% \end{definition}

% \subsection{The DKF Model}
% \label{s:Model}
% We may now formalize the discrete Kalman filter model of Figure~\ref{fig:DKFModel}.  
% \begin{definition}[Deep Kalman Filter]
% Let $d\in\mathbb{N}_+$, $T>0$, and an activation function $\sigma:\mathbb{R}\rightarrow \mathbb{R}$.  
% A function $\hat{F}:C([0:T],\mathbb{R}^d)\rightarrow \mathcal{N}_d$ is called a discrete Kalman Filter if it admits the representation
% \begin{equation}
% \label{eq:DKF_formalization}
%         \hat{f}
%     =
%             \operatorname{g-attn}_N^{\vartheta}
%         \circ 
%             \hat{f}
%         \circ 
%             \operatorname{attn}_T^{\theta}
% \end{equation}
% where $\operatorname{g-attn}_N^{\vartheta}$ is as in Definition~\ref{defn:GeometricAttentionMechanism}, $\operatorname{attn}_T^{\theta}$ is as in Definition~\ref{defn:PathAttention}, and $\hat{f}$ is an MLP as in~\eqref{eq:MLP}; such that the composition~\eqref{eq:DKF_formalization} is well-defined.
% \end{definition}



% \section{Main Result}
% \label{s:Main_Results}

% We are now ready to state our main theorem.
% \begin{theorem}[The DKF Can Approximate the Optimal Filter]
% \label{thrm:MAIN}
% Let $d\in \mathbb{N}_+$ and $K\subset C([0:T],\mathbb{R}^d)$ satisfy Assumption~\ref{ass:reg_compact}.  Suppose that the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies Assumption~\eqref{ass:technical_evolution_conditions}.  % and let $f^{\star}$ denote its associated optimal filter~\eqref{id:ConditionalDistribution}.  
% For every $T>0$ there exists a DKF $\hat{F}:C([0:T],\mathbb{R}^d)\rightarrow\mathcal{N}$ satisfying the uniform estimate
% \[
%     \max_{y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})
%             ,
%                 \hat{F}(y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, Table~\ref{tab:ComplexityMain} records the complexity estimates of $\hat{F}$.
% \end{theorem}

% \begin{table}[H]%[ht!]
%     \centering
%     \caption{{Complexity Estimates for the DKF model $\hat{F}$ in Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:ComplexityMain}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}



% \subsection{Proof Overview}
% \label{s:Theoretical_Analysis}
% This section overviews the derivation of our main result, namely, Theorem~\ref{thrm:MAIN}.
% \paragraph{Summary of What is Known}
% % \label{s:Theoretical_Analysis__ss:LipsterShiryaevSummary}
% Results in \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, they denote an explicit formulation of the resulting distribution which can then analyze directly. 
% Under Assumption~\ref{ass:technical_evolution_conditions}, \citep[Theorem 12.6]{LipShiryaev_II_2001} and we deduce that $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, meaning that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.


% A function is uniformly approximable by a deep learning model if it is continuous.  If there is no clear favourable structure in the function being approximated, e.g.\ smoothness \cite{yarotsky2020phase,gonon2023approximation} or neural network-like structure \cite{cheridito2021efficient,mhaskar2016deep}, then the best available approximation rates are those corresponding to those where the target function is Lipschitz; see \cite{DaubechiesDeVoreFoucartHaninPetrova_CA_KnotFreeReLU_2022}. %devore1993constructive,
% Thus, the first step to obtaining approximability guarantees for the optimal filter, by deep neural networks, which depend on relatively few trainable parameters, is to show that the optimal filter is a locally-Lipschitz function of observed paths.
% \begin{proposition}[Local Lipschitz-Continuity of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter}
% \hfill\\\anastasis{group into simple assumption environment.}\\
%     Fix $t \in [0, T]$. Under the assumptions of \Cref{lem:LipschitzSigma} and \Cref{lem:LipschitzMu}, $f_t$ from \eqref{id:ConditionalDistribution} is locally Lipschitz-continuous. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t 
%     \end{align*}
% \end{proposition}

% Having established the regularity of the optimal filter for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, we need to verify that maps sharing the same domain (input space), codomain (output space), and regularity as the optimal filter are approximable by the proposed DKF model.  This is the content of the next proposition, which acts as its standalone approximation theorem for the DKF.


% \begin{table}[H]%[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}

% \begin{proposition}[Approximation Capacity of DKFs]
% \label{prop:Universal_Approximation_Theorem__PathToNd}
% Let $d\in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}.  
% For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:(K,\|\cdot\|_{\infty})\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ there exists a DKF $\hat{F}$ 
% % \[
% %         \hat{t}(x)
% %     \eqdef
% %         \mathcal{N}_d\Biggl(
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     m^{(n)}
% %             ,
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     (A^{(n)})^{\top}A^{(n)})
% %         \Biggr)
% % \]
% % \anastasis{Update representation/simplify ofc + explain notation} 
% satisfying the uniform estimate 
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{F}(x)
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(N)$ and Decoding dimension $(M)$ are all recorded in Table~\ref{tab:approximationrates__nonFlatVersion} depending on the the choice of activation function $\sigma$.
% \end{proposition}


% We now have at our disposal, the tools to prove our main result.  
% \begin{proof}[{Proof of Theorem~\ref{thrm:MAIN}}]
% Since the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies Assumption~\eqref{ass:technical_evolution_conditions}, then Proposition~\ref{prop:LocLipReg_OptimFilter} implies that the optimal filter $f: y_{[0:t]}\mapsto \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})$ is a locally-Lipschitz map from $(C([0:T],\mathbb{R}^d),\|\cdot\|_T)$ to $(\mathcal{N}_d,\mathcal{W}_2)$.  Since $K\subseteq C([0:T],\mathbb{R}^d)$ is compact then, $f|_K$ is Lipschitz.  

% Since $K\subset C([0:T],\mathbb{R}^d)$ satisfies Assumption~\ref{ass:reg_compact} and $0<\varepsilon<1/2$ then, Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd} implies that there is a DKF $\hat{F}:C([0,T],\mathbb{R}^d)\rightarrow\mathbb{N}_d$ with representation~\eqref{eq:DKF_formalization} and complexity recorded in Table~\ref{tab:approximationrates__nonFlatVersion} satisfying
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{F}(x)
%         \big)
%     < 
%         \varepsilon
% .
% \]
% This completes the proof of Theorem~\ref{thrm:MAIN}.
% \end{proof}


% \section{Proofs of Auxiliary Results}
% \label{s:Proof}
% This section contains the derivations of our paper's results.

% \subsection{Proofs of Auxiliary Results}
% \label{s:Proof__ss:AuxResults}
% \begin{proof}[{Proof of Proposition~\ref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^d)$, given by $f\mapsto \big(f(\cdot /T),0,\dots,0\big)$, is an isometric embedding; then $\phi\eqdef \phi_3\circ\phi_2\circ \phi_1$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^d)$.
% \end{proof}

% \subsection{Stability of the Optimal Filter - Proof of \texorpdfstring{Proposition~\ref{prop:LocLipReg_OptimFilter}}{Lipschitz Continuity}}
% We now prove the local Lipschitz stability of the optimal filter~\eqref{id:ConditionalDistribution}, for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, as a function of its observed/input path.  The proof builds on a series of Lemmata, which demonstrate the local Lipschitz continuity of the parameters defining the optimal filter.  


% We first observe that, Assumption~\ref{ass:technical_evolution_conditions} grants us access to \citep[Theorem 12.7]{LipShiryaev_II_2001}, which implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
% \notag
%     d\mu_t 
%         =&[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\intercal}(t,y_{[0:t]})](B\circ B)^{-1}(t,y_{[0:t]})\\
%         &\times [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt] \label{id:ClosedFormMu}
%     \\
% \notag
%     \partial_t\Sigma_t =& a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\intercal}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]}) - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]}) ]
%         \\
%         & \times (B\circ B)^{-1} (t,y_{[0:t]}) [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]})]^{\intercal} \label{id:ClosedFormSigma}
% \end{align}
% with initial conditions $\mu_0=\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\intercal}|Y_0]$; where
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\intercal + B_2B_2^\intercal, \quad 
%     b \circ B \eqdef b_1B_1^\intercal + b_2B_2^\intercal, \quad 
%     b \circ b \eqdef b_1b_1^\intercal + b_2b_2^\intercal.
% \end{align*}
% Furthermore, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\Sigma_t$ is positive definite for all $t \in [0,T]$ since we have assume that $\Sigma_0$ in Assumption~\ref{ass:technical_evolution_conditions}.

% To clarify the argument's direction, we first record the proof of Proposition~\ref{prop:LocLipReg_OptimFilter}.  We subsequently derive the lemmata on which it relies.
% \begin{proof}[{Proof of Proposition~\ref{prop:LocLipReg_OptimFilter}}]
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a constant $\bar{K} < \infty$ s.t.
%     \begin{align*}
%     \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         &\leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{align*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma} that there exists a constant $K < \infty$, s.t.
%     \begin{align*}
%             \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \quad 
%             \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%     \end{align*}
%     so we obtain 
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%     \end{align*}
%     and the statement follows. 
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]\label{lem:LipschitzMu}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:TimeLipschitzMu}, $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%  \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%  \end{align*} 
% \end{lemma}
% \begin{proof}
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) \notag \\
%   & \quad \quad - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \label{id:Phi1} \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu}, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0, s]}) d y_{[0, s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align} 
%  & \mu^{(1)}_t - \mu^{(2)}_t \notag \\
%  & =   \mu_0^{(1)} - \mu_0^{(2)} 
%   + \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds 
%   + \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \notag \\ 
%  & \quad + \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \notag  
%   + \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\,
% (\mu^{(1)}_s - \mu^{(2)}_s ) ds .  \notag
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} 
%   + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwalls inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$. As a next step, let $\mySet{[s_{i-1}:s_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Moreover, by the use of integration by parts, we have
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         - \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         + \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq t} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% (Time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:t]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 
%       \leq \epsilon_I + K t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that $\eqref{t:gammaB} \leq K \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t$. Eventually, consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to Lipschitz continuity of $\Phi_1$. We conclude, since $\max_{s \in [0:t]} \|\mu^{(2)}_s \|_2 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\eqref{t:gammaC} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$, and therefore $\gamma(t)\leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.
% \medskip

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%         \left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)
%      \notag  
% \end{align} 
% As $\Phi_1$ is (time-)Lipschitz continuous, implying $\max_{s \in [0:t]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$ we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}

% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the assumptions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{align*}
%             \| \mu_t - \mu_s \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0, u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0, u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{align*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 
%         \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwalls inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_0^t a_0(u, y_{[0, u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{ \eqdef  \alpha(t)}
%           + \int_0^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0, s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0, u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi1}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_1$, $ (b \circ B)$, $(B\circ B)^{-1}$, $ A_0$, and $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
% \begin{enumerate}[wide]
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_0$, $(b \circ B)$, $(B\circ B)^{-1}$, $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}[wide]
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:LipschitzA1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq K \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left hand side refers to the Forbenius norm.
% \end{lemma} 
% \begin{proof} 
% From \eqref{id:ClosedFormSigma}, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
% \Sigma_t = & \Sigma_0 + \int_0^t
% a_1(t,y_{[0:s]}) \Sigma_s + \Sigma_s a_1^{\intercal}(s,y_{[0:s]}) + (b\circ b)(s,y_{[0:s]}) - [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]}) ]
%    \notag      \\
%         & \hspace{3cm} \times (B\circ B)^{-1} (s,y_{[0:s]}) [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]})]^{\intercal} ds . \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{align*} 
% & \Sigma^{(1)}_t - \Sigma^{(2)}_t \\
% & = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
% & \quad + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) + 
% \Xi_2^\intercal (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{align*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\intercal(s, y^{(1)}_{[0:s]}) - a_1^\intercal(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{align} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef & \big[ a_1^\intercal(s, y^{(2)}_s) 
%  + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) (b\circ B) (s, y^{(1)}_{[0:s]}) \notag \\ 
% &\quad + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
% \big] .   \label{Xi2} 
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{align} 
%  &\big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\
% & \leq  
% \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%  \notag \\ 
%  & \quad  + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot \notag \\ 
%  & \quad \qquad \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{align}  
% From \Cref{lem:LipschitzA1}, we have that 
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{align} 
%  & \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\ 
% &\quad \leq  
% \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big) 
% \cdot \notag \\ 
% &\quad  \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
% \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{align} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$
%  and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is also uniformly bounded, according to \eqref{Xi2}. 
%  Therefore, from \eqref{Sigma1-2bddXi2} we obtain that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% K ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}

% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and assume local Lipschitz continuity in the path component as well as time-continuity of $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\delta > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \delta$ holds
% \begin{align*} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component, we conclude that $a_1$, $b \circ b$, $A_1^\intercal(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\intercal (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\intercal$ have the same property. By this, together with the triangular inequality, 
%     \begin{align*}
% \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  & \leq  
%  2K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) + \\
% & \qquad + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2 + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \\
% & =  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(1+ \Vert\Sigma^{(1)}_s \big\Vert_2 + \Vert\Sigma^{(2)}_s \big\Vert_2 + \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2 \Big).
% \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < \bar{K} \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in $y_{[0:t]}$, for any $\epsilon>0$, there exists $\delta>0$ such that 
% when 
% $\| y^{(1)}_t - y^{(2)}_t \|_2 < \delta$,  
% $\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \|_2 < \epsilon$, and therefore 
% \begin{align*} 
% \big\| \Sigma^{(2)}_t \big\|_2 \leq \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 + \big\| \Sigma^{(1)}_t \big\|_2 
% \leq \epsilon + K . %\label{Sigma2bdd} 
% \end{align*} 
% \end{proof}

% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let $a_1, b \circ b, b \circ B, (B \circ B)^{-1}, b \circ B, A_1$ be continuous. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\intercal}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma}, then there exists an $r > 0$, s.t. for all times $t \in [0,T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ holds that 
%     \begin{align*}
%         \Sigma_t - r \cdot I_{d_X}
%     \end{align*}
%     is positive semi-definite.
% \end{lemma}
% \yannick{TODO. Assumptions are highlighted below.}
% \begin{proof}
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\intercal(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\intercal(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ being positive semi-definite} at 
%     \begin{align*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal )
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\intercal
%                     \right)
%                 ds.
%     \end{align*}
%     As \byyan{$G_t(y_{[0:t]})$ is positive definite}, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%                 (G_t(y_{[0:t]})^{-1})^\intercal
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%             )
%     \end{align*}
%     and 
%     \begin{align*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\intercal
%             \right)
%         \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{align*}
%     As we \byyan{assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$} as well as \byyan{$K_3 > 0$ s.t. $\tr(A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$} we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\intercal(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]




% \subsection{Stable and Lossless Encoding by Pathwise Attention - Proof of Propositions~\ref{prop:Lossless_Encoding}}
% \label{s:Proof__ss:Encoding}



% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(N)}$ in $C([0:T],\mathbb{R}^d)$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map]
% \label{lem:Good_Feature_Map}
% Under Assumption~\ref{ass:reg_compact} (ii).  
% There is a constant $C_{D_K}>0$, depending only on $D_K$, and a $\delta>0$ depending only on $(M,g)$ such that: for and $\delta$-packing $\{y^{(n)}\}_{n=1}^N$ of $K$, there are matrices $A,B,b,V,U,C$ and vectors $a,b$ for which the parameter $\theta$, as in Definition~\ref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{N+1}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{N+1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\| \in \mathcal{O}(N^2)$.

% \noindent Moreover, if $(M,g)$ is aspherical then:
% \begin{enumerate}
%     \item[(i)] $\delta \in \mathcal{O}( \operatorname{Vol}(M,g)^{1/D_K} )$
%     \item[(ii)] $\|\theta\| \in \mathcal{O}(N^2)$,
%     \item[(iii)] $C_{D_K}\in \mathcal{O}(D_K^{3(D_K+1)/2})$
%     % $0<C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
%     % \item[(i)] $\|A\|_0=2N$, 
%     % \item[(ii)] $\|B\|_0=2N$, 
%     % \item[(iii)] $\|a\|_0=1$, 
%     % \item[(iv)] $\|b\|_0=0$, 
%     % \item[(v)] $\|C\|_0= N_1$, 
%     % \item[(vii)] $\|U\|_0=0$, 
%     % \item[(viii)] $\|V\|_0= N^2_1$,
%     % \item[(ix)] $0<C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
% \end{enumerate}
% % \anastasis{perhaps I tally into a single parameter estimate} like $\|\theta\| \in \mathcal{O}(N^2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map}}]
% \noindent\textbf{Step 1 - Estimating $N$ on the Riemannian Manifold $(M,g)$}
% \hfill\\
% %%
% Since $(K,\|\cdot\|_T)$ be isometric to $(M,d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $D_K$-dimensional Riemannian manifold $(M,g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $M$ denoted by $\operatorname{sys}(M)$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(M) 
%     \le
%     \,\tilde{C}_{D_K}
%     \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \end{equation}
% where $\operatorname{Vol}(M,g)$ denotes the Riemannian volume of $(M,g)$ and $\lesssim$ hides a constant depending only on the dimension $D_K$, for a universal constant $\tilde{C}_{D_K}>0$ satisfying
% \[
%         0
%     <
%         \tilde{C}_{D_K}
%     <
%         6 (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}
% \,
% .
% \]
% By Stirling's approximation, $\sqrt{(D_K+1)!} \in \mathcal{O}(D_K^{(D_K+1)/2}$; whence, $\tilde{C}_{D_K}\in 
% % \mathcal{O}(D_K^{D_K+1}\, D_K^{(D_K+1)/2})$
% \mathcal{O}(D_K^{3(D_K+1)/2})$.

% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(M)/10$ then the given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(M,g)$, the map $\varphi_2:(M,d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{D_K}\eqdef \tilde{C}_{D_K}/10$, $N\eqdef \#\widetilde{\mathbb{X}}$, and enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^N$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{D_N}
%         \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     .
% \]
% We note that, if $K$ is not aspherical, then but it is only closed, then the conclusion still holds however, without the quantitative upper-bound on $\delta$.
% \hfill\\
% \noindent\textbf{Step 2 - Building the Feature Map with Well-posed Inverse}
% \hfill\\
% %%
% Let $\varphi_1:(M,d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have assumed to exist.  Set $\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^N$ where, for $n=1,\dots,N$ we set $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\varphi: C([0,T],\mathbb{R}^d)\rightarrow \mathbb{R}^N$ by $y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^N$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^N
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^N
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^N
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^N
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $M$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \hfill\\
% \noindent\textbf{Step 3 - Aligning to a Hyperplane in $\mathbb{R}^{N+1}$ with a Shallow ReLU Neural Network}
% \hfill\\
% Set $N_1\eqdef N+1$.  Let $b$ be the zero vector in $\mathbb{R}^N$.
% A mild variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $N\times 2N$ and $2N\times N$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_N & \vert & -I_N
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_N \\
%             \-- \\
%             -I_N
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^N\rightarrow \mathbb{R}^N$ defined by $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^N$.  Consider the $N_1\times N$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{N_1}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_N & 0 \\
%             0 & 0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,N\\
%             1 & \mbox{ if } i=N_1
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \hfill\\
% \noindent\textbf{Step 4 - Injectivity of Softmax Function on Hyperplane}
% \hfill\\
% Note that, for each $u\in \mathbb{R}^N$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^N$ onto the $N$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^N\}$ in $\mathbb{R}^{N_1}$.  Observe that the Softmax function $\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^N\,e^{u_k})_{j=1}^N$ maps $H$ surjectively and continuously onto the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})\subset \operatorname{int}(\Delta_N)\eqdef \{v\in [0,1]^{N_1}:\,\sum_{i=1}^{N_1}\,v_i=1\}$; i.e.\ of the interior of the $N_1$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{N_1}) + 1\big)_{i=1}^{N}
% \end{equation}
% is a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})$ then, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{N_1})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$.  Since, $\Psi$ was constructed to be an instance of $\operatorname{attn}_T$.  
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_N)$ of the $N_1$-simplex then, $C^{\star}\eqdef \max_{u\in \Phi(K)}\,\min_{v\in \Delta_{N_1}\setminus \operatorname{int}(\Delta_{N_1})}\,\|u-v\|>0$.  Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{N_1}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{N_1})
%             +
%             \bar{\Delta}_{N_1}
%         \}
% \]
% where $\bar{\Delta}_{N_1}\eqdef (1/N_1,\dots,1/N_1)$ is the barycenter of the $N_1$-simplex $\Delta_{N_1}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{N_1}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is Lipschitz\footnote{\anastasis{Add details about Lipschitzness? or Obvious?}} on $\Delta_{N_1}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image since it is the composition of Lipschitz functions with Lipschitz inverses.  
% \hfill\\
% \textbf{Step 5 - Representation as an Attention Mechanism}
% \hfill\\
% Set $\theta_0 = (A,B,a,b, \{y^{(n)}_{\cdot}\}_{n=1}^{N_1})$ and observe that the map $\Psi$ is of the form~\eqref{eq:featuremap}.  
% Let $U$ be the $N_1\times N_1$-dimensional zero matrix, and let $V$ be the $N\times N$-dimensional matrix whose entries are all $1$s.  Set $\theta_1\eqdef (U,V,\{n/{N_1}\}_{n=1}^{N_1})$.  Let $C$ be the $N_1\times N_1 d$-dimensional matrix given by $Cx = (x_i)_{i=1}^{N_1}$ for every $x\in \mathbb{R}^{N_1 d}$.  Set $\theta\eqdef (\theta_0,\theta_1,C)$ and observe that 
% \[
%         \operatorname{attn}_T^{\theta}(y_{\cdot}) 
%     \eqdef
%             C\,
%             \operatorname{vec}\big(
%                     \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%                 \odot
%                     \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%             \big)
%     = 
%         \Psi(y_{\cdot})
% \]
% for each $y_{\cdot}\in K.$. Consequentially, $\operatorname{attn}_T^{\theta_{\cdot}}$ is a bi-Lipschitz embedding of $K$ to $\mathbb{R}^M$.  Note that $\|C\|_0= N_1$, $\|U\|_0=0$, and $\|V\|_0= N^2$.  Thus, $\|\theta\|_0\in \mathcal{O}(N^2)$.  
% This concludes the proof.
% \end{proof}

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Finite Version]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under Assumption~\ref{ass:reg_compact} (i) and let $k\eqdef \#K$.  
% Set $N=192\lceil\log(k)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There is a parameter $\theta$ as in Definition~\ref{defn:PathAttention} defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{192\lceil \log(k)\rceil}$ which restricts to a $(2^{-1/2},(3N/6)^{1/2})$-bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{192\lceil \log(k)\rceil},\|\cdot\|_2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}
% \begin{proof}
% We argue similarly to the proof of Lemma~\ref{lem:Good_Feature_Map}, with only Steps $1$ and $2$ of its proof being replaced with the following argument.  
% \hfill\\
% \noindent\textbf{Step 1 and 2 - Modified- Building the Feature Map}
% \hfill\\
% Enumerate $K=\{x_n\}_{n=1}^N$.  The map $\phi_1:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^N,\|\cdot\|_{\infty})$ given by $x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^N$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le N^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^N$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^N,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^N,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% By the Johnson-Lindenstrauss Lemma, as derived in \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $4*48$ as opposed to $4*200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , there is a linear map $\phi_3:(\mathbb{R}^N,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\lceil192\,\ln(N)\rceil},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $(\lceil48\,\ln(N)\rceil)\times N$-matrix $A_0$, satisfying: for every $u,v\in \mathbb{R}^N$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, $\varphi:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3N/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_{t}
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         N^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3N/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_t 
% .
% \end{align*}
% \noindent\textbf{Remaining Steps:}
% \hfill\\
% The rest of the proof is identical to the proof of Lemma~\ref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_N\,\vert \,I_N)^{\top}$.
% \end{proof}


% \begin{lemma}[Bi-Lipschitz Embedding of Piecewise Linear Paths]
% \label{lem:biLip_pw_lin}
% Fix $N\in \mathbb{N}_+$, $0=t_0<\dots<t_N=T$, and a constant $C_K>0$.
% Let $K\subset C([0:T],\mathbb{R}^d)$ be such that $y_{\cdot}\in K$ if:
% \begin{enumerate}
%     \item[(i)] For $i=0,\dots,N-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^d$ satisfying
%     \[
%     \begin{aligned}
%         & y(t)=A^{(i)}\,t+b^{(i)}
%         \,
%         &
%         \,
%         \mbox{ for all } t\in (t_i,t_{i+1})
%     ,
%     \end{aligned}
%     \]
%     \item[(ii)] $y_0=0$,
%     \item[(iii)] $\max_{i=1,\dots,N}\,|y(t_i)|\le C_K$.
% \end{enumerate}
% There is a parameter $\theta$, as in Definition~\ref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{Nd}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{Nd},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0\in \mathcal{O}(Nd)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:biLip_pw_lin}}]
% Set $N_1=N$.  Let $A,B$ be the $N_1\times N_1$-dimensional zero matrix and $a,b$ be the zero vector in $\mathbb{R}^{N_1}$.  Set $\theta_0=(A,B,a,b)$.  Observe that 
% \[
% \operatorname{sim}_T^{\theta_0}(y_{\cdot})_i = 1
% \]
% for all $y\in C([0:T],\mathbb{R}^d)$ and each $i=1,\dots,d$.  
% Let $V$ be the $N_1\times N_1$-dimensional zero matrix, $U=I_{N}$ where $I_N$ is the $N\times N$-dimensional identity matrix, and\footnote{The point $t_0$ is not sampled since every path $y_{\cdot}$ in $K$ satisfies $y_0=0$, and thus, there is no need to sample it at time $0$.} $\theta_1=(U,V,\{t_n\}_{n=1}^N)$.  Then, 
% \begin{equation}
% \label{eq:bijection_sampling}
%         \operatorname{pos}_T^{\theta_1}(y_{\cdot})
%     =
%         (y_1,\dots,y_N).
% \end{equation}
% In particular, the map $\operatorname{pos}_T^{\theta_1}$ in ~\eqref{eq:bijection_sampling} defines a linear bijection between $\mathcal{K}$ and the set $[-C_K,C_K]^N$.  Since $[-C_K,C_K]^N$ a subset of the finite-dimensional Banach space $(\mathbb{R}^N,\|\cdot\|_2)$ and all norms on a finite-dimensional normed are equivalent, then, $\operatorname{sim}_T^{\theta_1}$ is a bi-Lipschitz embedding of $K$ into $(\mathbb{R}^N,\|\cdot\|_2)$.  

% Let $C$ be the $Nd\times Nd$-dimensional matrix with $C_{i,j}=1$ for $i,j=1,\dots,Nd$.  Set $\theta=(\theta_0,\theta_1,C)$.  By construction $\|\theta\|_0\in \mathcal{O}(Nd)$.  
% Then, 
% \begin{equation}
% \label{eq:bijection_sampling__RelabelingStuff}
%         \operatorname{attn}_T^{\theta}(y_{\cdot})
%     \eqdef 
%         C\,
%         \operatorname{vec}\big(
%                 \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%             \odot
%                 \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%         \big)
%     =
%         (y_1,\dots,y_N)
%     .
% \end{equation}
% Together,~\eqref{eq:bijection_sampling} and~\eqref{eq:bijection_sampling} imply that $\operatorname{attn}_T^{\theta}$ defines a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \end{proof}

% \begin{proof}[{Proof of Proposition~\ref{prop:Lossless_Encoding}}]
% Follows directly from Lemmata~\ref{lem:Good_Feature_Map},~\ref{lem:Good_Feature_Map__FiniteVariant}, and~\ref{lem:biLip_pw_lin}.
% \end{proof}

% \subsection{Approximability of Locally Lipschitz Maps By DKFs - Proof Propositions~\ref{TBD}}
% We now prove our main universal approximation theorem, Propositions~\ref{TBD}.  We show that the target space/codomain of any considered DKF is geometrically regular, in the sense of \cite{Acciaio2022_GHT,kratsios2023transfer}.  Using this fact, we then combine and apply the results of \cite{kratsios2021universal,kratsios2023transfer} to deduce the result.

% % HERE!

% \subsubsection{Step A - Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}
% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d\in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d}$ denote the set of $d\times d$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d\times d$ matrices.  Here the $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.  Consider the $2$-product metric on $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ defined for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ by sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ will serve to quantize $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^d\times \operatorname{Sym}_{0,d})^{N} \rightarrow 
% \mathbb{R}^d\times \operatorname{Sym}_{0,d}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:QAS_Space_Sym0d}]  
% We first show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% \hfill\\
% \textbf{QAS Space Structure}
% \hfill\\
% Since $\operatorname{Sym}_{0,d}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the normed space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ as sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big)
%     = &
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     = &
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     \le &
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad            
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     \le &
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     = &
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\mathcal{Q},\eta)$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
% \hfill\\
% \textbf{Barycentricity}
% \hfill\\
% Consider the map $\sigma:(\mathbb{R}^d\times \operatorname{Sym}_{0,d})^2\times [0,1]$ given for any $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and $t\in [0,1]$ by
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),t
%         \big)
%     \eqdef 
%         \eta\big(
%             (m,A),(\tilde{m},B),(t,1-t)
%         \big)
%     .
% \]
% Since geodesics in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ are line segments, since $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the inner-product space $(\mathbb{R}^d\times \operatorname{Sym}_d)$, with inner-product given by the product of the Euclidean and Frobenius inner-products, then clearly for each $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ the map $t\mapsto \sigma\big((m,A),(\tilde{m},B),t\big)$ is a geodesic in the global NPC space, as defined in \citep[Definition 2.1]{Sturm_2003}, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$.  Thus, $\sigma$ is a \textit{geodesic bicombing} in the sense of \citep[page 1]{basso2018fixed}.  Since 
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
%     =
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
% \]
% then \citep[Theorem 3.4]{basso2018fixed} applies; whence $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is barycentric with $1$-Lipschitz barycenter map explicitly given therein.  

% Since is a barycentric QAS space then, \citep[Setting 3.6]{kratsios2023transfer} (iii) is satisfied.
% \end{proof}

% Having established the barycentricity and the QAS space structure of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\eta,\mathcal{Q}_{\cdot})$, we are now ready to prove the following result.
% \anastasis{Here in transcription}
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ there is a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ satisfying
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x_{\cdot}),f(x_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{t}(x_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^M\,
%                 P_{\Delta_M}(\hat{f}\circ \operatorname{attn}_T(x_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $M\in \mathbb{N}_+$, $m^{(1)},\dots,m^{(M)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(M)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_M}:\mathbb{R}^M\rightarrow\Delta_M$ is the Euclidean (orthogonal) projection onto the $M$-simplex, and an MLP $\hat{f}:\mathbb{R}^N\rightarrow \mathbb{R}^M$ with activation function $\sigma$.  The depth, width, encoding dimension (N), and decoding dimension (M) are recorded in Table~\ref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{D_K}\operatorname{Vol}(M,g)^{1/D_K})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:approximation_Sym}}]
% \anastasis{Relabel $N$ (index) as $M$}
% \hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% We will apply \citep[Theorem 3.7]{kratsios2023transfer}, which requires us to verify each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \paragraph{Step 1 - Implementing a Bi-Lipschitz Feature Map with the Attention Layer}
% \hfill\\
% \textbf{Remark:} \textit{We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap} can be chosen such that $\operatorname{attn}_T$ is a suitable feature map}.
% \hfill\\
% \begin{comment}
% \paragraph{Case (i) - The Continuous and Injective Case} 
% \anastasis{come back to this shortly...}
% \paragraph{Case (ii) - The Bi-Lipschitz Case} 
% \noindent 
% \end{comment}
% Let $N$ denote the $C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(\mathcal{M},d_g)$.  Since $(K,\|\cdot\|_T)$ and $(\mathcal{M},d_g)$ are isometric, then $N$ is the $C_{D_K} \operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(K,\|\cdot\|_T)$.  
% By Lemma~\ref{lem:Good_Feature_Map}, there are matrices $A,B$, $a$, and $b$ with $\|A\|_0=2N=\|B_0\|$, $\|a\|_0=1$, and $\|b\|_0=0$ such that $\varphi\eqdef \operatorname{attn}_T$, as defined in~\eqref{lem:Good_Feature_Map}, is a bi-Lipschitz embedding of $(K,\|\cdot\|_{T})$ to $(\mathbb{R}^N,\|\cdot\|_2)$.  Set $\{(K,\varphi)\}$, let $\nu$ denote the normalized (uniform) Volume probability measure on $(\mathcal{M},g)$, and let $\mu\eqdef \varphi_{\#}\nu$ be its pushforward to $(K,\|\cdot\|_T)$.  Since every bi-Lipschitz map is a quasi-symmetry\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}, then \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(M,d_g)$ is a doubling metric space, as defined on \citep[10.13; page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  This verifies \citep[Setting 3.6 (i)]{kratsios2023transfer}.




% \paragraph{Step 2 - Feature Space Geometry}\hfill\\
% Since the codomain of $\phi$ is simply a Euclidean space, then the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^N}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^N$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^N$, 
% \[
%     \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
% \]
% and the operator norm $\|1_{\mathbb{R}^N}\|_{op}$ of $1_{\mathbb{R}^N}$, thus of $T^i$ for every $i\in \mathbb{N}_+$, is uniformly bounded above by $1$.  
% Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} is holds.

% \paragraph{Step 3 - Geometry of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$}
% \hfill\\
% By Lemma~\ref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $N\in\mathbb{N}_+$, $u\in \mathbb{R}^N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 P_{\Delta_N}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \paragraph{Step 4 - Determining The Euclidean Universal Approximator}
% \hfill\\
% \textbf{Remark:} \textit{We now verify that the class of all MLPs with activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition} satisfies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.}\\
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le d+D+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy Assumption~\ref{ass:KLCondition} then, \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \paragraph{Step 5 - Applying~{\citep[Theorem 3.7]{kratsios2023transfer}}}
% Steps $1$ though $5$ verify that the conditions of Theorem~\citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the Feature Decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, Theorem~\citep[Theorem 3.7]{kratsios2023transfer} implies, thus for every $\varepsilon>0$ there is a map $\hat{t}:K\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{t}(x_{\cdot})
%     = &
%         \beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^N
%             \,
%                 \big(
%                     P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $x_{\cdot}\in K$ satisfying 
% \[
%     \sup_{x_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{t}(x_{\cdot})
%         ,
%             f(x_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ (which exists by Lemma~\ref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a right-inverse of the map $\mathbb{R}^d\times \operatorname{Sym}_{0,d}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$, where $\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially,~\eqref{eq:transformer_pre_mapped_BEGIN}-~\ref{eq:transformer_pre_mapped_END} reduces to~\eqref{lem:approximation_Sym__approximation___representation}.  


% \paragraph{Step 6 - Tallying Parameters}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $N=\mathcal{N}_{\operatorname{pack}}\big(K,C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in Table~\ref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $N$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             N
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{proof}

% \subsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool.  The proof method is summarized visually in Figure~\ref{fig:Approximation_Theorem}.


% \anastasis{t and t hat}
% \begin{figure}[H]
%     \centering
%     \begin{tikzcd}
%     \big(C([0:T],\mathbb{R}^d),\|\cdot\|_{\infty}\big) & (\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2) \\
%     (K,\|\cdot\|_{\infty}) 
%     \arrow[hookrightarrow]{u}{\iota} 
%     \arrow{r}{f} 
%     % \arrow[swap]{d}{\varphi} 
%     \arrow{dr}{\varrho\circ f}
%     & ({\mathcal{N}}_d,\mathcal{W}_2) 
%     \arrow[hookrightarrow]{u}{i}
%     \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
%     & (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
%     \end{tikzcd}
%     \caption{Summary of Proof Strategy for Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd} \anastasis{details}.}
%     \label{fig:Approximation_Theorem}
% \end{figure}


% \begin{proof}[{Proof of Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}}]
% \hfill\\
% \textbf{Step 1 - Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$}
% By Lemma~\ref{lem:LipschitzManifold_Nd} the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^d,\operatorname{Sym}_{0,d},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous then the map
% \[
%     g: (K,\|\cdot\|_T)\ni x \mapsto 
%     \pi\circ \varrho\circ f(x)
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d\times d$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain is achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; i.e.
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_d$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% \anastasis{Add reference to Lemma~\ref{lem:LoewnerBound} here.}
% Consequentially, Lemma~\ref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \hfill\\
% \textbf{Step 2 - Approximating $\varrho \circ f$ on $K$}
% \hfill\\
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%                     \,\operatorname{diam}(K) + 1
%                 }
%                 }
%         \biggr\}
% .
% \end{equation}
% We many now apply Lemma~\ref{lem:approximation_Sym} to deduce that there exists a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x),\varrho\circ f(x))
%     <
%         \delta
% .
% \end{equation}
% Since Lemma~\ref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  Set $t\eqdef \varrho^{-1}\circ \hat{t}$ and 
% denote the $1$-thickening of $\varrho\circ f(K)$ by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}:\,(\exists x\in K)\, d_{2,F}(f(x),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{t}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate} and Lemma~\ref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% = & 
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{t}(x)
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{x\in K}\,
%         d_{2,F}\big(
%                 \hat{t}(x)
%             ,
%                 \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% \le &
%     \sqrt{d}2\sqrt{
%             L
%             \,\operatorname{diam}(K) + 1
%         }
%     \,
%     \varepsilon
%     \,
%     \frac1{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:Approxim_LEMMA__END}
% = & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from Lemma~\ref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B} followed from the estimate~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009}, then estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% %\label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_p\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \textbf{Step 3 - Counting Parameters}
% Using $\delta$, as defined in~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in Table~\ref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \anastasis{Add computations tomorrow}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_d}$ denote the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_d}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_d}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_d},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_d}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of Lemma~\ref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_d}$ sending any $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_d}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_d}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_d}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_d},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_d}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_d}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}



% \appendix
% \section{Auxiliary Lemmata}
% \label{s:AuxLemmata}
% This section records auxiliary lemmata used in our proofs but proven elsewhere.
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% it holds that
% \[
% \begin{aligned}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     \\
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{aligned}
% \]
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzManifold_Nd}}]
% The proof is due to \textit{Iosif Pinelis}, and is given in \cite{LocalLipschitz_Pinelis}.  We only note that, $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$ where $\|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})$ denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}

% \section{Background: Riemannian Geometry and Algebraic Topology}
% \label{s:Background_Geo}



% \bibliographystyle{abbrvnat}
% \bibliography{Bookkeaping/2_References}


% \newpage
% \section{Algorithms}
% \input{Sections/Practical_Approach}

% \newpage
% \newpage
% \section{Applications}

% In this section, we will discuss exemplary applications that leverage the possibility to approximate a Kalman filter setting with our suggested framework. 
% For this, we first discuss how to fit and solve a filtering problem on the basis of sample paths for $Y_{[0:T]}$.
% We begin by revisiting the training procedure of Deep Kalman filters suggested in \cite{KrishnanShalitSontag17}, which motivates an approach that aligns more with our framework.

% \subsection{Training a Deep Kalman Filter as in \texorpdfstring{\cite{KrishnanShalitSontag17}}{Krishnan et al. (2017)}}
% For this, we reduce the setting of our filtering problem \eqref{eq:filtering_dynamics__signal},  \eqref{eq:filtering_dynamics__observation} such that the desired training framework is applicable. For this, functions $a_0$, $a_1$, $b_1$ are replaced with constants, we assume independence of the stochastic components, i.e. $b_2 \equiv B_1 \equiv 0$, and $A_0$, $A_1$, $B_1$ are assumed to be Markovian, i.e. functions mapping from $\R^{d_Y}$ to the corresponding space. Then, the former constants are treated as parameters and the latter functions are approximated by MLPs, and we denote their combined (learnable) parameters by $\phi$. We then denote the resulting filtering setting by
% \begin{align*}
%     dX_t & = [a^\phi_0 + a^\phi_1 X_t]dt +  b^\phi_1 dW^{(1)}_t \\
%     dY_t & = [A^\phi_0(Y_{t}) + A^\phi_1(Y_{t}) X_t]dt + B^\phi_2(Y_{t})dW^{(2)}_t. 
% \end{align*}
% This is then discretized by an Euler scheme for time steps $0 = t_0 < t_1 < \ldots < t_N = T$, $N \in \N$, with $\Delta t_n := t_{n}- t_{n-1}$, s.t. 
% \begin{align*}
%     X_{t_{n}} & \sim  \mathcal{N}\left(
%             (a^\phi_0 + a^\phi_1 X_{t_{n-1}})
%             \Delta t_n
%         ,
%             b^\phi_1
%             \Delta t_n
%     \right)
%     \\
%     Y_{t_{n}} & \sim \mathcal{N}\left(
%             (A^\phi_0(Y_{t_{n-1}}) + A^\phi_1(Y_{t_{n-1}}) X_{t_{n}})
%             \Delta t_n
%         ,
%             B^\phi_2(Y_{t_{n-1}})
%             \Delta t_n
%     \right)
% \end{align*}
% In the following, we denote for $n \in \myset{1}{N}$ the likelihood of $Y_{t_n} = y_{t_n} \in \R^{d_Y}$ under the parametrization $\phi$ by $p_\phi(y_t)$ and the likelihood conditional on $Y_{t_n} = y_{t_n}$ by $p_\phi( \cdot \vert y_{t_{n}})$. We can extend this notation to paths, i.e. for $Y_{[t_0:t_n]} = y_{[t_0:t_n]}$, we write $p_\phi(y_{[t_0:t_n]})$ and $p_\phi( \cdot \vert y_{[t_0:t_n]})$. Then, the fitting procedure is based on the observation that 
% \begin{align*}
%         \log p_\phi(y_{[t_0:t_N]}) 
%     & =  \log \int
%             \frac{
%                 p_\phi\left(
%                     y_{[t_0:t_N]}
%                 \middle|
%                     x_{[t_0:t_N]} 
%                 \right)
%                 p_\phi(x_{[t_0:t_N]} )
%             }{
%                 p_\phi\left(
%                     x_{[t_0:t_N]}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)
%             }
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%         dx_{[t_0:t_N]} \\ 
%     & \geq \int 
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%             \log \frac{
%                 p_\phi\left(
%                     y_{[t_0:t_N]}
%                 \middle|
%                     x_{[t_0:t_N]}
%                 \right)
%                 p_\phi(
%                     x_{[t_0:t_N]}
%                 )
%             }{
%                 p_\phi\left(
%                     x_{[t_0:t_N]}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)
%             }
%         dx_{[t_0:t_N]}  \\
%     & =
%         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
%             \log p_\phi\left(
%                 y_{[t_0:t_N]}
%             \mid
%                 x_{[t_0:t_N]}
%             \right)
%         \right]
%     -
%         \mathrm{KL} \left(
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%         \middle\Vert
%             p_\phi(
%                 x_{[t_0:t_N]}
%             )
%         \right)
% \end{align*}
% which can be factorized due to the Markovian property of $Y$ and $X$ to 
% \begin{align*}
%         \log p_\phi(y_{[t_0:t_N]}) 
%     & \geq
%         -
%             \mathrm{KL} \left(
%                 p_\phi\left(
%                     x_{t_0}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)           
%             \middle\Vert
%                 p_\phi(
%                     x_{t_0}
%                 )
%             \right) 
%         +
%             \sum_{n=0}^N
%             \mathbb{E}_{p_\phi(x_{t_n} \vert y_{[t_0:t_N]})} \left[
%                 \log p_\phi\left(
%                     y_{t_n}
%                 \mid
%                     x_{t_n}
%                 \right)
%             \right] \\ 
%         &\quad -
%             \sum_{n=1}^N
%             \mathbb{E}_{
%                 p_\phi(x_{t_{n-1}} \vert y_{[t_0:t_N]})
%             } \left[
%                 \mathrm{KL} \left(
%                     p_\phi\left(
%                         x_{t_n}
%                     \middle|
%                         x_{t_{n-1}}, y_{[t_0:t_N]}
%                     \right)
%                 \middle\Vert
%                     p_\phi\left(
%                         x_{t_n}
%                     \middle|
%                         x_{t_{n-1}}
%                     \right)
%                 \right)
%             \right].
% \end{align*}
% In the above expression, all terms are known in analytical form, except for $p_\phi( x_{t_n} | y_{[t_0:t_N]})$ and $p_\phi( x_{t_n} | x_{t_{n-1}}, y_{[t_0:t_N]})$, which is approximated a machine learning structure, that can be learned simultaneously in the process. One key feature of this structure is its capability to produce the posterior distribution both, conditional and unconditional, on $x_{t_{n-1}}$. This argument is valid due to the fact that the lower bound of $\log p_\phi(y_{[t_0:t_N]})$ is tight, when the produced posterior coincides with the (intractable) conditional distribution under $\phi$ with respect to the Kullback-Leibler divergence. \byyan{Since the Wasserstein distance used in this article is bounded by the Kullback-Leibler divergence, our result in \Cref{thrm:MAIN} can be used to show that this approximation argument holds.} 

% \subsection{Fitting the general filtering problem}
% In this section, we extend our filtering framework by removing the constraints that were introduced in the previous section. Specifically, we no longer enforce the restrictions on our filtering setting. To approximate the functions \(a_0\), \(a_1\), \(b_1\), \(b_2\), \(B_1\), \(A_0\), \(A_1\), and \(B_1\), we employ MLPs. Upon discretizing the system using the Euler scheme, we obtain the following dynamical equations:
% \begin{align}
%         X_{t_{n}}
%     & \approx
%             X_{t_{n-1}}
%         +
%             [a_0(t_{n-1},Y_{[0:t_{n-1}]}) + a_1(t_{n-1},Y_{[0:t_{n-1}]}) X_{t_{n-1}}] \Delta t_n
%         +
%             \sum_{i=1}^2\, b_i(t,Y_{[0:t_{n-1}]})\sqrt{\Delta t_n} Z_n^{(i)}
%     \label{id:Discretized_Signal}\\
%         Y_{t_{n}}
%     &
%             \approx Y_{t_{n-1}}
%         + 
%             [A_0(t,Y_{[0:t_{n-1}]}) + A_1(t,Y_{[0:t_{n-1}]}) X_{t_{n}}]\Delta t_n
%         +
%             \sum_{i=1}^2\, B_i(t,Y_{[0:t_{n-1}]})\sqrt{\Delta t_n}Z_n^{(i)},
%     \label{id:Discretized_Observation}
% \end{align}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables.

% We can now proceed with a similar observation as before
% \begin{align*}
%         \log p_\phi(
%             y_{t_n}
%         |
%             y_{[t_0:t_{n-1}]}
%         ) 
%     & =  \log \int
%             \frac{
%                 p_\phi\left(
%                     y_{t_n}
%                 \middle|
%                     x_{t_n},
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%             }{
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_n]}
%                 \right)
%             }
%             p_\phi\left(
%                 x_{t_n}
%             \middle|
%                 y_{[t_0:t_n]}
%             \right)
%         d x_{t_n} \\ 
%     & \geq \int 
%             p_\phi\left(
%                 x_{t_n}
%             \middle|
%                 y_{[t_0:t_n]}
%             \right)
%             \log \frac{
%                 p_\phi\left(
%                     y_{t_n}
%                 \middle|
%                     x_{t_n},
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%             }{
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_n]}
%                 \right)
%             }
%         d x_{t_n} \\ 
%     & =
%         \mathbb{E}_{
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_n]}
%             )
%         } [
%             \log
%             p_\phi(
%                 y_{t_n}
%             |
%                 x_{t_n},
%                 y_{[t_0:t_{n-1}]}
%             )
%         ]
%     -
%         \mathrm{KL}(
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_n]}
%             )
%         \Vert
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_{n-1}]}
%             )
%         ),
% \end{align*}
% Further, note that 
% \begin{align*}
%         p_\phi(
%             x_{t_n}
%         |
%             y_{[t_0:t_{n-1}]}
%         )
%     =
%         \mathbb{E}_{
%             p_\phi(
%                 x_{t_{n-1}}
%             |
%                 y_{[t_0:t_{n-1}]}
%             )
%         } \left[
%             p_\phi(
%                 x_{t_{n}}
%             |
%                 x_{t_{n-1}},
%                 y_{[t_0:t_{n-1}]}
%             )
%         \right]
% \end{align*}
% and therefore
% \begin{align*}
%         \log p_\phi\left(
%             y_{[t_0:t_{N}]}
%         \right) 
%     & =    
%         \log p_\phi\left(
%             y_{t_0}
%         \right) 
%         +
%         \sum_{n=1}^N
%         \log p_\phi\left(
%             y_{t_n}
%         \middle|
%             y_{[t_0:t_{n-1}]}
%         \right) \\
%     &\gtrapprox 
%         \log p_\phi\left(
%             y_{t_0}
%         \right) 
%         +
%         \sum_{n=1}^N
%         \mathbb{E}_{
%             X_{t_n} \sim f_\theta(y_{[t_0, t_n]})
%         } \left[
%             \log p_\phi\left(
%                 y_{t_n}
%             \middle|
%                 X_{t_n},
%                 y_{[t_0:t_{n-1}]}
%             \right)
%         \right] \\
%     &\hspace{3cm} -
%         \sum_{n=1}^N
%         \mathrm{KL}\left(
%             f_\theta(y_{[t_0, t_n]})
%         \middle\Vert
%             \mathbb{E}_{
%                 X_{t_{n-1}} \sim f_\theta(y_{[t_0, t_{n-1}]})
%             } \left[
%                 p_\phi(
%                     x_{t_{n}}
%                 |
%                     x_{t_{n-1}},
%                     y_{[t_0:t_{n-1}]}
%                 )
%             \right]
%         \right).
% \end{align*}
% We can now maximize the term on the right-hand side using stochastic gradient ascent in the parameters $\phi, \theta$. Note that the optimum is obtained when $\mathrm{KL}(f_\theta(y_{[t_0, t_n]}) \Vert  p_\phi(x_{t_{n}}|y_{[t_0:t_{n}]})) = 0$, as this results in the lower boundary being tight. \byyan{The approximation argument holds again due to the fact that the Wasserstein distance is dominated by the Kullback-Leibler divergence and \Cref{thrm:MAIN}.}

% \begin{remark}[Alternative MC-based training for \texorpdfstring{$\theta$}{theta}]
%     As there is no guarantee that the stochastic gradient descent actually converges against the right $\theta$, one can alternatively use Monte-Carlo simulations of \eqref{id:Discretized_Observation}, \eqref{id:Discretized_Signal} to fit $f_\theta$ under the current filtering system defined by $\phi$ with respect to the Wasserstein distance.
% \end{remark}

% % \textbf{\byyan{Approach 1.}} Note that the derivation of 
% % \begin{align*}
% %         \log p_\phi(y_{[t_0:t_N]}) 
% %     & \geq
% %         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{[t_0:t_N]}
% %             \mid
% %                 x_{[t_0:t_N]}
% %             \right)
% %         \right]
% %     -
% %         \mathrm{KL} \left(
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %         \middle\Vert
% %             p_\phi(
% %                 x_{[t_0:t_N]}
% %             )
% %         \right)
% % \end{align*}
% % does not use any of the properties assumed in the last section. We see that 
% % \begin{align*}
% %         & \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{[t_0:t_N]}
% %             \mid
% %                 x_{[t_0:t_N]}
% %             \right)
% %         \right] \\
% %     & \qquad = 
% %         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{t_0}
% %             \right)
% %             +
% %             \sum_{n=1}^N
% %                 \log p_\phi\left(
% %                     y_{[t_0:t_n]}
% %                 \mid
% %                     y_{[t_0:t_{n-1}]},
% %                     x_{t_n}
% %                 \right)
% %         \right] \\
% %     & \qquad = 
% %             \log p_\phi\left(
% %                 y_{t_0}
% %             \right)
% %         +
% %             \sum_{n=1}^N
% %                 \mathbb{E}_{p_\phi(x_{t_n} \vert y_{[t_0:t_n]})} \left[
% %                     \log p_\phi\left(
% %                         y_{[t_0:t_n]}
% %                     \mid
% %                         y_{[t_0:t_{n-1}]},
% %                         x_{t_n}
% %                     \right)
% %                 \right],
% % \end{align*}
% % and 
% % \begin{align*}
% %         & \mathrm{KL} \left(
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %         \middle\Vert
% %             p_\phi(
% %                 x_{[t_0:t_N]}
% %             )
% %         \right) \\
% %     & \qquad =
% %         \int
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %             \log \frac{
% %                 p_\phi\left(
% %                     x_{[t_0:t_N]}
% %                 \middle|
% %                     y_{[t_0:t_N]}
% %                 \right)
% %             }{
% %                 p_\phi(
% %                     x_{[t_0:t_N]}
% %                 )
% %             }
% %         dx_{[t_0:t_N]} \\
% %     & \qquad =
% %         \int
% %             \prod_{m=1}^N
% %             p_\phi\left(
% %                 x_{t_m}
% %             \middle|
% %                 x_{t_{m-1}},
% %                 y_{[t_0:t_m]}
% %             \right)
% %             \sum_{n=1}^N
% %                 \log \frac{
% %                     p_\phi\left(
% %                         x_{t_n}
% %                     \middle|
% %                         x_{t_{n-1}},
% %                         y_{[t_0:t_n]}
% %                     \right)
% %                 }{
% %                     p_\phi(
% %                         x_{t_n}
% %                     |
% %                         x_{t_{n-1}}
% %                     )
% %                 }
% %         dx_{[t_0:t_N]} \\
% %         & \qquad \byyan{=}
% %             \sum_{n=1}^N
% %             \mathbb{E}_{
% %                 p_\phi\left(
% %                     x_{t_{n-1}}
% %                 \middle|
% %                     y_{[t_0:t_n]}
% %                 \right)
% %             } \left[
% %                 \mathrm{KL} \left(
% %                     p_\phi\left(
% %                         x_{t_n}
% %                     \middle|
% %                         x_{t_{n-1}},
% %                         y_{[t_0:t_n]}
% %                     \right)
% %                 \middle|
% %                     p_\phi(
% %                         x_{t_n}
% %                     |
% %                         x_{t_{n-1}}
% %                     )
% %                 \right)
% %             \right]
% % \end{align*}


% \subsection{(Conditional) simulation of the observation process}

% \yannick{TODO. Remove duplicate content with above and clarify benefits of transformer representation of $f_\theta$ when it comes to sampling.} Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation} and are known by the agent. For a fixed time $t \in [0:T]$, the objective is now to simulate the process $Y$ at times $t \leq s \leq T$. If both, $X, Y$ are observable, then a typical Euler-scheme for $Y_{[t:T]}$ is usually given by fixing a time-discretization $t  \eqdef  t_0 < t_1  < \cdots < t_N  \eqdef  T$ with $N \in \N$ and approximating
% \begin{align*}
%     X_{t_{n+1}} & \approx X_{t_{n}} + [a_0(t,Y_{[0:t_n]}) + a_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, b_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)} \\
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)}
% \end{align*}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables. Note that we have a slight abuse of notation, as $a_0, a_1, b_1, b_2, A_0, A_1, B_1, B_2$ are now approximations from discretized paths instead of the continuous counterparts.

% In our setting, however, the component $X$ is not observable. To overcome this, we have to rely on standalone simulations of $Y_{[t:T]}$, while inferring $X$ conditional on $Y$. This means, 
% \begin{align*}
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n} \vert  Y_{[0:t_n]}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)},
% \end{align*}
% where $X_{t_n} \vert Y_{[0:t_n]}$ refers to the conditional law described by \eqref{id:ConditionalDistribution}.

% \yannick{If we want to do these simulations fast and efficient, we are reliant on fast access to $X_{t_n} \vert Y_{[0:t_n]}$.}


% % \subsection{Optimal control and BSDEs in finance}
 
% % Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}. While there are numerous settings where this structure is applicable, the reader may regard the observation process $Y$ as an asset price process and assume that the signal process $X$ constitutes a stochastic drift model that is generally not observable. 
% % 
% % We now consider an optimal control problem of the form 
% % \begin{align}
% %     J(u) \eqdef \mathbb{E}\left[\int_0^T r(t, Y_t, (u \bdot Y)_t, u_t) dt + g(Y_T, (u \bdot Y)_T) \right] \label{id:OptimalControl}
% % \end{align}
% % for a measurable function $r: \R_+ \times \R^{d_Y} \times \R^{d_Y} \times \R^{d_Y}$, a concave function $g: \R^{d_Y} \times \R^{d_Y} \to \R$, and $u$ being a predictable control process with values in $\R^{d_Y}$. We write 
% % \begin{align*}
% %     (u \bdot Y)_t  \eqdef  \int_0^t u_s dY_s \quad \forall t \in [0:T], 
% % \end{align*}
% % which is interpreted as trading with rate $u$ on the asset $Y$. Furthermore, $r$ refers to the running reward that accumulates over all times $s \in [0,T]$ and $g$ is interpreted as the terminal reward which is received at maturity. 
% % 
% % \begin{example}[Optimal control problems in finance]
% % \begin{enumerate}[wide]
% %     \item \emph{Hedging European options.} In the following, let $h: \R^{d_Y} \to \R$ denote the payoff of a European contingent claim, and set $r \equiv 0$, $g(y, z)  \eqdef  - (z - h(y))^2$. \yannick{Concave?} Then, the optimization task reads as 
% %     \begin{align*}
% %         J(u) \eqdef - \mathbb{E}\left[  \left(h(Y_T) - (u \bdot Y)_T) \right)^2 \right],
% %     \end{align*}
% %     which is tantamount to minimizing the $L^2$-distance of the wealth process at terminal time to the option's payoff.
% %     \item \emph{Optimal Liquidation.} Assume $d_Y \eqdef 2$ with the first component of $Y$ representing the asset price and let the second component of $Y$ constitute the constant process, i.e. $(Y)_{2} \eqdef 1$, therefore $d((u)_{2} \cdot (Y)_{2})_t = u_t dt$ corresponds to the inventory if we require $(u)_1 \equiv (u)_2$. Now, define $alpha: \R \to \R$ as a (concave) utility function and $\beta: \R \to \R$ as a (convex) inventory penalty. If we set $g(y, z) \eqdef \alpha((y)_1) - \beta((y)_1)$ and define by $r(t, y, z, u) \eqdef \Tilde{r}(t, (y)_1, (u)_1)$ the trading cost of $u$ at time $t$ and asset price $(y)_1$, we arrive at a classical optimal liquidation task.
% %     \item ...
% % \end{enumerate}
% % \end{example}
% % 
% % In order to solve \eqref{id:OptimalControl}, we assume conditions XXX. Then we can define the generalized Hamiltonian
% % \begin{align*}
% %     H:
% %     \begin{array}{ccc}
% %         \R_+ \times (\R^{d_Y})^{\times 3} \times \R^{d_Y} & \longrightarrow & \\
% %          & \longmapsto &
% %     \end{array}
% % \end{align*}

% \subsection{Model ambiguity}
% Let $x_{[0:T]} \in XXX$ and assume the dynamics of $Y$ are given by \eqref{eq:filtering_dynamics__observation}. Then,  $Y \vert \lbrace X = x \rbrace$ which is defined via $(Y \vert \lbrace X = x \rbrace)_t \eqdef Y_t \vert \lbrace X_t = x_{t} \rbrace$ for all $t \in [0:T]$ represents an ordinary SDE with full observability. 
% \begin{example}\label{exa:UncertaintyHeston}
%     For any $t \in [0:T]$ and $y_{[0:t]} \in XXX$ consider $A_0(t, y_{[0:t]}) \eqdef (\mu, - \kappa y_t^2)$, $A_1(t, y_{[0:t]}) \eqdef (0, \kappa)$, $B_1(t, y_{[0:t]}) \eqdef 0$, $B_2(t, y_{[0:t]})^1 \eqdef (y_t^1\sqrt{y_t^2}, 0)$, and $B_2(t, y_{[0:t]})^1 \eqdef (\sigma \rho \sqrt{y_t^2}, \sigma \sqrt{1-\rho^2} \sqrt{y_t^2})$, where $\mu \in \R$, $\kappa, \sigma > 0$, and $\rho \in [-1:1]$. This corresponds to the Heston model with (stochastic) mean-reversion parameter $X_t$,
%     \begin{align*}
%             d 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \\
%                     Y_t^2
%                 \end{matrix}
%             \right)
%         = 
%             \left(
%                 \begin{matrix}
%                     \mu \\
%                     \kappa X_t - \kappa Y_t^2
%                 \end{matrix}
%             \right)
%             dt
%         + 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \sqrt{Y_t^2}  \\
%                     \sigma \sqrt{Y_t^2} 
%                 \end{matrix}
%             \right)
%             \left(
%                 \begin{matrix}
%                     1 & \rho \\
%                     \rho & 1
%                 \end{matrix}
%             \right)^{1/2}
%             dW^{(2)}_t, \quad  \forall t \in [0:T],
%     \end{align*}
%     and $Y \vert \lbrace X \equiv \theta \rbrace$, $\theta > 0$ represents the Heston model with deterministic (and constant) mean-reversion parameter $\theta$.
% \end{example}

% In the following, let $g: A \times XXX \mapsto \R$, define a control problem, where the control $a \in A$ acts on the path $y \in XXX$ to obtain the payoff $g(a, y)$. Further, let $u: \R \to \R$ denote a utility (concave) function. Then, under the model assumption $X = x$, the (ambiguity-unaware) control problem reads as follows,
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}} \mathbb{E}\left[
%         u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)
%     \right].
% \end{align*}
% In terms of \Cref{exa:UncertaintyHeston}, one could for instance consider the hedging task $g(a, y)  \eqdef  (a \bdot y^1)_T - h(y_T^1)$ of the European option with payoff structure $h: \R \to \R$, where $\mathcal{A}$ is the set of previsible trading strategies on $Y^1$.

% In \cite{KlibanoffMarinacciMukerji05}, the authors suggest considering not only one choice of model (as we did above with $X = x$) but instead a distribution of models, which are evaluated with a second expected utility. Let $r: \R \to \R$ denote a second (concave) utility function and since 
% \begin{align*}
%         \mathbb{E}\left[u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)\right]    
%     =
%         \mathbb{E}\left[u \circ g(\alpha, Y) \mid \lbrace X = x \rbrace \right],
% \end{align*}
% ambiguity-aware control problem reads as follows, 
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}}
%         \mathbb{E}\left[
%             r \left(
%             \mathbb{E}\left[
%                 u \circ g(\alpha, Y)
%             \mid
%                 X
%             \right]
%             \right)
%         \right].
% \end{align*}
% \yannick{TODO. Explain how a DKF setting applies as the model-process is unobservable.}

% \end{document}




==> OLD/Historical_Versions/Bookkeaping/1_mathcommands.tex <==
\usepackage{amsthm}
% \smartqed  % flush right qed marks, e.g. at end of proof
\usepackage{graphicx}
% \usepackage{geometry}
%  \geometry{
%  a4paper,
%  % total={170mm,257mm},
%  left=17.5mm,
%  right=17.5mm,
%  top=20mm,
%  }

%-------%
% Fonts % 
%-------%
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables


% General Packages
%------------------%
\usepackage{amsfonts,amssymb,bbm}
\usepackage{amsmath}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage[table]{xcolor}
    \usepackage{adjustbox}
\usepackage[UKenglish]{isodate}
\usepackage{graphicx}
\usepackage{silence}
\WarningFilter{caption}{Unknown document class (or package)}
\usepackage[format=default,font=small,labelfont=it]{caption}
\usepackage{subcaption}
\usepackage{hyperref} 
    \hypersetup{
    	colorlinks = true,
    	linkcolor = blue,
    	anchorcolor = blue,
    	citecolor = blue,
    	filecolor = blue,
    	urlcolor = blue
    }
\usepackage{cleveref}
\crefname{lemma}{lemma}{lemmata}
\Crefname{lemma}{Lemma}{Lemmata}

\usepackage{float}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage{rotating}
    %%% Tikz
    \usepackage{tikz}
    \usepackage{tikz-cd} 
    \pgfdeclarelayer{edgelayer}
    \pgfdeclarelayer{nodelayer}
    \pgfsetlayers{edgelayer,nodelayer,main}
    %%%% Custom Node styles
    \tikzstyle{new style 0}=[fill={rgb,255: red,255; green,94; blue,247}, draw=black, shape=circle]
    \tikzstyle{pointy}=[fill=white, draw=black, shape=circle]
    %%%% Custom Edge styles
    \tikzstyle{pointy}=[->]
\usepackage{fontawesome}


%To display labels in the PDF. Comment at the end!
% Code
\usepackage{algpseudocode}
\usepackage[linesnumbered,lined,boxed,commentsnumbered,ruled,longend]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

% TABLE Formatting
\raggedbottom
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength\heavyrulewidth{0.3ex}
\usepackage{lscape}



\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother


\DeclareMathOperator{\Leb}{Leb}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\tr}{tr}
\newcommand{\n}{\mathbbm{n}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\II}{I_{\varepsilon,\Gamma}}

%Modifiche comode 
\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\lam}{\lambda}
\newcommand{\Ll}{\left}
\newcommand{\rr}{\mathbb{R}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
%\def\mathsf{1}{\mathds{1}}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\newcommand{\essinf}{\operatornamewithlimits{ess\,inf}}
\newcommand{\paren}[1]{\left( \left. #1 \right. \right)}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\BL}{BL}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\rhoseason}{m_{\rho}}%\rho_{\mathrm{season}}}% name of the seasonality function: m_{\rho} in [Arlot 2004]
\newcommand{\rhoseasondiscrete}[1]{m_{\rho,#1}}
\newcommand{\rhomin}{\ensuremath{\mu_{\min}}} %changed by Duccio
\newcommand{\rhomax}{\ensuremath{\mu_{\max}}} %changed by Duccio
\newcommand{\croch}[1]{\left[ \left. #1 \right. \right]}
\newcommand{\survival}{\ensuremath{\mathbb{S}}}

% Processes
\newcommand{\process}[3]{{#1}({#2})_{#3}}
\newcommand{\myset}[2]{\lbrace{#1}, \ldots, {#2}\rbrace}
\newcommand{\mySet}[2]{\left\lbrace {#1} \middle\vert {#2} \right\rbrace}


% Mathbb
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Cg}{\mathfrak{C}}
\newcommand{\bdot}{\boldsymbol{\cdot}}


% Calligrafiche
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Kk}{K}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Xx}{\mathcal{X}}

\newcommand{\eqdef}{\ensuremath{\,\raisebox{-1pt}{$\stackrel{\mbox{\upshape\tiny def.}}{=}$}}\,}
% \newcommand{\eqdef}{\stackrel{\mathclap{\tiny\mbox{def.}}}{=}}


\newcommand{\sdim}{{N_\mathrm{sim}}} %Similarity score encoding dimension
\newcommand{\pdim}{{N_\mathrm{pos}}} %Positional encoding dimension
\newcommand{\edim}{{N}} % Encoding dimension
\newcommand{\ddim}{{N'}} % Decoding dimension (target dimension of MLP)
\newcommand{\rdim}{{N_\mathrm{ref}}} %Number of reference paths
\newcommand{\tdim}{{N_\mathrm{time}}} %Number of reference time points
\newcommand{\pldim}{{N_\mathrm{p}}} %Number of time points between linear pieces
\newcommand{\ldim}{{d_K}} %Latent dimension, was {d_K}

% Cose del modello
\newcommand{\rhosummer}{\rho}% name of the length of summer
\newcommand{\rhowinter}{\rho}% name of the length of winter

\newtheorem{atheorem}{Theorem}
\renewcommand{\theatheorem}{\Alph{atheorem}} % "letter-numbered" theorems
\newtheorem*{InformalTheorem}{Informal Theorem}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{notation}{Notation}
\newtheorem{setting}{Setting}[section]
\newtheorem{assumptions}{Assumptions}[section]
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{question}{Question}

% QED Symbol 
\usepackage{etoolbox}
\newcommand{\addQEDstyle}[2]{\AtBeginEnvironment{#1}{\pushQED{\qed}\renewcommand{\qedsymbol}{#2}}\AtEndEnvironment{#1}{\popQED}}
\addQEDstyle{remark}{$\triangleleft$}
\addQEDstyle{example}{$\triangleleft$}



%%%% COMMENTING (Temporary)
\NewDocumentCommand{\luca}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{green}{ 
                            \textbf{L:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
\NewDocumentCommand{\giulia}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{red}{ 
                            \textbf{GL:}
                            \textit{{#1}}
                            }
                        }}
        }
}
\NewDocumentCommand{\anastasis}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{violet}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }
                    
\NewDocumentCommand{\cody}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{orange}{ 
                            \textbf{A:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\newcommand{\byyan}[1]{\textcolor{cyan}{#1}}
\NewDocumentCommand{\yannick}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{cyan}{ 
                            \textbf{Y:}
                            \textit{{#1}}
                            }
                        }}
        }
                    } 

\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\NewDocumentCommand{\xuwei}{mo}{
    \IfValueF{#2}{
    %%%%% NO Margin Note
                        {{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
    %%%% Margin Note
    \IfValueT{#2}{
                        \marginnote{{\scriptsize
                            \textcolor{darkgreen}{ 
                            \textbf{X:}
                            \textit{{#1}}
                            }
                        }}
        }
                    }

\usepackage{appendix}




\newcounter{termcounter}
\renewcommand{\thetermcounter}{\Roman{termcounter}}
\crefname{term}{term}{terms}
\creflabelformat{term}{#2\textup{(#1)}#3}

\makeatletter
\def\term{\@ifnextchar[\term@optarg\term@noarg}%]
\def\term@optarg[#1]#2{%
  \textup{#1}%
  \def\@currentlabel{#1}%
  \def\cref@currentlabel{[][2147483647][]#1}%
  \cref@label[term]{#2}}
\def\term@noarg#1{%
  \refstepcounter{termcounter}%
  \textup{(\thetermcounter)}%
  \cref@label[term]{#1}}
\makeatother


%  \setcounter{termcounter}{0}


\usepackage{comment}

==> OLD/Historical_Versions/OLD/Historical_Versions/2023_09_15.tex <==
% % https://mcmaster.zoom.us/j/2601491351


% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% \documentclass[preprint,12pt,authoryear]{elsarticle}
% \usepackage{amssymb}

% \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}



% \begin{document}

% \begin{frontmatter}
% \title{Deep Kalman Filters Can Filter}
% % \title{Deep Kalman Filters Are Approximately-Optimal Stochastic Filters}

% % \author[inst1]{Matheus Grasselli}
% \author[inst2,inst3]{Blanka Horvath}
% \author[inst1,inst4]{Anastasis Kratsios}
% \author[inst2,inst3]{Yannick Limmer}
% \author[inst1]{Xuwei Yang}


% \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
%             % addressline={Hamilton, Ontario}, 
%             city={Hamilton},
%             % postcode={00000}, 
%             % state={Ontario},
%             country={Canada}}

% \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             % state={Oxfordshire},
%             country={United Kingdom}}

% \affiliation[inst3]{organization={Oxford-MAN Instute for Quantitative Finance, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             % state={Oxfordshire},
%             country={United Kingdom}}
            
% \affiliation[inst4]{organization={Vector Institute},
%             % addressline={Address Two}, 
%             city={Toronto},
%             % postcode={22222}, 
%             % state={Ontario},
%             country={Canada}}
            

% \begin{abstract}
% Deep Kalman filters (DKFs) are a class of neural network models that generate Gaussian probability measures from sequential data.  Though DKFs are inspired by the Kalman filter, they lack concrete theoretical ties to the stochastic filtering problem, thus limiting their applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-times measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  
% \end{abstract}


% \begin{keyword}
% %% keywords here, in the form: keyword \sep keyword
% Stochastic Filtering \sep Conditionally Gaussian Processes \sep Geometric Deep Learning
% %% PACS codes here, in the form: \PACS code \sep code
% % \PACS 0000 \sep 1111
% %% MSC codes here, in the form: \MSC code \sep code
% %% or \MSC[2008] code \sep code (2000 is the default)
% \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% \end{keyword}

% \end{frontmatter}


% \section{Introduction}
% \label{s:Introduction_Deep_Filtering}

% % \byyan{Opening.}\hfill\\
% In several scientific problems, especially in mathematical finance, one is typically interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$; both of which have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0,T]},\mathbb{P})$.  For example, market sentiment impacts market prices, however, only the latter of these two can be reliably measured.  The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is for any time $t>0$ to identify a continuous function $f_t:C([0,t],\mathbb{R}^d)\rightarrow \mathcal{P}(\mathbb{R}^D)$ satisfying 
% \begin{align}
%     \label{goal:Robust_Filtering}
%         f_t(y_{[0:t]})
%     =
%         \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)
%     ,
% \end{align}
% conditioned on any continuous path $y_{[0:t]}$ realized the $d$-dimensional observable process $Y_{\cdot}$ up time $t>0$; where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $D$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0,t]}$.  The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^D$, denoted by $\mathcal{P}(\mathbb{R}^D)$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^d$, denoted by $C([0,t],\mathbb{R}^d)$, with the uniform norm. 

% % \byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
% When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^d)$.  These robust representations are particularly invaluable in mathematical finance where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

% % \byyan{Do Optimal Filters Exist?.}\hfill\\
% In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,Sirjaev1965Filtering,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued processes, make the problem computationally intractable.  

% % \byyan{Computational Challenges}\hfill\\
% The exception to this rule is so-called finite-dimensional filters, which are rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

% % \byyan{Numerical Approaches.}\hfill\\
% The intractability of the computational general filtering problem has the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} when it admits a square-integrable density.  The latter two approaches work well if the coupled system $(X_{\cdot},Y_{\cdot})$ follows the postulated dynamics, and the former particle-filtering approach is well-suited to low-dimensional settings.  

% % \byyan{Why Deep Learning?.}\hfill\\
% The ability of deep neural networks to efficiently solve a variety of problems has inspired the use of deep learning approaches to the numerical stochastic filtering problems; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering}, and the development of measure-valued deep learning models; e.g.~\cite{Acciaio2022_GHT}.  In particular, the need for a more generic approximate stochastic filtering toolbox has motivated the deep learning community to introduce deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, which is the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered model, are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem.  

% This paper constructs a DKF model which can uniformly approximate the map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering}, to arbitrary precision, for any pair of non-Markovian $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0,T]}$-adapted \textit{conditionally Gaussian} stochastic processes studied by \cite{LipShiryaev_II_2001}.  
% %%%%
% %%%%
% %%%%
% \begin{InformalTheorem}[The DKF is a Universal Conditionally-Gaussian Robust Filter]
% \label{Informal_Theorem_Main:Informal_Theorem}
% Fix $t>0$ and let $(X_{\cdot},Y_{\cdot})$ be the partially-observed system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} below, subject to mild regularity conditions.  For any suitable compact subset $K\subseteq C([0:t],\mathbb{R}^d)$, and any approximation error $\varepsilon>0$ there exists a DKF model $\hat{f}:C([0:t],\mathbb{R}^d)\rightarrow \mathcal{N}_d$ satisfying
% \[
%         \sup_{y_{[0:t]}\in K}\,
%             \mathcal{W}_2\big(
%                 f(y_{[0:t]})
%             ,
%                 \hat{f}(y_{[0:t]})
%             \big)
%     <
%         \varepsilon
%     .
% \]
% \end{InformalTheorem}
% %%%%
% %%%%
% %%%%
% Our uniform estimates hold for coupled stochastic differential equations governed by
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% % \tag{Sig}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% % \tag{Obs}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
% We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$, of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% \subsection{The Deep Kalman Filter Model}
% \label{s:Introduction_Deep_Filtering__ss:ModelDetails}
% The proposed deep Kalman filter (DKF), illustrated in Figure~\ref{fig:DKFModel}, generates predictions on the finite-dimensional metric space $(\mathcal{N}_d,\mathcal{W}_2)$ whose points are non-singular Gaussian measures, and whose distance between points is quantified by the $2$-Wasserstein distance.  These predictions are generated from the continuous input paths via the following three-phase process.  
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
%     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
%     \label{fig:DKFModel}
% \end{figure}
% \paragraph{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^d)$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% \paragraph{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% \paragraph{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_d$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.

% \paragraph{Organization of Paper}
% Section~\eqref{s:Setting} formalizes the basic required regularity conditions on the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} and it overviews the required background in optimal transport.  Section~\ref{s:Model} rigersouly introduces the relevant DKF model.  Section~\ref{s:Main_Results} contains the paper's main theoretical results, as well as an overview of the proof methodology.  Several results of independant interest, both concerning the approximation capacity of the DKF model and the local Lipschitz regularity of the robust filtering map~\eqref{goal:Robust_Filtering} are discussed.  Detailed proofs of our results are relegated to Section~\ref{s:Proof}. 

% \section*{Notation}
% % \label{s:Notation}
% \noindent This section serves as a reference, which records the notation used throughout our manuscript.  In what follows, $N,I,J\in \mathbb{N}_+$, $A$ is an arbitrary $I\times J$ matrix, $x,x_1,\dots,x_J\in \mathbb{R}^N$, $f$ is an arbitrary real-valued function on $\mathbb{R}$, and $t\in \mathbb{R}$.
% \begin{enumerate}
%     \item \textbf{Componentwise Composition:} $f\bullet x\eqdef (f(x_n))_{n=1}^N$ for any $N\in \mathbb{N}_+$.%, $x\in \mathbb{R}^N$, and $f:\mathbb{R}\rightarrow \mathbb{R}$.
%     \item \textbf{Rectified Linear Unit (ReLU):} $\operatorname{ReLU}:\mathbb{R}\rightarrow\mathbb{R}$ given by $\operatorname{ReLU}(t)\eqdef \max\{0,t\}$.
%     \item \textbf{Rowwise Product:} $v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}$.% for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
%     \item \textbf{Softmax Function:} $\operatorname{Softmax}(x)\eqdef \big(e^{x_n}/\sum_{i=1}^N\,e^{x_i}\big)_{n=1}^N$.% for any $N\in \mathbb{N}_+$ and any $x\in \mathbb{R}^N$.
%     \item \textbf{Sparsity:} $\|(A_{i,j})_{i,j=1}^{I,J}\|_0\eqdef \#\{A_{i,j}\neq 0:\,i,j=1,\dots,I\}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
%     \item \textbf{Vector Concatenation:} $\oplus_{j=1}^N x_j\eqdef (x_1,\dots,x_J)^{\top}$ is the $J\times N$-matrix whose $j^{th}$ row is $x_j$.%, for $j=1,\dots,N$.
%     \item \textbf{Vectorization:} $\operatorname{vec}((A_{i,j})_{i,j=1}^{I,J})\eqdef (A_{1,1},\dots,A_{I,J})$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
% \end{enumerate}

% \section{The Setting}
% \label{s:Setting}
% This section formalizes the setting in which our analysis takes place.  We begin by specifying the dynamics of the stochastic processes in the filtering problem.  Next, the source space of paths considered is introduced.  Subsequently, we formulate the target space of probability measures wherein the optimal filter lies.

% \subsection{Regularity Conditions on the Partially-Observed System}
% % \label{s:Preliminaries__ss:Dynamics}
% % This section formulates the theoretical problem which this paper addresses.
% % % Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% % % Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  
% % These processes evolve according to the coupled dynamics
% % \begin{align}
% % \label{eq:filtering_dynamics__signal}
% % dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% % \label{eq:filtering_dynamics__observation}
% % dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% % \end{align}
% % where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.
% % 
% % 
% % Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% % \begin{align}
% % \label{id:ConditionalDistribution}
% %     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) 
% % \end{align}
% % where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of the theoretical foundations of DKFs.
% % \begin{question}
% % \label{question:main}
% % Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$?
% % \end{question}
% During our analysis, we maintain the following basic regularity assumptions on the dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
% %%
% \begin{assumption}[Regularity Conditions: Dynamics]
% \label{ass:technical_evolution_conditions}
% We will assume the following uniform bounds:
% \begin{align*}
%     \vert \process{a_1}{t, x}{i, j}\vert \le L
%     \mbox{ and }
%     \vert \process{A_1}{t, x}{k, j}\vert \le L
% \end{align*}
% for $x \in C([0:t], \R^{d_Y})$, $t \in [0:T]$, $i,j=1,\dots,d_X$, and $k=1,\dots,d_Y$.  
% Further, we require the following integrability conditions:\footnote{In particular, the integrability conditions imply that $\bE\bigg[\sum_{j = 1}^{d_X}(X_0)_j^4\bigg] < \infty$.}
% \begin{enumerate}
%     \item[(i)] $\int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item[(ii)] $\int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item[(iii)] $\int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt < \infty$,
%     \item[(iv)] $\int_0^T (\process{b_2}{t, y_{[0:t]}}{i, k})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{k, i})^2 dt < \infty$
%     \item[(v)] $\int_0^T (\process{A_0}{t, y_{[0:t]}}{k})^2 + (\process{B_2}{t, y_{[0:t]}}{k, l})^2 dt < \infty$
% \end{enumerate}
% hold for $i,j=1,\dots,d_X$, and $k,l=1,\dots,d_Y$ and all paths $y_{[0:T]} \in C([0:T], \R^{d_Y})$.  We require that the matrix $B \circ \process{B}{t,x}{}  \eqdef  \process{B_1}{t,x}{} \process{B_1}{t,x}{}^\intercal + \process{B_2}{t,x}{} \process{B_2}{t,x}{}^\intercal$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% \begin{enumerate}
%     \item[(vi)] $\vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%         \le
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2$,
%     \item[(vii)] $(B_k)_{i,j}(t, x)^2  
%         \le 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2)$,
%     \item[(viii)] $\int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt < \infty$,
%     \item[(ix)] $\bE[\vert (X_t)_j \vert] < \infty, \quad \forall t \in [0:T]$,
%     \item[(x)] $\bP\left( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \right) = 1$
% \end{enumerate}
% for indices $i=1,\dots,d_Y$ and $j=1,\dots,d_X$, where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$.  Lastly, we require that the covariance matrix $\Sigma_0$ is positive definite.\anastasis{where is $\Sigma_0$ defined?}
% \end{assumption}
% \begin{comment}
% Moreover, under mild regularity conditions ensuring that $f$ is sufficiently continuous the geometric deep learning results of \cite{kratsios2021universal} and \cite{Acciaio2022_GHT} guarantee that it can be approximated with a class of transformer models.  However, their analysis equally reveals that the required number of parameters to approximate each $f_t$ can depend highly non-favourably on the dimensions $d_X$ and $d_Y$, as a function of the local uniform approximation error, if nothing is assumed of $f_t$.  In these results, the \textit{uniform} (on compact sets) approximation of the probability measure-valued functions $f_{t}$ by a sequential learning model $\hat{f}_t$ \anastasis{dets later} is quantified by
% \[
%     \sup_{y_{[0:T]}\in K}\, \sup_{0\le t\le T}\,
%         \mathcal{W}_2\big(f_t(y_{[0:t]},\hat{f}_t(y_{[0:t]})\big)
%     ,
% \]
% where $K$ is a (non-empty) compact subset of the path-space $\dots$.  \anastasis{Make comment about adapted Wasserstein when predicting multiple steps forward it time.}
% \end{comment}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Setting__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^d)$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^d$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^d$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically\footnote{dets later; obvious.} embed any path $f\in C([0:t],\mathbb{R}^d)$ into a path $F\in C([0:T],\mathbb{R}^d)$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     F(s)\eqdef \begin{cases}
%         f(s) &: \mbox{ if } 0\le s \le t\\
%         f(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $f\mapsto F$ is a linear isometric embedding of the Banach space $C([0:t],\mathbb{R}^d)$ into $C([0:T],\mathbb{R}^d)$ since
% \[
% \|F\|_T = \max_{0\le s\le T}\, \|f(s)\|_2
% = \max_{0\le s\le t}\, \|f(s)\|_2 = \|f\|_t, 
% \]
% since $f(s)=f(t)$ for all $t<s\le T$.  Conversely, the restriction $F_{[0:t]}$ of a path $F\in C([0:T],\mathbb{R}^d)$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^d)$ to $C([0:t],\mathbb{R}^d)$ since
% \[
%         \|F_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|F_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|F_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|F(s)\|_2 
%     =
%         \|F\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^d)$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot by approximated by standard deep neural networks parameterized determined by a number trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing} for general rates.   

% The curse of dimensionality cannot be broken, by can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space, as is the case in our results, shows that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}, however, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are either isometric to some compact Riemannian manifold or they are comprised of piecewise linear paths with finitely many pieces.  In particular, we exclude fractal-like subsets of the path space $C([0:T],\mathbb{R}^d)$ which needn't be compressible into finitely many dimensions without ``loosing information'' (i.e.\ for which there is no bi-Lipschitz embedding into a finite-dimensional normed space).  

% In what follows, we denote the Riemannian volume of a connected $(C^2)$ Riemannian manifold $(M,g)$ by $\operatorname{Vol}(M,g)$.  We denote its geodesic distance function by $d_g$.
% \begin{assumption}[Domain Regularity]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^d)$ and a ``latent dimension $D_K\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}
%     \item[(i)] \textbf{Finite Domains:} $K$ is finite,
%     \item[(ii)] \textbf{Smooth Domains:} There exists a compact and connected $D_K$-dimensional Riemannian manifold $(M,g)$ for which $(M,d_g)$ is isometric to $(K,\|\cdot\|_T)$,
%     \anastasis{I think, I can do a bit better here, and get a compact subset of ...}
%     \item[(iii)] \textbf{Piecewise Linear Domains:} There are $N\in \mathbb{N}_+$, $0=t_0<\dots<t_N=T$, and $C_K>0$ such that $y_{\cdot}\in K$ if and only if:
%         \begin{enumerate}
%             \item[(a)] For $i=0,\dots,N-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^d$ satisfying
%             \[
%             \begin{aligned}
%                 & y(t)=A^{(i)}\,t+b^{(i)}
%                 \,
%                 &
%                 \,
%                 \mbox{ for all } t\in (t_i,t_{i+1})
%             ,
%             \end{aligned}
%             \]
%             \item[(b)] $y_0=0$,
%             \item[(c)] $\max_{i=1,\dots,N}\,|y(t_i)|\le C_K$.
%         \end{enumerate}
% \end{enumerate}
% \end{assumption}
% Evidently, their domains $K$ satisfying Assumption~\ref{ass:reg_compact} (i) are easily exhibited, and they correspond to any \textit{training set}.  One can interpret results in this case as paralleling interpolation results for deep learning, e.g.\ \cite{CristaJosefMartin_2020_UnivInterpol,vershynin2020memory,KratsiosDevarnotDokmanic_SmallTransformers_JMLR2023}, but allowing for some arbitrarily small error as in \cite{park2021provable}.

% Compact subsets of the path-space $C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact} (ii) are also plentiful.  The following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}, and related results such as~\cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}, illustrate this by guaranteeing that $C([0:T],\mathbb{R}^d)$ contains isometric copies of any compact metric space.  Consequentially, $C([0:T],\mathbb{R}^d)$ contains isometric copies of any compact and connected Riemannian manifold.
% \begin{proposition}[Isometric Copies of Every Compact Riemannian Manifold in The Path Space]
% \label{prop:Non_Vaccousness}
% Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^d)$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}

% We obtain explicit estimates for the case where $(K,d_{\cdot})$ satisfies Assumption~\ref{ass:reg_compact} (ii), if the ``model'' smooth manifold $M$ is topologically regular, in that sense that it is \textit{aspherical}.
% This means that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$ (see \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups).  E.g.\ $M$ can be a Torus.

% Domains $K$ satisfying Assumption~\ref{ass:reg_compact} include any piecewise linear interpolation of real-world financial time-series data, or simulated data.  This is because only a finite number of inflection points can be observed, and prices are not unbounded.  

% In this way, Assumption~\ref{ass:reg_compact} summarizes a rich family of compact subsets of the path-space $C([0:T],\mathbb{R}^d)$ which possess a sufficient degree of structure to be losslessly encoded into finitely many dimensions by our model's encoding layer, called its \textit{pathwise attention mechanism}.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Setting__ss:OutputSpace}

% The $2$-Wasserstein space $\mathcal{P}_2(\mathbb{R}^d)$ consists of all probability measures on $\mathbb{R}^d$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_2(\mathbb{R}^d)$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^2]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_2$ on $\mathbb{P}_2(\mathbb{R}^d)$ is given by minimizing the opimtal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_2(\mathbb{P}, \mathbb{Q})^2
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
%     .
% \]
% Generally, the $2$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, the $2$-Wasserstein distance is not always computationally in tractable and in the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite{dowson1982frechet} showed that it admits the following closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^d)$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^d)$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% % This section introduces our attention-based model, our deep Kalman filter (DKF) model, illustrated in Figure~\ref{fig:DKFModel}.  The proposed DKF generates a prediction on the space $(\mathcal{N}_d,\mathcal{W}_2)$ from any observed continuous path in $C([0:T],\mathbb{R}^d)$, via a three-phase process.  

% % \begin{figure}[hpt!]%[H]%
% %     \centering
% %         \centering
% %         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
% %     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
% %     \label{fig:DKFModel}
% % \end{figure}

% % \paragraph{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^d)$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% % \paragraph{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% % \paragraph{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_d$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.


% \subsection{Phase 1 - Encoding via Pathwise Attention}
% \label{s:Model__ss:PathwiseAttention}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and the graph attention mechanism of \cite{velivckovic2017graph} to the context of continuous-time path sources/inputs.  Our attention mechanism, called \textit{pathwise attention}, encodes key information about a novel path $y_{\cdot}$ and like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``know/previously generated paths''.  

% \begin{figure}[hpt!]%[H]%
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.9\linewidth]{Graphics/Similarity_Score.pdf}
%         \caption{\label{fig:Similarity_Score} The \textit{similarity score} component $\operatorname{sim}_t^{\theta_0}$ encodes a path into finite-dimensional vectorial data, by relating its similarity to a dictionary of previously observed ``contextual paths''.}  
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.9\linewidth]{Graphics/Positional_Emcoding.pdf}
%         \caption{\label{fig:PositionalEncoding} The \textit{positional encoding} component $\operatorname{pos}_t^{\theta_0}$ of the attention mechanism allows the similarity scores to further adapt to any novel path by extracting sample-positions on the novel paths.}
%     \end{subfigure}
%     \caption[1]{Our \textit{pathwise attention mechanism} $\operatorname{attn}_t^{\theta}$, in Definition~\ref{defn:PathAttention}, relies on two methods for adaptive feature extraction.  The first component of the mechanism, in~\ref{fig:Similarity_Score}, in is a similarity score which ranks the similarity of any novel path $x_{\cdot}$ to a dictionary of ``recognized/saved'' reference paths.  The second component of the mechanism, in~\ref{fig:PositionalEncoding}, samples points on the novel path $x_{\cdot}$ and perturbs the similarity scores by them.  The adeptness of the pathwise attention mechanism, unlike basis-based methods, is rooted in the fact that nearly all of its the parameters are trainable, which allows it to be tasks-specific (similarly to the advantage of deep MLPs have over regression via basis-functions).}
%     \label{fig:Attention_Is_All_You_Need}
% \end{figure}


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $N$, $N_1$, $d$, and a ``time horizon'' $t> 0$.  
% Given a set of $N$ distinct paths $\{y^{(n)}\}_{n=1}^N$ in $C([0,1],\mathbb{R}^d)$, a $B$ is an $N_1\times N$-matrix, $b\in \mathbb{R}^{N_1}$, $A$ is an $N_1\times N_1$-matrix, and $a\in \mathbb{R}^{N_1}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^N)$.\\
% \noindent The \textit{similarity score}, is a map $\operatorname{sim}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$ by
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{sim}_t^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%             \operatorname{Softmax}
%         \circ
%             \biggl(
%                 A\operatorname{ReLU}\bullet 
%             \Big(
%                     B
%                     \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^N
%                 +
%                     b
%             \Big)
%                 +
%                     a
%         \biggr)
%     ,
% \end{equation}
% where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$.
% \end{definition}

% Illustrated in Figure~\ref{fig:Attention_Is_All_You_Need}, our pathwise attention mechanism extracts features by reinterpreting two of the key features of attention mechanisms from natural language processing (NLP).  First, it utilizes \textit{similarity scores} which rank the likeness of any novel path against a dictionary of references paths.  These reference paths can either arise from real/stress historical (market) scenarios, they can be generated synthetically, or a combination of either.  These similarity scores are illustrated in Figure~\ref{fig:Similarity_Score}, and they serve as pathwise analogues of contextual keys and queries in attention mechanisms in NLP.

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of Definition~\ref{defn:Sim_Score}, fix a positive integer $N_2$, and set of query times $0\le t_1<\dots< t_N\le t$, an $N_2\times d$ matrix $V$, and a $N_2\times N$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^N)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{pos}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined by 
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{pos}_t^{\theta_1}
%         (y_{\cdot} )
%     \eqdef 
%         U \,
%         (\oplus_{j=1}^N \, y_{t_j})
%         + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$.
% \end{definition}

% Next, the \textit{positional encoding} of any novel path, illustrated in Figure~\ref{fig:PositionalEncoding}, encodes samples from the novel path.  These indicates changes in any sample path and they fully determined piecewise linear paths with finitely many pieces (as are generated in simulation studies).  This data is then combines with the weights of the similarity scores to produce the features encodings of our pathwise attention mechanism. 


% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of Definitions~\ref{defn:Sim_Score} and~\ref{defn:PositionalEncoding}, set $N_1=N_2$.  A \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1,C)$, is the map $\operatorname{attn}_t^{\theta}:C([0,1],\mathbb{R}^d)\rightarrow \mathbb{R}^{d\times N}$ with representation
% \[
%         \operatorname{attn}_t^{\theta}(y_{\cdot})
%     \eqdef 
%             C\,
%             \operatorname{vec}\big(
%                     \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%                 \odot
%                     \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%             \big)
% \]
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$, where $C$ is an $M\times (N_1 d)$-dimensional matrix.
% \end{definition}


% \begin{proposition}[Pathwise Attention Losslessly Encodes Regular Domains]
% \label{prop:Lossless_Encoding}
% \hfill\\
% Let $K\subseteq C([0:T],\mathbb{R}^d)$ satisfy Assumption~\ref{ass:reg_compact}.  Then, there exists an $N\in \mathbb{N}_+$ and a parameter $\theta$ as in Definition~\ref{defn:PathAttention} such that, $\operatorname{attn}_T^{\theta}$ restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^N,\|\cdot\|_2)$.
% \hfill\\
% Estimates for the encoding dimension $M$ are recorded in Table~\ref{tab:ATTENTION_Rates} on a case-by-base basis.
% \end{proposition}



% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for Lossless Pathwise Attention Encoding of Regular Compact Domains.}}
%     \label{tab:ATTENTION_Rates}
%     \begin{tabular}{lllll}
%     \toprule
%         Type of Compact Domain %& Complexity ($\|\theta\|_0$) 
%         & Encoding Dimension $(M)$ & Ass.~\ref{ass:reg_compact} \\
%     \midrule
%         Finite%& $\mathcal{O}(\cdot)$ 
%         & $\mathcal{O}(\log(\# K))$ 
%         & (i)
%         \\
%         Iso. Comp. Riemann.%& -- 
%         & Finite
%         & (ii)
%         \\
%         Iso. Comp. Riemann. + Aspherical %& -- 
%         & $\mathcal{O}\big(\mathcal{N}_{d_g}(M,\operatorname{Vol}(M,g)^{1/D_K} )\big)$
%         & (ii)
%         \\
%         P.W. Lin. (N. Pieces) %& - 
%         & $\mathcal{O}(Nd)$
%         & (iii)
%         \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Fix an $A\subset M$ and $\delta>0$.  The quantity $\mathcal{N}_{d_g}(A,\delta)$ denotes the minimum number, $I$, of points $\{x_i\}_{i=1}^I$ in $M$ for which every $x\in M$ is contained in a geodesic ball of radius $\delta$ about some $x_i$, for $i\in \{1,\dots,I\}$.}
% \end{table}

% \subsection{Phase 2 - Multi-Layered Perceptrons (MLPs) Transformation}
% \label{s:Model__ss:Review__MLPs}
% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an source dimension $d$ and a target dimension $D$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^d$ to $\mathbb{R}^D$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^d\rightarrow\mathbb{R}^D$ with iterative representation: for each $x\in \mathbb{R}^d$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=d$ and $d_{J+1}=D$.

% \subsection{Bloack 3 - Decoding via Geometric Attention Mechanism}
% \label{s:Model__ss:GeometricAttentionMechanism}

% Fix $N\in \mathbb{N}_+$.  In what follows, we denote the orthogonal projection of $\mathbb{R}^N$ onto the $N$-simplex 
% \[
%         \Delta_N
%     \eqdef 
%     \{
%         w \in [0,1]^N:\,
%         \sum_{n=1}^N\,w_n = 1
%     \}
% \]
% by $P_{\Delta_N}$.  We note that the closedness and convexity of $\Delta_N$ implies that $P_{\Delta_N}$ is a well-defined $1$-Lipschitz map, see \citep[Proposition 4.8]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017}.  

% \begin{definition}[Geometric Attention Mechanism]
% \label{defn:GeometricAttentionMechanism}
% Let $N,d\in \mathbb{N}_+$.  A geometric attention mechanism is a map $\operatorname{g-attn}_N:\mathbb{R}^N\rightarrow \mathcal{N}_d$ with representation
% \[
%         \operatorname{g-attn}_N^{\vartheta}(v)
%     =
%         \mathcal{N}_d\Biggl(
%                 \sum_{n=1}^N\,
%                     P_{\Delta_N}(v)_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^N\,
%                     P_{\Delta_N}(v)_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)})
%         \Biggr)
% \]
% where $m^{(1)},\dots,m^{(N)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(N)}$ are $d\times d$-matrices; and $\vartheta\eqdef (m^{(n)},A^{(n)})_{n=1}^N$.
% \end{definition}

% \subsection{The DKF Model}
% \label{s:Model}
% We may now formalize the discrete Kalman filter model of Figure~\ref{fig:DKFModel}.  
% \begin{definition}[Deep Kalman Filter]
% Let $d\in\mathbb{N}_+$, $T>0$, and an activation function $\sigma:\mathbb{R}\rightarrow \mathbb{R}$.  
% A function $\hat{F}:C([0:T],\mathbb{R}^d)\rightarrow \mathcal{N}_d$ is called a discrete Kalman Filter if it admits the representation
% \begin{equation}
% \label{eq:DKF_formalization}
%         \hat{f}
%     =
%             \operatorname{g-attn}_N^{\vartheta}
%         \circ 
%             \hat{f}
%         \circ 
%             \operatorname{attn}_T^{\theta}
% \end{equation}
% where $\operatorname{g-attn}_N^{\vartheta}$ is as in Definition~\ref{defn:GeometricAttentionMechanism}, $\operatorname{attn}_T^{\theta}$ is as in Definition~\ref{defn:PathAttention}, and $\hat{f}$ is an MLP as in~\eqref{eq:MLP}; such that the composition~\eqref{eq:DKF_formalization} is well-defined.
% \end{definition}



% \section{Main Result}
% \label{s:Main_Results}

% We are now ready to state our main theorem.
% \begin{theorem}[The DKF Can Approximate the Optimal Filter]
% \label{thrm:MAIN}
% Let $d\in \mathbb{N}_+$ and $K\subset C([0:T],\mathbb{R}^d)$ satisfy Assumption~\ref{ass:reg_compact}.  Suppose that the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies Assumption~\eqref{ass:technical_evolution_conditions}.  % and let $f^{\star}$ denote its associated optimal filter~\eqref{id:ConditionalDistribution}.  
% For every $T>0$ there exists a DKF $\hat{F}:C([0:T],\mathbb{R}^d)\rightarrow\mathcal{N}$ satisfying the uniform estimate
% \[
%     \max_{y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})
%             ,
%                 \hat{F}(y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, Table~\ref{tab:ComplexityMain} records the complexity estimates of $\hat{F}$.
% \end{theorem}

% \begin{table}[H]%[ht!]
%     \centering
%     \caption{{Complexity Estimates for the DKF model $\hat{F}$ in Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:ComplexityMain}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}



% \subsection{Proof Overview}
% \label{s:Theoretical_Analysis}
% This section overviews the derivation of our main result, namely, Theorem~\ref{thrm:MAIN}.
% \paragraph{Summary of What is Known}
% % \label{s:Theoretical_Analysis__ss:LipsterShiryaevSummary}
% Results in \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, they denote an explicit formulation of the resulting distribution which can then analyze directly. 
% Under Assumption~\ref{ass:technical_evolution_conditions}, \citep[Theorem 12.6]{LipShiryaev_II_2001} and we deduce that $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, meaning that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.


% A function is uniformly approximable by a deep learning model if it is continuous.  If there is no clear favourable structure in the function being approximated, e.g.\ smoothness \cite{yarotsky2020phase,gonon2023approximation} or neural network-like structure \cite{cheridito2021efficient,mhaskar2016deep}, then the best available approximation rates are those corresponding to those where the target function is Lipschitz; see \cite{DaubechiesDeVoreFoucartHaninPetrova_CA_KnotFreeReLU_2022}. %devore1993constructive,
% Thus, the first step to obtaining approximability guarantees for the optimal filter, by deep neural networks, which depend on relatively few trainable parameters, is to show that the optimal filter is a locally-Lipschitz function of observed paths.
% \begin{proposition}[Local Lipschitz-Continuity of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter}
% \hfill\\\anastasis{group into simple assumption environment.}\\
%     Fix $t \in [0, T]$. Under the assumptions of \Cref{lem:LipschitzSigma} and \Cref{lem:LipschitzMu}, $f_t$ from \eqref{id:ConditionalDistribution} is locally Lipschitz-continuous. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t 
%     \end{align*}
% \end{proposition}

% Having established the regularity of the optimal filter for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, we need to verify that maps sharing the same domain (input space), codomain (output space), and regularity as the optimal filter are approximable by the proposed DKF model.  This is the content of the next proposition, which acts as its standalone approximation theorem for the DKF.


% \begin{table}[H]%[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}

% \begin{proposition}[Approximation Capacity of DKFs]
% \label{prop:Universal_Approximation_Theorem__PathToNd}
% Let $d\in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}.  
% For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:(K,\|\cdot\|_{\infty})\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ there exists a DKF $\hat{F}$ 
% % \[
% %         \hat{t}(x)
% %     \eqdef
% %         \mathcal{N}_d\Biggl(
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     m^{(n)}
% %             ,
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     (A^{(n)})^{\top}A^{(n)})
% %         \Biggr)
% % \]
% % \anastasis{Update representation/simplify ofc + explain notation} 
% satisfying the uniform estimate 
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{F}(x)
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(N)$ and Decoding dimension $(M)$ are all recorded in Table~\ref{tab:approximationrates__nonFlatVersion} depending on the the choice of activation function $\sigma$.
% \end{proposition}


% We now have at our disposal, the tools to prove our main result.  
% \begin{proof}[{Proof of Theorem~\ref{thrm:MAIN}}]
% Since the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies Assumption~\eqref{ass:technical_evolution_conditions}, then Proposition~\ref{prop:LocLipReg_OptimFilter} implies that the optimal filter $f: y_{[0:t]}\mapsto \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})$ is a locally-Lipschitz map from $(C([0:T],\mathbb{R}^d),\|\cdot\|_T)$ to $(\mathcal{N}_d,\mathcal{W}_2)$.  Since $K\subseteq C([0:T],\mathbb{R}^d)$ is compact then, $f|_K$ is Lipschitz.  

% Since $K\subset C([0:T],\mathbb{R}^d)$ satisfies Assumption~\ref{ass:reg_compact} and $0<\varepsilon<1/2$ then, Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd} implies that there is a DKF $\hat{F}:C([0,T],\mathbb{R}^d)\rightarrow\mathbb{N}_d$ with representation~\eqref{eq:DKF_formalization} and complexity recorded in Table~\ref{tab:approximationrates__nonFlatVersion} satisfying
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{F}(x)
%         \big)
%     < 
%         \varepsilon
% .
% \]
% This completes the proof of Theorem~\ref{thrm:MAIN}.
% \end{proof}


% \section{Proofs of Auxiliary Results}
% \label{s:Proof}
% This section contains the derivations of our paper's results.

% \subsection{Proofs of Auxiliary Results}
% \label{s:Proof__ss:AuxResults}
% \begin{proof}[{Proof of Proposition~\ref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^d)$, given by $f\mapsto \big(f(\cdot /T),0,\dots,0\big)$, is an isometric embedding; then $\phi\eqdef \phi_3\circ\phi_2\circ \phi_1$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^d)$.
% \end{proof}

% \subsection{Stability of the Optimal Filter - Proof of \texorpdfstring{Proposition~\ref{prop:LocLipReg_OptimFilter}}{Lipschitz Continuity}}
% We now prove the local Lipschitz stability of the optimal filter~\eqref{id:ConditionalDistribution}, for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, as a function of its observed/input path.  The proof builds on a series of Lemmata, which demonstrate the local Lipschitz continuity of the parameters defining the optimal filter.  


% We first observe that, Assumption~\ref{ass:technical_evolution_conditions} grants us access to \citep[Theorem 12.7]{LipShiryaev_II_2001}, which implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
% \notag
%     d\mu_t 
%         =&[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\intercal}(t,y_{[0:t]})](B\circ B)^{-1}(t,y_{[0:t]})\\
%         &\times [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt] \label{id:ClosedFormMu}
%     \\
% \notag
%     \partial_t\Sigma_t =& a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\intercal}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]}) - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]}) ]
%         \\
%         & \times (B\circ B)^{-1} (t,y_{[0:t]}) [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]})]^{\intercal} \label{id:ClosedFormSigma}
% \end{align}
% with initial conditions $\mu_0=\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\intercal}|Y_0]$; where
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\intercal + B_2B_2^\intercal, \quad 
%     b \circ B \eqdef b_1B_1^\intercal + b_2B_2^\intercal, \quad 
%     b \circ b \eqdef b_1b_1^\intercal + b_2b_2^\intercal.
% \end{align*}
% Furthermore, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\Sigma_t$ is positive definite for all $t \in [0,T]$ since we have assume that $\Sigma_0$ in Assumption~\ref{ass:technical_evolution_conditions}.

% To clarify the argument's direction, we first record the proof of Proposition~\ref{prop:LocLipReg_OptimFilter}.  We subsequently derive the lemmata on which it relies.
% \begin{proof}[{Proof of Proposition~\ref{prop:LocLipReg_OptimFilter}}]
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a constant $\bar{K} < \infty$ s.t.
%     \begin{align*}
%     \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         &\leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{align*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma} that there exists a constant $K < \infty$, s.t.
%     \begin{align*}
%             \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \quad 
%             \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%     \end{align*}
%     so we obtain 
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%     \end{align*}
%     and the statement follows. 
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]\label{lem:LipschitzMu}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:TimeLipschitzMu}, $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%  \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%  \end{align*} 
% \end{lemma}
% \begin{proof}
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) \notag \\
%   & \quad \quad - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \label{id:Phi1} \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu}, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0, s]}) d y_{[0, s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align} 
%  & \mu^{(1)}_t - \mu^{(2)}_t \notag \\
%  & =   \mu_0^{(1)} - \mu_0^{(2)} 
%   + \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds 
%   + \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \notag \\ 
%  & \quad + \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \notag  
%   + \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\,
% (\mu^{(1)}_s - \mu^{(2)}_s ) ds .  \notag
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} 
%   + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwalls inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$. As a next step, let $\mySet{[s_{i-1}:s_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Moreover, by the use of integration by parts, we have
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         - \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         + \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq t} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% (Time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:t]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 
%       \leq \epsilon_I + K t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that $\eqref{t:gammaB} \leq K \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t$. Eventually, consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to Lipschitz continuity of $\Phi_1$. We conclude, since $\max_{s \in [0:t]} \|\mu^{(2)}_s \|_2 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\eqref{t:gammaC} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$, and therefore $\gamma(t)\leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.
% \medskip

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%         \left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)
%      \notag  
% \end{align} 
% As $\Phi_1$ is (time-)Lipschitz continuous, implying $\max_{s \in [0:t]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$ we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}

% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the assumptions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{align*}
%             \| \mu_t - \mu_s \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0, u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0, u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{align*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 
%         \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwalls inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_0^t a_0(u, y_{[0, u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{ \eqdef  \alpha(t)}
%           + \int_0^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0, s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0, u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi1}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_1$, $ (b \circ B)$, $(B\circ B)^{-1}$, $ A_0$, and $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
% \begin{enumerate}[wide]
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_0$, $(b \circ B)$, $(B\circ B)^{-1}$, $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}[wide]
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:LipschitzA1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq K \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left hand side refers to the Forbenius norm.
% \end{lemma} 
% \begin{proof} 
% From \eqref{id:ClosedFormSigma}, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
% \Sigma_t = & \Sigma_0 + \int_0^t
% a_1(t,y_{[0:s]}) \Sigma_s + \Sigma_s a_1^{\intercal}(s,y_{[0:s]}) + (b\circ b)(s,y_{[0:s]}) - [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]}) ]
%    \notag      \\
%         & \hspace{3cm} \times (B\circ B)^{-1} (s,y_{[0:s]}) [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]})]^{\intercal} ds . \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{align*} 
% & \Sigma^{(1)}_t - \Sigma^{(2)}_t \\
% & = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
% & \quad + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) + 
% \Xi_2^\intercal (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{align*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\intercal(s, y^{(1)}_{[0:s]}) - a_1^\intercal(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{align} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef & \big[ a_1^\intercal(s, y^{(2)}_s) 
%  + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) (b\circ B) (s, y^{(1)}_{[0:s]}) \notag \\ 
% &\quad + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
% \big] .   \label{Xi2} 
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{align} 
%  &\big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\
% & \leq  
% \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%  \notag \\ 
%  & \quad  + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot \notag \\ 
%  & \quad \qquad \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{align}  
% From \Cref{lem:LipschitzA1}, we have that 
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{align} 
%  & \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\ 
% &\quad \leq  
% \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big) 
% \cdot \notag \\ 
% &\quad  \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
% \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{align} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$
%  and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is also uniformly bounded, according to \eqref{Xi2}. 
%  Therefore, from \eqref{Sigma1-2bddXi2} we obtain that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% K ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}

% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and assume local Lipschitz continuity in the path component as well as time-continuity of $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\delta > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \delta$ holds
% \begin{align*} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component, we conclude that $a_1$, $b \circ b$, $A_1^\intercal(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\intercal (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\intercal$ have the same property. By this, together with the triangular inequality, 
%     \begin{align*}
% \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  & \leq  
%  2K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) + \\
% & \qquad + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2 + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \\
% & =  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(1+ \Vert\Sigma^{(1)}_s \big\Vert_2 + \Vert\Sigma^{(2)}_s \big\Vert_2 + \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2 \Big).
% \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < \bar{K} \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in $y_{[0:t]}$, for any $\epsilon>0$, there exists $\delta>0$ such that 
% when 
% $\| y^{(1)}_t - y^{(2)}_t \|_2 < \delta$,  
% $\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \|_2 < \epsilon$, and therefore 
% \begin{align*} 
% \big\| \Sigma^{(2)}_t \big\|_2 \leq \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 + \big\| \Sigma^{(1)}_t \big\|_2 
% \leq \epsilon + K . %\label{Sigma2bdd} 
% \end{align*} 
% \end{proof}

% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let $a_1, b \circ b, b \circ B, (B \circ B)^{-1}, b \circ B, A_1$ be continuous. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\intercal}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma}, then there exists an $r > 0$, s.t. for all times $t \in [0,T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ holds that 
%     \begin{align*}
%         \Sigma_t - r \cdot I_{d_X}
%     \end{align*}
%     is positive semi-definite.
% \end{lemma}
% \yannick{TODO. Assumptions are highlighted below.}
% \begin{proof}
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\intercal(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\intercal(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ being positive semi-definite} at 
%     \begin{align*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal )
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\intercal
%                     \right)
%                 ds.
%     \end{align*}
%     As \byyan{$G_t(y_{[0:t]})$ is positive definite}, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%                 (G_t(y_{[0:t]})^{-1})^\intercal
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%             )
%     \end{align*}
%     and 
%     \begin{align*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\intercal
%             \right)
%         \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{align*}
%     As we \byyan{assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$} as well as \byyan{$K_3 > 0$ s.t. $\tr(A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$} we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\intercal(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]




% \subsection{Stable and Lossless Encoding by Pathwise Attention - Proof of Propositions~\ref{prop:Lossless_Encoding}}
% \label{s:Proof__ss:Encoding}



% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(N)}$ in $C([0:T],\mathbb{R}^d)$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map]
% \label{lem:Good_Feature_Map}
% Under Assumption~\ref{ass:reg_compact} (ii).  
% There is a constant $C_{D_K}>0$, depending only on $D_K$, and a $\delta>0$ depending only on $(M,g)$ such that: for and $\delta$-packing $\{y^{(n)}\}_{n=1}^N$ of $K$, there are matrices $A,B,b,V,U,C$ and vectors $a,b$ for which the parameter $\theta$, as in Definition~\ref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{N+1}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{N+1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\| \in \mathcal{O}(N^2)$.

% \noindent Moreover, if $(M,g)$ is aspherical then:
% \begin{enumerate}
%     \item[(i)] $\delta \in \mathcal{O}( \operatorname{Vol}(M,g)^{1/D_K} )$
%     \item[(ii)] $\|\theta\| \in \mathcal{O}(N^2)$,
%     \item[(iii)] $C_{D_K}\in \mathcal{O}(D_K^{3(D_K+1)/2})$
%     % $0<C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
%     % \item[(i)] $\|A\|_0=2N$, 
%     % \item[(ii)] $\|B\|_0=2N$, 
%     % \item[(iii)] $\|a\|_0=1$, 
%     % \item[(iv)] $\|b\|_0=0$, 
%     % \item[(v)] $\|C\|_0= N_1$, 
%     % \item[(vii)] $\|U\|_0=0$, 
%     % \item[(viii)] $\|V\|_0= N^2_1$,
%     % \item[(ix)] $0<C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
% \end{enumerate}
% % \anastasis{perhaps I tally into a single parameter estimate} like $\|\theta\| \in \mathcal{O}(N^2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map}}]
% \noindent\textbf{Step 1 - Estimating $N$ on the Riemannian Manifold $(M,g)$}
% \hfill\\
% %%
% Since $(K,\|\cdot\|_T)$ be isometric to $(M,d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $D_K$-dimensional Riemannian manifold $(M,g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $M$ denoted by $\operatorname{sys}(M)$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(M) 
%     \le
%     \,\tilde{C}_{D_K}
%     \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \end{equation}
% where $\operatorname{Vol}(M,g)$ denotes the Riemannian volume of $(M,g)$ and $\lesssim$ hides a constant depending only on the dimension $D_K$, for a universal constant $\tilde{C}_{D_K}>0$ satisfying
% \[
%         0
%     <
%         \tilde{C}_{D_K}
%     <
%         6 (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}
% \,
% .
% \]
% By Stirling's approximation, $\sqrt{(D_K+1)!} \in \mathcal{O}(D_K^{(D_K+1)/2}$; whence, $\tilde{C}_{D_K}\in 
% % \mathcal{O}(D_K^{D_K+1}\, D_K^{(D_K+1)/2})$
% \mathcal{O}(D_K^{3(D_K+1)/2})$.

% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(M)/10$ then the given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(M,g)$, the map $\varphi_2:(M,d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{D_K}\eqdef \tilde{C}_{D_K}/10$, $N\eqdef \#\widetilde{\mathbb{X}}$, and enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^N$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{D_N}
%         \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     .
% \]
% We note that, if $K$ is not aspherical, then but it is only closed, then the conclusion still holds however, without the quantitative upper-bound on $\delta$.
% \hfill\\
% \noindent\textbf{Step 2 - Building the Feature Map with Well-posed Inverse}
% \hfill\\
% %%
% Let $\varphi_1:(M,d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have assumed to exist.  Set $\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^N$ where, for $n=1,\dots,N$ we set $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\varphi: C([0,T],\mathbb{R}^d)\rightarrow \mathbb{R}^N$ by $y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^N$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^N
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^N
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^N
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^N
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $M$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \hfill\\
% \noindent\textbf{Step 3 - Aligning to a Hyperplane in $\mathbb{R}^{N+1}$ with a Shallow ReLU Neural Network}
% \hfill\\
% Set $N_1\eqdef N+1$.  Let $b$ be the zero vector in $\mathbb{R}^N$.
% A mild variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $N\times 2N$ and $2N\times N$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_N & \vert & -I_N
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_N \\
%             \-- \\
%             -I_N
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^N\rightarrow \mathbb{R}^N$ defined by $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^N$.  Consider the $N_1\times N$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{N_1}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_N & 0 \\
%             0 & 0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,N\\
%             1 & \mbox{ if } i=N_1
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \hfill\\
% \noindent\textbf{Step 4 - Injectivity of Softmax Function on Hyperplane}
% \hfill\\
% Note that, for each $u\in \mathbb{R}^N$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^N$ onto the $N$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^N\}$ in $\mathbb{R}^{N_1}$.  Observe that the Softmax function $\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^N\,e^{u_k})_{j=1}^N$ maps $H$ surjectively and continuously onto the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})\subset \operatorname{int}(\Delta_N)\eqdef \{v\in [0,1]^{N_1}:\,\sum_{i=1}^{N_1}\,v_i=1\}$; i.e.\ of the interior of the $N_1$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{N_1}) + 1\big)_{i=1}^{N}
% \end{equation}
% is a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})$ then, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{N_1})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$.  Since, $\Psi$ was constructed to be an instance of $\operatorname{attn}_T$.  
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_N)$ of the $N_1$-simplex then, $C^{\star}\eqdef \max_{u\in \Phi(K)}\,\min_{v\in \Delta_{N_1}\setminus \operatorname{int}(\Delta_{N_1})}\,\|u-v\|>0$.  Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{N_1}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{N_1})
%             +
%             \bar{\Delta}_{N_1}
%         \}
% \]
% where $\bar{\Delta}_{N_1}\eqdef (1/N_1,\dots,1/N_1)$ is the barycenter of the $N_1$-simplex $\Delta_{N_1}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{N_1}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is Lipschitz\footnote{\anastasis{Add details about Lipschitzness? or Obvious?}} on $\Delta_{N_1}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image since it is the composition of Lipschitz functions with Lipschitz inverses.  
% \hfill\\
% \textbf{Step 5 - Representation as an Attention Mechanism}
% \hfill\\
% Set $\theta_0 = (A,B,a,b, \{y^{(n)}_{\cdot}\}_{n=1}^{N_1})$ and observe that the map $\Psi$ is of the form~\eqref{eq:featuremap}.  
% Let $U$ be the $N_1\times N_1$-dimensional zero matrix, and let $V$ be the $N\times N$-dimensional matrix whose entries are all $1$s.  Set $\theta_1\eqdef (U,V,\{n/{N_1}\}_{n=1}^{N_1})$.  Let $C$ be the $N_1\times N_1 d$-dimensional matrix given by $Cx = (x_i)_{i=1}^{N_1}$ for every $x\in \mathbb{R}^{N_1 d}$.  Set $\theta\eqdef (\theta_0,\theta_1,C)$ and observe that 
% \[
%         \operatorname{attn}_T^{\theta}(y_{\cdot}) 
%     \eqdef
%             C\,
%             \operatorname{vec}\big(
%                     \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%                 \odot
%                     \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%             \big)
%     = 
%         \Psi(y_{\cdot})
% \]
% for each $y_{\cdot}\in K.$. Consequentially, $\operatorname{attn}_T^{\theta_{\cdot}}$ is a bi-Lipschitz embedding of $K$ to $\mathbb{R}^M$.  Note that $\|C\|_0= N_1$, $\|U\|_0=0$, and $\|V\|_0= N^2$.  Thus, $\|\theta\|_0\in \mathcal{O}(N^2)$.  
% This concludes the proof.
% \end{proof}

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Finite Version]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under Assumption~\ref{ass:reg_compact} (i) and let $k\eqdef \#K$.  
% Set $N=192\lceil\log(k)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There is a parameter $\theta$ as in Definition~\ref{defn:PathAttention} defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{192\lceil \log(k)\rceil}$ which restricts to a $(2^{-1/2},(3N/6)^{1/2})$-bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{192\lceil \log(k)\rceil},\|\cdot\|_2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}
% \begin{proof}
% We argue similarly to the proof of Lemma~\ref{lem:Good_Feature_Map}, with only Steps $1$ and $2$ of its proof being replaced with the following argument.  
% \hfill\\
% \noindent\textbf{Step 1 and 2 - Modified- Building the Feature Map}
% \hfill\\
% Enumerate $K=\{x_n\}_{n=1}^N$.  The map $\phi_1:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^N,\|\cdot\|_{\infty})$ given by $x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^N$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le N^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^N$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^N,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^N,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% By the Johnson-Lindenstrauss Lemma, as derived in \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $4*48$ as opposed to $4*200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , there is a linear map $\phi_3:(\mathbb{R}^N,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\lceil192\,\ln(N)\rceil},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $(\lceil48\,\ln(N)\rceil)\times N$-matrix $A_0$, satisfying: for every $u,v\in \mathbb{R}^N$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, $\varphi:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3N/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_{t}
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         N^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3N/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_t 
% .
% \end{align*}
% \noindent\textbf{Remaining Steps:}
% \hfill\\
% The rest of the proof is identical to the proof of Lemma~\ref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_N\,\vert \,I_N)^{\top}$.
% \end{proof}


% \begin{lemma}[Bi-Lipschitz Embedding of Piecewise Linear Paths]
% \label{lem:biLip_pw_lin}
% Fix $N\in \mathbb{N}_+$, $0=t_0<\dots<t_N=T$, and a constant $C_K>0$.
% Let $K\subset C([0:T],\mathbb{R}^d)$ be such that $y_{\cdot}\in K$ if:
% \begin{enumerate}
%     \item[(i)] For $i=0,\dots,N-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^d$ satisfying
%     \[
%     \begin{aligned}
%         & y(t)=A^{(i)}\,t+b^{(i)}
%         \,
%         &
%         \,
%         \mbox{ for all } t\in (t_i,t_{i+1})
%     ,
%     \end{aligned}
%     \]
%     \item[(ii)] $y_0=0$,
%     \item[(iii)] $\max_{i=1,\dots,N}\,|y(t_i)|\le C_K$.
% \end{enumerate}
% There is a parameter $\theta$, as in Definition~\ref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^d)\rightarrow \mathbb{R}^{Nd}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{Nd},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0\in \mathcal{O}(Nd)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{in}$ on $K$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:biLip_pw_lin}}]
% Set $N_1=N$.  Let $A,B$ be the $N_1\times N_1$-dimensional zero matrix and $a,b$ be the zero vector in $\mathbb{R}^{N_1}$.  Set $\theta_0=(A,B,a,b)$.  Observe that 
% \[
% \operatorname{sim}_T^{\theta_0}(y_{\cdot})_i = 1
% \]
% for all $y\in C([0:T],\mathbb{R}^d)$ and each $i=1,\dots,d$.  
% Let $V$ be the $N_1\times N_1$-dimensional zero matrix, $U=I_{N}$ where $I_N$ is the $N\times N$-dimensional identity matrix, and\footnote{The point $t_0$ is not sampled since every path $y_{\cdot}$ in $K$ satisfies $y_0=0$, and thus, there is no need to sample it at time $0$.} $\theta_1=(U,V,\{t_n\}_{n=1}^N)$.  Then, 
% \begin{equation}
% \label{eq:bijection_sampling}
%         \operatorname{pos}_T^{\theta_1}(y_{\cdot})
%     =
%         (y_1,\dots,y_N).
% \end{equation}
% In particular, the map $\operatorname{pos}_T^{\theta_1}$ in ~\eqref{eq:bijection_sampling} defines a linear bijection between $\mathcal{K}$ and the set $[-C_K,C_K]^N$.  Since $[-C_K,C_K]^N$ a subset of the finite-dimensional Banach space $(\mathbb{R}^N,\|\cdot\|_2)$ and all norms on a finite-dimensional normed are equivalent, then, $\operatorname{sim}_T^{\theta_1}$ is a bi-Lipschitz embedding of $K$ into $(\mathbb{R}^N,\|\cdot\|_2)$.  

% Let $C$ be the $Nd\times Nd$-dimensional matrix with $C_{i,j}=1$ for $i,j=1,\dots,Nd$.  Set $\theta=(\theta_0,\theta_1,C)$.  By construction $\|\theta\|_0\in \mathcal{O}(Nd)$.  
% Then, 
% \begin{equation}
% \label{eq:bijection_sampling__RelabelingStuff}
%         \operatorname{attn}_T^{\theta}(y_{\cdot})
%     \eqdef 
%         C\,
%         \operatorname{vec}\big(
%                 \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%             \odot
%                 \operatorname{pos}_t^{\theta_1}(y_{\cdot})
%         \big)
%     =
%         (y_1,\dots,y_N)
%     .
% \end{equation}
% Together,~\eqref{eq:bijection_sampling} and~\eqref{eq:bijection_sampling} imply that $\operatorname{attn}_T^{\theta}$ defines a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \end{proof}

% \begin{proof}[{Proof of Proposition~\ref{prop:Lossless_Encoding}}]
% Follows directly from Lemmata~\ref{lem:Good_Feature_Map},~\ref{lem:Good_Feature_Map__FiniteVariant}, and~\ref{lem:biLip_pw_lin}.
% \end{proof}

% \subsection{Approximability of Locally Lipschitz Maps By DKFs - Proof Propositions~\ref{TBD}}
% We now prove our main universal approximation theorem, Propositions~\ref{TBD}.  We show that the target space/codomain of any considered DKF is geometrically regular, in the sense of \cite{Acciaio2022_GHT,kratsios2023transfer}.  Using this fact, we then combine and apply the results of \cite{kratsios2021universal,kratsios2023transfer} to deduce the result.

% % HERE!

% \subsubsection{Step A - Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}
% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d\in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d}$ denote the set of $d\times d$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d\times d$ matrices.  Here the $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.  Consider the $2$-product metric on $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ defined for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ by sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ will serve to quantize $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^d\times \operatorname{Sym}_{0,d})^{N} \rightarrow 
% \mathbb{R}^d\times \operatorname{Sym}_{0,d}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:QAS_Space_Sym0d}]  
% We first show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% \hfill\\
% \textbf{QAS Space Structure}
% \hfill\\
% Since $\operatorname{Sym}_{0,d}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the normed space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ as sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big)
%     = &
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     = &
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     \le &
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad            
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     \le &
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     = &
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\mathcal{Q},\eta)$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
% \hfill\\
% \textbf{Barycentricity}
% \hfill\\
% Consider the map $\sigma:(\mathbb{R}^d\times \operatorname{Sym}_{0,d})^2\times [0,1]$ given for any $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and $t\in [0,1]$ by
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),t
%         \big)
%     \eqdef 
%         \eta\big(
%             (m,A),(\tilde{m},B),(t,1-t)
%         \big)
%     .
% \]
% Since geodesics in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ are line segments, since $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the inner-product space $(\mathbb{R}^d\times \operatorname{Sym}_d)$, with inner-product given by the product of the Euclidean and Frobenius inner-products, then clearly for each $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ the map $t\mapsto \sigma\big((m,A),(\tilde{m},B),t\big)$ is a geodesic in the global NPC space, as defined in \citep[Definition 2.1]{Sturm_2003}, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$.  Thus, $\sigma$ is a \textit{geodesic bicombing} in the sense of \citep[page 1]{basso2018fixed}.  Since 
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
%     =
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
% \]
% then \citep[Theorem 3.4]{basso2018fixed} applies; whence $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is barycentric with $1$-Lipschitz barycenter map explicitly given therein.  

% Since is a barycentric QAS space then, \citep[Setting 3.6]{kratsios2023transfer} (iii) is satisfied.
% \end{proof}

% Having established the barycentricity and the QAS space structure of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\eta,\mathcal{Q}_{\cdot})$, we are now ready to prove the following result.
% \anastasis{Here in transcription}
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ there is a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ satisfying
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x_{\cdot}),f(x_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{t}(x_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^M\,
%                 P_{\Delta_M}(\hat{f}\circ \operatorname{attn}_T(x_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $M\in \mathbb{N}_+$, $m^{(1)},\dots,m^{(M)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(M)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_M}:\mathbb{R}^M\rightarrow\Delta_M$ is the Euclidean (orthogonal) projection onto the $M$-simplex, and an MLP $\hat{f}:\mathbb{R}^N\rightarrow \mathbb{R}^M$ with activation function $\sigma$.  The depth, width, encoding dimension (N), and decoding dimension (M) are recorded in Table~\ref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{D_K}\operatorname{Vol}(M,g)^{1/D_K})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:approximation_Sym}}]
% \anastasis{Relabel $N$ (index) as $M$}
% \hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% We will apply \citep[Theorem 3.7]{kratsios2023transfer}, which requires us to verify each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \paragraph{Step 1 - Implementing a Bi-Lipschitz Feature Map with the Attention Layer}
% \hfill\\
% \textbf{Remark:} \textit{We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap} can be chosen such that $\operatorname{attn}_T$ is a suitable feature map}.
% \hfill\\
% \begin{comment}
% \paragraph{Case (i) - The Continuous and Injective Case} 
% \anastasis{come back to this shortly...}
% \paragraph{Case (ii) - The Bi-Lipschitz Case} 
% \noindent 
% \end{comment}
% Let $N$ denote the $C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(\mathcal{M},d_g)$.  Since $(K,\|\cdot\|_T)$ and $(\mathcal{M},d_g)$ are isometric, then $N$ is the $C_{D_K} \operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(K,\|\cdot\|_T)$.  
% By Lemma~\ref{lem:Good_Feature_Map}, there are matrices $A,B$, $a$, and $b$ with $\|A\|_0=2N=\|B_0\|$, $\|a\|_0=1$, and $\|b\|_0=0$ such that $\varphi\eqdef \operatorname{attn}_T$, as defined in~\eqref{lem:Good_Feature_Map}, is a bi-Lipschitz embedding of $(K,\|\cdot\|_{T})$ to $(\mathbb{R}^N,\|\cdot\|_2)$.  Set $\{(K,\varphi)\}$, let $\nu$ denote the normalized (uniform) Volume probability measure on $(\mathcal{M},g)$, and let $\mu\eqdef \varphi_{\#}\nu$ be its pushforward to $(K,\|\cdot\|_T)$.  Since every bi-Lipschitz map is a quasi-symmetry\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}, then \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(M,d_g)$ is a doubling metric space, as defined on \citep[10.13; page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  This verifies \citep[Setting 3.6 (i)]{kratsios2023transfer}.




% \paragraph{Step 2 - Feature Space Geometry}\hfill\\
% Since the codomain of $\phi$ is simply a Euclidean space, then the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^N}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^N$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^N$, 
% \[
%     \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
% \]
% and the operator norm $\|1_{\mathbb{R}^N}\|_{op}$ of $1_{\mathbb{R}^N}$, thus of $T^i$ for every $i\in \mathbb{N}_+$, is uniformly bounded above by $1$.  
% Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} is holds.

% \paragraph{Step 3 - Geometry of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$}
% \hfill\\
% By Lemma~\ref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $N\in\mathbb{N}_+$, $u\in \mathbb{R}^N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 P_{\Delta_N}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \paragraph{Step 4 - Determining The Euclidean Universal Approximator}
% \hfill\\
% \textbf{Remark:} \textit{We now verify that the class of all MLPs with activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition} satisfies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.}\\
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le d+D+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy Assumption~\ref{ass:KLCondition} then, \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \paragraph{Step 5 - Applying~{\citep[Theorem 3.7]{kratsios2023transfer}}}
% Steps $1$ though $5$ verify that the conditions of Theorem~\citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the Feature Decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, Theorem~\citep[Theorem 3.7]{kratsios2023transfer} implies, thus for every $\varepsilon>0$ there is a map $\hat{t}:K\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{t}(x_{\cdot})
%     = &
%         \beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^N
%             \,
%                 \big(
%                     P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $x_{\cdot}\in K$ satisfying 
% \[
%     \sup_{x_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{t}(x_{\cdot})
%         ,
%             f(x_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ (which exists by Lemma~\ref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a right-inverse of the map $\mathbb{R}^d\times \operatorname{Sym}_{0,d}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$, where $\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially,~\eqref{eq:transformer_pre_mapped_BEGIN}-~\ref{eq:transformer_pre_mapped_END} reduces to~\eqref{lem:approximation_Sym__approximation___representation}.  


% \paragraph{Step 6 - Tallying Parameters}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $N=\mathcal{N}_{\operatorname{pack}}\big(K,C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in Table~\ref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $N$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             N
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{proof}

% \subsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool.  The proof method is summarized visually in Figure~\ref{fig:Approximation_Theorem}.


% \anastasis{t and t hat}
% \begin{figure}[H]
%     \centering
%     \begin{tikzcd}
%     \big(C([0:T],\mathbb{R}^d),\|\cdot\|_{\infty}\big) & (\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2) \\
%     (K,\|\cdot\|_{\infty}) 
%     \arrow[hookrightarrow]{u}{\iota} 
%     \arrow{r}{f} 
%     % \arrow[swap]{d}{\varphi} 
%     \arrow{dr}{\varrho\circ f}
%     & ({\mathcal{N}}_d,\mathcal{W}_2) 
%     \arrow[hookrightarrow]{u}{i}
%     \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
%     & (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
%     \end{tikzcd}
%     \caption{Summary of Proof Strategy for Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd} \anastasis{details}.}
%     \label{fig:Approximation_Theorem}
% \end{figure}


% \begin{proof}[{Proof of Proposition~\ref{prop:Universal_Approximation_Theorem__PathToNd}}]
% \hfill\\
% \textbf{Step 1 - Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$}
% By Lemma~\ref{lem:LipschitzManifold_Nd} the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^d,\operatorname{Sym}_{0,d},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous then the map
% \[
%     g: (K,\|\cdot\|_T)\ni x \mapsto 
%     \pi\circ \varrho\circ f(x)
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d\times d$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain is achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; i.e.
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_d$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% \anastasis{Add reference to Lemma~\ref{lem:LoewnerBound} here.}
% Consequentially, Lemma~\ref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \hfill\\
% \textbf{Step 2 - Approximating $\varrho \circ f$ on $K$}
% \hfill\\
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%                     \,\operatorname{diam}(K) + 1
%                 }
%                 }
%         \biggr\}
% .
% \end{equation}
% We many now apply Lemma~\ref{lem:approximation_Sym} to deduce that there exists a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x),\varrho\circ f(x))
%     <
%         \delta
% .
% \end{equation}
% Since Lemma~\ref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  Set $t\eqdef \varrho^{-1}\circ \hat{t}$ and 
% denote the $1$-thickening of $\varrho\circ f(K)$ by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}:\,(\exists x\in K)\, d_{2,F}(f(x),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{t}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate} and Lemma~\ref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% = & 
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{t}(x)
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{x\in K}\,
%         d_{2,F}\big(
%                 \hat{t}(x)
%             ,
%                 \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% \le &
%     \sqrt{d}2\sqrt{
%             L
%             \,\operatorname{diam}(K) + 1
%         }
%     \,
%     \varepsilon
%     \,
%     \frac1{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:Approxim_LEMMA__END}
% = & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from Lemma~\ref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B} followed from the estimate~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009}, then estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% %\label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_p\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \textbf{Step 3 - Counting Parameters}
% Using $\delta$, as defined in~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in Table~\ref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \anastasis{Add computations tomorrow}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_d}$ denote the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_d}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_d}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_d},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_d}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of Lemma~\ref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_d}$ sending any $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_d}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_d}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_d}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_d},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_d}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_d}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}



% \appendix
% \section{Auxiliary Lemmata}
% \label{s:AuxLemmata}
% This section records auxiliary lemmata used in our proofs but proven elsewhere.
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% it holds that
% \[
% \begin{aligned}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     \\
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{aligned}
% \]
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzManifold_Nd}}]
% The proof is due to \textit{Iosif Pinelis}, and is given in \cite{LocalLipschitz_Pinelis}.  We only note that, $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$ where $\|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})$ denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}

% \section{Background: Riemannian Geometry and Algebraic Topology}
% \label{s:Background_Geo}



% \bibliographystyle{abbrvnat}
% \bibliography{Bookkeaping/2_References}


% \newpage
% \section{Algorithms}
% \input{Sections/Practical_Approach}

% \newpage
% \newpage
% \section{Applications}

% In this section, we will discuss exemplary applications that leverage the possibility to approximate a Kalman filter setting with our suggested framework. 
% For this, we first discuss how to fit and solve a filtering problem on the basis of sample paths for $Y_{[0:T]}$.
% We begin by revisiting the training procedure of Deep Kalman filters suggested in \cite{KrishnanShalitSontag17}, which motivates an approach that aligns more with our framework.

% \subsection{Training a Deep Kalman Filter as in \texorpdfstring{\cite{KrishnanShalitSontag17}}{Krishnan et al. (2017)}}
% For this, we reduce the setting of our filtering problem \eqref{eq:filtering_dynamics__signal},  \eqref{eq:filtering_dynamics__observation} such that the desired training framework is applicable. For this, functions $a_0$, $a_1$, $b_1$ are replaced with constants, we assume independence of the stochastic components, i.e. $b_2 \equiv B_1 \equiv 0$, and $A_0$, $A_1$, $B_1$ are assumed to be Markovian, i.e. functions mapping from $\R^{d_Y}$ to the corresponding space. Then, the former constants are treated as parameters and the latter functions are approximated by MLPs, and we denote their combined (learnable) parameters by $\phi$. We then denote the resulting filtering setting by
% \begin{align*}
%     dX_t & = [a^\phi_0 + a^\phi_1 X_t]dt +  b^\phi_1 dW^{(1)}_t \\
%     dY_t & = [A^\phi_0(Y_{t}) + A^\phi_1(Y_{t}) X_t]dt + B^\phi_2(Y_{t})dW^{(2)}_t. 
% \end{align*}
% This is then discretized by an Euler scheme for time steps $0 = t_0 < t_1 < \ldots < t_N = T$, $N \in \N$, with $\Delta t_n := t_{n}- t_{n-1}$, s.t. 
% \begin{align*}
%     X_{t_{n}} & \sim  \mathcal{N}\left(
%             (a^\phi_0 + a^\phi_1 X_{t_{n-1}})
%             \Delta t_n
%         ,
%             b^\phi_1
%             \Delta t_n
%     \right)
%     \\
%     Y_{t_{n}} & \sim \mathcal{N}\left(
%             (A^\phi_0(Y_{t_{n-1}}) + A^\phi_1(Y_{t_{n-1}}) X_{t_{n}})
%             \Delta t_n
%         ,
%             B^\phi_2(Y_{t_{n-1}})
%             \Delta t_n
%     \right)
% \end{align*}
% In the following, we denote for $n \in \myset{1}{N}$ the likelihood of $Y_{t_n} = y_{t_n} \in \R^{d_Y}$ under the parametrization $\phi$ by $p_\phi(y_t)$ and the likelihood conditional on $Y_{t_n} = y_{t_n}$ by $p_\phi( \cdot \vert y_{t_{n}})$. We can extend this notation to paths, i.e. for $Y_{[t_0:t_n]} = y_{[t_0:t_n]}$, we write $p_\phi(y_{[t_0:t_n]})$ and $p_\phi( \cdot \vert y_{[t_0:t_n]})$. Then, the fitting procedure is based on the observation that 
% \begin{align*}
%         \log p_\phi(y_{[t_0:t_N]}) 
%     & =  \log \int
%             \frac{
%                 p_\phi\left(
%                     y_{[t_0:t_N]}
%                 \middle|
%                     x_{[t_0:t_N]} 
%                 \right)
%                 p_\phi(x_{[t_0:t_N]} )
%             }{
%                 p_\phi\left(
%                     x_{[t_0:t_N]}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)
%             }
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%         dx_{[t_0:t_N]} \\ 
%     & \geq \int 
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%             \log \frac{
%                 p_\phi\left(
%                     y_{[t_0:t_N]}
%                 \middle|
%                     x_{[t_0:t_N]}
%                 \right)
%                 p_\phi(
%                     x_{[t_0:t_N]}
%                 )
%             }{
%                 p_\phi\left(
%                     x_{[t_0:t_N]}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)
%             }
%         dx_{[t_0:t_N]}  \\
%     & =
%         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
%             \log p_\phi\left(
%                 y_{[t_0:t_N]}
%             \mid
%                 x_{[t_0:t_N]}
%             \right)
%         \right]
%     -
%         \mathrm{KL} \left(
%             p_\phi\left(
%                 x_{[t_0:t_N]}
%             \middle|
%                 y_{[t_0:t_N]}
%             \right)
%         \middle\Vert
%             p_\phi(
%                 x_{[t_0:t_N]}
%             )
%         \right)
% \end{align*}
% which can be factorized due to the Markovian property of $Y$ and $X$ to 
% \begin{align*}
%         \log p_\phi(y_{[t_0:t_N]}) 
%     & \geq
%         -
%             \mathrm{KL} \left(
%                 p_\phi\left(
%                     x_{t_0}
%                 \middle|
%                     y_{[t_0:t_N]}
%                 \right)           
%             \middle\Vert
%                 p_\phi(
%                     x_{t_0}
%                 )
%             \right) 
%         +
%             \sum_{n=0}^N
%             \mathbb{E}_{p_\phi(x_{t_n} \vert y_{[t_0:t_N]})} \left[
%                 \log p_\phi\left(
%                     y_{t_n}
%                 \mid
%                     x_{t_n}
%                 \right)
%             \right] \\ 
%         &\quad -
%             \sum_{n=1}^N
%             \mathbb{E}_{
%                 p_\phi(x_{t_{n-1}} \vert y_{[t_0:t_N]})
%             } \left[
%                 \mathrm{KL} \left(
%                     p_\phi\left(
%                         x_{t_n}
%                     \middle|
%                         x_{t_{n-1}}, y_{[t_0:t_N]}
%                     \right)
%                 \middle\Vert
%                     p_\phi\left(
%                         x_{t_n}
%                     \middle|
%                         x_{t_{n-1}}
%                     \right)
%                 \right)
%             \right].
% \end{align*}
% In the above expression, all terms are known in analytical form, except for $p_\phi( x_{t_n} | y_{[t_0:t_N]})$ and $p_\phi( x_{t_n} | x_{t_{n-1}}, y_{[t_0:t_N]})$, which is approximated a machine learning structure, that can be learned simultaneously in the process. One key feature of this structure is its capability to produce the posterior distribution both, conditional and unconditional, on $x_{t_{n-1}}$. This argument is valid due to the fact that the lower bound of $\log p_\phi(y_{[t_0:t_N]})$ is tight, when the produced posterior coincides with the (intractable) conditional distribution under $\phi$ with respect to the Kullback-Leibler divergence. \byyan{Since the Wasserstein distance used in this article is bounded by the Kullback-Leibler divergence, our result in \Cref{thrm:MAIN} can be used to show that this approximation argument holds.} 

% \subsection{Fitting the general filtering problem}
% In this section, we extend our filtering framework by removing the constraints that were introduced in the previous section. Specifically, we no longer enforce the restrictions on our filtering setting. To approximate the functions \(a_0\), \(a_1\), \(b_1\), \(b_2\), \(B_1\), \(A_0\), \(A_1\), and \(B_1\), we employ MLPs. Upon discretizing the system using the Euler scheme, we obtain the following dynamical equations:
% \begin{align}
%         X_{t_{n}}
%     & \approx
%             X_{t_{n-1}}
%         +
%             [a_0(t_{n-1},Y_{[0:t_{n-1}]}) + a_1(t_{n-1},Y_{[0:t_{n-1}]}) X_{t_{n-1}}] \Delta t_n
%         +
%             \sum_{i=1}^2\, b_i(t,Y_{[0:t_{n-1}]})\sqrt{\Delta t_n} Z_n^{(i)}
%     \label{id:Discretized_Signal}\\
%         Y_{t_{n}}
%     &
%             \approx Y_{t_{n-1}}
%         + 
%             [A_0(t,Y_{[0:t_{n-1}]}) + A_1(t,Y_{[0:t_{n-1}]}) X_{t_{n}}]\Delta t_n
%         +
%             \sum_{i=1}^2\, B_i(t,Y_{[0:t_{n-1}]})\sqrt{\Delta t_n}Z_n^{(i)},
%     \label{id:Discretized_Observation}
% \end{align}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables.

% We can now proceed with a similar observation as before
% \begin{align*}
%         \log p_\phi(
%             y_{t_n}
%         |
%             y_{[t_0:t_{n-1}]}
%         ) 
%     & =  \log \int
%             \frac{
%                 p_\phi\left(
%                     y_{t_n}
%                 \middle|
%                     x_{t_n},
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%             }{
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_n]}
%                 \right)
%             }
%             p_\phi\left(
%                 x_{t_n}
%             \middle|
%                 y_{[t_0:t_n]}
%             \right)
%         d x_{t_n} \\ 
%     & \geq \int 
%             p_\phi\left(
%                 x_{t_n}
%             \middle|
%                 y_{[t_0:t_n]}
%             \right)
%             \log \frac{
%                 p_\phi\left(
%                     y_{t_n}
%                 \middle|
%                     x_{t_n},
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_{n-1}]}
%                 \right)
%             }{
%                 p_\phi\left(
%                     x_{t_n}
%                 \middle|
%                     y_{[t_0:t_n]}
%                 \right)
%             }
%         d x_{t_n} \\ 
%     & =
%         \mathbb{E}_{
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_n]}
%             )
%         } [
%             \log
%             p_\phi(
%                 y_{t_n}
%             |
%                 x_{t_n},
%                 y_{[t_0:t_{n-1}]}
%             )
%         ]
%     -
%         \mathrm{KL}(
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_n]}
%             )
%         \Vert
%             p_\phi(
%                 x_{t_n}
%             |
%                 y_{[t_0:t_{n-1}]}
%             )
%         ),
% \end{align*}
% Further, note that 
% \begin{align*}
%         p_\phi(
%             x_{t_n}
%         |
%             y_{[t_0:t_{n-1}]}
%         )
%     =
%         \mathbb{E}_{
%             p_\phi(
%                 x_{t_{n-1}}
%             |
%                 y_{[t_0:t_{n-1}]}
%             )
%         } \left[
%             p_\phi(
%                 x_{t_{n}}
%             |
%                 x_{t_{n-1}},
%                 y_{[t_0:t_{n-1}]}
%             )
%         \right]
% \end{align*}
% and therefore
% \begin{align*}
%         \log p_\phi\left(
%             y_{[t_0:t_{N}]}
%         \right) 
%     & =    
%         \log p_\phi\left(
%             y_{t_0}
%         \right) 
%         +
%         \sum_{n=1}^N
%         \log p_\phi\left(
%             y_{t_n}
%         \middle|
%             y_{[t_0:t_{n-1}]}
%         \right) \\
%     &\gtrapprox 
%         \log p_\phi\left(
%             y_{t_0}
%         \right) 
%         +
%         \sum_{n=1}^N
%         \mathbb{E}_{
%             X_{t_n} \sim f_\theta(y_{[t_0, t_n]})
%         } \left[
%             \log p_\phi\left(
%                 y_{t_n}
%             \middle|
%                 X_{t_n},
%                 y_{[t_0:t_{n-1}]}
%             \right)
%         \right] \\
%     &\hspace{3cm} -
%         \sum_{n=1}^N
%         \mathrm{KL}\left(
%             f_\theta(y_{[t_0, t_n]})
%         \middle\Vert
%             \mathbb{E}_{
%                 X_{t_{n-1}} \sim f_\theta(y_{[t_0, t_{n-1}]})
%             } \left[
%                 p_\phi(
%                     x_{t_{n}}
%                 |
%                     x_{t_{n-1}},
%                     y_{[t_0:t_{n-1}]}
%                 )
%             \right]
%         \right).
% \end{align*}
% We can now maximize the term on the right-hand side using stochastic gradient ascent in the parameters $\phi, \theta$. Note that the optimum is obtained when $\mathrm{KL}(f_\theta(y_{[t_0, t_n]}) \Vert  p_\phi(x_{t_{n}}|y_{[t_0:t_{n}]})) = 0$, as this results in the lower boundary being tight. \byyan{The approximation argument holds again due to the fact that the Wasserstein distance is dominated by the Kullback-Leibler divergence and \Cref{thrm:MAIN}.}

% \begin{remark}[Alternative MC-based training for \texorpdfstring{$\theta$}{theta}]
%     As there is no guarantee that the stochastic gradient descent actually converges against the right $\theta$, one can alternatively use Monte-Carlo simulations of \eqref{id:Discretized_Observation}, \eqref{id:Discretized_Signal} to fit $f_\theta$ under the current filtering system defined by $\phi$ with respect to the Wasserstein distance.
% \end{remark}

% % \textbf{\byyan{Approach 1.}} Note that the derivation of 
% % \begin{align*}
% %         \log p_\phi(y_{[t_0:t_N]}) 
% %     & \geq
% %         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{[t_0:t_N]}
% %             \mid
% %                 x_{[t_0:t_N]}
% %             \right)
% %         \right]
% %     -
% %         \mathrm{KL} \left(
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %         \middle\Vert
% %             p_\phi(
% %                 x_{[t_0:t_N]}
% %             )
% %         \right)
% % \end{align*}
% % does not use any of the properties assumed in the last section. We see that 
% % \begin{align*}
% %         & \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{[t_0:t_N]}
% %             \mid
% %                 x_{[t_0:t_N]}
% %             \right)
% %         \right] \\
% %     & \qquad = 
% %         \mathbb{E}_{p_\phi(x_{[t_0:t_N]} \vert y_{[t_0:t_N]})} \left[
% %             \log p_\phi\left(
% %                 y_{t_0}
% %             \right)
% %             +
% %             \sum_{n=1}^N
% %                 \log p_\phi\left(
% %                     y_{[t_0:t_n]}
% %                 \mid
% %                     y_{[t_0:t_{n-1}]},
% %                     x_{t_n}
% %                 \right)
% %         \right] \\
% %     & \qquad = 
% %             \log p_\phi\left(
% %                 y_{t_0}
% %             \right)
% %         +
% %             \sum_{n=1}^N
% %                 \mathbb{E}_{p_\phi(x_{t_n} \vert y_{[t_0:t_n]})} \left[
% %                     \log p_\phi\left(
% %                         y_{[t_0:t_n]}
% %                     \mid
% %                         y_{[t_0:t_{n-1}]},
% %                         x_{t_n}
% %                     \right)
% %                 \right],
% % \end{align*}
% % and 
% % \begin{align*}
% %         & \mathrm{KL} \left(
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %         \middle\Vert
% %             p_\phi(
% %                 x_{[t_0:t_N]}
% %             )
% %         \right) \\
% %     & \qquad =
% %         \int
% %             p_\phi\left(
% %                 x_{[t_0:t_N]}
% %             \middle|
% %                 y_{[t_0:t_N]}
% %             \right)
% %             \log \frac{
% %                 p_\phi\left(
% %                     x_{[t_0:t_N]}
% %                 \middle|
% %                     y_{[t_0:t_N]}
% %                 \right)
% %             }{
% %                 p_\phi(
% %                     x_{[t_0:t_N]}
% %                 )
% %             }
% %         dx_{[t_0:t_N]} \\
% %     & \qquad =
% %         \int
% %             \prod_{m=1}^N
% %             p_\phi\left(
% %                 x_{t_m}
% %             \middle|
% %                 x_{t_{m-1}},
% %                 y_{[t_0:t_m]}
% %             \right)
% %             \sum_{n=1}^N
% %                 \log \frac{
% %                     p_\phi\left(
% %                         x_{t_n}
% %                     \middle|
% %                         x_{t_{n-1}},
% %                         y_{[t_0:t_n]}
% %                     \right)
% %                 }{
% %                     p_\phi(
% %                         x_{t_n}
% %                     |
% %                         x_{t_{n-1}}
% %                     )
% %                 }
% %         dx_{[t_0:t_N]} \\
% %         & \qquad \byyan{=}
% %             \sum_{n=1}^N
% %             \mathbb{E}_{
% %                 p_\phi\left(
% %                     x_{t_{n-1}}
% %                 \middle|
% %                     y_{[t_0:t_n]}
% %                 \right)
% %             } \left[
% %                 \mathrm{KL} \left(
% %                     p_\phi\left(
% %                         x_{t_n}
% %                     \middle|
% %                         x_{t_{n-1}},
% %                         y_{[t_0:t_n]}
% %                     \right)
% %                 \middle|
% %                     p_\phi(
% %                         x_{t_n}
% %                     |
% %                         x_{t_{n-1}}
% %                     )
% %                 \right)
% %             \right]
% % \end{align*}


% \subsection{(Conditional) simulation of the observation process}

% \yannick{TODO. Remove duplicate content with above and clarify benefits of transformer representation of $f_\theta$ when it comes to sampling.} Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation} and are known by the agent. For a fixed time $t \in [0:T]$, the objective is now to simulate the process $Y$ at times $t \leq s \leq T$. If both, $X, Y$ are observable, then a typical Euler-scheme for $Y_{[t:T]}$ is usually given by fixing a time-discretization $t  \eqdef  t_0 < t_1  < \cdots < t_N  \eqdef  T$ with $N \in \N$ and approximating
% \begin{align*}
%     X_{t_{n+1}} & \approx X_{t_{n}} + [a_0(t,Y_{[0:t_n]}) + a_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, b_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)} \\
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)}
% \end{align*}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables. Note that we have a slight abuse of notation, as $a_0, a_1, b_1, b_2, A_0, A_1, B_1, B_2$ are now approximations from discretized paths instead of the continuous counterparts.

% In our setting, however, the component $X$ is not observable. To overcome this, we have to rely on standalone simulations of $Y_{[t:T]}$, while inferring $X$ conditional on $Y$. This means, 
% \begin{align*}
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n} \vert  Y_{[0:t_n]}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)},
% \end{align*}
% where $X_{t_n} \vert Y_{[0:t_n]}$ refers to the conditional law described by \eqref{id:ConditionalDistribution}.

% \yannick{If we want to do these simulations fast and efficient, we are reliant on fast access to $X_{t_n} \vert Y_{[0:t_n]}$.}


% % \subsection{Optimal control and BSDEs in finance}
 
% % Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}. While there are numerous settings where this structure is applicable, the reader may regard the observation process $Y$ as an asset price process and assume that the signal process $X$ constitutes a stochastic drift model that is generally not observable. 
% % 
% % We now consider an optimal control problem of the form 
% % \begin{align}
% %     J(u) \eqdef \mathbb{E}\left[\int_0^T r(t, Y_t, (u \bdot Y)_t, u_t) dt + g(Y_T, (u \bdot Y)_T) \right] \label{id:OptimalControl}
% % \end{align}
% % for a measurable function $r: \R_+ \times \R^{d_Y} \times \R^{d_Y} \times \R^{d_Y}$, a concave function $g: \R^{d_Y} \times \R^{d_Y} \to \R$, and $u$ being a predictable control process with values in $\R^{d_Y}$. We write 
% % \begin{align*}
% %     (u \bdot Y)_t  \eqdef  \int_0^t u_s dY_s \quad \forall t \in [0:T], 
% % \end{align*}
% % which is interpreted as trading with rate $u$ on the asset $Y$. Furthermore, $r$ refers to the running reward that accumulates over all times $s \in [0,T]$ and $g$ is interpreted as the terminal reward which is received at maturity. 
% % 
% % \begin{example}[Optimal control problems in finance]
% % \begin{enumerate}[wide]
% %     \item \emph{Hedging European options.} In the following, let $h: \R^{d_Y} \to \R$ denote the payoff of a European contingent claim, and set $r \equiv 0$, $g(y, z)  \eqdef  - (z - h(y))^2$. \yannick{Concave?} Then, the optimization task reads as 
% %     \begin{align*}
% %         J(u) \eqdef - \mathbb{E}\left[  \left(h(Y_T) - (u \bdot Y)_T) \right)^2 \right],
% %     \end{align*}
% %     which is tantamount to minimizing the $L^2$-distance of the wealth process at terminal time to the option's payoff.
% %     \item \emph{Optimal Liquidation.} Assume $d_Y \eqdef 2$ with the first component of $Y$ representing the asset price and let the second component of $Y$ constitute the constant process, i.e. $(Y)_{2} \eqdef 1$, therefore $d((u)_{2} \cdot (Y)_{2})_t = u_t dt$ corresponds to the inventory if we require $(u)_1 \equiv (u)_2$. Now, define $alpha: \R \to \R$ as a (concave) utility function and $\beta: \R \to \R$ as a (convex) inventory penalty. If we set $g(y, z) \eqdef \alpha((y)_1) - \beta((y)_1)$ and define by $r(t, y, z, u) \eqdef \Tilde{r}(t, (y)_1, (u)_1)$ the trading cost of $u$ at time $t$ and asset price $(y)_1$, we arrive at a classical optimal liquidation task.
% %     \item ...
% % \end{enumerate}
% % \end{example}
% % 
% % In order to solve \eqref{id:OptimalControl}, we assume conditions XXX. Then we can define the generalized Hamiltonian
% % \begin{align*}
% %     H:
% %     \begin{array}{ccc}
% %         \R_+ \times (\R^{d_Y})^{\times 3} \times \R^{d_Y} & \longrightarrow & \\
% %          & \longmapsto &
% %     \end{array}
% % \end{align*}

% \subsection{Model ambiguity}
% Let $x_{[0:T]} \in XXX$ and assume the dynamics of $Y$ are given by \eqref{eq:filtering_dynamics__observation}. Then,  $Y \vert \lbrace X = x \rbrace$ which is defined via $(Y \vert \lbrace X = x \rbrace)_t \eqdef Y_t \vert \lbrace X_t = x_{t} \rbrace$ for all $t \in [0:T]$ represents an ordinary SDE with full observability. 
% \begin{example}\label{exa:UncertaintyHeston}
%     For any $t \in [0:T]$ and $y_{[0:t]} \in XXX$ consider $A_0(t, y_{[0:t]}) \eqdef (\mu, - \kappa y_t^2)$, $A_1(t, y_{[0:t]}) \eqdef (0, \kappa)$, $B_1(t, y_{[0:t]}) \eqdef 0$, $B_2(t, y_{[0:t]})^1 \eqdef (y_t^1\sqrt{y_t^2}, 0)$, and $B_2(t, y_{[0:t]})^1 \eqdef (\sigma \rho \sqrt{y_t^2}, \sigma \sqrt{1-\rho^2} \sqrt{y_t^2})$, where $\mu \in \R$, $\kappa, \sigma > 0$, and $\rho \in [-1:1]$. This corresponds to the Heston model with (stochastic) mean-reversion parameter $X_t$,
%     \begin{align*}
%             d 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \\
%                     Y_t^2
%                 \end{matrix}
%             \right)
%         = 
%             \left(
%                 \begin{matrix}
%                     \mu \\
%                     \kappa X_t - \kappa Y_t^2
%                 \end{matrix}
%             \right)
%             dt
%         + 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \sqrt{Y_t^2}  \\
%                     \sigma \sqrt{Y_t^2} 
%                 \end{matrix}
%             \right)
%             \left(
%                 \begin{matrix}
%                     1 & \rho \\
%                     \rho & 1
%                 \end{matrix}
%             \right)^{1/2}
%             dW^{(2)}_t, \quad  \forall t \in [0:T],
%     \end{align*}
%     and $Y \vert \lbrace X \equiv \theta \rbrace$, $\theta > 0$ represents the Heston model with deterministic (and constant) mean-reversion parameter $\theta$.
% \end{example}

% In the following, let $g: A \times XXX \mapsto \R$, define a control problem, where the control $a \in A$ acts on the path $y \in XXX$ to obtain the payoff $g(a, y)$. Further, let $u: \R \to \R$ denote a utility (concave) function. Then, under the model assumption $X = x$, the (ambiguity-unaware) control problem reads as follows,
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}} \mathbb{E}\left[
%         u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)
%     \right].
% \end{align*}
% In terms of \Cref{exa:UncertaintyHeston}, one could for instance consider the hedging task $g(a, y)  \eqdef  (a \bdot y^1)_T - h(y_T^1)$ of the European option with payoff structure $h: \R \to \R$, where $\mathcal{A}$ is the set of previsible trading strategies on $Y^1$.

% In \cite{KlibanoffMarinacciMukerji05}, the authors suggest considering not only one choice of model (as we did above with $X = x$) but instead a distribution of models, which are evaluated with a second expected utility. Let $r: \R \to \R$ denote a second (concave) utility function and since 
% \begin{align*}
%         \mathbb{E}\left[u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)\right]    
%     =
%         \mathbb{E}\left[u \circ g(\alpha, Y) \mid \lbrace X = x \rbrace \right],
% \end{align*}
% ambiguity-aware control problem reads as follows, 
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}}
%         \mathbb{E}\left[
%             r \left(
%             \mathbb{E}\left[
%                 u \circ g(\alpha, Y)
%             \mid
%                 X
%             \right]
%             \right)
%         \right].
% \end{align*}
% \yannick{TODO. Explain how a DKF setting applies as the model-process is unobservable.}

% \end{document}




==> OLD/Historical_Versions/OLD/OLD_DRAFT.tex <==
% % Zoom link:
% % https://mcmaster.zoom.us/j/2601491351


% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% \documentclass[preprint,12pt,authoryear]{elsarticle}
% \usepackage{amssymb}

% \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}



% \begin{document}

% \begin{frontmatter}
% % \title{Universality of Continuous-Time Deep Kalman Filters}
% % \title{Continuous-Time Deep Kalman Filters which are Universal Filters}
% \title{Deep Kalman Filters Approximate Conditionally Gaussian Filters}

% % \author[inst1]{Matheus Grasselli}
% \author[inst2,inst3]{Blanka Horvath}
% \author[inst1,inst4]{Anastasis Kratsios}
% \author[inst2,inst3]{Yannick Limmer}
% \author[inst1]{Xuwei Yang}


% \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
%             % addressline={Hamilton, Ontario}, 
%             city={Hamilton},
%             % postcode={00000}, 
%             state={Ontario},
%             country={Canada}}

% \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             state={Oxfordshire},
%             country={United Kingdom}}

% \affiliation[inst3]{organization={Oxford MAN Instute for Quantitative Finance, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             state={Oxfordshire},
%             country={United Kingdom}}
            
% \affiliation[inst4]{organization={Vector Institute},
%             % addressline={Address Two}, 
%             city={Toronto},
%             % postcode={22222}, 
%             state={Ontario},
%             country={Canada}}
            

% \begin{abstract}
% Deep Kalman filters (DKFs) form a broad class of neural network models which generate Gaussian probability measures; inspired by the discrete-time Kalman filter.  
% In this paper, we show that there are are DKFs which are generic conditionally Gaussian filters.  We do so by explicitly constructing a DKF model which can approximate the solution operator of a broad class of continuous-time stochastic filters, between a partially observed, conditionally-Gaussian, non-Markovian signal processes given the realized path a non-Markovian observation process.
% Our approximation guarantees are uniform over regular compact manifolds of paths.  We provide explicit parameter estimates depending on the dynamics and dimension of the signal and observation process as well as on the geometry of the compact set of paths over which the stochastic filtering problem's solution operator is approximated.  \hfill\\
% {\color{red} Numerical illustrations are used to validate our guarantees.}
% \end{abstract}


% \begin{keyword}
% %% keywords here, in the form: keyword \sep keyword
% Stochastic Filtering \sep Conditionally Gaussian Processes \sep Neural Networks
% %% PACS codes here, in the form: \PACS code \sep code
% % \PACS 0000 \sep 1111
% %% MSC codes here, in the form: \MSC code \sep code
% %% or \MSC[2008] code \sep code (2000 is the default)
% \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% \end{keyword}

% \end{frontmatter}


% \section{Introduction}
% \label{s:Algorithm}
% \fbox{\begin{minipage}{0.8\textwidth}
%     \textbf{Structure of introduction.}

%     \begin{enumerate}
%         \item Opening.
%         \item What are Kalman filters? 
%         \item What are Deep Kalman Filters?
%         \item Exemplary applications of (D)KF in finance.
%         \item Universality: Limitations of existing results and extensions.
%         \item Structure of the article. 
%     \end{enumerate}

%     BH: This is great, this is exactly what I was thinking to do.
% I'd suggest to add or consider the following aspects:
% \begin{enumerate}
%     \item Opening
%     \item What are Kalman filters and what are traditional use cases of Kalman filters in finance (and beyond)
%     \item What are Deep Kalman Filters (when/how) and why did they become popular and what (were) limitations of Kalman Filters that can be resolved by Deep Kalman Filters?
%     \item What is the main result in this paper and why is it useful? Universality: Limitations of existing results and extensions.
%     \item This is what we don't do (re: training) but "this is why it is ok"...
%     \item Structure of the article.
% \end{enumerate}
% \end{minipage}
% }\\


% Literature surrounding applications of filtering in Mathematical Finance: \\
% For a general motivation for the geometric (also: information geometric) idea behind Filtering problems in typical applications in mathematical finance, see the excellent overview presented in the the recent work \href{https://arxiv.org/pdf/2205.01594.pdf}{Brigo (2022)} and the expose in \href{https://arxiv.org/pdf/1303.6236.pdf}{Armstrong and Brigo (2013)} as well as well-known early works \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}. A gentle introduction to typical linear and nonlinear filtering problems in mathamatical finance can be found in the review article \href{ura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{Date and Ponomareva (2010)} and for a comprehensive introduction to stochastic filtering we direct to the eteemed monograph \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)} as the reference literature.\\


% \anastasis{I would mention that there are at-least two sources of ``complexity'' to the general filtering problem: 1) The infinite-dimensionality of the set of all probability measures (complexity of representing conditional densities/measures) and 2) The complexity of the dynamics governing the solution of the signal, observation, and conditional dynamics.  \\
% I would then say some like Kalman filters simplify both, the general conditional Gaussian filters studied in \cite{LipShiryaev_II_2001} provide a theoretical foundations for filtering when (1) is resolved by considering conditionally Gaussian filters.  Then somehow relate that we work in (1), by developing a universal model class, in the conditionally-Gaussian framework based on the ideas of deep Kalman filtering.}

% \paragraph{Historical development:} 
% The filtering problem consists in estimating the state of a stochastic differential system
% from noisy observations. \\ 
% The general solution of the filtering problem at a given time is given by the probability density
% of the unperturbed state of the system at that time, conditional on the perturbed observations
% up to the given time. When the unobserved signal and the observed signal evolve in continuous
% time, the filter density follows a stochastic partial differential equation (SPDE), see \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)}. 
% If the dynamic evolution of the unobserved
% system is linear, the observations are linear, the noise terms are Gaussian\footnote{The initial condition of the
% unperturbed signal are also assumed to be Gaussian or deterministic.}, then this is a setting that leads to the celebrated \emph{Kalman-Bucy filter}:
% \\
% Indeed, in the linear Gaussian case the problem was solved in discrete-time by Rudolf Kalman, and later in continuous time in \cite{TBD}\anastasis{(Bucy Paper)},
% who introduced what is known today as the \emph{Kalman filter} (see next paragraph), a finite dimensional system of equations
% for the first two conditional moments of the state of the stochastic system, given the observations:
% In such a case, the filter is Gaussian and its density can
% be characterized by a finite dimensional set of parameters, namely the mean vector and variance-covariance matrix of the resulting Gaussian distribution,
% %\\In classical Kalman Filters, the evolution of this system (both observable and unobservable parts) are modelled as linear functions
% %perturbed by Gaussian noise.
% %In a linear setting 
% these equations determine the whole conditional density of the state of the system given the observations,
% as this (Gaussian) density is fully characterized by the first two moments. \\
%  For real world applications the assumption of a linear evolution of this system\footnote{I.e. transition and emission distributions.}
% limits the capacity to model complex phenomena, and modifications to the functional form of Kalman Filters
% have been proposed.
% \\
% As indicated above, 
% in the  general
% nonlinear case, the filtering problem is far more complex as it consists in computing the conditional density of the
% state given the observations. This density is the solution of a stochastic partial differential
% equation which is referred to as the \emph{Kushner-Stratonovich equation} and the resulting nonlinear filter is in general not finite dimensional\footnote{I.e. it does not evolve in a finite dimensional
% statistical manifold.}. A well
% known approximation method is the extended Kalman filter (EKF), in which one linearizes around
% the current estimate obtaining a locally linear system, and then applies the Kalman filter
% equations in this (linearised) neighbourhood. Traditionally, this procedure was usually justified by heuristic considerations.  
% Though more recent linear approximations have also been considered, e.g.\ in \cite{LukasJosef_LinearizedFiltering}.
% Another choice in the nonlinear case is the Gaussian assumed density filter (GADF),
% obtained by assuming the conditional density to be Gaussian\footnote{This is dangerous, because by assuming a false hypothesis one can deduce anything as well as its opposite.}, which yields a finite dimensional filter. %However, this approach depends heavily on conditional Gaussianity, which is not necessarily fulfilled in many real-life applications.\\
% We are universal in the conditional Gaussian class.\\
% Contrast it with neural SDEs (no hidden suff (ANASTASISSSS)

% Hanzon suggested to project the SPDE equation in Stratonovich form for the evolution of the filter density onto a finite dimensional statistical manifold, using the Fisher metric/Hellinger distance. We call this “Stratonovich projection” and it consists in projecting the separate vector
% fields of the SPDE corresponding to the drift and diffusion part of the Stratonovich version. The projected equation would describe a finite dimensional density evolution, called projection filter, approximating the full filter evolution associated with the optimal filter.\\
% In 1987, Hanzon (BH: reference missing) introduced the projection filter (PF), which is a finite dimensional nonlinear filter based on a differential geometric approach: The projection filter is obtained by projecting the Kushner-Stratonovich equation onto the tangent space
% of a finite dimensional manifold of probability densities, according to the Fisher information metric.\\
% Hanzon and Hut (1991) (BH: add ref) showed that if one projects onto the
% tangent space of the finite dimensional manifold of Gaussian densities, the resulting projection filter
% coincides with an assumed density filter which is obtained as follows: one computes the first two conditional moments equations in McShane-Fisk-Stratonovich (MFS) form, and then assumes the conditional density to be Gaussian, closing in this way the equations for the first two moments.   
% It was also proven in Hanzon and Hut (1991) that what we described above is in general not the same as assuming a Gaussian density in the It\^{o} equations for the first two moments and then transforming the obtained filter in MFS form.
% The equivalence between the MFS-based GADF and the Gaussian Projection Filter is very important when generalized to
% exponential families (see \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}), because it gives a simple characterization of the exponential projection
% filter (EPF) which is independent of geometric concepts. \\

% For a comprehensive but introductory review of linear and non-linear filterin applications in mathematical finance see: \href{https://bura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{P. Date and K. Ponomareva (2010)} among which we will highlight some simple but heavily used (Gaussian or near-Gaussian) use cases
% \begin{itemize}
%     \item In stochatic volatility modelling Kalman Filters have traditionally been used to estimate (and forecast) spot and realised volatility.
%     \item Monoyios in \href{https://people.maths.ox.ac.uk/monoyios/docs/ima_final.pdf}{Monoyios (2007)} develops a filtering approach with applications to (optimal) hedging, in which the hedger updates her parameter estimates from
% observations of the asset prices, and where he finds an analytic solution to the hedger’s combined filtering and
% control problem in the case that the drift of the traded asset is known with certainty.
% \item Filtering has been traditionally heavily used in linear Gaussian interest rate models. \href{}{}
%     \end{itemize}
    

% \paragraph{Kalman filters} At a high level, a Kalman filter operates by combining a model of a system with partial state-observations to estimate the current overall state of the system. The filter uses two primary steps to make these estimates: a prediction step and an update step.
% \begin{itemize}
%     \item In the prediction step, the Kalman filter uses the model of the system to predict the state of the system at the next time step. This prediction is based on the current estimate of the system state, as well as any known inputs or disturbances in the system. The Kalman filter uses a probabilistic approach to estimate the state of the system, this means the prediction includes both the expected value of the state as well as an estimate of the uncertainty or error in the prediction.
%     \item In the update step, the Kalman filter uses the actual observation to correct the predicted state estimate. The filter compares the distribution of the predicted state to the actual observed state (which acknowledges uncertainty and is perceived as a distribution itself). The filter then adjusts the state estimate based on this difference.
% \end{itemize}

% \paragraph{Deep Kalman filters} The term, ``deep Kalman filter'' (DKF) refers to deep learning models, that bolster the capacity of traditional Kalman filter by leveraging a neural network component. The neural network component is used to learn the probabilistic model of the underlying system dynamics, thus allowing DKFs to generically adapt to any situation in which the conditional evolution of the signal process is Gaussian.  This generic flexibility, of DKFs is what has lead to their empirical predictive edge over traditional Kalman filters \cite{TBD}.

% The neural network component in a DKF is typically used to model the transition function of the system, which describes how the state of the system evolves over time. The neural network takes as input the current state of the system, as well as any control inputs or disturbances, and outputs a probability distribution over the possible next states of the system. This distribution is then used to make a prediction of the next state, as well as an estimate of the uncertainty or error in the prediction. 

% The traditional Kalman filter components are then used to combine the neural network predictions with actual observations in order to update the state estimate. The neural network component in a DKF can be trained using a variety of techniques, such as maximum likelihood or Bayesian inference. The training process involves minimizing the error between the predicted state and the actual state, as well as minimizing the uncertainty in the predictions.

% \paragraph{Exemplary (existing) applications of (D)KF in finance}
% \begin{enumerate}
%     \item Sequential calibration of options
%     \begin{itemize}
%         \item Problem: The parameter estimates are noisy and old data are typically discarded, as only the most recent data are used.
%         \item As a solution, the calibration is formulated as a filtering problem.
%         \item The observable process consists of market option prices, spot, strike, interest, and maturity.
%         \item The unobservable process consists of the difference between the modelled option price and the denoted option price, as well as the difference of the model's parameters to the day before.
%         \item See \cite{LindstroemStroejbyBrodenWiktorssonHolst08}, extensions \cite{LindstroemWiktorsson14}
%     \end{itemize}
%     \item Computing VaR in a stochastic volatility model, see \cite{LindstroemMadsenNielsen16}
%     \item Filtering with bond prices, see \cite{LindstroemMadsenNielsen16}
%     \begin{itemize}
%         \item The observable process constitutes the prices obtained from solving the ``bond pricing equation''
%         \item The unobservable variables are the parameters of the estimated model and the implied interest rate (by bond prices, not quoted)
%     \end{itemize}
%     \item Calibration of term structure models of commodity prices \cite{JavaheriLautierGalli03}
%     \item Dynamic pricing (this is probably more economics than finance), see \cite{CohenTreetanthiploet22}
%     \item Besides state estimation in control systems, Kalman filters have found applications in financial markets for constructing trading strategies. Two common approaches involve using Kalman filters to:
%     \begin{itemize}
%         \item Identify Mean-Reverting Patterns: Kalman filters can be utilized to detect instances where asset prices deviate from their long-term average, indicating potential mean-reverting behaviour. Traders can then develop strategies that take advantage of these deviations, expecting prices to eventually return to their mean.
%         \item Identify Momentum-Based Trends: Kalman filters can also be employed to identify momentum-based trends in asset prices, indicating sustained movements in a particular direction. Traders can develop strategies to follow and capitalize on these trends.
%         \item \yannick{References missing.}
%     \end{itemize}
%     \item Portfolio Optimization with Kalman Filters and Multi-Asset Models:
%     \begin{itemize}
%         \item Kalman filters applied to optimize asset portfolios by considering individual asset dynamics and correlations.
%         \item Particularly beneficial for multi-asset portfolios.
%         \item Estimation of assets' covariance matrix using Kalman filters.
%         \item Portfolio optimization based on the covariance matrix while adhering to specified constraints.
%         \item \yannick{References missing.}
%     \end{itemize}
%     \item  Risk Management and Stress Testing with Kalman Filters:
%     \begin{itemize}
%         \item Utilization of Kalman filters for risk management and stress testing purposes.
%         \item Estimation of portfolio risk and identification of potential risk sources.
%         \item Modelling asset behaviour under various market scenarios using Kalman filters.
%         \item Assessment of the portfolio's vulnerability to the impact of these scenarios.
%         \item \yannick{References missing.}
%     \end{itemize}
% \end{enumerate}


% \begin{comment}
% \paragraph{Limitations and contribution} The results \cite{kratsios2021universal, Acciaio2022_GHT} show that, while it is possible to universally approximate the function used above with a class of transformer models, the required number of parameters to approximate the function at each state in time can depend highly non-favourably on the dimensions of the (observable and unobservable) state. In this work, we suggest to best approximate the function at all times by a class of non-Euclidean kernel regressors, trained on a finite set of observations. 
% \end{comment}


% \section{The Setting}
% \label{s:Preliminaries}

% This section formulates the theoretical problem which this paper addresses.
% Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  These processes evolve according to the coupled dynamics
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d := \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.


% Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% \begin{align}
%     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) \label{id:ConditionalDistribution}
% \end{align}
% where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of theoretical foundations of DKFs.
% \begin{question}
% \label{question:main}
% Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$.
% \end{question}

% \begin{comment}
% Moreover, under mild regularity conditions ensuring that $f$ is sufficiently continuous the geometric deep learning results of \cite{kratsios2021universal} and \cite{Acciaio2022_GHT} guarantee that it can be approximated with a class of transformer models.  However, their analysis equally reveals that the required number of parameters to approximate each $f_t$ can depend highly non-favourably on the dimensions $d_X$ and $d_Y$, as a function of the local uniform approximation error, if nothing is assumed of $f_t$.  In these results, the \textit{uniform} (on compact sets) approximation of the probability measure-valued functions $f_{t}$ by a sequential learning model $\hat{f}_t$ \anastasis{dets later} is quantified by
% \[
%     \sup_{y_{[0:T]}\in K}\, \sup_{0\le t\le T}\,
%         \mathcal{W}_2\big(f_t(y_{[0:t]},\hat{f}_t(y_{[0:t]})\big)
%     ,
% \]
% where $K$ is a (non-empty) compact subset of the path-space $\dots$.  \anastasis{Make comment about adapted Wasserstein when predicting multiple steps forward it time.}
% \end{comment}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Preliminaries__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^d)$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^d$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^d$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically\footnote{dets later; obvious.} embed any path $f\in C([0:t],\mathbb{R}^d)$ into a path $F\in C([0:T],\mathbb{R}^d)$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     F(s)\eqdef \begin{cases}
%         f(s) &: \mbox{ if } 0\le s \le t\\
%         f(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $f\mapsto F$ is a linear isometric embedding of the Banach space $C([0:t],\mathbb{R}^d)$ into $C([0:T],\mathbb{R}^d)$ since
% \[
% \|F\|_T = \max_{0\le s\le T}\, \|f(s)\|_2
% = \max_{0\le s\le t}\, \|f(s)\|_2 = \|f\|_t, 
% \]
% since $f(s)=f(t)$ for all $t<s\le T$.  Conversely, the restriction $F_{[0:t]}$ of a path $F\in C([0:T],\mathbb{R}^d)$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^d)$ to $C([0:t],\mathbb{R}^d)$ since
% \[
%         \|F_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|F_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|F_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|F(s)\|_2 
%     =
%         \|F\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^d)$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot by approximated by standard deep neural networks parameterized determined by a number trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing} for general rates.   

% The curse of dimensionality cannot be broken, by can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space, as is the case in our results, shows that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}, however, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are isometric to some compact Riemannian manifold, thus we exclude fractal like subsets of the path space $C([0:T],\mathbb{R}^d)$.  We motivate the our condition with the following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}; and consequences thereof e.g.\ \cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}.

% \begin{proposition}[Isometric Copies of Every Compact Riemannian Manifold in The Path Space]
% \label{prop:Non_Vaccousness}
% Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^d)$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}
% \anastasis{Perhaps I create a simple example later.}

% We will additionally impose topological regularity on our compact sets \textit{aspherical}; such as tori.  This means, that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$ (see \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups).  
% \anastasis{Maybe I include a brief appendix on homotopy groups}

% \begin{assumption}[Regular Compact Sets]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^d)$ and a ``latent dimension $D_K\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}
%     % \item[(i)] \textbf{Qualitative Case:} There is an $D_K$-dimensional connected, homogeneous, geodesically complete Riemannian manifold $(M,g)$ and an isometric embedding $\psi:(M,d_g)\rightarrow C([0:T],\mathbb{R}^d)$ with $K\subseteq \psi(M)$.
%     % \item[(ii)] \textbf{Quantitative Case:} 
%     \item[(i)] $K$ is finite. 
%     \item[(ii)] There exists a compact aspherical $D_K$-dimensional Riemannian manifold $(M,g)$ for which $(M,d_g)$ is isometric to $(K,\|\cdot\|_T)$; where $d_g$ is the geodesic distance on $(M,g)$. 
% \end{enumerate}
% \end{assumption}
% In what follows, we denote the Riemannian volume of $(M,g)$, in Assumption~\ref{ass:reg_compact}, by $\operatorname{Vol}(M,g)$.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Preliminaries__ss:OutputSpace}

% The $2$-Wasserstein space $\mathcal{P}_2(\mathbb{R}^d)$ consists of all probability measures on $\mathbb{R}^d$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_2(\mathbb{R}^d)$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^2]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_2$ on $\mathbb{P}_2(\mathbb{R}^d)$ is given by minimizing the opimtal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_2(\mathbb{P}, \mathbb{Q})^2
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
%     .
% \]
% Generally, the $2$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, in \cite{TBD} it was show that the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$ admits the following exceptional closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^d)$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^d)$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% This section introduces our attention-based model.  

% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an source dimension $d$ and a target dimension $D$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^d$ to $\mathbb{R}^D$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^d\rightarrow\mathbb{R}^D$ with iterative representation: for each $x\in \mathbb{R}^d$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=d$ and $d_{J+1}=D$.


% \anastasis{place model here}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and in GNNs \cite{TBD} to the context of continuous-time path inputs and like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``know/previously generated paths''.  


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $N$, $N_1$, $d$, and a ``time horizon'' $t> 0$.  
% Given a set of $N$ distinct paths $\{y^{(n)}\}_{n=1}^N$ in $C([0,1],\mathbb{R}^d)$, a $B$ is an $N_1\times N$-matrix, $b\in \mathbb{R}^{N_1}$, $A$ is an $N_1\times N_1$-matrix, and $a\in \mathbb{R}^{N_1}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^N)$.\\
% \noindent The \textit{similarity score}, is a map $\operatorname{sim}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$ by
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{sim}_t^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%             \operatorname{Softmax}
%         \circ
%             \biggl(
%                 A\operatorname{ReLU}\bullet 
%             \Big(
%                     B
%                     \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^N
%                 +
%                     b
%             \Big)
%                 +
%                     a
%         \biggr)
%     ,
% \end{equation}
% where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$.
% \end{definition}

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of Definition~\ref{defn:Sim_Score}, fix a positive integer $N_2$, and set of query times $0\le t_1<\dots< t_N\le t$, an $N_2\times d$ matrix $V$, and a $N_2\times N$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^N)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{pos}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined by 
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{pos}_t^{\theta_1}:
%         y_{\cdot} 
%     \mapsto 
%            U \,(x_{t_n})_{n=1}^N + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$.
% \end{definition}

% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of Definitions~\ref{defn:Sim_Score} and~\ref{defn:PositionalEncoding}.  The \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1)$, is the map $\operatorname{attn}_t^{\theta}:C([0,1],\mathbb{R}^d)\rightarrow \mathbb{R}^{d\times N}$ given by
% \[
%         \operatorname{attn}_t^{\theta}(y_{\cdot})
%     \eqdef 
%             \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%         \odot
%             \operatorname{pos}_t^{\theta_1}(y_{\cdot})
% \]
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$, where $v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}$ for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
% \end{definition}

% % \[
% %     \hat{\phi}:
% %         u
% %     \mapsto 
% %         A\operatorname{ReLU}\bullet (Bu+ b)
% %     ,
% % \]  
% % where 

% % $D\in \mathbb{N}_+$, and each of the $W^{(d)}:\mathbb{R}^{F_{d-1}}\rightarrow \mathbb{R}^{F_d}$ (for $d=1,\dots,D$) is an ``invertible'' affine map defined for every $v\in \mathbb{R}^{F_{d-1}}$ by
% % \[
% %         W^{(d)}(v) 
% %     = 
% %         (A^{(d:1)},e^{A^{(d:0)}})v + b^{(d)}
% %     ,
% % \]
% % where $F_d>F_{d-1}$, $b\in \mathbb{R}^{F_d}$, $A^{(d:1)}$ is a $(F_d-F_{d-1})\times F_{d-1}$ matrix, and $e^{A^{(d:0)}}$ is the matrix exponential of a $F_{d-1}\times F_{d-1}$-matrix $A^{(d:0)}$.  Furthermore, $F_0\eqdef N$, and $F\eqdef F_d$.

% % \anastasis{We can perhaps sample these from some ``prior model we believe on the process $Y_{\cdot}$''?} \yannick{Is there any indicator in \Cref{lem:Good_Feature_Map} that yields what properties the paths $x_\cdot^{(1)}, x_\cdot^{(2)}, ...$ should have? Or to put it another way, if the paths are sampled from the actual distribution, they would do the job? }

% % \anastasis{Explain good feature map, Comment @Yannick the easiest explanation is found in ``Non-Euclidean Universal Approximation''.} \yannick{TODO.} 


% % \anastasis{The idea is to train $\operatorname{attn}_T$ on a set in a centralized manner, then update $\varphi$ in a decentralized way.}

% % Let us fix $(\operatorname{attn}_t)_{t\ge 0}$ using as in Lemma~\ref{lem:Good_Feature_Map}.  This allows us to reduce our deep-learning model class to a smaller hypothesis class $\mathcal{H}$ of non-Euclidean kernel regressors mapping paths in $C([0:T],\mathbb{R}_d)$ to non-singular Gaussian measures $\mathcal{N}_{d_X}$
% % %\yannick{its bijective characterization in $\mathbb{R}^{d_X+d_X(d_X+1)/2}$, right?}\anastasis{yes}
% % .  

% % At any given time $0\le t\le T$ and for each path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$, each kernel regressor $f_{\theta_{\cdot}}\in \mathcal{H}$ is determined by a $\mathcal{Y}_{\cdot}$-predictable process $\theta_{\cdot}\eqdef (\theta_t)_{0\le t\le T}$ via
% % \[
% %         f_{\theta_{\cdot}}
% %             (t,y_{[0:t]})
% %         \eqdef
% %             \psi\big(
% %                 \theta_t
% %                 \operatorname{attn}_t(y_{[0:t]})
% %             \big)
% %     ,
% % \]
% % where $\theta_t$ is a ${d_X+d_X(d_X+1)/2}\times F$-dimensional matrix.  NB, that $\psi$ is a homeomorphism between $\mathcal{N}_{d_X}$ and $\mathbb{R}^{d_X+d_X(d_X+1)/2}$. 




% % \subsection{The Objective Function}

% % Fix a set of realizations/sample paths from the process $Y_{\cdot}$, which we denote by $y_{[0:T]}^{(1)},\dots,y_{[0:T]}^{(N)}$ for some positive integer $N$.
% % We wish to select an optimal (dynamic) kernel regressor by minimizing the \textit{penalized regret functional}
% % \begin{equation}
% %         \mathcal{R}(\theta_{\cdot})
% %     \eqdef 
% %         \underbrace{
% %             \int_0^T\, 
% %                 \frac1{N}
% %                 \sum_{n=1}^N\,
% %                 \mathcal{W}_2^2\big(
% %                     f_t(y_{[0:t]}^{(n)})
% %                 ,   
% %                     \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})
% %                 \big)
% %                 -
% %                 \mathcal{R}^{\star}
% %             \,dt
% %             }_{
% %                 \mbox{$W_2$-Regret}
% %             }
% %         +
% %             \underbrace{
% %             \int_0^T
% %                 \lambda \,\|
% %                     \theta_t
% %                 \|_2^2
% %                 \,
% %             dt
% %             }_{
% %                 \mbox{Running Regularizer}
% %             }
% %     ,
% % \end{equation}
% % and $\lambda >0$ is a regularizing hyperparameter and where $\mathcal{R}^{\star}$ represents the minimal possible value which the running $\mathcal{W}_2^2$-SSEs loss can achieve
% % \[
% %     \mathcal{R}^{\star} 
% % \eqdef 
% %     \inf_{\theta_{\cdot}\in ...}
% %         \int_0^T\, 
% %             \frac1{N}
% %             \sum_{n=1}^N\,
% %             \mathcal{W}_2^2\big(
% %                 f_t(y_{[0:t]}^{(n)})
% %             ,   
% %                 \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})
% %         \big)
% %     dt
% % \]
% % \anastasis{Describe the set of controls...which determins our hypothesis class}\hfill\\
% % Minimizing the regret functional $\mathcal{R}$ is equivalent to minimizing the following energy/loss function, in the sense that their set of minimizers coincide.   
% % \anastasis{I'll add the details in this, and the diagonal, cass (this will be a proposition)}
% % \begin{equation}
% %         L(\theta_{\cdot})
% %     \eqdef 
% %         \int_0^T\, 
% %                 \frac1{N}
% %                 \sum_{n=1}^N\,
% %                     \| \mu_{n:t} - \hat{\mu}_{n:t} \|_2^2 
% %                         + 
% %                     \operatorname{tr}\big(
% %                         \Sigma_{n:t} + \hat{\Sigma}_{n:t}
% %                         -2
% %                         (
% %                             \hat{\Sigma}_{n:t}^{1/2}
% %                             \Sigma_{n:t} 
% %                             \hat{\Sigma}_{n:t}^{1/2}
% %                         )^{1/2}
% %                     \big)
% %         +
% %                 \|
% %                     \theta_t
% %                 \|_2^2
% %         \,
% %         dt
% %     ,\label{id:LossFunction}
% % \end{equation}
% % where we have made the abbreviations $\mathcal{N}(\byyan{\hat{\mu}_{n:t}}, \hat{\Sigma}_{n:t})\eqdef \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})$ and 
% % $\mathcal{N}(\byyan{\mu_{n:t}}, \Sigma_{n:t})\eqdef f_t(y_{[0:t]}^{(n)})$ for each $0\le t\le T$ and each $n\in \{1,\dots,N\}$.  
% % \anastasis{With Xuwei, we will identify when things are diagonal and derive the optimal control; i.e.\ optimal dynamic non-Euclidean kernel model.}
% % \yannick{(For next discussion:) How can we minimize \eqref{id:LossFunction}, as $f_t(y_{[0:t]}^{(n)}) [= \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)]$ is not observable? $\rightarrow$ we have closed form expressions for $\mu$, $\Sigma$ given by \eqref{id:ClosedFormMu}, \eqref{id:ClosedFormSigma}.} \yannick{I think $\lambda$ will occur in \eqref{id:LossFunction}?}



% % \newpage
% % \begin{definition}\label{defn:BV_Paths}
% % Fix a positive integer $d$.  A continuous path $x:[0:1]\rightarrow \mathbb{R}^d$ with $x(0)=0$ is said to be of bounded variation if $\|x\|_{BV}\eqdef \sup_{\pi}\, \sum_{i=1}^{l-1}\, \|h(t_{i+1})-h(t_i)\|_{\mathbb{R}^D}$ is finite, where the supremum is taken over all finite partitions $\pi=\{(t_i)_{i=1}^l:\, 0=t_1<\dots<t_l=1\}$ of $[0:1]$.  The set of all such paths denoted by $C^1_0([0:1],\mathbb{R}^d)$.
% % \end{definition}
% % Let $x_{\cdot}$ and $y_{\cdot}$ be paths in $C^1_0([0:1],\mathbb{R}^d)$, their we the component-wise Riemann-Stieltjes integral of $y_{\cdot}$ against $x_{\cdot}$ by $\int_0^1\,y(t)\,dx(t)\eqdef \big(\int_0^1\,y(t)_i\,dx_i(t)\big)_{i=1}^d$.  The Riemann-Stieltjes integrals are a type of ``polynomial features'' for paths in $C^1_0([0:1],\mathbb{R}^d)$ and their associated feature maps are the signatures of \cite{???}, defined as follows.
% % \begin{definition}[Signature of a BV-Path]\label{defn:Signatures}
% % Let $x_{\cdot}\in C^1_0([0:1],\mathbb{R}^$
% % \end{definition}



% \section{Main Result}
% \label{s:Main_Results}



















% \paragraph{The Feature Map}
% \anastasis{Explain why no sig, discrete/trivial topology analogy; and note that one could consider a variant of the model using sig if they needed the stronger p-variation topology.  But since we don't then its more efficient to consider approximators depending on fewer parameters.}


% \newpage
% \section{Applications}

% In this section, we will discuss exemplary applications that leverage the possibility to approximate a Kalman filter setting with our suggested framework. 

% \subsection{(Conditional) simulation of the observation process}

% Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation} and are known by the agent. For a fixed time $t \in [0:T]$, the objective is now to simulate the process $Y$ at times $t \leq s \leq T$. If both, $X, Y$ are observable, then a typical Euler-scheme for $Y_{[t:T]}$ is usually given by fixing a time-discretization $t := t_0 < t_1  < \cdots < t_N := T$ with $N \in \N$ and approximating
% \begin{align*}
%     X_{t_{n+1}} & \approx X_{t_{n}} + [a_0(t,Y_{[0:t_n]}) + a_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, b_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)} \\
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)}
% \end{align*}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables. Note that we have a slight abuse of notation, as $a_0, a_1, b_1, b_2, A_0, A_1, B_1, B_2$ are now approximations from discretized paths instead of the continuous counterparts.

% In our setting, however, the component $X$ is not observable. To overcome this, we have to rely on standalone simulations of $Y_{[t:T]}$, while inferring $X$ conditional on $Y$. This means, 
% \begin{align*}
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n} \vert  Y_{[0:t_n]}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)},
% \end{align*}
% where $X_{t_n} \vert Y_{[0:t_n]}$ refers to the conditional law described by \eqref{id:ConditionalDistribution}.

% \yannick{If we want to do these simulations fast and efficient, we are reliant on fast access to $X_{t_n} \vert Y_{[0:t_n]}$.}


% \subsection{Optimal control and BSDEs in finance}

% Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}. While there are numerous settings where this structure is applicable, the reader may regard the observation process $Y$ as an asset price process and assume that the signal process $X$ constitutes a stochastic drift model that is generally not observable. 

% We now consider an optimal control problem of the form 
% \begin{align}
%     J(u) \eqdef \mathbb{E}\left[\int_0^T r(t, Y_t, (u \bdot Y)_t, u_t) dt + g(Y_T, (u \bdot Y)_T) \right] \label{id:OptimalControl}
% \end{align}
% for a measurable function $r: \R_+ \times \R^{d_Y} \times \R^{d_Y} \times \R^{d_Y}$, a concave function $g: \R^{d_Y} \times \R^{d_Y} \to \R$, and $u$ being a predictable control process with values in $\R^{d_Y}$. We write 
% \begin{align*}
%     (u \bdot Y)_t := \int_0^t u_s dY_s \quad \forall t \in [0:T], 
% \end{align*}
% which is interpreted as trading with rate $u$ on the asset $Y$. Furthermore, $r$ refers to the running reward that accumulates over all times $s \in [0,T]$ and $g$ is interpreted as the terminal reward which is received at maturity. 

% \begin{example}[Optimal control problems in finance]
% \begin{enumerate}[wide]
%     \item \emph{Hedging European options.} In the following, let $h: \R^{d_Y} \to \R$ denote the payoff of a European contingent claim, and set $r \equiv 0$, $g(y, z) := - (z - h(y))^2$. \yannick{Concave?} Then, the optimization task reads as 
%     \begin{align*}
%         J(u) \eqdef - \mathbb{E}\left[  \left(h(Y_T) - (u \bdot Y)_T) \right)^2 \right],
%     \end{align*}
%     which is tantamount to minimizing the $L^2$-distance of the wealth process at terminal time to the option's payoff.
%     \item \emph{Optimal Liquidation.} Assume $d_Y \eqdef 2$ with the first component of $Y$ representing the asset price and let the second component of $Y$ constitute the constant process, i.e. $(Y)_{2} \eqdef 1$, therefore $d((u)_{2} \cdot (Y)_{2})_t = u_t dt$ corresponds to the inventory if we require $(u)_1 \equiv (u)_2$. Now, define $alpha: \R \to \R$ as a (concave) utility function and $\beta: \R \to \R$ as a (convex) inventory penalty. If we set $g(y, z) \eqdef \alpha((y)_1) - \beta((y)_1)$ and define by $r(t, y, z, u) \eqdef \Tilde{r}(t, (y)_1, (u)_1)$ the trading cost of $u$ at time $t$ and asset price $(y)_1$, we arrive at a classical optimal liquidation task.
%     \item ...
% \end{enumerate}
% \end{example}

% In order to solve \eqref{id:OptimalControl}, we assume conditions XXX. Then we can define the generalized Hamiltonian
% \begin{align*}
%     H:
%     \begin{array}{ccc}
%         \R_+ \times (\R^{d_Y})^{\times 3} \times \R^{d_Y} & \longrightarrow & \\
%          & \longmapsto &
%     \end{array}
% \end{align*}

% \subsection{Model ambiguity}
% Let $x_{[0:T]} \in XXX$ and assume the dynamics of $Y$ are given by \eqref{eq:filtering_dynamics__observation}. Then,  $Y \vert \lbrace X = x \rbrace$ which is defined via $(Y \vert \lbrace X = x \rbrace)_t \eqdef Y_t \vert \lbrace X_t = x_{t} \rbrace$ for all $t \in [0:T]$ represents an ordinary SDE with full observability. 
% \begin{example}\label{exa:UncertaintyHeston}
%     For any $t \in [0:T]$ and $y_{[0:t]} \in XXX$ consider $A_0(t, y_{[0:t]}) \eqdef (\mu, - \kappa y_t^2)$, $A_1(t, y_{[0:t]}) \eqdef (0, \kappa)$, $B_1(t, y_{[0:t]}) \eqdef 0$, $B_2(t, y_{[0:t]})^1 \eqdef (y_t^1\sqrt{y_t^2}, 0)$, and $B_2(t, y_{[0:t]})^1 \eqdef (\sigma \rho \sqrt{y_t^2}, \sigma \sqrt{1-\rho^2} \sqrt{y_t^2})$, where $\mu \in \R$, $\kappa, \sigma > 0$, and $\rho \in [-1:1]$. This corresponds to the Heston model with (stochastic) mean-reversion parameter $X_t$,
%     \begin{align*}
%             d 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \\
%                     Y_t^2
%                 \end{matrix}
%             \right)
%         = 
%             \left(
%                 \begin{matrix}
%                     \mu \\
%                     \kappa X_t - \kappa Y_t^2
%                 \end{matrix}
%             \right)
%             dt
%         + 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \sqrt{Y_t^2}  \\
%                     \sigma \sqrt{Y_t^2} 
%                 \end{matrix}
%             \right)
%             \left(
%                 \begin{matrix}
%                     1 & \rho \\
%                     \rho & 1
%                 \end{matrix}
%             \right)^{1/2}
%             dW^{(2)}_t, \quad  \forall t \in [0:T],
%     \end{align*}
%     and $Y \vert \lbrace X \equiv \theta \rbrace$, $\theta > 0$ represents the Heston model with deterministic (and constant) mean-reversion parameter $\theta$.
% \end{example}

% In the following, let $g: A \times XXX \mapsto \R$, define a control problem, where the control $a \in A$ acts on the path $y \in XXX$ to obtain the payoff $g(a, y)$. Further, let $u: \R \to \R$ denote a utility (concave) function. Then, under the model assumption $X = x$, the (ambiguity-unaware) control problem reads as follows,
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}} \mathbb{E}\left[
%         u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)
%     \right].
% \end{align*}
% In terms of \Cref{exa:UncertaintyHeston}, one could for instance consider the hedging task $g(a, y) := (a \bdot y^1)_T - h(y_T^1)$ of the European option with payoff structure $h: \R \to \R$, where $\mathcal{A}$ is the set of previsible trading strategies on $Y^1$.

% In \cite{KlibanoffMarinacciMukerji05}, the authors suggest considering not only one choice of model (as we did above with $X = x$) but instead a distribution of models, which are evaluated with a second expected utility. Let $r: \R \to \R$ denote a second (concave) utility function and since 
% \begin{align*}
%         \mathbb{E}\left[u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)\right]    
%     =
%         \mathbb{E}\left[u \circ g(\alpha, Y) \mid \lbrace X = x \rbrace \right],
% \end{align*}
% ambiguity-aware control problem reads as follows, 
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}}
%         \mathbb{E}\left[
%             r \left(
%             \mathbb{E}\left[
%                 u \circ g(\alpha, Y)
%             \mid
%                 X
%             \right]
%             \right)
%         \right].
% \end{align*}
% \yannick{TODO. Explain how a DKF setting applies as the model-process is unobservable.}




% \section{Theoretical Analysis}
% \label{s:Theoretical_Analysis}

% \subsection{The Structure of the Target Function: The Optimal Filter}

% In this section, we employ results of \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, and, denote an explicit formulation of the resulting distribution. For this, assume that
% \begin{align*}
%     \int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt &< \infty, \,\, \forall i  \in \myset{1}{d_X}\, \forall j \in  \myset{1}{d_X} \\
%     \int_0^T (\process{b_2}{t, y_{[0:t]}}{i, j})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{j, i})^2 dt &< \infty, \,\, \forall i \in  \myset{1}{d_X}  \,\forall j \in  \myset{1}{d_Y}\\
%     \int_0^T (\process{A_0}{t, y_{[0:t]}}{i})^2 + (\process{B_2}{t, y_{[0:t]}}{i, j})^2 dt &< \infty, \,\, \forall i \in \myset{1}{d_Y}\, \forall j \in \myset{1}{d_Y} 
% \end{align*}
% for all $y_{[0:T]} \in C([0:T], \R^{d_Y})$; the matrix $B \circ \process{B}{t,x}{} := \process{B_1}{t,x}{} \process{B_1}{t,x}{}^\intercal + \process{B_2}{t,x}{} \process{B_2}{t,x}{}^\intercal$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% % entry $g$ in $B_1, B_2$ holds
% \begin{align*}
%         \vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%     & \leq
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2, 
%     \\
%         (B_k)_{i,j}(t, x)^2  
%     & \leq 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2) 
% \end{align*}
% where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$; and we have
% \begin{align*}
%     \int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt & < \infty; \\
%     \bE[\vert (X_t)_j \vert] & < \infty, \quad \forall t \in [0:T]; \\
%     \bP\left( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \right) & = 1;
% \end{align*}
% for indices $i \in \myset{1}{d_Y}, j\in \myset{1}{d_X}$.

% This allows us to apply \citep[Theorem 12.6]{LipShiryaev_II_2001} and we deduce that $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, meaning that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.

% We assume further
% \begin{align*}
% \begin{array}{cc}
%     \vert \process{a_1}{t, x}{i, j}\vert \leq L, &\quad \forall i \in \myset{1}{d_X}, \\
%     \vert \process{A_1}{t, x}{i, j}\vert \leq L, &\quad \forall i \in \myset{1}{d_Y},
% \end{array} \quad \forall j \in \myset{1}{d_X},
% \end{align*}
% for $x \in C([0:t], \R^{d_Y})$, $t \in [0:T]$; as well as
% \begin{align*}
%     \begin{array}{cc}
%     \int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty, &\quad \forall j \in \myset{1}{d_X}, \\
%     \int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty, &\quad \forall j \in \myset{1}{d_Y}, \\
%     \end{array} \quad \forall i \in \myset{1}{d_X},
% \end{align*}
% and eventually
% \begin{align*}
%     \bE\bigg[\sum_{j = 1}^{d_X}(X_0)_j^4\bigg] < \infty.
% \end{align*}
% Then, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
% \notag
%     d\mu_t 
%         =&[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\intercal}(t,y_{[0:t]})](B\circ B)^{-1}(t,y_{[0:t]})\\
%         &\times [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt] \label{id:ClosedFormMu}
%     \\
% \notag
%     \partial_t\Sigma_t =& a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\intercal}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]}) - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]}) ]
%         \\
%         & \times (B\circ B)^{-1} (t,y_{[0:t]}) [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]})]^{\intercal} \label{id:ClosedFormSigma}
% \end{align}
% with initial conditions $\mu_0=\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\intercal}|Y_0]$. Note that we used the notation 
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\intercal + B_2B_2^\intercal, \quad 
%     b \circ B \eqdef b_1B_1^\intercal + b_2B_2^\intercal, \quad 
%     b \circ b \eqdef b_1b_1^\intercal + b_2b_2^\intercal.
% \end{align*}
% Eventually (again \cite{LipShiryaev_II_2001}, Theorem 12.7), we have that $\Sigma_t$ is positive definite for all $t \in [0,T]$ if $\Sigma_0$ is positive definite. 
% \anastasis{argue (as in page 34) that we may consider $B_0=0$ and $B\eqdef B_1$ and likewise for $b_i$ where $i=0,1$.}
% \anastasis{(which we assume to be known or tuneable?)}.

% \anastasis{@Xuwei, let's check conditions under which $\Sigma_t$ remains positive definite for all $t$ and all $y_{[0:t]}$.} 

% \begin{lemma}[Local Lipschitz-Continuity of the Optimal Filter]
%     Fix $t \in [0, T]$. Under the assumptions of \Cref{lem:LipschitzSigma} and \Cref{lem:LipschitzMu}, $f_t$ from \eqref{id:ConditionalDistribution} is locally Lipschitz-continuous. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t 
%     \end{align*}
% \end{lemma}



% \subsection{Proof of Lipschitz Continuity}
% \begin{proof}
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a constant $\bar{K} < \infty$ s.t.
%     \begin{align*}
%     \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         &\leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{align*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma} that there exists a constant $K < \infty$, s.t.
%     \begin{align*}
%             \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \quad 
%             \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%     \end{align*}
%     so we obtain 
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%     \end{align*}
%     and the statement follows. 
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]\label{lem:LipschitzMu}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:TimeLipschitzMu}, $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%  \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%  \end{align*} 
% \end{lemma}
% \begin{proof}
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) \notag \\
%   & \quad \quad - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \label{id:Phi1} \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu}, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0, s]}) d y_{[0, s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align} 
%  & \mu^{(1)}_t - \mu^{(2)}_t \notag \\
%  & =   \mu_0^{(1)} - \mu_0^{(2)} 
%   + \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds 
%   + \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \notag \\ 
%  & \quad + \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \notag  
%   + \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\,
% (\mu^{(1)}_s - \mu^{(2)}_s ) ds .  \notag
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} 
%   + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwalls inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$. As a next step, let $\mySet{[s_{i-1}:s_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Moreover, by the use of integration by parts, we have
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         - \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         + \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq t} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% (Time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:t]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 
%       \leq \epsilon_I + K t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that $\eqref{t:gammaB} \leq K \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t$. Eventually, consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to Lipschitz continuity of $\Phi_1$. We conclude, since $\max_{s \in [0:t]} \|\mu^{(2)}_s \|_2 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\eqref{t:gammaC} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$, and therefore $\gamma(t)\leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.
% \medskip

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%         \left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)
%      \notag  
% \end{align} 
% As $\Phi_1$ is (time-)Lipschitz continuous, implying $\max_{s \in [0:t]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$ we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}

% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the assumptions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{align*}
%             \| \mu_t - \mu_s \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0, u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0, u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{align*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 
%         \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwalls inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_0^t a_0(u, y_{[0, u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{:= \alpha(t)}
%           + \int_0^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0, s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0, u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi1}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_1$, $ (b \circ B)$, $(B\circ B)^{-1}$, $ A_0$, and $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
% \begin{enumerate}[wide]
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_0$, $(b \circ B)$, $(B\circ B)^{-1}$, $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}[wide]
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:LipschitzA1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq K \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left hand side refers to the Forbenius norm.
% \end{lemma} 
% \begin{proof} 
% From \eqref{id:ClosedFormSigma}, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
% \Sigma_t = & \Sigma_0 + \int_0^t
% a_1(t,y_{[0:s]}) \Sigma_s + \Sigma_s a_1^{\intercal}(s,y_{[0:s]}) + (b\circ b)(s,y_{[0:s]}) - [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]}) ]
%    \notag      \\
%         & \hspace{3cm} \times (B\circ B)^{-1} (s,y_{[0:s]}) [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]})]^{\intercal} ds . \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{align*} 
% & \Sigma^{(1)}_t - \Sigma^{(2)}_t \\
% & = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
% & \quad + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) + 
% \Xi_2^\intercal (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{align*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\intercal(s, y^{(1)}_{[0:s]}) - a_1^\intercal(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{align} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef & \big[ a_1^\intercal(s, y^{(2)}_s) 
%  + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) (b\circ B) (s, y^{(1)}_{[0:s]}) \notag \\ 
% &\quad + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
% \big] .   \label{Xi2} 
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{align} 
%  &\big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\
% & \leq  
% \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%  \notag \\ 
%  & \quad  + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot \notag \\ 
%  & \quad \qquad \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{align}  
% From \Cref{lem:LipschitzA1}, we have that 
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{align} 
%  & \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\ 
% &\quad \leq  
% \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big) 
% \cdot \notag \\ 
% &\quad  \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
% \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{align} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$
%  and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is also uniformly bounded, according to \eqref{Xi2}. 
%  Therefore, from \eqref{Sigma1-2bddXi2} we obtain that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% K ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}

% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and assume local Lipschitz continuity in the path component as well as time-continuity of $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\delta > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \delta$ holds
% \begin{align*} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component, we conclude that $a_1$, $b \circ b$, $A_1^\intercal(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\intercal (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\intercal$ have the same property. By this, together with the triangular inequality, 
%     \begin{align*}
% \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  & \leq  
%  2K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) + \\
% & \qquad + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2 + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \\
% & =  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(1+ \Vert\Sigma^{(1)}_s \big\Vert_2 + \Vert\Sigma^{(2)}_s \big\Vert_2 + \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2 \Big).
% \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < \bar{K} \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in $y_{[0:t]}$, for any $\epsilon>0$, there exists $\delta>0$ such that 
% when 
% $\| y^{(1)}_t - y^{(2)}_t \|_2 < \delta$,  
% $\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \|_2 < \epsilon$, and therefore 
% \begin{align*} 
% \big\| \Sigma^{(2)}_t \big\|_2 \leq \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 + \big\| \Sigma^{(1)}_t \big\|_2 
% \leq \epsilon + K . %\label{Sigma2bdd} 
% \end{align*} 
% \end{proof}

% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let $a_1, b \circ b, b \circ B, (B \circ B)^{-1}, b \circ B, A_1$ be continuous. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\intercal}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma}, then there exists an $r > 0$, s.t. for all times $t \in [0,T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ holds that 
%     \begin{align*}
%         \Sigma_t - r \cdot I_{d_X}
%     \end{align*}
%     is positive semi-definite.
% \end{lemma}
% \yannick{TODO. Assumptions are highlighted below.}
% \begin{proof}
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\intercal(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\intercal(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ being positive semi-definite} at 
%     \begin{align*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal )
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\intercal
%                     \right)
%                 ds.
%     \end{align*}
%     As \byyan{$G_t(y_{[0:t]})$ is positive definite}, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%                 (G_t(y_{[0:t]})^{-1})^\intercal
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%             )
%     \end{align*}
%     and 
%     \begin{align*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\intercal
%             \right)
%         \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{align*}
%     As we \byyan{assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$} as well as \byyan{$K_3 > 0$ s.t. $\tr(A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$} we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\intercal(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]


% \section{Proof of Approximation Theorem}
% \label{s:Proof}
% This section contains the derivations of our paper's main results.

% \subsection{ The Attention Layer Implements Good Feature Maps}
% \begin{proof}[{Proof of Proposition~\ref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^d)$, given by $f\mapsto \big(f(\cdot /T),0,\dots,0\big)$, is an isometric embedding; then $\phi\eqdef \phi_3\circ\phi_2\circ \phi_1$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^d)$.
% \end{proof}


% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Qualitative Version]
% \label{lem:Good_Feature_Map_Qualitative}
% Under Assumption~\ref{ass:reg_compact} (i).  There exist $y^{(1)},\dots,y^{(N)}\in \psi(M)\subset C([0:T],\mathbb{R}^d)$ and matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a continuous injective map.  
% Here, $N=D_K+1$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map_Qualitative}}]
% \anastasis{Add details:}
% Since $(M,g)$ is a connected, homogeneous, geodesically complete Riemannian manifold of dimension $D_K$ then, \citep[Corollary 3.7]{HeydarpourMaghsoudi_2015_MetricDimension_GeometricSpaces} implies that there exist $p^{(1)},\dots,p^{(N)}$, with $N=D_K+1$, such that the map $p\mapsto \big(d_g(p,p_n)\big)_{n=1}^N$ is injective.  Clearly, the map $\big(d_g(p,p_n)\big)_{n=1}^N$ is continuous since the metric $d_g$ is a continuous function.  
% \end{proof}


% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(N)}$ in $C([0:T],\mathbb{R}^d)$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Quantitative Version]
% \label{lem:Good_Feature_Map}
% Under Assumption~\ref{ass:reg_compact} (ii).  
% There exists a constant $C_{D_K}>0$ depending only on $D_K$ such that for and $\delta$-packing $\{y^{(n)}\}_{n=1}^N$ of $K$, and matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a bi-Lipschitz embedding
% of $K$ into $(\mathbb{R}^{N+1},\|\cdot\|_2)$ provided that
% \[
%         \delta 
%     \lesssim 
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \]
% where $\lesssim$ hides a constant $C_{D_K}>0$ depending only on $D_K$.  Furthermore\footnote{\anastasis{Define $\|\cdot\|_0$-notation.}}, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$, and $C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any sampling distribution $\mathbb{P}_{in}$ with support $K$.\anastasis{define in intro.}
% \hfill\\
% Moreover, if $K$ is not aspherical then the conclusion holds without a quantitative upper-bound on $\delta$, and therefore on $N$.
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map}}]
% \noindent\textbf{Step 1 - Estimating $N$ on the Riemannian Manifold $(M,g)$}
% \hfill\\
% %%
% Since $(K,\|\cdot\|_T)$ be isometric to $(M,d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $D_K$-dimensional Riemannian manifold $(M,g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $M$ denoted by $\operatorname{sys}(M)$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(M) 
%     \le
%     \,\tilde{C}_{D_K}
%     \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \end{equation}
% where $\operatorname{Vol}(M,g)$ denotes the Riemannian volume of $(M,g)$ and $\lesssim$ hides a constant depending only on the dimension $D_K$, for a universal constant $\tilde{C}_{D_K}>0$ satisfying
% \[
%         0
%     <
%         \tilde{C}_{D_K}
%     <
%         6 (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}
% \,
% .
% \]
% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(M)/10$ then the given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(M,g)$, the map $\varphi_2:(M,d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{D_K}\eqdef \tilde{C}_{D_K}/10$, $N\eqdef \#\widetilde{\mathbb{X}}$, and enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^N$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{D_N}
%         \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     .
% \]
% We note that, if $K$ is not aspherical, then but it is only closed, then the conclusion still holds however, without the quantitative upper-bound on $\delta$.
% \hfill\\
% \noindent\textbf{Step 2 - Building the Feature Map with Well-posed Inverse}
% \hfill\\
% %%
% Let $\varphi_1:(M,d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have assumed to exist.  Set $\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^N$ where, for $n=1,\dots,N$ we set $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\varphi: C([0,T],\mathbb{R}^d)\rightarrow \mathbb{R}^N$ by $y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^N$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^N
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^N
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^N
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^N
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $M$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \hfill\\
% \noindent\textbf{Step 3 - Aligning to a Hyperplane in $\mathbb{R}^{N+1}$ with a Shallow ReLU Neural Network}
% \hfill\\
% Set $N_1\eqdef N+1$.  Let $b$ be the zero vector in $\mathbb{R}^N$.
% A mild variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $N\times 2N$ and $2N\times N$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_N & \vert & -I_N
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_N \\
%             \-- \\
%             -I_N
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^N\rightarrow \mathbb{R}^N$ defined by $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^N$.  Consider the $N_1\times N$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{N_1}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_N & 0 \\
%             0 & 0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,N\\
%             1 & \mbox{ if } i=N_1
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \hfill\\
% \noindent\textbf{Step 4 - Injectivity of Softmax Function on Hyperplane}
% \hfill\\
% Note that, for each $u\in \mathbb{R}^N$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^N$ onto the $N$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^N\}$ in $\mathbb{R}^{N_1}$.  Observe that the Softmax function $\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^N\,e^{u_k})_{j=1}^N$ maps $H$ surjectively and continuously onto the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})\subset \operatorname{int}(\Delta_N)\eqdef \{v\in [0,1]^{N_1}:\,\sum_{i=1}^{N_1}\,v_i=1\}$; i.e.\ of the interior of the $N_1$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{N_1}) + 1\big)_{i=1}^{N}
% \end{equation}
% is a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})$ then, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{N_1})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$.  Since, $\Psi$ was constructed to be an instance of $\operatorname{attn}_T$.  
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_N)$ of the $N_1$-simplex then, $C^{\star}\eqdef \max_{u\in \Phi(K)}\,\min_{v\in \Delta_{N_1}\setminus \operatorname{int}(\Delta_{N_1})}\,\|u-v\|>0$.  Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{N_1}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{N_1})
%             +
%             \bar{\Delta}_{N_1}
%         \}
% \]
% where $\bar{\Delta}_{N_1}\eqdef (1/N_1,\dots,1/N_1)$ is the barycenter of the $N_1$-simplex $\Delta_{N_1}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{N_1}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is Lipschitz\footnote{\anastasis{Add details about Lipschitzness? or Obvious?}} on $\Delta_{N_1}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image, since it is the composition of Lipschitz functions with Lipschitz inverses.  This completes the proof.  

% \end{proof}

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Finite Version]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under Assumption~\ref{ass:reg_compact} (i) and let $k\eqdef \#K$.  
% Set $N=48\lceil\log(k)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There exists a matrices matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a $(2^{-1/2},(3N/6)^{1/2})$-bi-Lipschitz embedding
% of $K$ into $(\mathbb{R}^{48\lceil \log(k)\rceil},\|\cdot\|_2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any sampling distribution $\mathbb{P}_{in}$ with support $K$.\anastasis{define in intro.}
% \end{lemma}
% \begin{proof}
% We argue similarly to the proof of Lemma~\ref{lem:Good_Feature_Map}, with only Steps $1$ and $2$ of its proof being replaced with the following argument.  
% \hfill\\
% \noindent\textbf{Step 1 and 2 - Modified- Building the Feature Map}
% \hfill\\
% Enumerate $K=\{x_n\}_{n=1}^N$.  The map $\phi_1:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^N,\|\cdot\|_{\infty})$ given by $x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^N$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le N^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^N$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^N,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^N,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% By the Johnson-Lindenstrauss Lemma, as derived in \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $48$ as opposed to $200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , there is a linear map $\phi_3:(\mathbb{R}^N,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $(\lceil48\,\ln(N)\rceil)\times N$-matrix $A_0$, satisfying: for every $u,v\in \mathbb{R}^N$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, $\varphi:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3N/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_{t}
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         N^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3N/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_t 
% .
% \end{align*}
% \noindent\textbf{Remaining Steps:}
% \hfill\\
% The rest of the proof is identical to the proof of Lemma~\ref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_N\,\vert \,I_N)^{\top}$.
% \end{proof}

% \anastasis{Update Theorems to also include this case.}

% \subsection{Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}
% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d\in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d}$ denote the set of $d\times d$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d\times d$ matrices.  Here the $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.  Consider the $2$-product metric on $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ defined for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ by sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ will serve to quantize $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^d\times \operatorname{Sym}_{0,d})^{N} \rightarrow 
% \mathbb{R}^d\times \operatorname{Sym}_{0,d}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:QAS_Space_Sym0d}]  
% We first show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% \hfill\\
% \textbf{QAS Space Structure}
% \hfill\\
% Since $\operatorname{Sym}_{0,d}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the normed space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ as sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big)
%     = &
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     = &
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     \le &
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad            
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     \le &
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     = &
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\mathcal{Q},\eta)$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
% \hfill\\
% \textbf{Barycentricity}
% \hfill\\
% Consider the map $\sigma:(\mathbb{R}^d\times \operatorname{Sym}_{0,d})^2\times [0,1]$ given for any $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and $t\in [0,1]$ by
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),t
%         \big)
%     \eqdef 
%         \eta\big(
%             (m,A),(\tilde{m},B),(t,1-t)
%         \big)
%     .
% \]
% Since geodesics in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ are line segments, since $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the inner-product space $(\mathbb{R}^d\times \operatorname{Sym}_d)$, with inner-product given by the product of the Euclidean and Frobenius inner-products, then clearly for each $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ the map $t\mapsto \sigma\big((m,A),(\tilde{m},B),t\big)$ is a geodesic in the global NPC space, as defined in \citep[Definition 2.1]{Sturm_2003}, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$.  Thus, $\sigma$ is a \textit{geodesic bicombing} in the sense of \citep[page 1]{basso2018fixed}.  Since 
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
%     =
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
% \]
% then \citep[Theorem 3.4]{basso2018fixed} applies; whence $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is barycentric with $1$-Lipschitz barycenter map explicitly given therein.  

% Since is a barycentric QAS space then, \citep[Setting 3.6]{kratsios2023transfer} (iii) is satisfied.
% \end{proof}

% Having established the barycentricity and the QAS space structure of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\eta,\mathcal{Q}_{\cdot})$, we are now ready to prove the following result.
% \anastasis{Here in transcription}
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ there is a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ satisfying
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x_{\cdot}),f(x_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{t}(x_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^M\,
%                 P_{\Delta_M}(\hat{f}\circ \operatorname{attn}_T(x_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $M\in \mathbb{N}_+$, $m^{(1)},\dots,m^{(M)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(M)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_M}:\mathbb{R}^M\rightarrow\Delta_M$ is the Euclidean (orthogonal) projection onto the $M$-simplex, and an MLP $\hat{f}:\mathbb{R}^N\rightarrow \mathbb{R}^M$ with activation function $\sigma$.  The depth, width, encoding dimension (N), and decoding dimension (M) are recorded in Table~\ref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{D_K}\operatorname{Vol}(M,g)^{1/D_K})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:approximation_Sym}}]
% \anastasis{Relabel $N$ (index) as $M$}
% \hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% We will apply \citep[Theorem 3.7]{kratsios2023transfer}, which requires us to verify each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \paragraph{Step 1 - Implementing a Bi-Lipschitz Feature Map with the Attention Layer}
% \hfill\\
% \textbf{Remark:} \textit{We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap} can be chosen such that $\operatorname{attn}_T$ is a suitable feature map}.
% \hfill\\
% \begin{comment}
% \paragraph{Case (i) - The Continuous and Injective Case} 
% \anastasis{come back to this shortly...}
% \paragraph{Case (ii) - The Bi-Lipschitz Case} 
% \noindent 
% \end{comment}
% Let $N$ denote the $C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(\mathcal{M},d_g)$.  Since $(K,\|\cdot\|_T)$ and $(\mathcal{M},d_g)$ are isometric, then $N$ is the $C_{D_K} \operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(K,\|\cdot\|_T)$.  
% By Lemma~\ref{lem:Good_Feature_Map}, there are matrices $A,B$, $a$, and $b$ with $\|A\|_0=2N=\|B_0\|$, $\|a\|_0=1$, and $\|b\|_0=0$ such that $\varphi\eqdef \operatorname{attn}_T$, as defined in~\eqref{lem:Good_Feature_Map}, is a bi-Lipschitz embedding of $(K,\|\cdot\|_{T})$ to $(\mathbb{R}^N,\|\cdot\|_2)$.  Set $\{(K,\varphi)\}$, let $\nu$ denote the normalized (uniform) Volume probability measure on $(\mathcal{M},g)$, and let $\mu\eqdef \varphi_{\#}\nu$ be its pushforward to $(K,\|\cdot\|_T)$.  Since every bi-Lipschitz map is a quasi-symmetry\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}, then \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(M,d_g)$ is a doubling metric space, as defined on \citep[10.13; page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  This verifies \citep[Setting 3.6 (i)]{kratsios2023transfer}.




% \paragraph{Step 2 - Feature Space Geometry}\hfill\\
% Since the codomain of $\phi$ is simply a Euclidean space, then the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^N}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^N$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^N$, 
% \[
%     \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
% \]
% and the operator norm $\|1_{\mathbb{R}^N}\|_{op}$ of $1_{\mathbb{R}^N}$, thus of $T^i$ for every $i\in \mathbb{N}_+$, is uniformly bounded above by $1$.  
% Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} is holds.

% \paragraph{Step 3 - Geometry of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$}
% \hfill\\
% By Lemma~\ref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $N\in\mathbb{N}_+$, $u\in \mathbb{R}^N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 P_{\Delta_N}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \paragraph{Step 4 - Determining The Euclidean Universal Approximator}
% \hfill\\
% \textbf{Remark:} \textit{We now verify that the class of all MLPs with activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition} satisfies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.}\\
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le d+D+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy Assumption~\ref{ass:KLCondition} then, \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \paragraph{Step 5 - Applying~{\citep[Theorem 3.7]{kratsios2023transfer}}}
% Steps $1$ though $5$ verify that the conditions of Theorem~\citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the Feature Decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, Theorem~\citep[Theorem 3.7]{kratsios2023transfer} implies, thus for every $\varepsilon>0$ there is a map $\hat{t}:K\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{t}(x_{\cdot})
%     = &
%         \beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^N
%             \,
%                 \big(
%                     P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $x_{\cdot}\in K$ satisfying 
% \[
%     \sup_{x_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{t}(x_{\cdot})
%         ,
%             f(x_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ (which exists by Lemma~\ref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a right-inverse of the map $\mathbb{R}^d\times \operatorname{Sym}_{0,d}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$, where $\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially,~\eqref{eq:transformer_pre_mapped_BEGIN}-~\ref{eq:transformer_pre_mapped_END} reduces to~\eqref{lem:approximation_Sym__approximation___representation}.  


% \paragraph{Step 6 - Tallying Parameters}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $N=\mathcal{N}_{\operatorname{pack}}\big(K,C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in Table~\ref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $N$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             N
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{proof}

% \subsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool.  The proof method is summarized visually in Figure~\ref{fig:Approximation_Theorem}.


% \anastasis{t and t hat}
% \begin{figure}[H]
%     \centering
%     \begin{tikzcd}
%     \big(C([0:T],\mathbb{R}^d),\|\cdot\|_{\infty}\big) & (\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2) \\
%     (K,\|\cdot\|_{\infty}) 
%     \arrow[hookrightarrow]{u}{\iota} 
%     \arrow{r}{f} 
%     % \arrow[swap]{d}{\varphi} 
%     \arrow{dr}{\varrho\circ f}
%     & ({\mathcal{N}}_d,\mathcal{W}_2) 
%     \arrow[hookrightarrow]{u}{i}
%     \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
%     & (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
%     \end{tikzcd}
%     \caption{Summary of Proof Strategy for Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd} \anastasis{details}.}
%     \label{fig:Approximation_Theorem}
% \end{figure}

% \begin{lemma}
% \label{lem:Universal_Approximation_Theorem__PathToNd}
% Let $d\in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^d)$ be non-empty and regular compact set in the topology of uniform convergence.  For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:(K,\|\cdot\|_{\infty})\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ there exists a map $\hat{t}:C([0,T],\|\cdot\|_T)\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ with representation 
% \[
%         \hat{t}(x)
%     \eqdef
%         \mathcal{N}_d\Biggl(
%                 \sum_{n=1}^N\,
%                     P_{\Delta_q}(\mathcal{NN}(x))_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^N\,
%                     P_{\Delta_q}(\mathcal{NN}(x))_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)})
%         \Biggr)
% \]
% \anastasis{Update representation/simplify ofc + explain notation} 
% such that
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{t}(x)
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(N)$ and Decoding dimension $(M)$ are all recorded in Table~\ref{tab:approximationrates__nonFlatVersion} depending on the the choice of activation function $\sigma$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd}}]
% \hfill\\
% \textbf{Step 1 - Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$}
% By Lemma~\ref{lem:LipschitzManifold_Nd} the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^d,\operatorname{Sym}_{0,d},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous then the map
% \[
%     g: (K,\|\cdot\|_T)\ni x \mapsto 
%     \pi\circ \varrho\circ f(x)
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d\times d$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain is achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; i.e.
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_d$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% \anastasis{Add reference to Lemma~\ref{lem:LoewnerBound} here.}
% Consequentially, Lemma~\ref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \hfill\\
% \textbf{Step 2 - Approximating $\varrho \circ f$ on $K$}
% \hfill\\
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%                     \,\operatorname{diam}(K) + 1
%                 }
%                 }
%         \biggr\}
% .
% \end{equation}
% We many now apply Lemma~\ref{lem:approximation_Sym} to deduce that there exists a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x),\varrho\circ f(x))
%     <
%         \delta
% .
% \end{equation}
% Since Lemma~\ref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  Set $t\eqdef \varrho^{-1}\circ \hat{t}$ and 
% denote the $1$-thickening of $\varrho\circ f(K)$ by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}:\,(\exists x\in K)\, d_{2,F}(f(x),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{t}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate} and Lemma~\ref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% = & 
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{t}(x)
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{x\in K}\,
%         d_{2,F}\big(
%                 \hat{t}(x)
%             ,
%                 \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% \le &
%     \sqrt{d}2\sqrt{
%             L
%             \,\operatorname{diam}(K) + 1
%         }
%     \,
%     \varepsilon
%     \,
%     \frac1{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \nonumber
% \label{eq:Approxim_LEMMA__END}
% = & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from Lemma~\ref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_B} followed from the estimate~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009}, then estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-~\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_p\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \textbf{Step 3 - Counting Parameters}
% Using $\delta$, as defined in~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in Table~\ref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \anastasis{Add computations tomorrow}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_d}$ denote the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_d}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_d}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_d},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_d}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of Lemma~\ref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_d}$ sending any $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_d}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_d}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_d}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_d},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_d}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_d}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}



% \appendix
% \section{Auxiliary Lemmata}
% \label{s:AuxLemmata}
% This section records auxiliary lemmata used in our proofs but proven elsewhere.
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% it holds that
% \[
% \begin{aligned}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     \\
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{aligned}
% \]
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzManifold_Nd}}]
% The proof is due to Iosif Pinelis, and is given in \cite{LocalLipschitz_Pinelis}.  We only note that, $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$ where $\|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})$ denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}

% \section{Background: Riemannian Geometry and Algebraic Topology}
% \label{s:Background_Geo}



% \bibliographystyle{abbrvnat}
% \bibliography{Bookkeaping/2_References}


% \newpage
% \section{Algorithms}
% \input{Sections/Practical_Approach}

% \end{document}


==> OLD/Historical_Versions/OLD/Old_notes.tex <==
\newpage
\newpage
\anastasis{Please ignore this bit for now friends :)}
Let $X_{\cdot}\eqdef (X_t)_{t=0}^{\infty}$ be a discrete-time stochastic process defined on a filtered probability space $(\Omega,\mathcal{F},\mathbb{F}\eqdef (\mathcal{F}_t)_{t=0}^{\infty},\mathbb{P})$ taking values in $\mathbb{R}^d$.  Suppose that for $\P$-a.s.\ each $x_{\cdot}\in (\mathbb{R}^d)^{\mathbb{N}}$ the conditional law
\[
        \mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \eqdef 
        \mathbb{P}(X_{t+1}\in \cdot \vert x_{[0:t]})
    ,
\]
is absolutely continuous with respect to the $d$-dimensional Lebesgue measure and has finite moments.  This happens, for example in continuous time, for SDEs with sufficiently smooth drift and diffusion coefficients \cite{aida1993support,kusuoka2010existence,de2011smoothness}, possibly with jumps \cite{cass2009smooth}, driven by Gaussian processes with continuous paths of $p$-variations \cite{baudoin2014upper} such as fractional Brownian motions with Hurst parameter even in $[1/4,1/2]$ \cite{inahama2022positivity}, or even certain strong solutions to SDEs with H\"{o}lder drift \cite{olivera2019density}.  The discrete-time analogues of these results are immediately obtained by discretizing time
\anastasis{Provide a concrete example of a non-Markovian ``discrete-time" SDE.}


The conditional law of such a general process $X_{\cdot}$ can be a complicated high-dimensional object, which can make approximation of it computationally much more challenging \cite{kratsios2021universal} compared to approximation of functions in Euclidean spaces \cite{...} or smooth Riemannian manifolds \cite{kratsios2022universal}.  Since we will be interested in computationally tractable estimates of the conditional law of $X_{\cdot}$, then the starting point for our analysis is a low-dimensional non-degenerate Gaussian surrogate for $\mathcal{L}(X_{t+1} |x_{[0:t]})$ which preserves the maximum information possible of $\mathcal{L}(X_{t+1} |x_{[0:t]})$.

One possible surrogate function is formalized using the \textit{information projection}, or \textit{$I$-projection}.  More specifically, under the aforementioned conditions, \citep[Theorem 1]{CsiszarInfoProjRevisited2003IEEE} guarantees that there exists a unique Gaussian measure with non-singular covariance, which we denote by $\mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]})$, which best represents the conditional law $\mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]})$ 
\anastasis{Relate to dimension-reduction/regularization and capacity control :)}
\[
\operatorname{KL}\biggl(
        \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})
        ,
        \mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \biggr)
    =
    \min_{\mathbb{Q}}\,
    \operatorname{KL}\big(
    \mathbb{Q},\mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \big)
\]
where the minimum is taken over a suitable space of probability measures $\mathcal{Q}$ to be described below.

\subsection{Case 1 - $\mathcal{Q}$}
Suppose that $\mathcal{Q}\subseteq \mathcal{P}_1(\mathbb{R}^d)$ consists of all Gaussian measures on $\mathbb{R}^d$ with covariance of the form $\otimes_{i=1}^d\, \sigma_i$ for some $\sigma_1,\dots,\sigma_d>0$.
% That is, is the \textit{information projection} of the conditional law $\mathcal{L}(X_{t+1}\vert x_{[0:t]})$ onto the space $\otimes_{i=1}^d\,\mathcal{N}_1$ of $d$-dimensional Gaussian measures with non-singular diagonal covariance matrices; denoted by $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$.  
% \cite{Takatsu2011}
The measures in $\mathcal{Q}$ can be parameterized bijectively and continuously by
\[
\begin{aligned}
\psi:\mathbb{R}^{2d}& \rightarrow \otimes_{i=1}^d\,\mathcal{N}_1
\\
(\mu,\varsigma)& \mapsto \mathcal{N}_d\left(\mu,
\begin{pmatrix}
e^{\varsigma_1} & 0 & \dots & 0 \\
0 & e^{\varsigma_2} & \dots & 0 \\
0 & 0& \ddots & 0 \\
0 & 0& \dots & e^{\varsigma_d}
\end{pmatrix}
\right)
.
\end{aligned}
\]
If we were to fix a time $t\in \mathbb{N}_+$, a feature map $\varphi:\mathbb{R}^{t(d+1)}\rightarrow \mathbb{R}^F$, and consider the hypothesis class $\mathcal{F}$ of \textit{non-Euclidean kernel learners} $f_{\theta}:\mathbb{R}^{t(d+1)}\rightarrow \otimes_{i=1}^d\,\mathcal{N}_1$
\[
    \hat{f}_{\theta_{\cdot}}(x_{[0:t]})
    \eqdef 
    \psi\big(
        \theta_t^{\top}
        \varphi(x_{[0:t]})
    \big)
,
\]
where $\theta$ belongs to the parameter space $\Theta\eqdef \mathbb{R}^{d\times F}$ of $d\times F$-dimensional real-matrices.  \anastasis{Given examples of such $\varphi$, e.g.\ random NNs and discuss their properties$\dots$}.  
Then, given a set of i.i.d.\ sample paths $\{x^{(n)}_{[0:t]}\}_{n=1}^N$ from the process $X_{\cdot}$ up to time $t$, for some positive integer $N$, we can train the non-Euclidean kernel regressor to approximate the function $\mathcal{L}(X_{t+1} \vert x_{[0:t]})$ by optimizing the empirical risk functional
\begin{equation}
\tag{Static}
\label{eq:static_objective}
\min_{\theta}\,
    \frac1{N}\sum_{n=1}^N\,
        \mathcal{W}_2^2\big(
            \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}^{(n)})
            ,
            f_{\theta}(x_{[0:t]}^{(n)})
        \big)
,
\end{equation}
associated to the $2$-Wasserstein distance on $\mathcal{P}_2(\mathbb{R}^d)$. 

We are interested in optimizing the dynamic version of~\eqref{eq:static_objective} where our learners are of the form 
\[
\{f_{\theta_{\cdot}} :\, \theta_{\cdot}\in (\mathbb{R}^F)^{\mathbb{N}}\}
\]
and each $\hat{f}_{\theta_{\cdot}}$ is as above.  Our goal is to optimize the following regret functional
\begin{equation}
\tag{Regret}
\label{eq:dynamic_objective}
        \mathcal{R}(\theta_{[0:T]})
    \eqdef 
        \frac1{T N}\,
            \sum_{t=0}^{T-1}\,
                % \frac1{N}
                \sum_{n=1}^N\,
                \big(
                        \mathcal{W}_2^2\big(
                            \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}^{(n)})
                            ,
                            f_{\theta}(x_{[0:t]}^{(n)})
                        \big)
                +
                    \lambda\|\Delta_t\theta_t\|_2^2
            \big)
,
\end{equation}
where $\lambda>0$ is a regularizing hyperparameter and the minimization is performed $\mathcal{F}_T$ by optimizing over the set of controls in~\eqref{eq:control}.  Using coincidence results with the Wasserstein-$2$ distance, we can show that the regret functional~\eqref{eq:dynamic_objective} can be rewritten as
\begin{equation}
\label{eq:dynamic_objective__simplified}
        \mathcal{R}(\theta_{[0:T]})
    \eqdef 
        \frac1{T N}\,
            \sum_{t=0}^{T-1}\,
                % \frac1{N}
                \sum_{n=1}^N\,
                \Big(
                        \big(
                                \|\mathbb{E}(X_{t+1} \vert x_{[0:t]}^{(n)}) - \mu(\theta_t)\|_2^2
                            +
                                \|
                                    (\sqrt{\exp(\varsigma_i)}
                                    -
                                    \sqrt{\sigma_i})_{i=1}^d
                                \|_2^2
                        \big)
                +
                    \lambda\|\Delta_t\theta_t\|_2^2
            \Big)
,
\end{equation}

% \anastasis{%if we solve this, then perhaps we can extend to the mean-field N-player version where each player controls a mixture component...  Show that
% I will show this:
% \[
%         \mathcal{W}_2^2\big(
%             \mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]}^{(n)})
%             ,
%             f_{\theta}(x_{[0:t]}^{(n)})
%         \big)
%     =
%         \|\mathbb{E}(X_{t+1} \vert x_{[0:t]}^{(n)}) - \mu(\theta_t)\|_2^2
%         +
%         \|
%             (\sqrt{\exp(\varsigma_i)}
%             -
%             \sqrt{\sigma_i})_{i=1}^d
%         \|_2^2
% \]
% explain the notation later...\hfill\\
% @Xuwei, Note that this is now a linear-quadratic problem.  We can possibly optimize the weights like last time also.
% \hfill\\
% @Xuwei I wonder if we can introduce symmetry into the problem and view this as several agents controlling $\theta_{\cdot}$ then use our decentralization technique.
% \hfill\\
% @AK: I wonder if we can use a VMP-type estimate here to reduce the complexity of computing the OC, up to some error ofc.
% }

% \anastasis{Possibly extend to fancier exponential families later.}

% \anastasis{I'd suggest replacing the class of general controls in~\eqref{eq:control} with a class which is ``designed to look forward''; namely,
% \[
% \theta_t = f(\theta_{t-1},\nabla_{\theta} R(\theta_{t-1})
% \]
% We can use \citep[Theorem 3.18]{KrieglMichor_ConvenientBook_1997_AMS} to get a critical point of the regret functional $\mathcal{R}$:
% \begin{enumerate}
%     \item First compute the Gateau derivative of the regret functional (see \citep[Theorems 5 and 6]{pmlr-v134-casgrain21a}),
%     \item Then input the derivative of f into the chain-rule
%     \item Solve.
% \end{enumerate}
% }


% \subsection{Case 2 - $\mathcal{Q}$ Maximum Entropy Family}
% Let $\mathcal{Q}$

% Since $\otimes_{i=1}^d\mathcal{N}_1$ is an exponential family, then \citep[Theorem 1]{CsiszarInfoProjRevisited2003IEEE} guarantees that $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ exists. for each $x_{[0:t]}\in \mathbb{R}^{(1+t)d}$.  Since any such $\nu\eqdef \mathcal{N}(\mu,\otimes_{i=1}^d\,\sigma_i)$ is characterized by the moment constraints
% \[
% \mathbb{E}_{X\sim \nu}[X_i] = \mu_i \mbox{ and } \mathbb{E}_{X\sim \nu}[(X_i)^2] = \mu_i^2 + \sigma_i,
% \]
% for $i=1,\dots,d$, then \citep[Theorem 3.1]{csiszar1975divergence} implies that $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ is of the form
% \begin{equation}
% \label{eq:IprojForm}
% \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}) 
% \propto
% \exp\Big(\sum_{i=1}^d\,\beta_i\,u_i + \beta_{d+i}\,u_i^2\Big)
% d\lambda(u),
% \end{equation}
% where $\lambda$ is the $d$-dimensional Lebesgue measure, $\beta\in \mathbb{R}^{2d}$, and $\propto$ hides the unique constant ensuring that the measure on the right-hand side of~\eqref{eq:IprojForm} integrates to $1$.  Whence, $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ belongs to $\otimes_{i=1}^d\,\mathcal{N}_1$. \anastasis{redundant.}

==> OLD/Historical_Versions/OLD/Working_Introduction/Intro.tex <==
\begin{abstract}
% GPT
% Inspired by the Kalman filter, Deep Kalman Filters (DKFs) have lacked strong theoretical ties to the stochastic filtering problem, limiting their trustworthy applicability, in areas where traditional stochastic filtering has been applied mathematical finance. We present a class of continuous-time DKFs designed to approximate the conditional law of various non-Markovian, conditionally Gaussian signal processes using noisy measurements. Our approach quantifies approximation quality through worst-case 2-Wasserstein distance, computed uniformly computed over regular compact path spaces. Unlike other infinite-dimensional deep learning models, our DKF adapts to path space geometry and does not require a Schauder basis, enhancing its versatility for filtering tasks.
% ME - 1
% Deep Kalman filters (DKFs) are neural network models that generate Gaussian input probability measures.  However, beyond their inspiration from the Kalman filter, there are still weak theoretical ties between DKFs and the stochastic filtering problem where one tries best to reconstruct a partially observed signal from noisy measurements.  Nevertheless, without stronger clear ties to the filtering problem, the use of DKFs to numerically solve problems where stochastic filtering has traditionally deployed, e.g.\ XXX finance, is questionable.   We address this issue by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  Unlike other deep learning models defined on infinite-dimensional spaces, our DKF does not rely on a Schauder basis for the path space.  Rather, it adapts to the geometry of the compact set of paths on which it approximates the optimal filter.  
% Me -2 
Deep Kalman filters (DKFs) are a class of neural network models that generate Gaussian probability measures from sequential data.  Though DKFs are inspired by the Kalman filter, they lack concrete theoretical ties to the stochastic filtering problem, thus limiting their applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-times measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  
% Unlike most deep learning models defined on the infinite-dimensional domains, our DKF does not rely on a particular Schauder basis, and instead, it adapts to the geometry of a given path space.  
\end{abstract}


\section{Introduction}
\label{s:Algorithm}
%\fbox{\begin{minipage}{0.8\textwidth}
%    \textbf{Structure of introduction.}
%    \begin{enumerate}
%        \item Opening
%        \item What are Kalman filters and what are traditional use cases of Kalman filters in finance (and beyond)
%        \item What are Deep Kalman Filters (when/how) and why did they become popular and what (were) limitations of Kalman Filters that can be resolved by Deep Kalman Filters?
%        \item What is the main result in this paper and why is it useful? Universality: Limitations of existing results and extensions.
%        \item This is what we don't do (re: training) but "this is why it is ok"...
%        \item Structure of the article.
%    \end{enumerate}
%\end{minipage}
%}
%\bigskip

\byyan{Opening.}\hfill\\
In several scientific problems, especially in mathematical finance, one is typically interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$; both of which have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0,T]},\mathbb{P})$.  For example, market sentiment impacts market prices, however, only the latter of these two can be reliably measured.  
% Filtering
% Consequentially, an accurate estimation of the unobservable signal process implies reliable forecasts of all affected quantities.  The objective of the \textit{stochastic filtering problem}, is to recursively estimate the conditional law of the unobserved signal process $X_{\cdot}$, at any time given $t>0$, given the information contained in the $\sigma$-algebra generated by the observation process $Y_{\cdot}$ up to time $t$.
% Robust Filtering
The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is for any time $t>0$ to identify a continuous function $f_t:C([0,t],\mathbb{R}^d)\rightarrow \mathcal{P}(\mathbb{R}^D)$ satisfying 
\begin{align}
    \label{goal:Robust_Filtering}
        f_t(y_{[0:t]})
    =
        \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)%y_{[0:t]})
    ,
\end{align}
conditioned on any continuous path $y_{[0:t]}$ realized the $d$-dimensional observable process $Y_{\cdot}$ up time $t>0$; where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $D$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0,t]}$.  The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^D$, denoted by $\mathcal{P}(\mathbb{R}^D)$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^d$, denoted by $C([0,t],\mathbb{R}^d)$, with the uniform norm. 

\byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^d)$.  These robust representations are particularly 
% day2016deep,mishev2020evaluation
% Filtering problems, integral to the realm of stochastic systems, involve the challenging task of estimating the state of a dynamic system from observations contaminated by noise. These problems find widespread applications in diverse domains such as finance, control systems, and environmental monitoring, where accurate state estimation is paramount. At the heart of the filtering paradigm lies the concept of filter distribution—the conditional distribution describing the state of a stochastic system conditional on the noisy observations up to a given time. In this work, we demonstrate that in the case of a continuous-time conditionally Gaussian filter, this filtering distribution can be approximated universally by a transformer-like machine learning model uniformly in time.
% \medskip
% \byyan{Kalman filters.} \hfill\\
% The simplest form of a conditionally Gaussian filter is the well-known Kalman-Bucy filter, which is the case when the underlying system follows linear dynamics, observations are linear, and noise terms are Gaussian. Rudolf Kalman's work introduced the discrete-time Kalman filter \cite{Kalman60}, which later found a continuous-time counterpart in \cite{KalmanBucy61}. These filters provide finite-dimensional representations of the filter distribution, summarizing the first two conditional moments of the system's state based on observations. In the linear Gaussian scenario, the filter distribution is fully characterized by these first two moments, specifically, the mean vector and variance-covariance matrix of the resulting Gaussian distribution. The Kalman filter's elegance and utility have made it a staple in various fields, particularly when dealing with linear dynamics and Gaussian noise assumptions.
% Stochastic filters have proven to be 
invaluable in mathematical finance where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

\byyan{Do Optimal Filters Exist?.}\hfill\\
In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,Sirjaev1965Filtering,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued processes, make the problem computationally intractable.  

\byyan{Computational Challenges}\hfill\\
The exception to this rule is so-called finite-dimensional filters, which are rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

\byyan{Numerical Approaches.}\hfill\\
The intractability of the computational general filtering problem has the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} when it admits a square-integrable density.  The latter two instances work well if the coupled system $(X_{\cdot},Y_{\cdot})$ genuinely follows the postulated dynamics, and the former particle-filtering approach is effective for low-dimensional state space systems.  

\byyan{Why Deep Learning?.}\hfill\\
The ability of deep neural networks to efficiently solve a variety of problems has inspired the use of deep learning approaches to the numerical stochastic filtering problem; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering}, and example of deep neural network approximations to measure-valued processes; e.g.~\cite{Acciaio2022_GHT}.  In particular, the need for a more generic approximate stochastic filtering toolbox has motivated the deep learning community to introduce deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, which is the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered model, are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem.  

This paper confirms the ability of deep Kalman filters to map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering} for any pair of $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0,T]}$-adapted processes governed by the coupled dynamics
\begin{align}
\label{eq:filtering_dynamics__signal}
% \tag{Sig}
dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
\label{eq:filtering_dynamics__observation}
% \tag{Obs}
dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
\end{align}
where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$, of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  


% HERE!

% \begin{enumerate}
%     \item Optimal investment under partial information \cite{lakner1998optimal,BjorkDavis}
%     \item \textit{Volatility Estimation from Intra-day Stock Prices.}
%    \cite{Barndorff-NielsenShephard02} introduced the use of Kalman filters to estimate underlying volatility from observed intra-day stock prices. Volatility estimation is crucial in risk management, options pricing, and trading strategy development. By incorporating high-frequency price data into the Kalman filter framework, this approach provides more accurate and timely volatility estimates, enhancing decision-making in financial markets.
%    \item \textit{Fixed Income and Interest Rate Estimation Modeling} 
%    \cite{chen1993maximum,duan1999estimating}
%    \textit{Instantaneous Interest Rate Estimation from Bond Yields.}
%    Further research, including \cite{BabbsNowman99}, have applied Kalman filters to estimate underlying instantaneous interest rates, also known as short rates, from observed bond yields. This estimation is fundamental in fixed income markets, aiding in bond pricing, yield curve modelling, and interest rate risk analysis. The Kalman filter's ability to handle noisy and irregularly sampled bond yield data makes it an ideal choice for this application.
%    \item \textit{Spot Price Estimation from Futures Prices for Commodities.} Approaches as for instance \cite{Schwartz97}, \cite{ManoliuTompaidis02}, and \cite{LautierGalli04} employ Kalman filters to tackle this problem. By modelling the relationship between spot and futures prices, Kalman filters provide a dynamic framework for spot price estimation, allowing market participants to make informed decisions.
%    \item \textit{Estimation of Latent Factors Affecting Pricing.}
%    Kalman filters are also utilized to estimate latent factors that influence asset pricing, e.g.\ in commodity market model \cite{schwartz1997stochastic,schwartz2000short,Cody2007parameter}, energy future pricing \cite{manoliu2002energy}, and . These factors could include macroeconomic variables, market sentiment, or other unobservable drivers. By integrating observed asset prices and a dynamic state-space model, researchers can extract these latent factors, enhancing our understanding of market dynamics and improving pricing models.
%    \item \textit{Updating Estimates of Uncertain Drift Parameters.}
%    In the context of hedging strategies in incomplete markets, as explored by \cite{Monoyios07}, Kalman filters are employed to update estimates of uncertain drift parameters in the price process. This adaptation allows market participants to dynamically manage risk by adjusting their hedging positions as market conditions evolve.
%    \item Books \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear}
% \end{enumerate}


% In these financial applications, the Kalman filter's adaptability to handle noisy, irregular, and dynamic data has proven to be a significant advantage. Its ability to estimate unobservable variables, track market dynamics, and improve the precision of financial models has made it a staple tool in quantitative finance. However, it's important to acknowledge that the financial markets often present challenges that extend beyond the simplistic filtering dynamics of the Kalman-Bucy filter.

\byyan{Applications outside of Finance (high-level).}
The Kalman filter's versatility and effectiveness in dealing with linear dynamics and Gaussian noise assumptions have also led to its widespread use across various fields outside of finance: In aerospace and navigation, it plays a pivotal role in spacecraft navigation and autonomous vehicle positioning, providing accurate state estimates despite inherent uncertainties. In geophysics and seismology, it contributes to ground motion and structural response monitoring during seismic events, enhancing early warning systems and structural health assessments. Control engineering relies on the Kalman filter for state estimation in feedback control systems, benefiting industries such as manufacturing, robotics, and aerospace, where precise control is essential. In the realm of medical imaging, it improves image quality by reducing noise, leading to advancements in disease diagnosis and treatment planning. Environmental monitoring applications leverage the Kalman filter to estimate and predict environmental parameters, including pollutant concentrations, weather conditions, and ocean currents, supporting climate studies and disaster management. Additionally, robotics equipped with sensors use the Kalman filter to estimate their positions and orientations in unfamiliar environments.

\medskip
\byyan{More complex conditionally Gaussian filters.}
Many real-world situations deviate from these idealized assumptions, featuring nonlinear or non-Markovian dynamics. In such cases, the simplicity of the Bucy-Kalman filter may not suffice, prompting the need for more sophisticated filtering methods.

\yannick{Generalizations include
\begin{itemize}
    \item Non-linear, non-Markovian signal dynamics
    \item Non-linear, non-Markovian dependence of hidden state on signal dynamics
    \item Opening the door for learning procedures, where dynamics are (mostly model-freely) learned from data
\end{itemize}
}
    


\paragraph{The main result in this paper}

\paragraph{Structure of the article}

~\\ 
\bigskip

Literature surrounding applications of filtering in Mathematical Finance: \\
For a general motivation for the geometric (also: information geometric) idea behind Filtering problems in typical applications in mathematical finance, see the excellent overview presented in the the recent work \href{https://arxiv.org/pdf/2205.01594.pdf}{Brigo (2022)} and the expose in \href{https://arxiv.org/pdf/1303.6236.pdf}{Armstrong and Brigo (2013)} as well as well-known early works \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}. A gentle introduction to typical linear and nonlinear filtering problems in mathamatical finance can be found in the review article \href{ura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{Date and Ponomareva (2010)} and for a comprehensive introduction to stochastic filtering we direct to the eteemed monograph \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)} as the reference literature.\\


\anastasis{I would mention that there are at-least two sources of ``complexity'' to the general filtering problem: 1) The infinite-dimensionality of the set of all probability measures (complexity of representing conditional densities/measures) and 2) The complexity of the dynamics governing the solution of the signal, observation, and conditional dynamics.  \\
I would then say some like Kalman filters simplify both, the general conditional Gaussian filters studied in \cite{LipShiryaev_II_2001} provide a theoretical foundations for filtering when (1) is resolved by considering conditionally Gaussian filters.  Then somehow relate that we work in (1), by developing a universal model class, in the conditionally-Gaussian framework based on the ideas of deep Kalman filtering.}

\paragraph{Historical development:} 
The filtering problem consists in estimating the state of a stochastic differential system
from noisy observations. \\ 
The general solution of the filtering problem at a given time is given by the probability density
of the unperturbed state of the system at that time, conditional on the perturbed observations
up to the given time. When the unobserved signal and the observed signal evolve in continuous
time, the filter density follows a stochastic partial differential equation (SPDE), see \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)}. 
If the dynamic evolution of the unobserved
system is linear, the observations are linear, the noise terms are Gaussian\footnote{The initial condition of the
unperturbed signal are also assumed to be Gaussian or deterministic.}, then this is a setting that leads to the celebrated \emph{Kalman-Bucy filter}:
\\
Indeed, in the linear Gaussian case the problem was solved in discrete-time by Rudolf Kalman, and later in continuous time in \cite{TBD}\anastasis{(Bucy Paper)},
who introduced what is known today as the \emph{Kalman filter} (see next paragraph), a finite dimensional system of equations
for the first two conditional moments of the state of the stochastic system, given the observations:
In such a case, the filter is Gaussian and its density can
be characterized by a finite dimensional set of parameters, namely the mean vector and variance-covariance matrix of the resulting Gaussian distribution,
%\\In classical Kalman Filters, the evolution of this system (both observable and unobservable parts) are modelled as linear functions
%perturbed by Gaussian noise.
%In a linear setting 
these equations determine the whole conditional density of the state of the system given the observations,
as this (Gaussian) density is fully characterized by the first two moments. \\
 For real world applications the assumption of a linear evolution of this system\footnote{I.e. transition and emission distributions.}
limits the capacity to model complex phenomena, and modifications to the functional form of Kalman Filters
have been proposed.
\\
As indicated above, 
in the  general nonlinear case, the filtering problem is far more complex as it consists in computing the conditional density of the
state given the observations. This density is the solution of a stochastic partial differential
equation which is referred to as the \emph{Kushner-Stratonovich equation} and the resulting nonlinear filter is in general not finite dimensional\footnote{I.e. it does not evolve in a finite dimensional
statistical manifold.}. A well
known approximation method is the extended Kalman filter (EKF), in which one linearizes around
the current estimate obtaining a locally linear system, and then applies the Kalman filter
equations in this (linearised) neighbourhood. Traditionally, this procedure was usually justified by heuristic considerations.  
Though more recent linear approximations have also been considered, e.g.\ in \cite{LukasJosef_LinearizedFiltering}.
Another choice in the nonlinear case is the Gaussian assumed density filter (GADF),
obtained by assuming the conditional density to be Gaussian\footnote{This is dangerous, because by assuming a false hypothesis one can deduce anything as well as its opposite.}, which yields a finite dimensional filter. %However, this approach depends heavily on conditional Gaussianity, which is not necessarily fulfilled in many real-life applications.\\
We are universal in the conditional Gaussian class.\\
Contrast it with neural SDEs (no hidden suff (ANASTASISSSS)

Hanzon suggested to project the SPDE equation in Stratonovich form for the evolution of the filter density onto a finite dimensional statistical manifold, using the Fisher metric/Hellinger distance. We call this “Stratonovich projection” and it consists in projecting the separate vector
fields of the SPDE corresponding to the drift and diffusion part of the Stratonovich version. The projected equation would describe a finite dimensional density evolution, called projection filter, approximating the full filter evolution associated with the optimal filter.\\
In 1987, Hanzon (BH: reference missing) introduced the projection filter (PF), which is a finite dimensional nonlinear filter based on a differential geometric approach: The projection filter is obtained by projecting the Kushner-Stratonovich equation onto the tangent space
of a finite dimensional manifold of probability densities, according to the Fisher information metric.\\
Hanzon and Hut (1991) (BH: add ref) showed that if one projects onto the
tangent space of the finite dimensional manifold of Gaussian densities, the resulting projection filter
coincides with an assumed density filter which is obtained as follows: one computes the first two conditional moments equations in McShane-Fisk-Stratonovich (MFS) form, and then assumes the conditional density to be Gaussian, closing in this way the equations for the first two moments.   
It was also proven in Hanzon and Hut (1991) that what we described above is in general not the same as assuming a Gaussian density in the It\^{o} equations for the first two moments and then transforming the obtained filter in MFS form.
The equivalence between the MFS-based GADF and the Gaussian Projection Filter is very important when generalized to
exponential families (see \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}), because it gives a simple characterization of the exponential projection
filter (EPF) which is independent of geometric concepts. \\

For a comprehensive but introductory review of linear and non-linear filterin applications in mathematical finance see: \href{https://bura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{P. Date and K. Ponomareva (2010)} among which we will highlight some simple but heavily used (Gaussian or near-Gaussian) use cases
\begin{itemize}
    \item In stochatic volatility modelling Kalman Filters have traditionally been used to estimate (and forecast) spot and realised volatility.
    \item Monoyios in \href{https://people.maths.ox.ac.uk/monoyios/docs/ima_final.pdf}{Monoyios (2007)} develops a filtering approach with applications to (optimal) hedging, in which the hedger updates her parameter estimates from
observations of the asset prices, and where he finds an analytic solution to the hedger’s combined filtering and
control problem in the case that the drift of the traded asset is known with certainty.
\item Filtering has been traditionally heavily used in linear Gaussian interest rate models. 
    \end{itemize}
    

\paragraph{Kalman filters} At a high level, a Kalman filter operates by combining a model of a system with partial state-observations to estimate the current overall state of the system. The filter uses two primary steps to make these estimates: a prediction step and an update step.
\begin{itemize}
    \item In the prediction step, the Kalman filter uses the model of the system to predict the state of the system at the next time step. This prediction is based on the current estimate of the system state, as well as any known inputs or disturbances in the system. The Kalman filter uses a probabilistic approach to estimate the state of the system, this means the prediction includes both the expected value of the state as well as an estimate of the uncertainty or error in the prediction.
    \item In the update step, the Kalman filter uses the actual observation to correct the predicted state estimate. The filter compares the distribution of the predicted state to the actual observed state (which acknowledges uncertainty and is perceived as a distribution itself). The filter then adjusts the state estimate based on this difference.
\end{itemize}

\paragraph{Deep Kalman filters} The term, ``deep Kalman filter'' (DKF) refers to deep learning models, that bolster the capacity of traditional Kalman filter by leveraging a neural network component. The neural network component is used to learn the probabilistic model of the underlying system dynamics, thus allowing DKFs to generically adapt to any situation in which the conditional evolution of the signal process is Gaussian.  This generic flexibility, of DKFs is what has lead to their empirical predictive edge over traditional Kalman filters \cite{TBD}.

The neural network component in a DKF is typically used to model the transition function of the system, which describes how the state of the system evolves over time. The neural network takes as input the current state of the system, as well as any control inputs or disturbances, and outputs a probability distribution over the possible next states of the system. This distribution is then used to make a prediction of the next state, as well as an estimate of the uncertainty or error in the prediction. 

The traditional Kalman filter components are then used to combine the neural network predictions with actual observations in order to update the state estimate. The neural network component in a DKF can be trained using a variety of techniques, such as maximum likelihood or Bayesian inference. The training process involves minimizing the error between the predicted state and the actual state, as well as minimizing the uncertainty in the predictions.

\paragraph{Exemplary (existing) applications of (D)KF in finance}
\begin{enumerate}
    \item Sequential calibration of options
    \begin{itemize}
        \item Problem: The parameter estimates are noisy and old data are typically discarded, as only the most recent data are used.
        \item As a solution, the calibration is formulated as a filtering problem.
        \item The observable process consists of market option prices, spot, strike, interest, and maturity.
        \item The unobservable process consists of the difference between the modelled option price and the denoted option price, as well as the difference of the model's parameters to the day before.
        \item See \cite{LindstroemStroejbyBrodenWiktorssonHolst08}, extensions \cite{LindstroemWiktorsson14}
    \end{itemize}
    \item Computing VaR in a stochastic volatility model, see \cite{LindstroemMadsenNielsen16}
    \item Filtering with bond prices, see \cite{LindstroemMadsenNielsen16}
    \begin{itemize}
        \item The observable process constitutes the prices obtained from solving the ``bond pricing equation''
        \item The unobservable variables are the parameters of the estimated model and the implied interest rate (by bond prices, not quoted)
    \end{itemize}
    \item Calibration of term structure models of commodity prices \cite{JavaheriLautierGalli03}
    \item Dynamic pricing (this is probably more economics than finance), see \cite{CohenTreetanthiploet22}
    \item Besides state estimation in control systems, Kalman filters have found applications in financial markets for constructing trading strategies. Two common approaches involve using Kalman filters to:
    \begin{itemize}
        \item Identify Mean-Reverting Patterns: Kalman filters can be utilized to detect instances where asset prices deviate from their long-term average, indicating potential mean-reverting behaviour. Traders can then develop strategies that take advantage of these deviations, expecting prices to eventually return to their mean.
        \item Identify Momentum-Based Trends: Kalman filters can also be employed to identify momentum-based trends in asset prices, indicating sustained movements in a particular direction. Traders can develop strategies to follow and capitalize on these trends.
        \item \yannick{References missing.}
    \end{itemize}
    \item Portfolio Optimization with Kalman Filters and Multi-Asset Models:
    \begin{itemize}
        \item Kalman filters applied to optimize asset portfolios by considering individual asset dynamics and correlations.
        \item Particularly beneficial for multi-asset portfolios.
        \item Estimation of assets' covariance matrix using Kalman filters.
        \item Portfolio optimization based on the covariance matrix while adhering to specified constraints.
        \item \yannick{References missing.}
    \end{itemize}
    \item  Risk Management and Stress Testing with Kalman Filters:
    \begin{itemize}
        \item Utilization of Kalman filters for risk management and stress testing purposes.
        \item Estimation of portfolio risk and identification of potential risk sources.
        \item Modelling asset behaviour under various market scenarios using Kalman filters.
        \item Assessment of the portfolio's vulnerability to the impact of these scenarios.
        \item \yannick{References missing.}
    \end{itemize}
\end{enumerate}


\begin{comment}
\paragraph{Limitations and contribution} The results \cite{kratsios2021universal, Acciaio2022_GHT} show that, while it is possible to universally approximate the function used above with a class of transformer models, the required number of parameters to approximate the function at each state in time can depend highly non-favourably on the dimensions of the (observable and unobservable) state. In this work, we suggest to best approximate the function at all times by a class of non-Euclidean kernel regressors, trained on a finite set of observations. 
\end{comment}

==> OLD/Historical_Versions/Sections/Practical_Approach.tex <==
\subsection{Practical approach with known dynamics}
Our objective is to lean the conditional distribution of a process $(X_n)_{n=0}^{\infty}$ given noisy measurements in another stochastic process $(Y_n)_{n=0}^{\infty}$, without assuming we know how these processes evolve, and only assuming some ``basic structural conditions''.  


Fix continuous functions $a_0,a_1,b_0$ which continuously mapping $\mathbb{R}^{1+d}$ to $\mathbb{R}^d$.  
\begin{example}
$\alpha_i(t,x)\eqdef \cos(x)$ and $b_0(t,x)=1$.
\end{example}
These functions define the evolution of the stochastic process $X_{\cdot}\eqdef (X_t)_{t=0}^{\infty}$ whose conditional distribution which we are interested in predicting
\begin{align}
\label{eq:filtering_dynamics__signal___discrete}
X_{t+1} & = [a_0(t,Y_t) + a_1(t,Y_{t}) X_t]\Delta + b_0(t,Y_{t})\sqrt{\Delta}\,W_t,
\end{align}
where $X_0=0$, $W_0,\dots,W_T$ are i.i.d.\ standard normal random variables, $\Delta>0$ is some hyperparameter, and $Y_{\cdot}\eqdef (Y_t)_{t=0}^{\infty}$ is a sequence of noisy measurements from $X_{\cdot}$.  These noisy measurements are defined iteratively by
\begin{align}
\label{eq:filtering_dynamics__observation___discrete}
Y_{t+1}  = [A_0(t,Y_t) + A_1(t,Y_t) X_t]\Delta + B_0(t,Y_t)\sqrt{\Delta}Z_t
,
\end{align}
where $Y_0$ is fixed, $a_0,a_1,b_0$ are continuously mapping $\mathbb{R}^{1+d}$ to $\mathbb{R}^d$, and $Z_0,\dots,Z_T$ are i.i.d.\ standard normal random variables which are also independent of $W_0,\dots,W_T$.

Our deep Kalman filter operates in three phases.  First, it encodes a realized time-series, up to the current point in time $T$, into an ${F+M}$-dimensional feature vector
\[
    \operatorname{attention}_t:(y_0,\dots,y_T) 
        \mapsto 
        \biggl(
            \frac1{T_F}
            \,
            \sum_{i=0}^{T_F-1}\,
                y_{jT_F + i}
        \biggr)_{j=0}^{F-1}
        \oplus
        (y_{T-M},\dots,y_T)
    ,
\]
where $T_F=\lfloor \frac{T-M}{F} \rfloor$, the parameters $T,M$ are positive integers, and $\oplus$ denotes the $np.append$ operation.  The last $M$ features generated by $\operatorname{attention}_T$ exactly reproduce the ``recent'' time-series, and the first $F$ features pool the time series' ``distant past''.

The next portion of the learning model produces an adaptive low-dimensional feature representation using a geometric deep neural network (GDN) of \cite{kratsios2022universal}.  This map is given by
\[
        f_{\theta}(u) 
    \eqdef 
        \rho(\operatorname{MLP}(u))
\]
where $\operatorname{MLP}$ is an standard feedforward neural network mapping inputs in $\mathbb{R}^{F+M}$ to outputs in $\mathbb{R}^{\byyan{d}(d+3)/2}$.  The decoder layer $\rho$ sends any real vector $(u_1,\dots,u_{\byyan{d}(d+3)/2})$ to the pair of a $d$-dimensional vector $\mu$ and a $d\times d$ non-singular covariant matrix $\Sigma$ via
\begin{align}
        (\mu,\Sigma)\eqdef 
        \Big(
            \begin{pmatrix}
                u_1 \\
                \vdots \\
                u_d
                \end{pmatrix}
        ,
            \operatorname{exp}\left(
                \begin{pmatrix}
                u_{d+1} & u_{d+2} & \dots & u_{\byyan{d(d+1)/2+1}} \\
                u_{d+2} & u_{d+3} & \dots & u_{\byyan{d(d+1)/2+2}} \\
                \vdots & \vdots& \ddots & \vdots \\
                u_{\byyan{d(d+1)/2+1}} & u_{\byyan{d(d+1)/2+2}} & \dots & u_{\byyan{d}(d+3)/2}
                \end{pmatrix}
            \right)
        \Big) \label{id:Encoding}
\end{align}


\begin{algorithm}[H]
\caption{Generate Time Series}
\label{alg:GenerateTimeSeries}
\SetAlgoLined
\KwIn{Initial values $Y_0$, $X_0$; standard normal samples $(Z_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$, $(W_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$}
\KwOut{Time series realizations $(X_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$, $(Y_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$}
\DontPrintSemicolon
\For{$t=0,\dots,T-1$}{
    \For{$k=1,\dots,K$}{
        $Y_{t+1}^{(k)}  \leftarrow [A_0(t-1,Y_t^{(k)}) + A_1(t,Y_t^{(k)}) X_t^{(k)}]\Delta + B_0(t,Y_t^{(k)})\sqrt{\Delta}Z_t^{(k)}$ \\
        $X_{t+1}^{(k)} \leftarrow [a_0(t,Y_t^{(k)}) + a_1(t,Y_t^{(k)}) X_t^{(k)}]\Delta + b_0(t,Y_t^{(k)})\sqrt{\Delta}\,W_t^{(k)}$
    }
}
\end{algorithm} 

\begin{algorithm}[H]
\caption{Generate Labels}
\label{alg:GenerateLables}
\SetAlgoLined
\KwIn{Time series realizations $(X_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$, $(Y_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$}
\KwOut{Estimated distributions of unobservable state $(\hat{\Sigma}_{t+1}^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$, $(\hat{\mu}_{t+1}^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$}
\DontPrintSemicolon
\For{$t=0,\dots,T-1$}{
    \For{$k=1,\dots,K$}{
            $\boldsymbol{X}_{t+1}^{(k)}=\{\,\}$\;
            \For{$n=1,\dots,N$}{
                $
                    \boldsymbol{X}_{t+1}^{(k)}\leftarrow \operatorname{APPEND}\left(\boldsymbol{X}_{t+1}^{(k)}
                    ,
                        \mathcal{N}\Big(
                            X_{t}^{(k)} 
                            +
                            [a_0(t,Y_t^{(k)}) + a_1(t,Y_{t}^{(k)}) X_t^{(k)}]\Delta,
                            \byyan{b_0(t,Y_t^{(k)}) \sqrt{\Delta}}
                        \Big)
                    \right)
                $
                \tcp*{$\mathcal{N}(\mu, \Sigma)$ generates normally distributed samples with mean $\mu$ and covariance matrix $\Sigma$}
            }
        $\hat{\mu}_{t+1}^{(k)} \leftarrow \operatorname{Mean}(\boldsymbol{X}_{t+1}^{(k)})$ \;
        $\hat{\Sigma}_{t+1}^{(k)} \leftarrow \operatorname{Cov}(\boldsymbol{X}_{t+1}^{(k)})$ \;
    }
}
\end{algorithm} 

\begin{algorithm}[H]
\caption{Train MLP}
\label{alg:TrainMLP}
\SetAlgoLined
\KwIn{Observations $(Y_t^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$; Lables $(\hat{\Sigma}_{t+1}^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$, $(\hat{\mu}_{t+1}^{(k)})_{t = 0, ..., T-1; k = 1, ..., K}$}
\KwOut{}
\DontPrintSemicolon
\For{$t=0,\dots,T-1$}{
    \For{$k=1,\dots,K$}{
        $\operatorname{attention}_t^k \leftarrow \operatorname{attention}_t(\byyan{(Y_{0}^{(k)}, ..., Y_{t+1}^{(k)})})$ \;
        $\hat{u}_{t+1}^{(k)} \leftarrow (\hat{\mu}_{t+1}^{(k)},\operatorname{logm}(\hat{\Sigma}_{t+1}^{(k)}))$ \;
        \tcp*{$\operatorname{logm}$ is the decoding of \eqref{id:Encoding}}
    }
}
    $
    \operatorname{MLP} \leftarrow \operatorname{argmin}\,
        \sum_{t,k}\,
        \|
            \operatorname{MLP}(\operatorname{attention}_t^k) - \hat{u}_{t+1}^{(k)}
        \|_2^2
    $
\end{algorithm} 


\newpage
\subsection{Unknown dynamics}

In the pursuit of refining our understanding of sequential observations, this section aims to establish an appropriate filtering setup. The primary objective is to effectively fit the filtering setup to a given sequence of observations, allowing us to infer meaningful insights from the data. Accomplishing this entails the integration of two fundamental components: a generative model characterizing the observable process and the formulation of the law governing the signal process conditional on the realizations of the observable process. To achieve our goal, we adopt a principled approach by stipulating priors for both the generative model and the conditional distribution. These priors serve as our initial beliefs about the underlying processes before observing any data. After each new observation, we update the both components to maximize the likelihood of the observation under the prevailing filtering setup.


Specify time steps $0 = t_0 < t_1 < \ldots < t_N = T$ for some $N \in \N$. The Kalman filter is defined via
\begin{align*}
        X_{t_n} \vert y_{[t_0:t_n]}
    &\sim
        \mathcal{N}\left(f_\theta(y_{[t_0:t_n]})\right)
    \\
        Y_{t_n} \vert x_{t_n}, y_{[t_0:t_{n-1}]} 
    &\sim
        \mathcal{N}\left(a_\iota(y_{[t_0:t_{n-1}]}) + x_{t_n} b_\kappa(y_{[t_0:t_{n-1}]}), c_\eta(y_{[t_0:t_{n-1}]})\right),
\end{align*}
whereat $f_\theta$ is defined as in \Cref{eq:featuremap} and $a_\iota, b_\kappa, c\eta$ are MLPs, each defined via the corresponding parameters, and we write $\phi \eqdef \lbrace \theta, \iota, \kappa, \eta \rbrace$. 


Then, by an application of the Bayes formula, we obtain the lower bound on the likelihood of a realization $y \in XXX$
\begin{align*}
        \log p_\phi(y_{[t_0:t_n]}) 
    & =  \log \mathbb{E}\left[
            p_\phi\left(
                y_{[t_0:t_n]}
            \mid
                X_{[t_0:t_n]} 
            \right)
        \right] 
    \geq 
        \sum_{n=1}^N
            \mathbb{E}\left[
                \log p_\phi\left(
                    y_{t_n}
                \mid
                    (X_{t_n} \vert y_{[t_0:t_n]})
                \right)
            \right] 
    \eqdef
        \mathcal{L}(y, \phi),
\end{align*}
where we used the factorization of the likelihood 
\begin{align*}
        p_\phi\left(
            y_{[t_0:t_n]}
        \mid
            (X_{[t_0:t_n]} \vert y_{[t_0:t_n]})
        \right) 
    = 
        \prod_{n = 1}^N
            p_\phi\left(
                y_{t_n}
            \mid
                (X_{t_n} \vert y_{[t_0:t_n]})
            \right)
\end{align*}
together with Jensen's inequality.



\yannick{We write a training algorithm where we can produce arbitrary many realizations of $Y$}

\yannick{Is the above true? In particular 
\begin{align*}
        \log p_\phi(y) 
    & =  \log \mathbb{E}\left[
            p_\phi\left(
                y
            \mid
                (X \vert y)
            \right)
        \right] ?
\end{align*}}


==> OLD/Main_AAP.tex <==
% % \documentclass[aap]{imsart}
% % Theorems with 
% % \theoremstyle{plain}
% \documentclass[twoside,11pt]{article}


% % Any additional packages needed should be included after jmlr2e.
% % Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% % and defines many common macros, such as 'proof' and 'example'.
% %
% % It also sets the bibliographystyle to plainnat; for more information on
% % natbib citation styles, see the natbib documentation, a copy of which
% % is archived at http://www.jmlr.org/format/natbib.pdf

% % Available options for package jmlr2e are:
% %
% %   - abbrvbib : use abbrvnat for the bibliography style
% %   - nohyperref : do not load the hyperref package
% %   - preprint : remove JMLR specific information from the template,
% %         useful for example for posting to preprint servers.
% %
% % Example of using the package with custom options:
% %
% % \usepackage[abbrvbib, preprint]{jmlr2e}
% \usepackage[abbrvbib, preprint]{jmlr2e}

% % \documentclass[aap]{imsart}

% %% Packages
% % \RequirePackage{amsmath,amsfonts,amssymb}
% % \usepackage{amsthm}
% % \RequirePackage[numbers,sort&compress]{natbib}
% %\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
% % \RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
% % \RequirePackage{graphicx}

% % \startlocaldefs

% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% % \documentclass[preprint,12pt,authoryear]{elsarticle}
% % \usepackage{amssymb}
% % \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}

% % Springer
% % \raggedbottom
% % \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% % \setlength\heavyrulewidth{0.3ex}
% % \usepackage{lscape}


% \ShortHeadings{Deep Kalman Filters Can Filter:
% Universality in the class of non-Markovian Conditionally Gaussian Filters}{Hovarth, Kratsios, Limmer, and Yang}

% \begin{document}



% % AAP
% % \begin{frontmatter}
% \title{Deep Kalman Filters Can Filter:
% Approximation Guarantees for Non-Markovian Conditionally Gaussian Filters}


% \author{\name Blanka Horvath \email horvath@maths.ox.ac.uk \\
%         \addr Department of Mathematics, University of Oxford\\
%         Oxford-Man Institute for Quantitative Finance
%         \AND
%         \name Anastasis Kratsios\email kratsioa@mcmaster.ca \\
%         \addr Department of Mathematics, McMaster University \\
%         Vector Institute
%         \AND
%         \name Yannick Limmer \email limmery@maths.ox.ac.uk \\
%         \addr Department of Mathematics, University of Oxford\\
%         Oxford-Man Institute for Quantitative Finance
%         \AND    
%         \name Xuwei Yang \email yangx212@mcmaster.ca\\
%         \addr Department of Mathematics, McMaster University}

% % \editor{TBD}

% \maketitle

% % \begin{aug}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %% Only one address is permitted per author. %%
% % %% Only division, organization and e-mail is %%
% % %% included in the address.                  %%
% % %% Additional information can be included in %%
% % %% the Acknowledgments section if necessary. %%
% % %% ORCID can be inserted by command:         %%
% % %% \orcid{0000-0000-0000-0000}               %%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % \author[inst1]{Matheus Grasselli}
% % \author[A,D]{\fnms{Blanka}~\snm{Hovarth}\ead[label=e1]{horvath@maths.ox.ac.uk}},
% % \author[B,C]{\fnms{Anastasis}~\snm{Kratsios}\ead[label=e2]{kratsioa@mcmaster.ca}},%\orcid{0000-0000-0000-0000}}
% % \author[A,D]{\fnms{Yannick}~\snm{Limmer}\ead[label=e3]{limmery@maths.ox.ac.uk}},
% % \author[B]{\fnms{Xuwei}~\snm{Yang}\ead[label=e4]{yangx212@mcmaster.ca}}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %% Addresses                                %%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \address[A]{Department of Mathematics,
% % University of Oxford \printead[presep={,\ }]{e1}\printead[presep={,\ }]{e3}}
% % \address[D]{Oxford Man Institute for Quantitative Finance, University of Oxford}
% % \address[B]{Department of Mathematics,
% % McMaster University\printead[presep={,\ }]{e2}\printead[presep={,\ }]{e4}}
% % \address[C]{Vector Institute}
% % % Elseview
% % % \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
% % %             % addressline={Hamilton, Ontario}, 
% % %             city={Hamilton},
% % %             % postcode={00000}, 
% % %             % state={Ontario},
% % %             country={Canada}}

% % % \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
% % %             % addressline={Address Two}, 
% % %             city={Oxford},
% % %             % postcode={22222}, 
% % %             % state={Oxfordshire},
% % %             country={United Kingdom}}

% % % \affiliation[inst3]{organization={Oxford-MAN Instute for Quantitative Finance, University of Oxford},
% % %             % addressline={Address Two}, 
% % %             city={Oxford},
% % %             % postcode={22222}, 
% % %             % state={Oxfordshire},
% % %             country={United Kingdom}}
            
% % % \affiliation[inst4]{organization={Vector Institute},
% % %             % addressline={Address Two}, 
% % %             city={Toronto},
% % %             % postcode={22222}, 
% % %             % state={Ontario},
% % %             country={Canada}}
% % \end{aug}

% \begin{abstract}
% Deep Kalman filters (DKFs) are a class of neural network models that generate conditionally Gaussian outputs from sequential data, inspired by the Kalman filter.  Though DKFs have seen significant success in Bayesian deep learning, they still lack concrete theoretical ties to the stochastic filtering problem, limiting their sound applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-time measurements.  Our approximation guarantees hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case $2$-Wasserstein distance computed uniformly over the given compact set of paths.  
% \end{abstract}


% % \begin{keyword}
% % %% keywords here, in the form: keyword \sep keyword
% % Stochastic Filtering \sep Conditionally Gaussian Processes \sep Geometric Deep Learning
% % %% PACS codes here, in the form: \PACS code \sep code
% % % \PACS 0000 \sep 1111
% % %% MSC codes here, in the form: \MSC code \sep code
% % %% or \MSC[2008] code \sep code (2000 is the default)
% % \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% % \end{keyword}

% % \begin{keyword}[class=MSC]
% % \kwd[Primary ]{62M20}
% % \kwd{62M45}
% % \kwd[; secondary ]{93E11}
% % \end{keyword}

% % \begin{keyword}
% % \kwd{Robust Filtering}
% % \kwd{Deep Kalman Filtering}
% % \kwd{Partial Information}
% % \end{keyword}

% % \end{frontmatter}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Please use \tableofcontents for articles %%
% %% with 50 pages and more                   %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\tableofcontents
% % \end{frontmatter}
% % \hbadness=10000

% \section{Introduction}
% \label{s:Introduction_Deep_Filtering}

% % \byyan{Opening.}\hfill\\
% In several scientific problems, e.g. in mathematical finance, one is interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$. Here both of the processes are often assumed to have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0:T]},\mathbb{P})$.  For example, market sentiment(signal) impacts market prices(observations), however, only the latter of these two can be directly measured.  The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is to identify a continuous function $f_t:C([0:t],\mathbb{R}^{d_Y})\rightarrow \mathcal{P}(\mathbb{R}^{d_X})$, with $d_X, d_Y \in \N$ for $t>0$, satisfying 
% \begin{align}
%     \label{goal:Robust_Filtering}
%         f_t(Y_{[0:t]})
%     =
%         \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)
%     ,
% \end{align}
% where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $d_X$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0:t]}$. The key innovation in \eqref{goal:Robust_Filtering} is the continuity, and the uniqueness, of $f_t$.  In contrast, a Borel $f_t$ satisfying \eqref{goal:Robust_Filtering} exists by elementary measure-theoretic \citep[Theorem 6.3]{Kallenberg_2021__FoundationsOfModernProbability}. 
% The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^{d_X}$, denoted by $\mathcal{P}(\mathbb{R}^{d_X})$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^{d_Y}$, denoted by $C([0:t],\mathbb{R}^{d_Y})$, with the uniform norm.

% % \byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
% When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^{d_Y})$.  These robust representations are particularly invaluable in mathematical finance, where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

% % \byyan{Do Optimal Filters Exist?.}\hfill\\
% In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued path-dependent processes, make the problem computationally intractable. 

% % \byyan{Computational Challenges}\hfill\\
% The exception to this rule is so-called finite-dimensional filters. These encapsulate rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

% % \byyan{Numerical Approaches.}\hfill\\
% The computational intractability of the general filtering problem leads to the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} where it can be tracked using finitely parameterized representations.  The latter two approaches work well if the coupled system $(X_{\cdot},Y_{\cdot})$ follows the postulated affine dynamics, and the former particle-filtering approach is well-suited to low-dimensional settings. Nevertheless, one would like to have access to (approximate) optimal finite dimensional filters for a broader range of situations.    

% % \byyan{Why Deep Learning?.}\hfill\\
% One possibility could be via deep learning, since deep neural networks have demonstrated that they can efficiently solve a variety of previously intractable numerical problems. The expressivity of neural networks on classical learning problems has inspired the use of deep learning approaches to the numerical stochastic filtering problems; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering,pmlr-v80-ryder18a,de2019gru,herrera2021neural,krach2022optimal}, and the development of measure-valued deep learning models; e.g.~\cite{Acciaio2022_GHT}.  At the forefront of these methods, are the class of deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, these are the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered models are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem \eqref{goal:Robust_Filtering}. 

% This paper constructs a DKF model which can uniformly approximate the map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering}, to arbitrary precision, for any pair of non-Markovian $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0:T]}$-adapted \textit{conditionally Gaussian} stochastic processes studied by \cite{LipShiryaev_II_2001}.  
% %%%%
% %%%%
% %%%%
% \begin{InformalTheorem}[The DKF is a Universal Conditionally-Gaussian Filter]
% \label{Informal_Theorem_Main:Informal_Theorem}
% \hfill\\
% Let $(X_{\cdot},Y_{\cdot})$ be the partially-observed system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} below, subject to mild regularity conditions.  For any suitable compact subset $K\subseteq C([0:T],\mathbb{R}^{d_Y})$, every $T>0$, and any approximation error $\varepsilon>0$ there exists a DKF model $\hat{F}:[0:T]\times C([0:T]\times\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ satisfying the uniform estimate
% \[
%     \max_{0\le t\le T,\,y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:t]})
%             ,
%                 \hat{F}(t,y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.
% \end{InformalTheorem}
% %%%%
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=.4\linewidth]{Graphics/Mask.pdf}
%     \caption{The DKF model in Informal Theorem~\ref{Informal_Theorem_Main:Informal_Theorem} has two inputs: a time $t$ and a continuous path $y_{\cdot}$ defined up to some time $T\ge t$.  The first parameter $t$ acts as a mask hiding the future evolution of the observation (input) path $y_{\cdot}$ beyond the current time $t$.  We note that there is no loss of generality in assuming that the path $y_{\cdot}$ is defined up to time $T$, since any path can be trivially extended beyond the current time $t$ by setting $y_{s}=y_t$ for all $s\in [t,T]$; e.g.\ as in the Functional It\^{o} Calculus \cite{MR3939653,MR2782350,MR3059194}.
%     \\
%     The mask, i.e.\ the parameter $t$, fills the same analogous role to recursions in classical stochastic filters.  That is, by varying the time parameter $t$, the prediction of the DKFs evolves into the future without having to retrain the DKF model.}
%     \label{fig:Mask}
% \end{figure}
% %%%%
% Our uniform estimates hold for coupled stochastic differential equations governed by
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% % \tag{Sig}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% % \tag{Obs}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $\smash{([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})}$, and where $\smash{\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))}$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
% We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $\smash{W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}}$ and $\smash{W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}}$, of respective dimensions $d_X$ and $d_Y$, for positive integers $d_X$ and $d_Y$. The requirements for the dynamics \labelcref{eq:filtering_dynamics__signal,eq:filtering_dynamics__observation} are detailed in \Cref{ass:technical_evolution_conditions} below.

% \subsection{The Deep Kalman Filter Model}
% \label{s:Introduction_Deep_Filtering__ss:ModelDetails}
% The proposed deep Kalman filter (DKF), illustrated in \Cref{fig:DKFModel}, generates predictions on the finite-dimensional metric space $(\mathcal{N}_{d_X},\mathcal{W}_2)$ whose points are non-singular Gaussian measures, and whose distance between points is quantified by the $2$-Wasserstein distance.  These predictions are generated from the continuous input paths via the following three-phase process.  
% \begin{figure}[hpt!]%[H]%
%     \centering
%         \centering
%         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
%     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
%     \label{fig:DKFModel}
% \end{figure}

% \begin{enumerate}[wide,label=\emph{Phase \arabic*}.]
%     \item The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly, our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^{d_Y})$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ include classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifold.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is is devoid of any projection onto a finite-dimensional (Schauder) basis, and its parameters can be chosen to suit the specific geomet\textit{}ry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.
    
%     \item In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner, by adaptive to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
    
%     \item In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_{d_X}$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{goal:Robust_Filtering}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.
% \end{enumerate}


% \subsection{Organization of Paper}
% \Cref{s:Setting} formalizes the basic required regularity conditions on the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} and it overviews any background material.  \Cref{s:Model} rigorously introduces the relevant DKF model.  \Cref{s:Main_Results} contains the paper's main theoretical results, as well as an overview of the proof methodology.  Several results of independent interest, both concerning the approximation capacity of the DKF model and the local Lipschitz regularity of the robust filtering map~\eqref{goal:Robust_Filtering} are discussed.  Detailed proofs of our results are relegated to \Cref{s:Proof}. 

% \section*{Notation}
% % \label{s:Notation}
% This section serves as a reference, which records the notation used throughout our manuscript.  In what follows, $N,I,J\in \mathbb{N}_+$, $A$ is an arbitrary $I\times J$ matrix, $x,x_1,\dots,x_J\in \mathbb{R}^N$, $f$ is an ar\-bi\-trary real-valued function on $\mathbb{R}$, and $t\in \mathbb{R}$.
% \begin{enumerate}[itemsep=3pt]
%     \item \textit{Componentwise Composition:} $\smash{f\bullet x\eqdef (f(x_n))_{n=1}^N}$ for any $N\in \mathbb{N}_+$.%, $x\in \mathbb{R}^N$, and $f:\mathbb{R}\rightarrow \mathbb{R}$.
%     \item \textit{Rectified Linear Unit (ReLU):} $\operatorname{ReLU}:\mathbb{R}\rightarrow\mathbb{R}$ given by $\smash{\operatorname{ReLU}(t)\eqdef \max\{0,t\}}$.
%     \item \textit{Rowwise Product:} $\smash{v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}}$.% for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
%     \item \textit{Softmax Function:} $\smash{\operatorname{Softmax}(x)\eqdef (e^{x_n}/\sum_{i=1}^N\,e^{x_i})_{n=1}^N}$.% for any $N\in \mathbb{N}_+$ and any $x\in \mathbb{R}^N$.
%     \item \textit{Sparsity:} $\smash{\|(A_{i,j})_{i,j=1}^{I,J}\|_0\eqdef \#\{A_{i,j}\neq 0:\,i,j=1,\dots,I\}}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$.
%     \item \textit{Vector Concatenation:} $\smash{\oplus_{j=1}^N x_j\eqdef (x_1,\dots,x_J)^{\top}}$ is the $J\times N$-matrix whose $j^{th}$ row is $x_j$.%, for $j=1,\dots,N$.
%     \item \textit{Vectorization:} $\smash{\operatorname{vec}((A_{i,j})_{i,j=1}^{I,J})\eqdef (A_{1,1},\dots,,A_{I,1},\dots,A_{1, J}, \dots, A_{I,J})}$.% for any $I,J\in \mathbb{N}_+$ and any $I\times J$-matrix $A$. 
%     \item \textit{Euclidean Norm:} 
%     $\smash{\|A\| = (\sum_{i,j=1}^{I,J} |A_{i,j}|^2 )^{1/2}}$. 
%     \item \textit{Supremum Norm:} 
%     $\smash{\|A\|_\infty=\sup \{ A_{i,j} : \, i=1,..., I, j=1, ..., J \}}$. 
% \end{enumerate}

% \section{The Setting}
% \label{s:Setting}
% This section formalizes the setting in which our analysis takes place.  We begin by specifying the dynamics of the stochastic processes in the filtering problem.  Next, the source space of paths considered is introduced.  Subsequently, we formulate the target space of probability measures wherein the optimal filter lies.

% \subsection{Regularity Conditions on the Partially-Observed System}
% % \label{s:Preliminaries__ss:Dynamics}
% % This section formulates the theoretical problem which this paper addresses.
% % % Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% % % Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  
% % These processes evolve according to the coupled dynamics
% % \begin{align}
% % \label{eq:filtering_dynamics__signal}
% % dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% % \label{eq:filtering_dynamics__observation}
% % dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% % \end{align}
% % where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.
% % 
% % 
% % Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% % \begin{align}
% % \label{id:ConditionalDistribution}
% %     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) 
% % \end{align}
% % where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of the theoretical foundations of DKFs.
% % \begin{question}
% % \label{question:main}
% % Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$?
% % \end{question}
% We henceforth maintain the following basic regularity assumptions on the dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.
% %%
% \begin{assumption}[Regularity Conditions: Dynamics]
% \label{ass:technical_evolution_conditions}
% We will assume the following uniform bounds:
% \begin{align*}
%     \vert \process{a_1}{t, y}{i, j}\vert \le L
%     \mbox{ and }
%     \vert \process{A_1}{t, y}{k, j}\vert \le L
% \end{align*}
% for $y \in C([0:t], \R^{d_Y})$, $t \in [0:T]$, $i,j=1,\dots,d_X$, and $k=1,\dots,d_Y$.  
% Further, we require the following integrability conditions:\footnote{In particular, the integrability conditions imply that $\bE\big[\sum_{j = 1}^{d_X}(X_0)_j^4\big] < \infty$.}
% \begin{enumerate}[label=(\roman*)]
%     \item $\int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     \item $\int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty$,
%     % \item $\int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt < \infty$, \yannick{Follows from Lip-cont.}
%     % \item $\int_0^T (\process{b_2}{t, y_{[0:t]}}{i, k})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{k, i})^2 dt < \infty$, \yannick{Follows f. Lip-cont.}
%     % \item $\int_0^T (\process{A_0}{t, y_{[0:t]}}{k})^2 + (\process{B_2}{t, y_{[0:t]}}{k, l})^2 dt < \infty$, \yannick{Follows from Lip-cont.}
% \end{enumerate}
% hold for $i,j=1,\dots,d_X$, and $k,l=1,\dots,d_Y$ and all paths $y_{[0:T]} \in C([0:T], \R^{d_Y})$. We define 
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\top + B_2B_2^\top, \quad 
%     b \circ B \eqdef b_1B_1^\top + b_2B_2^\top, \quad 
%     b \circ b \eqdef b_1b_1^\top + b_2b_2^\top.
% \end{align*}
% and require that the matrix $B \circ B$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% \begin{enumerate}[label=(\roman*), resume]
%     \item $\vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%         \le
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2$,
%     \item $(B_k)_{i,j}(t, x)^2  
%         \le 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2)$,
%     \item $\int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt < \infty$,
%     \item $\bE[\vert (X_t)_j \vert] < \infty, \quad \forall t \in [0:T]$,
%     \item $\bP\big( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \big) = 1$,
% \end{enumerate}
% for indices $i=1,\dots,d_Y$ and $j=1,\dots,d_X$, where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$.  

%     We further impose the following assumptions on the dynamics \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}:
%     \begin{enumerate}[label=(\roman*), resume]
%         \item Local Lipschitz continuity in the path component uniformly in time\footnote{
%             By \emph{local Lipschitz continuity uniformly in time} we mean that there exists a constant that is a local Lipschitz-constant for the path at all times $t \in [0,T]$.
%         }, as well as global Lipschitz continuity in the time component of $a_0$, $a_1$, $b \circ b$, $b \circ B$, $ A_0$, $A_1$, $(b \circ B)$, $(B \circ B)^{-1}$ with respect to the $l^2$-norm, or Frobenius norm if matrix-valued. \label{asm:Regulartiy__1}
%         \item Positive semi-definiteness of $(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ for all times $t \in [0:T]$ and paths $y_{[0:T]} \in C^1([0:T], \R^{d_X})$. \label{asm:Regulartiy__2}
%         \item \label{asm:Regularity__3} Let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$ for any path $y_{[0:T]} \in C^1([0:T], \R^{d_X})$, where 
%         \begin{align*}
%             \Tilde{a}_1^\top(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%         \end{align*}
%         There exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$ as well as $K_3 > 0$ s.t. $\tr(A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$. 
%     \end{enumerate}

%     Eventually we require for the initial conditions that 
%     \begin{enumerate}[label=(\roman*), resume]
%         \item the conditional distribution of $X_0$ given $Y_0$ is normal,
%         \item the covariance matrix $\Sigma_0 := \mathbb{E}[(X_0 - \mu_0)(X_0 - \mu_0)^\intercal \vert Y_0]$ is positive definite, where $\mu_0 := \mathbb{E}[X_0 \vert Y_0]$, and that
%         \item \label{asm:Regularity__LipInit} Lipschitz continuity of $\mu_0, \Sigma_0$ in $Y_0$ w.r.t. the $\Vert \cdot \Vert_2$-norm holds. 
%     \end{enumerate}
% \end{assumption}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Setting__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^{d_Y})$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^{d_Y}$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^{d_Y})$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^{d_Y}$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically embed any path $y\in C([0:t],\mathbb{R}^{d_Y})$ into a path $\bar{y} \in C([0:T],\mathbb{R}^{d_Y})$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     \bar{y}(s)\eqdef \begin{cases}
%         y(s) &: \mbox{ if } 0\le s \le t\\
%         y(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $\bar{\cdot}: C([0:t],\mathbb{R}^{d_Y}) \to C([0:T],\mathbb{R}^{d_Y})$ is a linear isometric embedding of the Banach spaces, since
% \[
% \|\bar{y}\|_T = \max_{0\le s\le T}\, \|y(s)\|_2
% = \max_{0\le s\le t}\, \|y(s)\|_2 = \|y\|_t, 
% \]
% since $y(s)=y(t)$ for all $t<s\le T$.  Conversely, the restriction $\bar{y}_{[0:t]}$ of a path $\bar{y}\in C([0:T],\mathbb{R}^{d_Y})$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^{d_Y})$ to $C([0:t],\mathbb{R}^{d_Y})$ since
% \[
%         \|\bar{y}_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|\bar{y}_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|\bar{y}_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|\bar{y}(s)\|_2 
%     =
%         \|\bar{y}\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^{d_Y})$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot be approximated by standard deep neural networks parameterized determined by a number of trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing}.   

% The curse of dimensionality cannot be broken, but can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space -- as is the case in our results -- show that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}. However, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are either isometric to some compact Riemannian manifold or they are comprised of piecewise linear paths with finitely many pieces.  In particular, we exclude fractal-like subsets of the path space $C([0:T],\mathbb{R}^{d_Y})$ which need not be compressible into finitely many dimensions without ``loosing information'' (i.e.\ for which there is no bi-Lipschitz embedding into a finite-dimensional normed space).  

% In what follows, we denote the Riemannian volume of a connected $(C^2)$ Riemannian manifold $(\mathcal{M},g)$ by $\operatorname{Vol}(\mathcal{M},g)$.  We denote its geodesic distance function by $d_g$.
% \begin{assumption}[Domain Regularity]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ and a ``latent dimension $\ldim\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}[label=(\roman*)]
%     \item  \label{ass:reg_compact_finite}\emph{Finite Domains:} $K$ is finite.
%     \item \label{ass:reg_compact_linear} \emph{Piecewise Linear Domains:} There are $\pldim \in \mathbb{N}_+$, $0=t_0<\dots<t_\pldim=T$, and $C_K>0$ such that $y_{\cdot}\in K$ if and only if:
%         \begin{enumerate}[label=(\alph*)]
%             \item For $i=0,\dots,\pldim-1$ there is a $d\times d$ matrix $A^{(i)}$ and a $b^{(i)}\in \mathbb{R}^{d_Y}$ satisfying
%             \[
%             \begin{aligned}
%                 & y(t)=A^{(i)}\,t+b^{(i)}
%                 \,
%                 &
%                 \,
%                 \mbox{ for all } t\in (t_i,t_{i+1})
%             ,
%             \end{aligned}
%             \]
%             \item $y_0=0$,
%             \item $\max_{i=1,\dots,\pldim}\,|y(t_i)|\le C_K$.
%         \end{enumerate}
%     \item \label{ass:reg_compact_riemann}\emph{Smooth Domains:} There exists a compact and connected $\ldim$-dimensional Riemannian manifold $(\mathcal{M},g)$ for which $(\mathcal{M},d_g)$ is isometric to $(K,\|\cdot\|_T)$.
%     %\anastasis{I think, I can do a bit better here, and get a compact subset of ...}
% \end{enumerate}
% \end{assumption}
% Evidently, their domains $K$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_finite} are easily exhibited, and they correspond to any \textit{training set}.  One can interpret results in this case as paralleling interpolation results for deep learning, e.g.\ \cite{CristaJosefMartin_2020_UnivInterpol,vershynin2020memory,KratsiosDevarnotDokmanic_SmallTransformers_JMLR2023}, but allowing for some arbitrarily small error as in \cite{park2021provable}.

% Compact subsets of the path-space $C([0:T],\mathbb{R}^{d_Y})$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann} are also plentiful.  The following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}, and related results such as~\cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}, illustrate this by guaranteeing that $C([0:T],\mathbb{R}^{d_Y})$ contains isometric copies of any compact metric space.  Consequentially, $C([0:T],\mathbb{R}^{d_Y})$ contains isometric copies of any compact and connected Riemannian manifold.
% \begin{proposition}[Isometric Copies of All Compact Riemannian Manifolds]
% \label{prop:Non_Vaccousness}
% \sloppy Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}

% We obtain explicit estimates for the case where $(K,d_{\cdot})$ satisfies \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann}, if the ``model'' smooth manifold $\mathcal{M}$ is topologically regular, in that sense that it is \textit{aspherical}.
% This means that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$, what is for instance the case if $\mathcal{M}$ is a Torus. See e.g. \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups.  

% Domains $K$ satisfying \Cref{ass:reg_compact} \ref{ass:reg_compact_linear} include any piecewise linear interpolation of real-world financial time-series data, or simulated data.  This is because only a finite number of inflection points can be observed, and prices are not unbounded.  

% In this way, \Cref{ass:reg_compact} summarizes a rich family of compact subsets of the path-space $C([0:T],\mathbb{R}^{d_Y})$ which possess a sufficient degree of structure to be losslessly encoded into finitely many dimensions by our model's encoding layer, called its \textit{pathwise attention mechanism}.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Setting__ss:OutputSpace}

% Fix $1 \leq p \leq 2$. The $p$-Wasserstein space $\mathcal{P}_p(\mathbb{R}^{d_X})$ consists of all probability measures on $\mathbb{R}^{d_X}$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_p(\mathbb{R}^{d_X})$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^p]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_p$ on $\mathbb{P}_p(\mathbb{R}^{d_X})$ is given by minimizing the optimal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_p(\mathbb{P}, \mathbb{Q})^p
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^p]
%     .
% \]
% Generally, the $p$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, the $2$-Wasserstein distance is not always computationally intractable as for instance in the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^{d_X}$, \cite{dowson1982frechet} showed that it admits the following closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^{d_X})$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^{d_X})$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^{d_X}$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% %\yannick{Until here $d_X, d_Y$ is fixed, needs to be done in what follows.}

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% % This section introduces our attention-based model, our deep Kalman filter (DKF) model, illustrated in \Cref{fig:DKFModel}.  The proposed DKF generates a prediction on the space $(\mathcal{N}_{d_X},\mathcal{W}_2)$ from any observed continuous path in $C([0:T],\mathbb{R}^{d_Y})$, via a three-phase process.  

% % \begin{figure}[hpt!]%[H]%
% %     \centering
% %         \centering
% %         \includegraphics[width=1\linewidth]{Graphics/Model.pdf}
% %     \caption{Architecture of a Deep Kalman Filter which can approximate the conditional law of the signal process $X_{\cdot}$ given source paths, possibly (but not necessarily) taken by the observation process.}
% %     \label{fig:DKFModel}
% % \end{figure}

% % \subsubsection{Phase 1:} The observed infinite-dimensional continuous path is encoded into a finite-length real vector.  Surprisingly our proposed encoding layer, coined the \textit{pathwise attention mechanism}, adaptively implements a stable and lossless encoding for a broad class of compact subsets of $K$ paths in $C([0:T],\mathbb{R}^{d_Y})$.  By \textit{losslessness}, we mean that it is injective for a broad class of compact subsets of $K$ including classes of piecewise linear paths, any finite (training) set, any $K$ which is isometric to a closed Riemannian manifolds.  By stability, we mean it in the sense of constructive approximation theory, e.g.~\cite{MR4433109,MR4577400}, namely that the map encoding layer is Lipschitz and so is its inverse.  \textit{Stability} is desirable since it implies that minor numerical errors, e.g.\ rounding, do not lead to drastically different downstream predictions.  Finally, by \textit{adaptivity} we mean that the encoding layer is (Schauder) basis-free, and its parameters can be chosen to suit the specific geometry of the compact set of paths $K$ on which the approximation of the optimal filter is to be performed.

% % \subsubsection{Phase 2:} In the next phase, the DKF processes the vectors encoding the observed paths and generates ``deep features'' which are then passed along to the output layer for prediction generation.  This phase leverages the efficient approximation capacity of MLPs, e.g.~\cite{yarotsky2018optimal,pmlr-v125-kidger20a,kratsios2021universal,LuShenYangZhang_2021_UATRegularTargets}, to flexibly process the encoded features in a task-specific manner by adapting to specific dynamics of the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.

% % \subsubsection{Phase 3:} In its final processing phase, the DKF decodes the ``deep features'' generated by the MLP to $\mathcal{N}_{d_X}$-valued predictions, which are then used to approximately implement the predictions of the optimal filter~\eqref{id:ConditionalDistribution}.  This decoder is a modified instance of the \textit{geometric attention mechanism} of \cite{Acciaio2022_GHT}.  Intuitively, this layer translates Euclidean data to a point in a generalized geodesic convex hull of a finite number containing the image of $K$ under the optimal filter.


% \subsection{Phase 1 - Encoding via Pathwise Attention}
% \label{s:Model__ss:PathwiseAttention}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and the graph attention mechanism of \cite{velivckovic2017graph} to the context of continuous-time path sources/inputs.  Our attention mechanism, called \textit{pathwise attention}, encodes key information about a novel path $y_{\cdot}$ and, like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``known/previously generated paths''.  

% \begin{figure}[hpt!]%[H]%
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.8\linewidth]{Graphics/Similarity_Score.pdf}
%         \caption{\label{fig:Similarity_Score} The \textit{similarity score} component $\operatorname{sim}_T^{\theta_0}$ encodes a path into finite-dimensional vectorial data, by relating its similarity to a dictionary of previously observed ``contextual paths''.}  
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \includegraphics[width=.8\linewidth]{Graphics/Positional_Emcoding.pdf}
%         \caption{\label{fig:PositionalEncoding} The \textit{positional encoding} component $\operatorname{post}_T^{\theta_0}$ of the attention mechanism allows the similarity scores to further adapt to any novel path by extracting sample-positions on the novel paths.}
%     \end{subfigure}
%     \caption[1]{Our \textit{pathwise attention mechanism} $\operatorname{attn}_t^{\theta}$, in \Cref{defn:PathAttention}, relies on two methods for adaptive feature extraction.  The first component of the mechanism, in~\ref{fig:Similarity_Score}, in is a similarity score which ranks the similarity of any novel path $x_{\cdot}$ to a dictionary of ``recognized/saved'' reference paths.  The second component of the mechanism, in~\ref{fig:PositionalEncoding}, samples points on the novel path $x_{\cdot}$ and perturbs the similarity scores by them.  The adeptness of the pathwise attention mechanism, unlike basis-based methods, is rooted in the fact that nearly all of its parameters are trainable, which allows it to be tasks-specific (similarly to the advantage of deep MLPs have over regression via basis-functions).}
%     \label{fig:Attention_Is_All_You_Need}
% \end{figure}


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $\rdim$, $\sdim$, $d_Y$, and a ``time horizon'' $T> 0$.  
% Given a set of $\rdim$ distinct paths $\{y^{(n)}\}_{n=1}^\rdim$ in $C([0,1],\mathbb{R}^{d_Y})$, an $\sdim \times \rdim$-matrix  $B$, $b\in \mathbb{R}^{\sdim}$, an $\sdim \times \sdim$-matrix $A$, and $a\in \mathbb{R}^{\sdim}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^\rdim)$.

% The \textit{similarity score}, is a map $\operatorname{sim}_T^{\theta_0}:C([0,1],\mathbb{R}^{d_Y})\rightarrow\mathbb{R}^\sdim$, mapping any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$ to
% \begin{equation}
% \label{eq:sim_score}
%     \operatorname{sim}_T^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%         \operatorname{Softmax}
%             \biggl(
%                     A\operatorname{ReLU}\bullet 
%                 \Big(
%                         B
%                         \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^\rdim
%                     +
%                         b
%                 \Big)
%                     +
%                         a
%             \biggr)
%     .
% \end{equation}
% % where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$. 
% % \yannick{The definition of $\bullet, \operatorname{Softmax}, \operatorname{ReLU}$ is also in the Notation section.}
% \end{definition}

% Illustrated in \Cref{fig:Attention_Is_All_You_Need}, our pathwise attention mechanism extracts features by reinterpreting two of the key features of attention mechanisms from natural language processing (NLP).  First, it utilizes \textit{similarity scores} which rank the likeness of any novel path against a dictionary of references paths.  These reference paths can either arise from real/stress historical (market) scenarios, they can be generated synthetically, or a combination of either.  These similarity scores are illustrated in \Cref{fig:Similarity_Score}, and they serve as pathwise analogues of contextual keys and queries in attention mechanisms in NLP.

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of \Cref{defn:Sim_Score}, fix a positive integer $\pdim$, and set of query times $0\le t_1<\dots< t_\tdim\le T$, an $\pdim\times {d_Y}$ matrix $V$, and an $\pdim\times \tdim$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^\tdim)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{post}_T^{\theta_0}:C([0,1],\mathbb{R}^{d_Y})\rightarrow\mathbb{R}^{\pdim \times d_Y}$, defined by 
% \begin{equation}
% \label{eq:pos_encoding}
%     \operatorname{post}_T^{\theta_1}
%         (y_{\cdot} )
%     \eqdef 
%         U \,
%         (\oplus_{j=1}^\tdim \, y_{t_j})
%         + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$.
% \end{definition}

% Next, the \textit{positional encoding} of any novel path, illustrated in \Cref{fig:PositionalEncoding}, encodes snapshots of this path at various times.  These indicate changes in any sample path, and they fully determined piecewise linear paths with finitely many pieces (as are generated in simulation studies).  This data then combines with the weights of the similarity scores to produce the features encodings of our pathwise attention mechanism. 


% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of \Cref{defn:Sim_Score,defn:PositionalEncoding}, set $\sdim=\pdim$.  A \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1,C)$, is the map $\operatorname{attn}_T^{\theta}:[0,T]\times C([0,T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim + 1}$ with representation
% \begin{align}
%     \label{eq:featuremap}
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot})
%     \eqdef 
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
% \end{align}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^{d_Y})$ and $0\le t\le T$, where $C$ is an $\edim \times (\sdim d_Y)$-dimensional matrix.
% \end{definition}


% \begin{proposition}[Pathwise Attention Losslessly Encodes Regular Domains]
% \label{prop:Lossless_Encoding}
% \sloppy Let $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact}.  Then, there exists an $\edim \in \mathbb{N}_+$ and a parameter $\theta$ as in \Cref{defn:PathAttention} such that, $\operatorname{attn}_T^{\theta}$ restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim+1},\|\cdot\|_2)$.

% Estimates for the encoding dimension $\edim$ are recorded in \Cref{tab:ATTENTION_Rates} on a case-by-base basis.
% \end{proposition}



% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for Lossless Pathwise Attention Encoding of Regular Compact Domains.}}
%     \label{tab:ATTENTION_Rates}
%     \begin{tabular}{lllll}
%     \toprule
%         Type of Compact Domain %& Complexity ($\|\theta\|_0$) 
%         & Encoding Dimension ($\edim$) & Ass.~\ref{ass:reg_compact} \\
%     \midrule
%         Finite%& $\mathcal{O}(\cdot)$ 
%         & $\mathcal{O}(\log(\# K))$ 
%         & \ref{ass:reg_compact_finite}
%         \\
%         P.W. Lin. ($\pldim$ Pieces) %& - 
%         & $\mathcal{O}(\pldim d)$
%         & \ref{ass:reg_compact_linear}
%         \\
%         Iso. Comp. Riemann.%& -- 
%         & Finite
%         & \ref{ass:reg_compact_riemann}
%         \\
%         Iso. Comp. Riemann $\&$ Aspherical %& -- 
%         & $\smash{\mathcal{O}\big(\mathfrak{N}_{d_g}(\mathcal{M},\operatorname{Vol}(\mathcal{M},g)^{1/\ldim} )\big)}$
%         & \ref{ass:reg_compact_riemann}
%         \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Fix an $A\subset \mathcal{M}$ and $\delta>0$.  The quantity $\mathfrak{N}_{d_g}(A,\delta)$ denotes the minimum number, $I$, of points $\{x_i\}_{i=1}^I \subseteq A$ for which every $x\in A$ is contained in a geodesic ball of radius $\delta$ about some $x_i$, for $i\in \{1,\dots,I\}$.}
% \end{table}

% \subsection{Phase 2 - Multi-Layered Perceptrons (MLPs) Transformation}
% \label{s:Model__ss:Review__MLPs}
% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an encoding dimension $\edim$ and a target dimension $\ddim$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^\edim$ to $\mathbb{R}^\ddim$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^\edim\rightarrow\mathbb{R}^\ddim$ with iterative representation: for each $x\in \mathbb{R}^\edim$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=\edim$ and $d_{J+1}=\ddim$.

% \subsection{Phase 3 - Decoding via Geometric Attention Mechanism}
% \label{s:Model__ss:GeometricAttentionMechanism}

% Fix $\ddim \in \mathbb{N}_+$.  In what follows, we denote the orthogonal projection of $\mathbb{R}^\ddim$ onto the $\ddim$-simplex 
% \[
%         \Delta_\ddim
%     \eqdef 
%     \Big\{
%         w \in [0,1]^\ddim:\,
%         \sum_{n=1}^\ddim\,w_n = 1
%     \Big\} 
% \]
% by $P_{\Delta_\ddim}$.  We note that the closedness and convexity of $\Delta_\ddim$ implies that $P_{\Delta_\ddim}$ is a well-defined $1$-Lipschitz map, see \citep[Proposition 4.8]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017}.  

% \begin{definition}[Geometric Attention Mechanism]
% \label{defn:GeometricAttentionMechanism}
% Let $\ddim,d_X \in \mathbb{N}_+$.  A geometric attention mechanism is a map $\operatorname{g-attn}_\ddim: \mathbb{R}^\ddim \rightarrow \mathcal{N}_{d_X}$ with representation
% \[
%         \operatorname{g-attn}_\ddim^{\vartheta}(v)
%     =
%         \mathcal{N}_{d_X}\Biggl(
%                 \sum_{n=1}^\ddim\,
%                     P_{\Delta_\ddim}(v)_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^\ddim\,
%                     P_{\Delta_\ddim}(v)_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)}
%         \Biggr)
% \]
% where $m^{(1)},\dots,m^{(\ddim)}\in \mathbb{R}^{d_X}$, $A^{(1)},\dots,A^{(\ddim)} \in \R^{d_X\times d_X}$; and $\vartheta\eqdef (m^{(n)},A^{(n)})_{n=1}^\ddim$.
% \end{definition}

% \subsection{The DKF Model}
% \label{s:Model__ss:DKFModel}
% We may now formalize the discrete Kalman filter model of \Cref{fig:DKFModel}.  
% \begin{definition}[Deep Kalman Filter]
% Let $d_X, d_Y \in\mathbb{N}_+$, $T>0$, and an activation function $\sigma:\mathbb{R}\rightarrow \mathbb{R}$.  
% A function $\hat{F}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathcal{N}_{d_X}$ is called a discrete Kalman Filter if it admits the representation
% \begin{equation}
% \label{eq:DKF_formalization}
%         \hat{F}
%     =
%             \operatorname{g-attn}_\ddim^{\vartheta}
%         \circ 
%             \hat{f}
%         \circ 
%             \operatorname{attn}_T^{\theta}
% \end{equation}
% where $\operatorname{g-attn}_\ddim^{\vartheta}$ is as in \Cref{defn:GeometricAttentionMechanism}, $\operatorname{attn}_T^{\theta}$ is as in \Cref{defn:PathAttention}, and $\hat{f}$ is an MLP as in~\eqref{eq:MLP}; such that the composition~\eqref{eq:DKF_formalization} is well-defined.
% \end{definition}



% \section{Main Result}
% \label{s:Main_Results}

% We are now ready to state our main theorem, which shows that the DKF~\eqref{eq:DKF_formalization} is indeed capable of asymptotically optimally filtering the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}.  Our guarantees are of a non-asymptotic form; in that they depend on the complexity of the network.
% \begin{theorem}[The DKF Can Approximate the Optimal Filter]
% \label{thrm:MAIN}
% \sloppy Let $d_X, d_Y \in \mathbb{N}_+$ and $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact}.  Suppose that the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies \Cref{ass:technical_evolution_conditions}.  % and let $f^{\star}$ denote its associated optimal filter~\eqref{id:ConditionalDistribution}.  
% For every $T>0$ there exists a DKF $\hat{F}:[0:T]\times C([0:T]\times\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ satisfying the uniform estimate
% \[
%     \max_{0\le t\le T,\,y_{\cdot}\in K}\,
%         \mathcal{W}_p\big(
%                 % f^{\star}(y_{\cdot})
%                 \mathbb{P}(X_t \in \cdot \vert y_{[0:T]})
%             ,
%                 \hat{F}(t,y_{\cdot})
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, \Cref{tab:ComplexityMain} records the complexity estimates of $\hat{F}$.
% \end{theorem}

% \begin{table}[H]%[ht!]
%     \centering
%     \caption{{Complexity Estimates for the DKF model $\hat{F}$ in~\Cref{thrm:MAIN}.}}
%     \label{tab:ComplexityMain}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 \varepsilon^{-\ddim}
%             \big)
%         }
%     	$
%         & 
%         $        
%         \smash{
%             \mathcal{O}\big(
%                 \varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          \smash{
%          \mathcal{O}\big(
%             \varepsilon^{-4\ddim-1}
%          \big)
%     	 }
%          $
%          &
%          $ \ddim + \edim +3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%          \smash{
%          \mathcal{O}\big(
%             \varepsilon^{-8\ddim-6}
%          \big)
%     	 }
%          $
%          & 
%          $\ddim+\edim+4$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(\varepsilon^{-1}\big)$
%          \\
%          Non-Smooth $\&$ Non-poly.
%             &
%         Finite
%         &
%         $\ddim+\edim+3$
%          & $\mathcal{O}(1)$ & $\smash{\mathcal{O}\big(\varepsilon^{-1}\big)}$
%          \\
%     \bottomrule
%     \end{tabular}
%     } % END Resize
% \end{table}



% \subsection{Proof Overview}
% \label{s:Theoretical_Analysis}
% This section overviews the derivation of our main result, namely, \Cref{thrm:MAIN}.

% %\subsubsection{Summary of What is Known}
% % \label{s:Theoretical_Analysis__ss:LipsterShiryaevSummary}
% Results in \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, they denote an explicit formulation of the resulting distribution which can then analyze directly. 
% In particular, \Cref{ass:technical_evolution_conditions} allows the application of \citep[Theorem 12.6]{LipShiryaev_II_2001} and we obtain that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.


% A function is uniformly approximable by a deep learning model if it is continuous.  If there is no clear favourable structure in the function being approximated, e.g.\ smoothness \cite{yarotsky2020phase,gonon2023approximation} or neural network-like structure \cite{cheridito2021efficient,mhaskar2016deep}, then the best available approximation rates are those corresponding to those where the target function is Lipschitz; see \cite{DaubechiesDeVoreFoucartHaninPetrova_CA_KnotFreeReLU_2022}. %devore1993constructive,
% Thus, the first step to obtaining approximability guarantees for the optimal filter by deep neural networks, which depend on relatively few trainable parameters, is to show that the optimal filter is a locally-Lipschitz function of observed paths.

% \begin{proposition}[Local Lipschitz-Continuity of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter}
%     Under \Cref{ass:technical_evolution_conditions}, $f_t$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous. In particular, for every time $t \in [0:T]$, path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$ there exists constant $C \ge 0$ such that for all times $s \in [0:T]$ and paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\vert t -s \vert < \epsilon$, $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]}))
%         \leq C 
%             \big(
%                 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T 
%             + 
%                 \vert t - s \vert
%             \big).
%     \end{align*}
% \end{proposition}

% Having established the regularity of the optimal filter for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, we need to verify that maps sharing the same domain (input space), codomain (output space), and regularity as the optimal filter are approximable by the proposed DKF model.  This is the content of the next proposition, which acts as its standalone approximation theorem for the DKF.


% \begin{table}[H]%[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{F}$ in \Cref{prop:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{@{}lllll@{}}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$) \\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 (LV( L))^{-\ddim}\,\varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & 
%         $
%         \smash{
%             \mathcal{O}\big(
%                 (LV(L))^{-\ddim}\,\varepsilon^{-\ddim}
%             \big)
%         }
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          \smash{
%         \mathcal{O}\big(
%             L^{4\ddim+1}\, \varepsilon^{-4\ddim-1}
%         \big)
%     	}
%          $
%          &
%          $ \ddim + \edim +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%          \smash{
%         \mathcal{O}\big(
%             L^{8\ddim+6}\, \varepsilon^{-8\ddim-6}
%         \big)
%     	}
%          $
%          & 
%          $\ddim+\edim+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Non-Sm. $\&$ Non-poly.
%             &
%         Finite
%         &
%         $\ddim+\edim+2$
%          & $\mathcal{O}(1)$ & $\smash{\mathcal{O}\big(L\varepsilon^{-1}\big)}$
%          \\
%     \bottomrule
%     \end{tabular}
%     } % END Resize
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
% \end{table}

% \begin{proposition}[Approximation Capacity of DKFs]
% \label{prop:Universal_Approximation_Theorem__PathToNd}
% Let $d_X, d_Y \in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfying \Cref{ass:reg_compact}.  
% For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:([0,T]\times K,|\cdot| \times \|\cdot\|_{\infty})\rightarrow (\mathcal{N}_{d_X},\mathcal{W}_2)$ there exists a DKF $\smash{\hat{F}}$ 
% % \[
% %         \hat{t}(x)
% %     \eqdef
% %         \mathcal{N}_{d_X}\Biggl(
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     m^{(n)}
% %             ,
% %                 \sum_{n=1}^N\,
% %                     P_{\Delta_N}(\mathcal{NN}(x))_n
% %                     \cdot
% %                     (A^{(n)})^{\top}A^{(n)})
% %         \Biggr)
% % \]
% % \anastasis{Update representation/simplify ofc + explain notation} 
% satisfying the uniform estimate 
% \[
%     \sup_{t, x\in [0:T]\times K}\,
%         \mathcal{W}_p\big(
%         f(t, x_\cdot) ,
%         \hat{F}(t,x_\cdot) 
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(\edim)$ and Decoding dimension $(\ddim)$ are all recorded in \Cref{tab:approximationrates__nonFlatVersion} depending on the activation function $\sigma$.
% \end{proposition}


% We now have at our disposal, the tools to prove our main result.  
% \begin{proof}\textbf{of \Cref{thrm:MAIN}}\hfill\\
% % \begin{proof}[{Proof of \Cref{thrm:MAIN}}]
% Since the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation} satisfies \Cref{ass:technical_evolution_conditions}, \Cref{prop:LocLipReg_OptimFilter} implies that the optimal filter $f_T$ in \eqref{goal:Robust_Filtering} 
% is a locally-Lipschitz map from $([0:T],  C([0:T],\mathbb{R}^{d_Y}),\vert \cdot \vert \times \|\cdot\|_T)$ to $(\mathcal{N}_{d_X},\mathcal{W}_2)$.  Since $K\subseteq C([0:T],\mathbb{R}^{d_Y})$ is compact then, $f|_K$ is Lipschitz.  

% Since $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfies \Cref{ass:reg_compact} and $0<\varepsilon<1/2$ then, \Cref{prop:Universal_Approximation_Theorem__PathToNd} implies that there is a DKF $\hat{F}:C([0:T],\mathbb{R}^{d_Y})\rightarrow\mathcal{N}_{d_X}$ with representation~\eqref{eq:DKF_formalization} and complexity recorded in \Cref{tab:approximationrates__nonFlatVersion} satisfying
% \[
% 	\sup_{t, y\in [0:T]\times K}\,
% 		\mathcal{W}_p\big(
% 			f(t,y)
% 		,
% 			\hat{F}(t,y)
% 		\big)
% 	< 
% 		\varepsilon
% 	.
% \]
% This completes the proof of \Cref{thrm:MAIN}.
% \end{proof}

% \section{Discussion and Future Work}
% \label{s:Discussion}
% Our main result, namely Theorem~\ref{thrm:MAIN}, showed that there are deep Kalman filters which can solve the approximately stochastic filtering problem in continuous time for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, to arbitrary accuracy.  This complements the experimental work of \cite{KrishnanShalitSontag15,KrishnanShalitSontag17}, which shows that deep Kalman filters can be trained to offer state-of-the-art empirical performance.  

% From the theory perspective, it would be interesting to analyze the statistical learning theoretic properties of DKFs.  One would expect that elementary generalization bounds could be derived by using the bounds on VC-dimension derived in \cite{MR3960917} and a version of the results of \cite{MR1984026} or by directly modifying the transport theoretic arguments of \cite{hou2022instance}, to incorporate the effects of the pathwise and geometric attention layers in~\eqref{eq:DKF_formalization}.  Nevertheless, for problems in mathematical finance where one only observes a single training path (one-shot learning), the most interesting question in that direction is: \textit{How to train the DKFs in a way such that they have robust statistical guarantees when only a single training path is observed}.

% \section{Proofs}
% \label{s:Proof}
% This section contains the derivations of our paper's results.

% \subsection{Isometric Copies of Every Compact Riemannian Manifold in the Path Space -- Proof of \texorpdfstring{\Cref{prop:Non_Vaccousness}}{Proposition 1}}
% \label{s:Proof__ss:AuxResults}
% \begin{proof}\textbf{of \Cref{prop:Non_Vaccousness}}\hfill\\
% % \begin{proof}[{Proof of \Cref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^{d_Y})$, given by $f\mapsto (f(\cdot /T),0,\dots,0)$, is an isometric embedding; then $\smash{\phi\eqdef \phi_3\circ\phi_2\circ \phi_1}$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^{d_Y})$.
% \end{proof}

% \subsection{Stability of the Optimal Filter - Proof of \texorpdfstring{\Cref{prop:LocLipReg_OptimFilter}}{Lipschitz Continuity}}
% We now prove the local Lipschitz stability of the optimal filter~\eqref{goal:Robust_Filtering}, for the coupled system~\eqref{eq:filtering_dynamics__signal}-\eqref{eq:filtering_dynamics__observation}, as a function of its observed/input path.  The proof builds on a series of Lemmata, which demonstrate the local Lipschitz continuity of the parameters defining the optimal filter.  

% We first observe that, \Cref{ass:technical_evolution_conditions} grants us access to \citep[Theorem 12.7]{LipShiryaev_II_2001}, which implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
%     d\mu_t 
%         &=[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\top}(t,y_{[0:t]})]\label{id:ClosedFormMu}
%         \\
%         & \pushright{
%              \times (B\circ B)^{-1}(t,y_{[0:t]}) [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt]  \notag
%         }
%         \\
%     \partial_t\Sigma_t
%         & = a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\top}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]})
%         \label{id:ClosedFormSigma} \\
%         & \pushright{
%               - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\top}(t,y_{[0:t]}) ]
%               (B\circ B)^{-1} (t,y_{[0:t]})} \notag \\
%         & \pushright{\times [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\top}(t,y_{[0:t]})]^{\top} }
%          \notag
% \end{align}
% with initial conditions $\mu_0\eqdef\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\top}|Y_0]$; where
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\top + B_2B_2^\top, \quad 
%     b \circ B \eqdef b_1B_1^\top + b_2B_2^\top, \quad 
%     b \circ b \eqdef b_1b_1^\top + b_2b_2^\top.
% \end{align*}
% Furthermore, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\Sigma_t$ is positive definite for all $t \in [0:T]$ since we have assume that $\Sigma_0$ in \Cref{ass:technical_evolution_conditions}.

% To clarify the argument's direction, we first record the proof of \Cref{prop:LocLipReg_OptimFilter}.  We subsequently derive the lemmata on which it relies.

% \begin{proof}\textbf{of \Cref{prop:LocLipReg_OptimFilter}}\hfill\\
% % \begin{proof}[{Proof of \Cref{prop:LocLipReg_OptimFilter}}]
%     Fix $t \in [0:T]$, a path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$.
%     By \Cref{prop:LocLipReg_OptimFilter_Time} we can fix a $K_1 > 0$ such that for every time $0 < s < T$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})) \leq K_1 \vert t-s \vert_t.
%     \end{align*}
%     By \Cref{prop:LocLipReg_OptimFilter_Path} we can fix a $K_2 > 0$ such that for every path $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$ holds
%     \begin{align*}
%             \mathcal{W}_2(
%                 \mathbb{P}(X_u \in \cdot \vert y^{(1)}_{[0:u]})
%             ,
%                 \mathbb{P}(X_u \in \cdot \vert y^{(2)}_{[0:u]})
%             )
%         \leq
%             K_2 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T.
%     \end{align*}
    
%     We see by the triangular inequality of the $\mathcal{W}_2$-distance (that holds as we handle normal distributions, see \eqref{id:LipsterShiryaevRepresentation}),
%     \begin{align*}
%         &
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]})) \\
%         & \quad \leq 
%                 \mathcal{W}_2(
%                     \mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]})
%                 ,
%                     \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})
%                 )
%             + 
%                 \mathcal{W}_2(
%                     \mathbb{P}(X_s \in \cdot \vert y^{(1)}_{[0:s]})
%                 ,
%                     \mathbb{P}(X_s \in \cdot \vert y^{(2)}_{[0:s]})
%                 )
%             \\
%         & \quad \leq \max\{ K_1, K_2 \} 
%             \big(
%                 \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T 
%             + 
%                 \vert t - s \vert
%             \big)
%     \end{align*}
%     what concludes the proof.
% \end{proof}

% \subsubsection{Lipschitz-Continuity in the Path-Component of the Optimal Filter}

% \begin{lemma}[Local Lipschitz - the Path-Component of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter_Path}
%     \sloppy Under \Cref{ass:technical_evolution_conditions}, $f$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous uniformly in time. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ and $\epsilon > 0$ there exists constant $C \ge 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq C \Vert y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \Vert_T, \quad \forall t \in [0:T].
%     \end{align*}
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{prop:LocLipReg_OptimFilter_Path}}
% % \begin{proof}[{Proof of Lemma~\ref{prop:LocLipReg_OptimFilter_Path}}]
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a non-negative constant $\bar{K} < \infty$ satisfying the following for every pair of paths $y^{(1)}_{\cdot},y^{(2)}_{\cdot} \in C([0:T],\|\cdot\|_2)$ and all time $t \in [0:T]$
%     \begin{multline*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%     \\
%         \leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{multline*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma}, there exists a non-negative constant $K < \infty$, satisfying
%     \begin{align*}
%         \begin{split}
%                 \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%             & \leq
%                 K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \\ 
%                 \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%             & \leq
%                 K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%         \end{split}
%         \qquad \forall t \in [0:T]
%     \end{align*}
%     Therefore, for each $y_{\cdot}^{(1)},y^{(2)}_{\cdot}\in C([0:T],\mathbb{R}^{d_Y})$ we have  
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t,
%         \qquad \forall t \in [0:T]
%     \end{align*}
%     and the statement follows. 
% \end{proof}


% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]
% \label{lem:LipschitzMu}
%     Under \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous uniformly in time. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}  
%             \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%         \leq
%             K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t,
%         \qquad \forall t \in [0:T].
%     \end{align*} 
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzMu}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzMu}}]
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) 
%    - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\top}}(s, y_{[0:s]}) ] \label{id:Phi1} \\ 
%  & \hspace{3cm} \times  (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \notag \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\top}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu} and for $t \in [0,T]$, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0:s]}) d y_{[0:s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align*}
%     \mu^{(1)}_t - \mu^{(2)}_t 
% & =   
%         \mu_0^{(1)} - \mu_0^{(2)} 
%     + 
%         \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \\
%     & \quad +   
%         \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0:s]}
%     - 
%         \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \\
%     & \quad +
%         \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds
%     +
%         \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\, (\mu^{(1)}_s - \mu^{(2)}_s ) ds .
% \end{align*} 
% By the triangle inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0:s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} \\ 
%   & + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwall's inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz with constant $K_1 < \infty$,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K_1 \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K_1 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K_2^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$ uniformly in time with constant $K_2 < \infty$, given by \Cref{lem:LipschitzPhi2}. Next, let $\lbrace [s_{i-1}:s_{i}] \vert i \in \myset{1}{I}\rbrace$, $I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K_2^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K_2^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K_2\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Integrating by parts, we find that
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         \notag \\
%     & \pushright{- \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2} \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         \notag \\
%     & \pushright{+ \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2} \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq T} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% \Cref{lem:LipschitzPhi2} yields (time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:T]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 =: K_3 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ uniformly in time with constant $K_4 < \infty$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 \\
%     & \leq \epsilon_I + K_4 t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that 
% \begin{align*}
% \eqref{t:gammaB} \leq \left(K_2 \sqrt{T} + K_3 + K_4 T\right) \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t.
% \end{align*}
% Next, we consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K_5 t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to (path-)Lipschitz continuity of $\Phi_1$ uniformly in time with constant $K_5$ which is obtained by \Cref{lem:LipschitzPhi1}. We conclude, since $\max_{s \in [0:T]} \|\mu^{(2)}_s \|_2 := K_6 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\gamma(t) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ with $K := K_1 + K_2 \sqrt{T} + K_3 + K_4 T + K_5 K_6 T$.

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \notag \\
%         & \pushright{\left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)}
%      \notag  
% \end{align} 
% Note that $\Phi_1$ is (time-)Lipschitz continuous, as shown in \Cref{lem:LipschitzPhi1}, therefore implying that $\max_{s \in [0:T]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$. As constants $K_1$, $K_2$, $K_3$, $K_3$, $K_4$, $K_5$, and $K_6$ were chosen independently of $t \in [0:T]$ and \Cref{ass:technical_evolution_conditions} \ref{asm:Regularity__LipInit} holds, we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}


% \begin{lemma}\label{lem:LipschitzPhi1}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists a constant $C\ge 0$ such that for all $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:T]} - y^{(2)}_{[0:T]} \|_T < \epsilon$, and times $t \in [0:T]$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq C \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzPhi1}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzPhi1}}]
% \begin{enumerate}[wide]
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component uniformly in time. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) uniformly in time, this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $C\ge 0$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq C \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $C\ge 0$, such that for all $\epsilon > 0$,  paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $t \in [0:T]$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq C \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzPhi2}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzPhi2}}]
%     \begin{enumerate}[wide]
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%     Under \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous uniformly in time. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $C \in \R$ such that for all $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $t \in [0:T]$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq C \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left-hand side refers to the Frobenius norm.
% \end{lemma} 
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzSigma}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzSigma}}] 
% From \eqref{id:ClosedFormSigma} and for $t \in [0:T]$, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
%         \Sigma_t
%     =
%         & \Sigma_0 + \int_0^t
%                 a_1(t,y_{[0:s]}) \Sigma_s
%             +
%                 \Sigma_s a_1^{\top}(s,y_{[0:s]})
%             +
%                 (b\circ b)(s,y_{[0:s]}) \hspace{3cm}
%             \notag\\
%                 &\pushright{- [
%                     (b\circ B)(s,y_{[0:s]})
%                 +
%                     \Sigma_s A_1^{\top}(s,y_{[0:s]})
%                 ]
%                 (B\circ B)^{-1} (s,y_{[0:s]}) } \hspace{1cm} \notag \\
%                 &\pushright{\times[
%                     (b\circ B)(s,y_{[0:s]}) 
%                 +
%                     \Sigma_s A_1^{\top}(s,y_{[0:s]})
%                 ]^{\top}
%         ds.} \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{multline*} 
% \Sigma^{(1)}_t - \Sigma^{(2)}_t
%  = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
%  + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \\
%  + 
% \Xi_2^\top (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{multline*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\top(s, y^{(1)}_{[0:s]}) - a_1^\top(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\top (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\top (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\top (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\top (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\top(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\top(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{multline} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef  a_1^\top(s, y^{(2)}_s) 
%  + A_1^\top(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]})  \\ 
%  \times(b\circ B) (s, y^{(1)}_{[0:s]})  
%  + A_1^\top(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
%  .   \label{Xi2} 
% \end{multline} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{multline} 
%     \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%     \leq  
%     \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%      \\ 
%   + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot  \\ 
%  \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \cdot \\ \cdot \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{multline}  
% From \Cref{lem:LipschitzA1}, we know that there exists a constant $K \in \R$ such that
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{multline}
%         \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
%     \leq  
%         \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big)  \cdot 
%         \\ 
%         \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 \cdot 
%         \\
%         \cdot \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{multline} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$ and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is uniformly bounded, according to \eqref{Xi2}. Therefore, from \eqref{Sigma1-2bddXi2} we obtain a constant $C \in \R$ such that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% C ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}
% We conclude the proof due to \Cref{ass:technical_evolution_conditions} \ref{asm:Regularity__LipInit}.
% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ there exists constant $K \in \R$, such that for all  $\epsilon > 0$, paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$, and times $s \in [0:T]$ holds
% \begin{align*} 
%          \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%      \leq
%          K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzA1}}
% % \begin{proof}[Proof of Lemma~\ref{lem:LipschitzA1}]
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component uniformly over all times, we conclude that $a_1$, $b \circ b$, $A_1^\top(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\top (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\top$ have the same property. By this, together with the triangular inequality, there exists a constant $K_1 \in \R$
%     \begin{align*}
%     &
%             \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  
%     \\& \quad
%         \leq  
%                 2K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) 
%             +
%                 K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2
%     \\ &
%             \pushright{
%             +
%                 K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s 
%             }
%     \\& \quad  
%         =
%             K_1 \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s
%             \Big(
%                     1
%                 +
%                     2 \Vert\Sigma^{(1)}_s \big\Vert_2
%                 +
%                     2 \Vert\Sigma^{(2)}_s \big\Vert_2 
%                 + 
%                     \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2
%             \Big).
%     \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < {K}_2$ for some $K_2 \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in the path-component and the closure of the set 
% \begin{align*}
%     \{y \in C^{1}([0:T]) \,:\, \Vert y_{[0:t]} - y^{(1)}_{[0:t]} \Vert_2 < \epsilon \}
% \end{align*}
% is compact, we know $\Vert\Sigma^{(2)}_s \Vert_2$ is bounded.
% \end{proof}

% \subsubsection{Lipschitz-Continuity in the Time-Component of the Optimal Filter}

% \begin{lemma}[Global Lipschitz-Cont. in the Time-Comp. of the Optimal Filter]
% \label{prop:LocLipReg_OptimFilter_Time}
%     \sloppy Under \Cref{ass:technical_evolution_conditions}, $f_t$ from \eqref{goal:Robust_Filtering} is locally Lipschitz-continuous in the time-component. In particular, for every path $y_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$, $t \in [0:T]$, and  $\epsilon > 0$ there exists constant $C \ge 0$ such that for all times $s \in [0:T]$ with $\| t - s \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]})) \leq C \vert t - s \vert.
%     \end{align*}
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{prop:LocLipReg_OptimFilter_Time}}
% % \begin{proof}[{Proof of Lemma~\ref{prop:LocLipReg_OptimFilter_Time}}]
%     As in the proof of \Cref{prop:LocLipReg_OptimFilter_Path}, we argue that by \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a non-negative constant $\bar{K} < \infty$ satisfying the following for every path $y_{\cdot} \in C([0:T],\|\cdot\|_2)$ and all times $t, s \in [0:T]$
%     \begin{multline*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]}))
%     \\
%         \leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}) - \mu(y_{[0:s]}) \|_2^2 + \|\Sigma(y_{[0:t]})-\Sigma(y_{[0:s]} \|_2^2}.
%     \end{multline*}
%     We see from \Cref{lem:TimeLipschitzMu} and \Cref{lem:TimeLipschitzSigma} that there exists a non-negative Lipschitz-constant $K < \infty$ for both $\mu$ and $\Sigma$ such that
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y_{[0:t]}), \mathbb{P}(X_s \in \cdot \vert y_{[0:s]})) \leq \sqrt{2}\bar{K}K \vert t - s \vert,
%     \end{align*}
%     and the statement follows. 
% \end{proof}


% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:TimeLipschitzMu}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:TimeLipschitzMu}}]
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{multline*}
%             \| \mu_t - \mu_s \|_2 
%         \\ \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0:u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0:u]})dy_{[0:u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0:u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{multline*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 \\
%         & \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwall's inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \le &
%             \overbrace{\Big\Vert \int_0^t a_0(u, y_{[0:u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0:u]})dy_{[0:u]} \Big\Vert_2}^{ \eqdef  \alpha(t)} \\
%           & + \int_0^t \big\Vert \Phi_1(u, y_{[0:u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0:s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0:u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0:u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}


% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__1} hold. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:TimeLipschitzSigma}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:TimeLipschitzSigma}}]
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\top}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\top}(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\top}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\top} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\top}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\top}(u,y_{[0:u]})^{\top} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \subsubsection{Lower Loewner order bound}

% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma} and \Cref{ass:technical_evolution_conditions} \ref{asm:Regulartiy__2}, \ref{asm:Regularity__3}, hold. Then there exists an $r > 0$, s.t. for all times $t \in [0:T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0:T], \R^{d_Y})$ holds that 
%     $\Sigma_t \preccurlyeq r I_d$. 
%     %$\Sigma_t - r \cdot I_{d_X}$ 
%     %is positive semi-definite.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LoewnerBound}}
% % \begin{proof}[{Proof of Lemma~\ref{lem:LoewnerBound}}]
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\top(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\top(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to $(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ being positive semi-definite at 
%     \begin{multline*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top ) \\
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\top
%                     \right)
%                 ds.
%     \end{multline*}
%     As $G_t(y_{[0:t]})$ is positive definite, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top
%                 (G_t(y_{[0:t]})^{-1})^\top
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\top
%             )
%     \end{align*}
%     and 
%     \begin{multline*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\top
%             \right)
%         \\ \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{multline*}
%     As we assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$ as well as $K_3 > 0$ s.t. $\tr(A_1^\top(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$ we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\top(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\top(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\top(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]




% \subsection{Stable and Lossless Encoding by Pathwise Attention - Proof of \texorpdfstring{\Cref{prop:Lossless_Encoding}}{Proposition 2}}
% \label{s:Proof__ss:Encoding}



% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(\rdim)}$ in $C([0:T],\mathbb{R}^{d_Y})$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[Stable Lossless Feature Maps -- Riemannian Case]
% \label{lem:Good_Feature_Map}
% \sloppy Under \Cref{ass:reg_compact} \ref{ass:reg_compact_riemann}, there exists a constant $C_{\ldim}>0$, depending only on $\ldim$, and a $\delta>0$ depending only on $(M,g)$ such that any $\delta$-packing $\{y^{(n)}\}_{n=1}^\ldim$ of $K$, there are matrices $A,B,b,V,U,C$ and vectors $a,b$ for which the parameter $\theta$, as in \Cref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim}$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim+1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0 \in \mathcal{O}(\edim^2)$.

% \noindent Moreover, if $(\mathcal{M},g)$ is aspherical then:
% \begin{enumerate}
%     \item[(i)] $\delta \in \mathcal{O}( \operatorname{Vol}(\mathcal{M},g)^{1/\ldim} )$
%     \item[(ii)] $\|\theta\|_0 \in \mathcal{O}(\edim^2)$,
%     \item[(iii)] $C_{\ldim}\in \mathcal{O}(\ldim^{3(\ldim+1)/2})$
%     % $0<C_{\ldim}< (3/5)\, (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}$.
%     % \item[(i)] $\|A\|_0=2N$, 
%     % \item[(ii)] $\|B\|_0=2N$, 
%     % \item[(iii)] $\|a\|_0=1$, 
%     % \item[(iv)] $\|b\|_0=0$, 
%     % \item[(v)] $\|C\|_0= N_1$, 
%     % \item[(vii)] $\|U\|_0=0$, 
%     % \item[(viii)] $\|V\|_0= N^2_1$,
%     % \item[(ix)] $0<C_{\ldim}< (3/5)\, (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}$.
% \end{enumerate}
% % \anastasis{perhaps I tally into a single parameter estimate} like $\|\theta\| \in \mathcal{O}(N^2)$.

% In particular, the attention mechanism $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any Borel probability measure $\mathbb{P}_{\mathrm{in}}$ on $K$.
% \end{lemma}

% \begin{proof}\textbf{of Lemma~\ref{lem:Good_Feature_Map}}\hfill
% % \begin{proof}[{Proof of \Cref{lem:Good_Feature_Map}}]\hfill
% \begin{enumerate}[label=\emph{Step \arabic*:}, ref=\arabic*, wide]
%     \item \label{step:GFM_1}\emph{Estimating $\rdim$ on the Riemannian Manifold $(\mathcal{M},g)$.}
% Since $(K,\|\cdot\|_T)$ be isometric to $(\mathcal{M},d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $\ldim$-dimensional Riemannian manifold $(\mathcal{M},g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $\mathcal{M}$ denoted by $\operatorname{sys}(\mathcal{M})$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(\mathcal{M}) 
%     \le
%     \,\tilde{C}_{\ldim}
%     \,
%         \operatorname{Vol}(\mathcal{M},g)^{1/\operatorname{dim}(\mathcal{M})}
%     ,
% \end{equation}
% where $\operatorname{Vol}(\mathcal{M},g)$ denotes the Riemannian volume of $(\mathcal{M},g)$ and $\tilde{C}_{\ldim}>0$ is a universal constant only depending on $\ldim$ satisfying
% \begin{align*}
%         0
%     <
%         \Tilde{C}_{\ldim}
%     <
%         6 (\ldim+1)\ldim^{\ldim}\,\sqrt{(\ldim+1)!}
% \,
% .
% \end{align*}
% By Stirling's approximation, $\sqrt{(\ldim+1)!} \in \mathcal{O}(\ldim^{(\ldim+1)/2})$; whence it follows that $\tilde{C}_{\ldim}\in 
% % \mathcal{O}(\ldim^{\ldim+1}\, \ldim^{(\ldim+1)/2})$
% \mathcal{O}(\ldim^{3(\ldim+1)/2})$.

% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(\mathcal{M})/10$ then given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(\mathcal{M},g)$, the map $\varphi_2:(\mathcal{M},d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{\ldim}\eqdef \tilde{C}_{\ldim}/10$ and $\rdim\eqdef \#\widetilde{\mathbb{X}}$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{\ldim}
%         \,
%         \operatorname{Vol}(\mathcal{M},g)^{1/\ldim}
%     .
% \]
% Enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^\rdim$.
% We note that if $K$ is not aspherical but if it is only isometric to a closed Riemannian manifold, then the conclusion still holds, however, without this explicit upper bound on $\delta$.
% \item \label{step:GFM_2} \emph{Building the Feature Map with Well-posed Inverse.}
% Let $\varphi_1:(\mathcal{M},d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have postulated to exist.  Set $\smash{\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^\rdim}$ where, for $n=1,\dots,\rdim$ we define $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\smash{\varphi: C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^\rdim}$ by $\smash{y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^\rdim}$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^\rdim
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\varphi_1(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^\rdim
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^\rdim
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^\rdim
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\varphi_1(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $\mathcal{M}$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $\rdim$-dimensional Euclidean space.

% \item \label{step:GFM_3} \emph{Aligning to a Hyperplane in $\mathbb{R}^{\sdim}$ with a Shallow ReLU Neural Network.}
% Set $\sdim \eqdef \rdim+1$.  Let $b$ be the zero vector in $\mathbb{R}^{2\rdim}$.
% We now consider a variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $\rdim \times 2\rdim$ and $2\rdim\times \rdim$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_\rdim & ~ -I_\rdim
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_\rdim \\
%             -I_\rdim
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^\rdim\rightarrow \mathbb{R}^\rdim$, with $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^\rdim$.  Consider the $\sdim\times \rdim$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{\sdim}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_\rdim \\
%             0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,\rdim\\
%             1 & \mbox{ if } i=\sdim
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2\rdim$, $\|B\|_0=2\rdim$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \item \label{step:GFM_4} \emph{Injectivity of Softmax Function on Hyperplane.}
% Note that, for each $u\in \mathbb{R}^\rdim$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^\rdim$ onto the $\rdim$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^\rdim\}$ in $\mathbb{R}^{\sdim}$.  Observe that the Softmax function, given for any $u\in \mathbb{R}^{\sdim}$ by $\smash{\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^\rdim\,e^{u_k})_{j=1}^\sdim}$, maps $H$ surjectively and continuously onto the image set 
% \begin{align*}
%     \operatorname{Softmax}(\mathbb{R}^{\sdim})\subseteq \operatorname{int}(\Delta_\sdim)\eqdef \Big\{v\in [0,1]^{\sdim}:\,\sum_{i=1}^{\sdim}\,v_i=1\Big\}; 
% \end{align*}
% i.e.\ of the interior of the $\sdim$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{\sdim}) + 1\big)_{i=1}^{\sdim}
% \end{equation}
% is a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{\sdim})$, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{\sdim})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$. 
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_\sdim)$ of the $\sdim$-simplex, then, 
% \begin{align*}
% 	 C^{\star}\eqdef \max_{u\in \Phi(K)}~\min_{v\in \Delta_{\sdim}\setminus \operatorname{int}(\Delta_{\sdim})}\,\|u-v\|>0.
% \end{align*}
%   Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{\sdim}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{\sdim})
%             +
%             \bar{\Delta}_{\sdim}
%         \}
% \]
% where $\bar{\Delta}_{\sdim}\eqdef (1/\sdim,\dots,1/\sdim)$ is the barycenter of the $\sdim$-simplex $\Delta_{\sdim}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{\sdim}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is locally Lipschitz on $\operatorname{int}(\Delta_\sdim)$, it is Lipschitz on the compact set $\Delta_{\sdim}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image since it is the composition of Lipschitz functions with Lipschitz inverses.  
% \item \label{step:GFM_5} \emph{Representation as an Attention Mechanism.}
% Set $\theta_0 = (A,B,a,b, \{y^{(n)}_{\cdot}\}_{n=1}^\rdim)$ and observe that the map $\Psi$ is of the form~\eqref{eq:sim_score}.  
% We continue by choosing a map of the form \eqref{eq:pos_encoding}. For this, let $\tdim \in \N$, set $\pdim \eqdef \sdim$ and let $U$ be the $\pdim \times \tdim$-dimensional zero matrix, and let $V$ be the $\pdim \times d_Y$-dimensional matrix whose entries are all equal to $1$.  Set $\theta_1\eqdef (U,V,\{n/{\pdim}\}_{n=1}^{\tdim})$.  Define the encoding dimension $\edim \eqdef \sdim$ and let $C$ be the $\edim \times \edim\cdot  d_Y$-dimensional matrix given by $Cx = (x_{n \cdot d_Y})_{n=1}^{\edim}$ for every $x\in \mathbb{R}^{\edim d_Y}$.  Set $\theta\eqdef (\theta_0,\theta_1,C)$ and observe that 
% \[
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot}) 
%     \eqdef
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
%     = 
%         \big(1_{[0:T]}\times \Psi\big)
%             (t,y_{\cdot})
% \]
% for each $y_{\cdot}\in K.$ and every $y\in [0:T]$. 
% Consequentially, $\operatorname{attn}_T^{\theta_{\cdot}}$ is a bi-Lipschitz embedding of $[0:T]\times K$ to $\mathbb{R}^{1 + \edim}$.  Note that $\|C\|_0= \pdim$, $\|U\|_0=0$, and $\|V\|_0= \pdim d_Y$.  Thus, $\|\theta\|_0\in \mathcal{O}(\pdim \cdot d_Y + \rdim)$.
% \end{enumerate}
% This concludes the proof.
% \end{proof}

% \begin{lemma}[Stable Lossless Feature Maps -- Finite Case]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under \Cref{ass:reg_compact} \ref{ass:reg_compact_finite} and let $\rdim \eqdef \#K$.  
% Set $\edim=192\lceil\log(\rdim)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There is a parameter $\theta$ as in \Cref{defn:PathAttention} defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim}$ which restricts to a $(2^{-1/2},(3\rdim/6)^{1/2})$-bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{1+\edim},\|\cdot\|_2)$.

% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer}. 
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:Good_Feature_Map__FiniteVariant}}
% % \begin{proof}[{Proof of~\Cref{lem:Good_Feature_Map__FiniteVariant}}]
% We argue similarly to the proof of \Cref{lem:Good_Feature_Map}, with only Steps \ref{step:GFM_1} and \ref{step:GFM_2} of its proof being replaced with the following argument.  
% \begin{enumerate}[label=\emph{Step \arabic*:}, ref=\arabic*, wide]
% \item[\emph{Steps 1-2}] \textit{(Modified): Building the Feature Map.}\hfill\\
% Enumerate $\smash{K=\{x_n\}_{n=1}^\rdim}$.  The map $\smash{\phi_1:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^\rdim,\|\cdot\|_{\infty})}$ given for every $x\in K$ by $\smash{x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^\rdim}$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le \rdim^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^\rdim$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^\rdim,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^\rdim,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% Define $\sdim \eqdef \lceil48\,\ln(\rdim)\rceil$.
% By the Johnson-Lindenstrauss Lemma, with ``small'' constant given in the derivation of \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $4*48$ as opposed to $4*200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , exists a linear map $\phi_3:(\mathbb{R}^\rdim,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\sdim},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $\sdim \times \rdim$-matrix $A_0$, satisfying: For every $u,v\in \mathbb{R}^\rdim$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, the map $\varphi:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^{\sdim},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3\rdim/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_T
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         \rdim^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3\rdim/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_T 
% .
% \end{align*}
% \item[\emph{Remaining Steps.}]
% % \textit{Remaining Steps}\hfill\\
% The rest of the proof is identical to Steps \labelcref{step:GFM_3,step:GFM_4,step:GFM_5}\footnote{Here $\sdim$ corresponds to $\sdim - 1$ in Step \ref{step:GFM_3}.} of the proof of \Cref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_\sdim\, \,I_\sdim)^{\top}$.
% \end{enumerate}
% This concludes the proof.
% \end{proof}


% \begin{lemma}[Stable Lossless Feature Maps -- Linear Case]
% \label{lem:biLip_pw_lin}
% Fix $\pldim \in \mathbb{N}_+$, $0=t_0<\dots<t_\pldim=T$, and a constant $C_K>0$.
% Let $K\subset C([0:T],\mathbb{R}^{d_Y})$ satisfy \Cref{ass:reg_compact} \ref{ass:reg_compact_linear}. 
% Then, there is a parameter $\theta$, as in \Cref{defn:PathAttention}, defining a pathwise attention mechanism $\operatorname{attn}_T^{\theta}:C([0:T],\mathbb{R}^{d_Y})\rightarrow \mathbb{R}^{\edim + 1}$, with $\edim \eqdef \pldim \cdot d_Y$ which restricts to a bi-Lipschitz embedding of $(K,\|\cdot\|_T)$ into $(\mathbb{R}^{\edim + 1},\|\cdot\|_2)$.
% Furthermore, $\|\theta\|_0\in \mathcal{O}(\pldim \cdot d_Y)$.

% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:biLip_pw_lin}}\hfill\\
% % \begin{proof}[{Proof of \Cref{lem:biLip_pw_lin}}]
% Let $\rdim \in \N_+$, set $\sdim \eqdef \pldim$, and define $A, B$ as zero-matrices as well as $a, b$ as zero-vectors according to the dimensions in \Cref{defn:Sim_Score}.
% By fixing $\theta_0=(A,B,a,b)$, we observe that 
% \begin{align}
% \label{eq:bijection_samplingA}
%     \operatorname{sim}_T^{\theta_0}(y_{\cdot}) = 1 \in \R^{\pldim}
% \end{align}
% for all $y\in C([0:T],\mathbb{R}^{d_Y})$.  

% Set $\tdim \eqdef \pdim \eqdef \pldim$. Then, let $V$ be the zero matrix and $U$ the identity matrix according to the dimensions in \Cref{defn:PositionalEncoding}\footnote{The point $t_0$ is not sampled since every path $y_{\cdot}$ in $K$ satisfies $y_0=0$ and, thus, there is no need to sample it at time $0$.}. Set $\theta_1=(U,V,\{t_n\}_{n=1}^\pldim)$ and with that, 
% \begin{equation}
% \label{eq:bijection_samplingB}
%         \operatorname{pos}_T^{\theta_1}(y_{\cdot})
%     =
%         (y_1,\dots,y_\pldim).
% \end{equation}
% In particular, the map $\operatorname{pos}_T^{\theta_1}$ in \eqref{eq:bijection_samplingB} defines a linear bijection between $K$ and the set $B_{C_K}(0)^\pldim$, where $B_{C_K}(0) := \lbrace z \in \R^{d_Y} : \vert z \vert \leq C_K\rbrace$.  Since $B_{C_K}(0)^\pldim$ is a subset of the finite-dimensional Banach space $(\mathbb{R}^{\pldim \times d_Y},\|\cdot\|_2)$ and all norms on a finite-dimensional normed are equivalent, then, $\operatorname{pos}_T^{\theta_1}$ is a bi-Lipschitz embedding of $K$ into $(\mathbb{R}^{\pldim \times d_Y},\|\cdot\|_2)$.  

% Fix $\edim \eqdef \pldim \cdot d_Y$ and let $C$ be the $\edim \times \edim$-dimensional matrix with $C_{i,j}=1$ for $i,j=1,\dots,\edim$.  Set $\theta=(\theta_0,\theta_1,C)$.  By construction $\|\theta\|_0\in \mathcal{O}(\pldim \cdot d_Y)$.  
% Then, 
% \begin{equation}
% \label{eq:bijection_sampling__RelabelingStuff}
%         \operatorname{attn}_T^{\theta}(t,y_{\cdot})
%     \eqdef 
%         \Big(
%                 t
%             ,
%                 C\,
%                 \operatorname{vec}\big(
%                         \operatorname{sim}_T^{\theta_0}(y_{\cdot}) 
%                     \odot
%                         \operatorname{post}_T^{\theta_1}(y_{\cdot})
%                 \big)
%         \Big)
%     =
%         \big(t,(y_1,\dots,y_\pldim)\big)
%     .
% \end{equation}
% Together, \labelcref{eq:bijection_samplingA,eq:bijection_samplingB} imply that $\operatorname{attn}_T^{\theta}$ defines a bi-Lipschitz embedding of $K$ into the $\edim+1$-dimensional Euclidean space.
% \end{proof}

% \begin{proof}\textbf{of \Cref{prop:Lossless_Encoding}}\hfill\\
% % \begin{proof}[{Proof of \Cref{prop:Lossless_Encoding}}]
% Follows directly from \Cref{lem:Good_Feature_Map,lem:Good_Feature_Map__FiniteVariant,lem:biLip_pw_lin}.
% \end{proof}

% \subsection{Approximability of Locally Lipschitz Maps By DKFs - Proof of \texorpdfstring{\Cref{prop:Universal_Approximation_Theorem__PathToNd}}{Proposition 4}}
% We now prove our main universal approximation theorem, \Cref{prop:Universal_Approximation_Theorem__PathToNd}.  We show that the target space/codomain of any considered DKF is geometrically regular, in the sense of \cite{Acciaio2022_GHT,kratsios2023transfer}.  Using this fact, we then combine and apply the results of \cite{kratsios2021universal,kratsios2023transfer} to deduce the result.

% \subsubsection{Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}

% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d_X \in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d_X}$ denote the set of $d_X\times d_X$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d_X\times d_X$ matrices.\footnote{The $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d_X}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.}  Consider the $2$-product metric on $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ given for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d_X+d_X^2}\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ by sending any $(m,A)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ quantizes $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})^{N} \rightarrow 
% \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d_X^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is a barycentric QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:QAS_Space_Sym0d}}\hfill\\
% % \begin{proof}[Proof of \Cref{lem:QAS_Space_Sym0d}]  
% We begin by showing that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% % \begin{itemize}
%     % \item[\emph{QAS Space Structure.}]
% \hfill\\
% \textit{QAS Space Structure}
% \hfill\\
% Since $\operatorname{Sym}_{0,d_X}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ is a closed and convex subset of the normed linear space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ as sending any $(m,A)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         & d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big) \\
%     \notag
%     & \quad = 
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     & \quad = 
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     & \quad \le
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     & \quad \le
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     & \quad = 
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $\smash{(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F},\mathcal{Q},\eta)}$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     % \item[\emph{Barycentricity.}]
% \hfill\\
% \textit{Barycentricity}
% \hfill\\
% Since $(\mathbb{R}^{d_X}\times \operatorname{Sym}_d,d_{2,F})$ is a normed linear space then \cite{BruHeinicheLootgieter1993} shows that the only contracting barycenter map is given by $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{d},d_{2,F})\ni \mathbb{P}\rightarrow \mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{d}$. 
% Since $\operatorname{Sym}_{0,d_X}$ is a closed convex subset of the normed linear space $\operatorname{Sym}_d$ then Jensen's inequality, as formulated in \citep[Theorem 10.2.6]{DudleyRealAnalysisandPRobabilityBook1989Revised2002}, implies that for each $\mathbb{P}\in \mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ we have $\mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$; where $\mathbb{E}_{X\sim \mathbb{P}}[X]$ denote the Bochner integral of a random variable with law $\mathbb{P}$.  Consequentially, 
% $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})\ni \mathbb{P}\rightarrow \mathbb{E}_{X\sim \mathbb{P}}[X]\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ is a contracting barycenter map.  Thus, $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is barycentric metric space.

% Since is a barycentric QAS space then, \citep[Setting 3.6 (iii)]{kratsios2023transfer} is satisfied.
% \end{proof}

% We are now ready to prove the following result, as we have established the barycentricity and the QAS space structure of $(\mathbb{R}^{d_X}\times\operatorname{Sym}_{0,d_X}, d_{2,F},\eta,\mathcal{Q}_{\cdot})$, 
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying \Cref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^{d_X})$ satisfying \Cref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:[0:T]\times K \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ there is a map $\hat{g}: [0:T]\times C([0:T],\mathbb{R}^{d_Y}) \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ satisfying the uniform estimate
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K}\,
%         d_{2,F}(\hat{g}(t,y_{\cdot}),f(t, y_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{g}(t, y_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^\ddim\,
%                 P_{\Delta_\ddim}(\hat{f}\circ \operatorname{attn}^\theta(t, y_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $\ddim \in \mathbb{N}_+$, $m^{(1)},\dots,m^{(\ddim)}\in \mathbb{R}^{d_X}$, $A^{(1)},\dots,A^{(\ddim)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_\ddim}:\mathbb{R}^\ddim\rightarrow\Delta_\ddim$ is the Euclidean (orthogonal) projection onto the $\ddim$-simplex, and an MLP $\hat{f}:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with activation function $\sigma$.  The depth, width, encoding dimension ($\edim$), and decoding dimension ($\ddim$) are recorded in \Cref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{\ldim}\operatorname{Vol}(M,g)^{1/\ldim})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \scriptsize
%     \caption{{Complexity Estimates for transformer-type model $\hat{g}$ in \Cref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode ($\edim$) & Decode ($\ddim$)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-\edim-1}\,\varepsilon^{-\edim-1}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-\edim-1}\,\varepsilon^{-\edim-1}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4\edim+5}\, \varepsilon^{-4\edim-5}
%         \right)
%          $
%          &
%          $ \mathcal{O}(L\epsilon^{-1} + \edim +3)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8\edim+14}\, \varepsilon^{-8m-14} %m=(\edim-1)
%         \big)
%          $
%          & 
%          $\mathcal{O}(L\epsilon^{-1} + \edim +4)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $\mathcal{O}(L\epsilon^{-1} + \edim +3)$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}\textbf{of Lemma~\ref{lem:approximation_Sym}}\hfill\\
% % \begin{proof}[{Proof of \Cref{lem:approximation_Sym}}]
% %\anastasis{Relabel $N$ (index) as $M$}
% %\hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% Our objective is to apply \citep[Theorem 3.7]{kratsios2023transfer} by verifying each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \begin{enumerate}[label=\emph{Step \arabic*:}, wide]
%     \item \emph{Implementing a Bi-Lipschitz Feature Map with the Attention Layer.}
%         \begin{remark}
%             We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap}  can be chosen such that $\operatorname{attn}^\theta$ is a suitable feature map.  
%         \end{remark}

%         When convenient, let $\operatorname{attn}^{\theta}$ be as in either of \Cref{lem:Good_Feature_Map,lem:Good_Feature_Map__FiniteVariant,lem:biLip_pw_lin} depending on which assumption of Assumptions~\ref{ass:reg_compact} (i), (ii), or (iii) holds.  For convenience, we denote the map $\operatorname{attn}$ by $\varphi$.  These lemmata show that the map $\varphi$ is a bi-Lipschitz embedding of $([0:T]\times K,\|\cdot\|\times \|\cdot\|_T)$ into a Euclidean space $(\mathbb{R}^N,\|\cdot\|_2)$.
    
%         We also observe that every bi-Lipschitz map is a quasi-symmetric map\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.  Thus, \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(\mathcal{M},d_g)$ is a doubling metric space, as defined on \citep[page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  Thus, $([0:T]\times K,\|\cdot\|\times \|\cdot\|_T)$ is a doubling metric space.  We have thus verified \citep[Setting 3.6 (i)]{kratsios2023transfer}.
%     \item \emph{Feature Space Geometry.}
%         Since the codomain of $\phi$ is simply a Euclidean space, then, the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^{\edim+1}}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^{\edim+1}$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^{\edim+1}$, 
%         \[
%             \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
%         \]
%         and the operator norm $\|1_{\mathbb{R}^{\edim+1}}\|_{\mathrm{op}}=1$. Thus, $(T^i)_{i\in \mathbb{N}}$ implements the $1$-BAP ($1$-bounded approximation property) on $\mathbb{R}^{\edim+1}$ for every $i$.  Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} holds.

% \item \emph{Geometry of $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$.}
% \Cref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},\mathcal{Q},\eta)$ is barycentric and it is a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $\ddim \in\mathbb{N}_+$, $u\in \mathbb{R}^\ddim$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(\ddim)})\in \mathbb{R}^{d_X}\times \mathbb{R}^{d_X^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^\ddim
%     \big)
%         \eqdef 
%             \sum_{n=1}^\ddim\,
%                 P_{\Delta_\ddim}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \item \emph{Determining The Euclidean Universal Approximator.}
% \begin{remark}
%     We now verify that the class of all MLPs with activation function $\sigma$ satisfying \Cref{ass:KLCondition}, thus assumption \citep[Setting 3.6 (iv)]{kratsios2023transfer} holds.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.
% \end{remark}
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $\edim,\ddim,c\in \mathbb{N}_+$ let $\mathcal{F}_{\edim, \ddim, c}$ denote the family of maps $f:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le \edim+\ddim+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy \Cref{ass:KLCondition} then by \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $\edim,\ddim,c\in \mathbb{N}_+$ let $\mathcal{F}_{\edim,\ddim,c}$ denote the family of maps $f:\mathbb{R}^\edim\rightarrow \mathbb{R}^\ddim$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \item \emph{Applying \citep[Theorem 3.7]{kratsios2023transfer}.}
% Steps $1$ though $5$ verify that the conditions of \citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the feature decomposition $\{([0,T]\times K,\varphi)\}$ of $([0,T]\times K,\|\cdot\|_T)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, by~\citep[Lemma 5.10]{kratsios2023transfer} for every $\varepsilon>0$ there is a map $\hat{F}:[0,T]\times K\rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{F}(y_{\cdot})
%     = &
%         \beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot}),(Z_n)_{n=1}^\edim)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot}),(Z_n)_{n=1}^\edim)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^\ddim
%             \,
%                 \big(
%                     P_{\Delta_\ddim}\circ \hat{f}_n\circ \phi(y_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $y_{\cdot}\in K$ satisfying 
% \[
%     \sup_{y_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{F}(y_{\cdot})
%         ,
%             f(y_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\smash{\beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ (which exists by \Cref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}}$ is a right-inverse of the map $\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})$, where $\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially, \labelcref{eq:transformer_pre_mapped_BEGIN,eq:transformer_barycentercancellation,eq:transformer_pre_mapped_END} reduces to \eqref{lem:approximation_Sym__approximation___representation}.  


% \item \emph{Tallying Parameters.}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $\edim=\mathcal{N}_{\operatorname{pack}}\big(K,C_{\ldim}\,\operatorname{Vol}(\mathcal{M},g)^{1/\ldim}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in \Cref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $\ddim$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             \ddim
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{enumerate}
% This concludes the proof.
% \end{proof}

% \subsubsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool, namely, \Cref{prop:Universal_Approximation_Theorem__PathToNd}.   
% %\begin{figure}[H]
% %    \centering
% %    \begin{tikzcd}
% %\big(C([0:T],\mathbb{R}^d), %\|\cdot\|_{\infty}\big) & %(\mathcal{P}_2(\mathbb{R}^d),
% %\mathcal{W}_2) \\
% %    (K,\|\cdot\|_{\infty}) 
% % \arrow[hookrightarrow{u}
% %{\iota} 
% %    \arrow{r}{f, \hat{t}} 
%     % \arrow[swap]{d}{\varphi} 
% %    \arrow{dr}{\varrho\circ f}
% % & ({\mathcal{N}}_d,
% %\mathcal{W}_2) 
% %   \arrow[hookrightarrow]{u}{i}
% %    \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
% %    & (\mathbb{R}^d\times \operatorname{Sym}_{0,d_X},\|\cdot\|\times \|\cdot\|_F)
% %    \end{tikzcd}
% %    \caption{Visual summary of the relationship between the spaces appearing in the proof of Proposition 4.}
% %\label{fig:Approximation_Theorem}
% %\end{figure}

% \begin{proof}\textbf{of \Cref{prop:Universal_Approximation_Theorem__PathToNd}}\hfill
% % \begin{proof}[{Proof of \Cref{prop:Universal_Approximation_Theorem__PathToNd}}] \hfill
% \begin{enumerate}[label=\emph{Step \arabic*:}, wide]
% \item \emph{Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$.}
% By \Cref{lem:LipschitzManifold_Nd}, the map $\varrho:(\mathcal{N}_{d_X},\mathcal{W}_2)\rightarrow (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^{d_X},\operatorname{Sym}_{0,d_X},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d_X},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous, then the map
% \[
%     g: ([0,T]\times K, 
%     | \cdot | \times \|\cdot\|_T)\ni (t,y_{\cdot}) \mapsto 
%     \pi\circ \varrho\circ f(t,y_{\cdot})
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d_X},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d_X \times d_X$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; by which we mean that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_{d_X}$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% By \Cref{lem:LoewnerBound}, we have that there is an $r>0$ such that $r=\lambda_{\operatorname{min}}(\Sigma_t)$ for all $0\le t\le T$. 
% Consequentially, \Cref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_{d_X},\mathcal{W}_2)\rightarrow (\mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \item \emph{Approximating $\varrho \circ f$ on $K$.}
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%     \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
%                     }}
%         \biggr\}
% .
% \end{equation}

% We apply \Cref{lem:approximation_Sym} to deduce that there exists a map $\hat{F}: [0:T]\times K \rightarrow \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K }\,
%         d_{2,F}(\hat{F}(t, y_\cdot),\varrho\circ f(t,y_\cdot))
%     <
%         \delta
% .
% \end{equation}
% Since \Cref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  
% Consider the $1$-thickening of $\varrho\circ f(K)$ defined by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^{d_X}\times \operatorname{Sym}_{0,d_X}:\,(\exists (t,y_{\cdot} )\in [0:T]\times K )\, d_{2,F}(f(t, y_\cdot),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{F}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate} and \Cref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     & \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         \mathcal{W}_2\big(
%                 \rho^{-1}\circ F(t,y_{\cdot})
%             ,
%                 f(t,y_{\cdot})
%         \big)
% \\
% \nonumber
% = & 
%     \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{F}(t,y_{\cdot})
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(t,y_{\cdot})
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{(t,y_{\cdot})\in [0:T]\times K}\,
%         d_{2,F}\big(
%                 \hat{F}(t,y_{\cdot})
%             ,
%                 \varrho\circ f(t,y_{\cdot})
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
% \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
%     }
%     }
% \\
% % \label{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% % \le &
% %     \sqrt{d}2\sqrt{
% %             L
% %     \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
% %         }
% %     \,
% %     \varepsilon
% %     \,
% %     \frac1{
% %     \sqrt{d}2\sqrt{
% %         L
% % \,\sqrt{T^2+\operatorname{diam}(K)^2} + 1
% %     }
% %     }
% % \\
% \label{eq:Approxim_LEMMA__END}
% \le & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from \Cref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:Approxim_LEMMA__END} followed from the estimate~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho} for $\operatorname{Lip}( \varrho^{-1}  | \bar{B}_1 )$.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009} then, the estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% %\label{eq:Approxim_LEMMA__BEGIN}
%     \max_{(t,y_{\cdot}) \in [0:T]\times K}\,
%         \mathcal{W}_p\big(
%                 \hat{F}(t,y), f(y)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \item \emph{Counting Parameters.}
% Using $\delta$, as defined in~\eqref{eq:prop:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in \Cref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \end{enumerate}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_{d_X}}$ denote the set of Gaussian measure on $\mathbb{R}^{d_X}$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_{d_X}}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_{d_X}}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_{d_X}},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_{d_X}}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of \Cref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_{d_X}}$ sending any $(m,A)\in \mathbb{R}^{d_X}\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_{d_X}}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_{d_X}}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_{d_X}}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_{d_X}}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_{d_X}}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_{d_X}},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_{d_X}}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_{d_X}}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}


% \appendix
% \section{An Auxiliary Lemma - I.\ Pinelis}
% \label{s:AuxLemmata}
% This section records an auxiliary lemma due to Iosif Pinelis, \cite{LocalLipschitz_Pinelis}.  We include the result and its proof here to keep our manuscript self-contained.  
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% then the following lower-bound holds
% \begin{align*}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     .
% \end{align*}
% Moreover, the following upper-bound also holds
% \begin{align*}
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{align*}
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}\textbf{of Lemma~\ref{lem:LipschitzManifold_Nd}}\hfill\\
% % \begin{proof}[{Proof of \Cref{lem:LipschitzManifold_Nd}}]
% By \citep[Proposition 7]{GivensShortt_ClassofWassersteinMetricforProbDists_1984} the $2$-Wasserstein distance between $\mathcal{N}(m^{(1)},A)$ and $\mathcal{N}(m^{(2)},B)$ satisfies
% \begin{equation*}
% 	\mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B))=\sqrt{\|m^{(1)}-m^{(2)}\|^2+W_2(\mathcal{N}(0,A),\mathcal{N}(0,B))^2}.
%  \label{10}
% \end{equation*}
% Thus, $\|m^{(1)}-m^{(2)}\|\le \mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B))$.  Moreover, for any unit vector $u\in\R^n=\R^{n\times1}$ we have
% \begin{align*}
% 	\mathbb{E}_{X\sim \mathcal{N}(0,A),\,Y\sim \mathcal{N}(0,B)}\|X-Y\|^2
%     \ge &
%         \mathbb{E}_{X\sim \mathcal{N}(0,A),\,Y\sim \mathcal{N}(0,B)}(u^\top X-u^\top Y)^2
%     \\
%     \ge& 
%         (\sqrt{u^\top A u}-\sqrt{u^\top B u})^2,
% \end{align*}
% where the last inequality holds since $u^\top X$ and $u^\top Y$ have Gaussian law with zero-mean random with respective variances $u^\top A u$ and $u^\top B u$.
% Again using the inequality $\|m^{(1)}-m^{(2)}\|\le \mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B))$, for any unit vector $u\in\R^n=\R^{n\times1}$, we have
% \begin{equation*}
% \begin{aligned}
% 	\mathcal{W}_2(\mathcal{N}(a,A),\mathcal{N}(b,B))&\ge \mathcal{W}_2(\mathcal{N}(0,A),\mathcal{N}(0,B)) \\ 
% 	&\ge|\sqrt{u^\top A u}-\sqrt{u^\top B u}| \\ 
% 	&=\frac{|u^\top A u-u^\top B u|}{\sqrt{u^\top A u}+\sqrt{u^\top B u}} \\ 
% 	&\ge\frac{|u^\top(A-B)u|}{\sqrt{\|A\|}+\sqrt{\|B\|}} \\  
% 	&=\frac{\|A-B\|}{\sqrt{\|A\|}+\sqrt{\|B\|}} 
% \end{aligned}
% \end{equation*}
% for some unit vector $u\in\R^n=\R^{n\times1}$, where $\|M\|$ is the spectral norm of a matrix $M$. 
% So, 
% \begin{equation*}
% 	\|A-B\|\le(\sqrt{\|A\|}+\sqrt{\|B\|\,})\, \mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B)). \label{30}
% \end{equation*}
% The conclusion follows upon combining $\|m^{(1)}-m^{(2)}\|\le \mathcal{W}_2(N(m^{(1)},A),N(m^{(2)},B))$ and 
% $\|A-B\|\le (\sqrt{\|A\|}+\sqrt{\|B\|}) \mathcal{W}_2(\mathcal{N}(m^{(1)},A),\mathcal{N}(m^{(2)},B))$ together with the observation that $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$; where 
% \[
% \|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})
% \]
% denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}


% % \bibliographystyle{imsart-number} 
% \bibliography{Bookkeaping/2_References}


% \end{document}




==> OLD/OLD_DRAFT.tex <==
% % Zoom link:
% % https://mcmaster.zoom.us/j/2601491351


% %% 
% %% Copyright 2007-2020 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% \documentclass[preprint,12pt,authoryear]{elsarticle}
% \usepackage{amssymb}

% \journal{Stochastic Processes and Their Applications}

% % % SCIMODS_Wrapped_2022
% % \documentclass[11pt]{article}


% \usepackage[utf8]{inputenc}
% % \usepackage[10pt]{extsizes} % <- Override Spring Size


% \input{Bookkeaping/1_mathcommands}
% \usepackage{natbib}



% \begin{document}

% \begin{frontmatter}
% % \title{Universality of Continuous-Time Deep Kalman Filters}
% % \title{Continuous-Time Deep Kalman Filters which are Universal Filters}
% \title{Deep Kalman Filters Approximate Conditionally Gaussian Filters}

% % \author[inst1]{Matheus Grasselli}
% \author[inst2,inst3]{Blanka Horvath}
% \author[inst1,inst4]{Anastasis Kratsios}
% \author[inst2,inst3]{Yannick Limmer}
% \author[inst1]{Xuwei Yang}


% \affiliation[inst1]{organization={Department of Mathematics, McMaster University},%Department and Organization
%             % addressline={Hamilton, Ontario}, 
%             city={Hamilton},
%             % postcode={00000}, 
%             state={Ontario},
%             country={Canada}}

% \affiliation[inst2]{organization={Department of Mathematics, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             state={Oxfordshire},
%             country={United Kingdom}}

% \affiliation[inst3]{organization={Oxford MAN Instute for Quantitative Finance, University of Oxford},
%             % addressline={Address Two}, 
%             city={Oxford},
%             % postcode={22222}, 
%             state={Oxfordshire},
%             country={United Kingdom}}
            
% \affiliation[inst4]{organization={Vector Institute},
%             % addressline={Address Two}, 
%             city={Toronto},
%             % postcode={22222}, 
%             state={Ontario},
%             country={Canada}}
            

% \begin{abstract}
% Deep Kalman filters (DKFs) form a broad class of neural network models which generate Gaussian probability measures; inspired by the discrete-time Kalman filter.  
% In this paper, we show that there are are DKFs which are generic conditionally Gaussian filters.  We do so by explicitly constructing a DKF model which can approximate the solution operator of a broad class of continuous-time stochastic filters, between a partially observed, conditionally-Gaussian, non-Markovian signal processes given the realized path a non-Markovian observation process.
% Our approximation guarantees are uniform over regular compact manifolds of paths.  We provide explicit parameter estimates depending on the dynamics and dimension of the signal and observation process as well as on the geometry of the compact set of paths over which the stochastic filtering problem's solution operator is approximated.  \hfill\\
% {\color{red} Numerical illustrations are used to validate our guarantees.}
% \end{abstract}


% \begin{keyword}
% %% keywords here, in the form: keyword \sep keyword
% Stochastic Filtering \sep Conditionally Gaussian Processes \sep Neural Networks
% %% PACS codes here, in the form: \PACS code \sep code
% % \PACS 0000 \sep 1111
% %% MSC codes here, in the form: \MSC code \sep code
% %% or \MSC[2008] code \sep code (2000 is the default)
% \MSC 60G35 \sep 62M45 \sep 68T07 \sep 65J22
% \end{keyword}

% \end{frontmatter}


% \section{Introduction}
% \label{s:Algorithm}
% \fbox{\begin{minipage}{0.8\textwidth}
%     \textbf{Structure of introduction.}

%     \begin{enumerate}
%         \item Opening.
%         \item What are Kalman filters? 
%         \item What are Deep Kalman Filters?
%         \item Exemplary applications of (D)KF in finance.
%         \item Universality: Limitations of existing results and extensions.
%         \item Structure of the article. 
%     \end{enumerate}

%     BH: This is great, this is exactly what I was thinking to do.
% I'd suggest to add or consider the following aspects:
% \begin{enumerate}
%     \item Opening
%     \item What are Kalman filters and what are traditional use cases of Kalman filters in finance (and beyond)
%     \item What are Deep Kalman Filters (when/how) and why did they become popular and what (were) limitations of Kalman Filters that can be resolved by Deep Kalman Filters?
%     \item What is the main result in this paper and why is it useful? Universality: Limitations of existing results and extensions.
%     \item This is what we don't do (re: training) but "this is why it is ok"...
%     \item Structure of the article.
% \end{enumerate}
% \end{minipage}
% }\\


% Literature surrounding applications of filtering in Mathematical Finance: \\
% For a general motivation for the geometric (also: information geometric) idea behind Filtering problems in typical applications in mathematical finance, see the excellent overview presented in the the recent work \href{https://arxiv.org/pdf/2205.01594.pdf}{Brigo (2022)} and the expose in \href{https://arxiv.org/pdf/1303.6236.pdf}{Armstrong and Brigo (2013)} as well as well-known early works \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}. A gentle introduction to typical linear and nonlinear filtering problems in mathamatical finance can be found in the review article \href{ura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{Date and Ponomareva (2010)} and for a comprehensive introduction to stochastic filtering we direct to the eteemed monograph \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)} as the reference literature.\\


% \anastasis{I would mention that there are at-least two sources of ``complexity'' to the general filtering problem: 1) The infinite-dimensionality of the set of all probability measures (complexity of representing conditional densities/measures) and 2) The complexity of the dynamics governing the solution of the signal, observation, and conditional dynamics.  \\
% I would then say some like Kalman filters simplify both, the general conditional Gaussian filters studied in \cite{LipShiryaev_II_2001} provide a theoretical foundations for filtering when (1) is resolved by considering conditionally Gaussian filters.  Then somehow relate that we work in (1), by developing a universal model class, in the conditionally-Gaussian framework based on the ideas of deep Kalman filtering.}

% \paragraph{Historical development:} 
% The filtering problem consists in estimating the state of a stochastic differential system
% from noisy observations. \\ 
% The general solution of the filtering problem at a given time is given by the probability density
% of the unperturbed state of the system at that time, conditional on the perturbed observations
% up to the given time. When the unobserved signal and the observed signal evolve in continuous
% time, the filter density follows a stochastic partial differential equation (SPDE), see \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)}. 
% If the dynamic evolution of the unobserved
% system is linear, the observations are linear, the noise terms are Gaussian\footnote{The initial condition of the
% unperturbed signal are also assumed to be Gaussian or deterministic.}, then this is a setting that leads to the celebrated \emph{Kalman-Bucy filter}:
% \\
% Indeed, in the linear Gaussian case the problem was solved in discrete-time by Rudolf Kalman, and later in continuous time in \cite{TBD}\anastasis{(Bucy Paper)},
% who introduced what is known today as the \emph{Kalman filter} (see next paragraph), a finite dimensional system of equations
% for the first two conditional moments of the state of the stochastic system, given the observations:
% In such a case, the filter is Gaussian and its density can
% be characterized by a finite dimensional set of parameters, namely the mean vector and variance-covariance matrix of the resulting Gaussian distribution,
% %\\In classical Kalman Filters, the evolution of this system (both observable and unobservable parts) are modelled as linear functions
% %perturbed by Gaussian noise.
% %In a linear setting 
% these equations determine the whole conditional density of the state of the system given the observations,
% as this (Gaussian) density is fully characterized by the first two moments. \\
%  For real world applications the assumption of a linear evolution of this system\footnote{I.e. transition and emission distributions.}
% limits the capacity to model complex phenomena, and modifications to the functional form of Kalman Filters
% have been proposed.
% \\
% As indicated above, 
% in the  general
% nonlinear case, the filtering problem is far more complex as it consists in computing the conditional density of the
% state given the observations. This density is the solution of a stochastic partial differential
% equation which is referred to as the \emph{Kushner-Stratonovich equation} and the resulting nonlinear filter is in general not finite dimensional\footnote{I.e. it does not evolve in a finite dimensional
% statistical manifold.}. A well
% known approximation method is the extended Kalman filter (EKF), in which one linearizes around
% the current estimate obtaining a locally linear system, and then applies the Kalman filter
% equations in this (linearised) neighbourhood. Traditionally, this procedure was usually justified by heuristic considerations.  
% Though more recent linear approximations have also been considered, e.g.\ in \cite{LukasJosef_LinearizedFiltering}.
% Another choice in the nonlinear case is the Gaussian assumed density filter (GADF),
% obtained by assuming the conditional density to be Gaussian\footnote{This is dangerous, because by assuming a false hypothesis one can deduce anything as well as its opposite.}, which yields a finite dimensional filter. %However, this approach depends heavily on conditional Gaussianity, which is not necessarily fulfilled in many real-life applications.\\
% We are universal in the conditional Gaussian class.\\
% Contrast it with neural SDEs (no hidden suff (ANASTASISSSS)

% Hanzon suggested to project the SPDE equation in Stratonovich form for the evolution of the filter density onto a finite dimensional statistical manifold, using the Fisher metric/Hellinger distance. We call this “Stratonovich projection” and it consists in projecting the separate vector
% fields of the SPDE corresponding to the drift and diffusion part of the Stratonovich version. The projected equation would describe a finite dimensional density evolution, called projection filter, approximating the full filter evolution associated with the optimal filter.\\
% In 1987, Hanzon (BH: reference missing) introduced the projection filter (PF), which is a finite dimensional nonlinear filter based on a differential geometric approach: The projection filter is obtained by projecting the Kushner-Stratonovich equation onto the tangent space
% of a finite dimensional manifold of probability densities, according to the Fisher information metric.\\
% Hanzon and Hut (1991) (BH: add ref) showed that if one projects onto the
% tangent space of the finite dimensional manifold of Gaussian densities, the resulting projection filter
% coincides with an assumed density filter which is obtained as follows: one computes the first two conditional moments equations in McShane-Fisk-Stratonovich (MFS) form, and then assumes the conditional density to be Gaussian, closing in this way the equations for the first two moments.   
% It was also proven in Hanzon and Hut (1991) that what we described above is in general not the same as assuming a Gaussian density in the It\^{o} equations for the first two moments and then transforming the obtained filter in MFS form.
% The equivalence between the MFS-based GADF and the Gaussian Projection Filter is very important when generalized to
% exponential families (see \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}), because it gives a simple characterization of the exponential projection
% filter (EPF) which is independent of geometric concepts. \\

% For a comprehensive but introductory review of linear and non-linear filterin applications in mathematical finance see: \href{https://bura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{P. Date and K. Ponomareva (2010)} among which we will highlight some simple but heavily used (Gaussian or near-Gaussian) use cases
% \begin{itemize}
%     \item In stochatic volatility modelling Kalman Filters have traditionally been used to estimate (and forecast) spot and realised volatility.
%     \item Monoyios in \href{https://people.maths.ox.ac.uk/monoyios/docs/ima_final.pdf}{Monoyios (2007)} develops a filtering approach with applications to (optimal) hedging, in which the hedger updates her parameter estimates from
% observations of the asset prices, and where he finds an analytic solution to the hedger’s combined filtering and
% control problem in the case that the drift of the traded asset is known with certainty.
% \item Filtering has been traditionally heavily used in linear Gaussian interest rate models. \href{}{}
%     \end{itemize}
    

% \paragraph{Kalman filters} At a high level, a Kalman filter operates by combining a model of a system with partial state-observations to estimate the current overall state of the system. The filter uses two primary steps to make these estimates: a prediction step and an update step.
% \begin{itemize}
%     \item In the prediction step, the Kalman filter uses the model of the system to predict the state of the system at the next time step. This prediction is based on the current estimate of the system state, as well as any known inputs or disturbances in the system. The Kalman filter uses a probabilistic approach to estimate the state of the system, this means the prediction includes both the expected value of the state as well as an estimate of the uncertainty or error in the prediction.
%     \item In the update step, the Kalman filter uses the actual observation to correct the predicted state estimate. The filter compares the distribution of the predicted state to the actual observed state (which acknowledges uncertainty and is perceived as a distribution itself). The filter then adjusts the state estimate based on this difference.
% \end{itemize}

% \paragraph{Deep Kalman filters} The term, ``deep Kalman filter'' (DKF) refers to deep learning models, that bolster the capacity of traditional Kalman filter by leveraging a neural network component. The neural network component is used to learn the probabilistic model of the underlying system dynamics, thus allowing DKFs to generically adapt to any situation in which the conditional evolution of the signal process is Gaussian.  This generic flexibility, of DKFs is what has lead to their empirical predictive edge over traditional Kalman filters \cite{TBD}.

% The neural network component in a DKF is typically used to model the transition function of the system, which describes how the state of the system evolves over time. The neural network takes as input the current state of the system, as well as any control inputs or disturbances, and outputs a probability distribution over the possible next states of the system. This distribution is then used to make a prediction of the next state, as well as an estimate of the uncertainty or error in the prediction. 

% The traditional Kalman filter components are then used to combine the neural network predictions with actual observations in order to update the state estimate. The neural network component in a DKF can be trained using a variety of techniques, such as maximum likelihood or Bayesian inference. The training process involves minimizing the error between the predicted state and the actual state, as well as minimizing the uncertainty in the predictions.

% \paragraph{Exemplary (existing) applications of (D)KF in finance}
% \begin{enumerate}
%     \item Sequential calibration of options
%     \begin{itemize}
%         \item Problem: The parameter estimates are noisy and old data are typically discarded, as only the most recent data are used.
%         \item As a solution, the calibration is formulated as a filtering problem.
%         \item The observable process consists of market option prices, spot, strike, interest, and maturity.
%         \item The unobservable process consists of the difference between the modelled option price and the denoted option price, as well as the difference of the model's parameters to the day before.
%         \item See \cite{LindstroemStroejbyBrodenWiktorssonHolst08}, extensions \cite{LindstroemWiktorsson14}
%     \end{itemize}
%     \item Computing VaR in a stochastic volatility model, see \cite{LindstroemMadsenNielsen16}
%     \item Filtering with bond prices, see \cite{LindstroemMadsenNielsen16}
%     \begin{itemize}
%         \item The observable process constitutes the prices obtained from solving the ``bond pricing equation''
%         \item The unobservable variables are the parameters of the estimated model and the implied interest rate (by bond prices, not quoted)
%     \end{itemize}
%     \item Calibration of term structure models of commodity prices \cite{JavaheriLautierGalli03}
%     \item Dynamic pricing (this is probably more economics than finance), see \cite{CohenTreetanthiploet22}
%     \item Besides state estimation in control systems, Kalman filters have found applications in financial markets for constructing trading strategies. Two common approaches involve using Kalman filters to:
%     \begin{itemize}
%         \item Identify Mean-Reverting Patterns: Kalman filters can be utilized to detect instances where asset prices deviate from their long-term average, indicating potential mean-reverting behaviour. Traders can then develop strategies that take advantage of these deviations, expecting prices to eventually return to their mean.
%         \item Identify Momentum-Based Trends: Kalman filters can also be employed to identify momentum-based trends in asset prices, indicating sustained movements in a particular direction. Traders can develop strategies to follow and capitalize on these trends.
%         \item \yannick{References missing.}
%     \end{itemize}
%     \item Portfolio Optimization with Kalman Filters and Multi-Asset Models:
%     \begin{itemize}
%         \item Kalman filters applied to optimize asset portfolios by considering individual asset dynamics and correlations.
%         \item Particularly beneficial for multi-asset portfolios.
%         \item Estimation of assets' covariance matrix using Kalman filters.
%         \item Portfolio optimization based on the covariance matrix while adhering to specified constraints.
%         \item \yannick{References missing.}
%     \end{itemize}
%     \item  Risk Management and Stress Testing with Kalman Filters:
%     \begin{itemize}
%         \item Utilization of Kalman filters for risk management and stress testing purposes.
%         \item Estimation of portfolio risk and identification of potential risk sources.
%         \item Modelling asset behaviour under various market scenarios using Kalman filters.
%         \item Assessment of the portfolio's vulnerability to the impact of these scenarios.
%         \item \yannick{References missing.}
%     \end{itemize}
% \end{enumerate}


% \begin{comment}
% \paragraph{Limitations and contribution} The results \cite{kratsios2021universal, Acciaio2022_GHT} show that, while it is possible to universally approximate the function used above with a class of transformer models, the required number of parameters to approximate the function at each state in time can depend highly non-favourably on the dimensions of the (observable and unobservable) state. In this work, we suggest to best approximate the function at all times by a class of non-Euclidean kernel regressors, trained on a finite set of observations. 
% \end{comment}


% \section{The Setting}
% \label{s:Preliminaries}

% This section formulates the theoretical problem which this paper addresses.
% Fix $T>0$ and let $(X,Y)_{\cdot}\eqdef (X_t,Y_t)_{0\le t\le T}$ be a stochastic process defined on a complete filtered probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ where $\mathbb{F}\eqdef (F_t)_{0\le t\le T}$ is a right-continuous filtration thereon.  Let $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$ be independent $\mathbb{F}$-adapted Brownian motions of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  

% Consider a pair of $\mathbb{F}$-adapted processes, called the recordable \textit{observation} process $Y_{\cdot}\eqdef (Y_t)_{0\le t\le T}$ and the unobservable \textit{signal} process $X_{\cdot}\eqdef (X_t)_{0\le t\le T}$ of respective dimensions $d_Y$ and $d_X$.  These processes evolve according to the coupled dynamics
% \begin{align}
% \label{eq:filtering_dynamics__signal}
% dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
% \label{eq:filtering_dynamics__observation}
% dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
% \end{align}
% where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d := \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.


% Our objective is to approximate to \textit{optimally filter} $X_{\cdot}$ given partial observations generated by $Y_{\cdot}$ using a deep learning model whose inductive bias is tailored the coupled system~\eqref{eq:filtering_dynamics__signal}, namely, a deep Kalman filter (DKF).  The information contained in $Y_{\cdot}$ up to any given time is captured by the filtration which it generates $\mathcal{Y}_{\cdot}\eqdef \sigma(\{Y_s\}_{0\le s\le t})$, where $\sigma(\{Y_s\}_{0\le s\le t}$ denotes the $\sigma$-algebra generated by the collection of random variables $\{Y_s\}_{0\le s\le t}$.  By \cite[Theorems 6.3]{Kallenberg_2021__FoundationsOfModernProbability} the $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ regular conditional distributions can be written as
% \begin{align}
%     \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t) = f_t(Y_{[0:t]}) \label{id:ConditionalDistribution}
% \end{align}
% where $f_t: C([0: t], \R^{d_Y}) \rightarrow \mathcal{P}(\mathbb{R}^{d_X})$ is a Borel measurable function.  In this paper, we affirmatively answer the following question, lying at the core of theoretical foundations of DKFs.
% \begin{question}
% \label{question:main}
% Can one design a deep Kalman filter which can approximate the regular conditional distribution function~\eqref{id:ConditionalDistribution} uniformly on suitable compact subsets of the path-space $C([0:t],\mathbb{R}^{d_Y})$.
% \end{question}

% \begin{comment}
% Moreover, under mild regularity conditions ensuring that $f$ is sufficiently continuous the geometric deep learning results of \cite{kratsios2021universal} and \cite{Acciaio2022_GHT} guarantee that it can be approximated with a class of transformer models.  However, their analysis equally reveals that the required number of parameters to approximate each $f_t$ can depend highly non-favourably on the dimensions $d_X$ and $d_Y$, as a function of the local uniform approximation error, if nothing is assumed of $f_t$.  In these results, the \textit{uniform} (on compact sets) approximation of the probability measure-valued functions $f_{t}$ by a sequential learning model $\hat{f}_t$ \anastasis{dets later} is quantified by
% \[
%     \sup_{y_{[0:T]}\in K}\, \sup_{0\le t\le T}\,
%         \mathcal{W}_2\big(f_t(y_{[0:t]},\hat{f}_t(y_{[0:t]})\big)
%     ,
% \]
% where $K$ is a (non-empty) compact subset of the path-space $\dots$.  \anastasis{Make comment about adapted Wasserstein when predicting multiple steps forward it time.}
% \end{comment}

% \subsection{Source Spaces: Regular Compact Subsets of Path Space}
% \label{s:Preliminaries__ss:InputSpace}
% Fix a time-horizon $T>0$.  For every $0<t\le T$, let $C([0:t],\mathbb{R}^d)$ denote the set of continuous ``paths'', i.e.\ functions, from $[0:t]$ to the $d$-dimensional Euclidean space $\mathbb{R}^d$.  We equip this set with the uniform norm, making it a Banach space, where the norm of a path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$ is defined by 
% \[
%         \|y\|_t
%     \eqdef 
%         \max_{0\le s\le t}\, \|y_s\|_2,
% \]
% where $\|\cdot\|_2$ is the Euclidean norm on $\mathbb{R}^d$.  

% For every $0<t\le T$, similarly to the Horizontal Extension of a path in the Functional It\^{o} calculus \citep[Section 5.2.1]{fournierRama}, we may canonically\footnote{dets later; obvious.} embed any path $f\in C([0:t],\mathbb{R}^d)$ into a path $F\in C([0:T],\mathbb{R}^d)$ via by extending the ``frozen version after time $t$'' defined by
% \[
%     F(s)\eqdef \begin{cases}
%         f(s) &: \mbox{ if } 0\le s \le t\\
%         f(t) & : \mbox{ if } t<s\le T.
%     \end{cases}
% \]
% Moreover, note that the map $f\mapsto F$ is a linear isometric embedding of the Banach space $C([0:t],\mathbb{R}^d)$ into $C([0:T],\mathbb{R}^d)$ since
% \[
% \|F\|_T = \max_{0\le s\le T}\, \|f(s)\|_2
% = \max_{0\le s\le t}\, \|f(s)\|_2 = \|f\|_t, 
% \]
% since $f(s)=f(t)$ for all $t<s\le T$.  Conversely, the restriction $F_{[0:t]}$ of a path $F\in C([0:T],\mathbb{R}^d)$ to any shorter time-interval $[0:t]$ for $0\le t\le T$ defines a non-expansive linear operator from $C([0:T],\mathbb{R}^d)$ to $C([0:t],\mathbb{R}^d)$ since
% \[
%         \|F_{[0:t]}\|_t 
%     = 
%        \max_{0\le s\le t}\, \|F_{[0:t]}(s)\|_2 
%     \le
%         \max_{0\le s\le T}\, \|F_{[0:t]}(s)\|_2 
%     =
%         \max_{0\le s\le T}\, \|F(s)\|_2 
%     =
%         \|F\|_T.
% \]
% Therefore, in what follows, we will always consider the domain of our path space to be the Banach space $C([0:T],\mathbb{R}^d)$.  
% As show in \citep[Proposition A.3]{lanthaler2023curse}, even in finite dimensions, there are rather regular functions which cannot by approximated by standard deep neural networks parameterized determined by a number trainable parameters which is a polynomial in the reciprocal approximation error.  In other words, the curse of dimensionality is generally unavoidable when approximating rather regular functions between finite-dimensional Banach spaces, and thus the problem can only be exacerbated in finite-dimensions; see \citep{galimberti2022designing} for general rates.   

% The curse of dimensionality cannot be broken, by can typically be avoided either by restricting the class of functions being approximated, e.g.\ in~\cite{adcock2022near,marcati2023exponential,siegel2023characterization,gonon2023approximation}, or the regularity of the compact subsets of the input space on which the uniform approximation is to hold; e.g.\ in~\cite{kratsios2021universal,lu2021deep,kratsios2022universal}.  Recent advances in infinite-dimensional approximation of functions not taking values in a linear space, as is the case in our results, shows that such restrictions are a sufficient requirement for obtaining universality, see \cite{kratsios2023transfer}, however, the necessity of such restrictions on compact subsets is still unknown.  The explicit effects of restricting the (fractal) dimension and diameter of compact sets of which a deep neural network approximation is to hold is explicitly studied in \citep[Proposition 3.10]{Acciaio2022_GHT}.

% In this paper, we adopt the second approach, since we cannot restrict the function class which is determined by the stochastic filtering problem.  
% We therefore restrict to compact subsets $K$ of the input space which are regular, in that they are isometric to some compact Riemannian manifold, thus we exclude fractal like subsets of the path space $C([0:T],\mathbb{R}^d)$.  We motivate the our condition with the following consequence of the Banach-Mazur theorem \cite{BanachMazurTheoremBook1955}; and consequences thereof e.g.\ \cite{Rodriguez_1995_Embedding,Stanislav_EmbeddingNowhereSmooth}.

% \begin{proposition}[Isometric Copies of Every Compact Riemannian Manifold in The Path Space]
% \label{prop:Non_Vaccousness}
% Let $\mathcal{X}$ be a compact metric space.  For every $T>0$ and each $d\in \mathbb{N}_+$, there exists a compact subset $K\subseteq C([0:T],\mathbb{R}^d)$ and an isometry from $\mathcal{X}$ onto $K$.
% \end{proposition}
% \anastasis{Perhaps I create a simple example later.}

% We will additionally impose topological regularity on our compact sets \textit{aspherical}; such as tori.  This means, that their homotopy groups $\pi_i(K)$ all vanish for all indices $i\ge 2$ (see \citep[Chapter 7]{spanier1989algebraic} for definitions and details on homotopy groups).  
% \anastasis{Maybe I include a brief appendix on homotopy groups}

% \begin{assumption}[Regular Compact Sets]
% \label{ass:reg_compact}
% Fix a compact $K\subseteq C([0:T],\mathbb{R}^d)$ and a ``latent dimension $D_K\in \mathbb{N}_+$''.
% Suppose either that:
% \begin{enumerate}
%     % \item[(i)] \textbf{Qualitative Case:} There is an $D_K$-dimensional connected, homogeneous, geodesically complete Riemannian manifold $(M,g)$ and an isometric embedding $\psi:(M,d_g)\rightarrow C([0:T],\mathbb{R}^d)$ with $K\subseteq \psi(M)$.
%     % \item[(ii)] \textbf{Quantitative Case:} 
%     \item[(i)] $K$ is finite. 
%     \item[(ii)] There exists a compact aspherical $D_K$-dimensional Riemannian manifold $(M,g)$ for which $(M,d_g)$ is isometric to $(K,\|\cdot\|_T)$; where $d_g$ is the geodesic distance on $(M,g)$. 
% \end{enumerate}
% \end{assumption}
% In what follows, we denote the Riemannian volume of $(M,g)$, in Assumption~\ref{ass:reg_compact}, by $\operatorname{Vol}(M,g)$.

% \subsection{Target Space - The \texorpdfstring{$2$-Wasserstein}{2-Wasserstein} Space of Probability Measures}
% \label{s:Preliminaries__ss:OutputSpace}

% The $2$-Wasserstein space $\mathcal{P}_2(\mathbb{R}^d)$ consists of all probability measures on $\mathbb{R}^d$ with finite second moment; i.e.\ $\mathbb{P}\in \mathcal{P}_2(\mathbb{R}^d)$ if
% \[
% \mathbb{E}_{X\sim \mathbb{P}}[\|X\|^2]<\infty
% .
% \]
% The $2$-Wasserstein metric $\mathcal{W}_2$ on $\mathbb{P}_2(\mathbb{R}^d)$ is given by minimizing the opimtal cost of transporting mass between any two measures $\mathbb{P}$ and $\mathbb{Q}$ via randomized transport plans.  This can be formalized by the Kanotovich problem
% \[
%         \mathcal{W}_2(\mathbb{P}, \mathbb{Q})^2
%     \eqdef
%         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
%             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
%     .
% \]
% Generally, the $2$-Wasserstein distance between measures can be computationally taxing, requiring a super-quadratic complexity to compute \cite{TBD}.  However, in \cite{TBD} it was show that the case where $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$ admits the following exceptional closed-form expression
% \begin{align}
%         \mathcal{W}_2(\mathbb{P},\mathbb{Q})^2
%     =
%             \| \mu^{(1)} - \mu^{(2)} \|_2^2 
%         + 
%             \operatorname{tr}(\Sigma^{(1)}) + \operatorname{tr}(\Sigma^{(2)})
%         -  
%             2
%             \,
%             \operatorname{tr}
%             \big(
%                 {\Sigma^{(2)}}^{1/2}
%                 \Sigma^{(1)}
%                 {\Sigma^{(2)}}^{1/2}
%             \big)^{1/2}
%     , \label{id:WassersteinExplicit}
% \end{align}
% provided that $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are invertible; in particular, they are positive-definite.
% % In the special case, where the covariance matrices $\Sigma^{(1)}$ and $\Sigma^{(2)}$ are also diagonal, then 
% % \[
% %         \mathcal{W}_2(\mathbb{P},\mathbb{Q})
% %     =
% %         \big(
% %                 \| \mu^{(1)} - \mu^{(2)} \|_2^2 
% %             + 
% %                 \|
% %                     \sigma^{(1)} - \sigma^{(2)}
% %                 \|_2^2
% %         \big)^{1/2}
% %     ,
% % \]
% % where $\sigma^{(i)}_j\eqdef \sqrt{\Sigma^{(i)}_{j,j}}$ for $i=1,2$ and $j=1,\dots,d$.

% % % mallasto2022entropy
% % \anastasis{It would be interesting to also consider the following:}\hfill\\
% % {\color{gray}
% % Recall that the relative entropy $\mathbb{D}$ (also called the KL-divergence) between two measures $\mathbb{P},\mathbb{Q}\in \mathcal{P}_2(\mathbb{R}^d)$ with Lebesgue densities $p$ and $q$ is
% % \[
% %         \mathbb{D}(\mathbb{P}\|\mathbb{Q})
% %     \eqdef
% %         -
% %         \mathbb{E}_{X\sim \mathbb{P}}\big[
% %             \log(p(X)/q(X))
% %         \big]
% %     .
% % \]
% % Our interest in the relative entropy is that it defines a \textit{regularized} version of the optimal transport problem between any two measures $\mathbb{P}$ and $\mathbb{Q}$ in $\mathcal{P}_2(\mathbb{R}^d)$ which can be solved in linear time \cite{TBD} using the Sinhorn-Knopp algorithm \byyan{\cite{chung2021turing}}.  This regularized transport problem is defined, for any $\varepsilon>0$, by
% % \[
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     \eqdef
% %         \inf_{(X_1,X_2)\sim \pi;\,X_1\sim \mathbb{P},\,X_2\sim \mathbb{Q}}\,
% %             \mathbb{E}_{\pi}[\|X_1-X_2\|^2]
% %         +
% %             \varepsilon\,
% %             \mathbb{D}(\pi\|\mathbb{P}\otimes \mathbb{Q})
% % \]
% % where\footnote{Note that, any transport plan $\pi$ has a $\mathbb{P}\otimes \mathbb{Q}$-density.} $\mathbb{P}\otimes \mathbb{Q}$ is the product measures on $\mathbb{R}^{2d}$ with marginals $\mathbb{P}$ and $\mathbb{Q}$.  

% % In the special case where both $\mathbb{P}=N(\mu^{(1)},\Sigma^{(1)})$ and $\mathbb{Q}=N(\mu^{(2)},{\Sigma^{(2)}})$ are Gaussian measures on $\mathbb{R}^d$, \cite[Corollary 1 and Theorem 1]{mallasto2022entropy} shows that the entropic regularized $2$-Wasserstein ``distance'' $\mathcal{W}_{\varepsilon:2}$ between $\mathbb{P}$ and $\mathbb{Q}$ admits the following closed-form expression
% % \begin{equation}
% % \label{eq:closed_form_ERWdist}
% %         \mathcal{W}_{\varepsilon:2}(\mathbb{P}\|\mathbb{Q})^2
% %     =
% %             \|\mu^{(1)}-\mu^{(2)}\|_2
% %         +
% %             \operatorname{tr}(\Sigma^{(1)})
% %             +
% %             \operatorname{tr}(\Sigma^{(2)})
% %         -
% %             \frac{\varepsilon}{2}
% %             \Big(
% %                     \operatorname{tr}(M^{\varepsilon})
% %                 -
% %                     \ln(\operatorname{det}(M^{\varepsilon}))
% %                 +
% %                     d\ln(2)-2d
% %             \Big)
% %     ,
% % \end{equation}
% % where $M^{\varepsilon}\eqdef I_d + \big(I_d + (\frac{4}{\varepsilon})^2 \Sigma^{(1)}\,{\Sigma^{(2)}} \big)^{1/2}$ and $I_d$ is the $d\times d$ identity matrix.
% % }

% \section{The Model: An Attention-Based Deep Kalman Filter}
% \label{s:Model}
% This section introduces our attention-based model.  

% Let us briefly recall the structure of a standard MLP, before formalizing our DKF. 
% In what follows, we fix a real-valued \textit{activation function} $\sigma$ defined on $\mathbb{R}$ satisfying:
% \begin{assumption}[{\cite{pmlr-v125-kidger20a}~Condition}]
% \label{ass:KLCondition}
% The activation function $\sigma$ is continuous, non-affine, and there exists an $t\in \mathbb{R}$ such that $\sigma$ is differentiable at $t$ and $\sigma^{\prime}(t)\neq 0$.
% \end{assumption}
% Examples of activation functions satisfying this condition are the $\operatorname{PReLU}$ function $t\mapsto \max\{0,t\}+a\min\{0,t\}$, for a hyperparameter $a\in \mathbb{R}$, the $\tanh$ function used in the numerical PDE literature \cite{de2021approximation}, the sine function used in SIRENs \cite{sitzmann2020implicit}, and the Swish map $t\mapsto \frac{t}{1+e^{-\beta t}}$ of \cite{ramachandran2017searching}, where $0\le \beta$ is a hyperparameter.  

% Fix an source dimension $d$ and a target dimension $D$; both of which are positive integers.  A \textit{multi-layer perceptron} (MLP), also called feedforward neural network, from $\mathbb{R}^d$ to $\mathbb{R}^D$ with activation function $\sigma$ is a map $\hat{f}:\mathbb{R}^d\rightarrow\mathbb{R}^D$ with iterative representation: for each $x\in \mathbb{R}^d$
% \begin{equation}
% \label{eq:MLP}
%     \begin{aligned}
%     \hat{f}(x) & \eqdef A^{(J)}\,x^{(J)}+b^{(J)},
%     \\
%     %
%     x^{(j+1)} & \eqdef  
%         \sigma%_{\bar{\alpha}^{(j)}}
%         \bullet 
%         \big( 
%             A^{(j)}
%             \,
%             x^{(j)}
%             +
%         b^{(j)}\big)
%         \qquad 
%             \mbox{for }  
%         j=0,\dots,J-1,
%     %
%     %
%     \\
%     x^{(0)} & \eqdef  x.
%     \end{aligned}
% \end{equation}
% where for $j=0,\dots,J-1$, each $A^{(j)}$ is a $d_{j+1}\times d_j$ matrix, $b^{(j)}\in \mathbb{R}^{d_{j+1}}$, $d_0=d$ and $d_{J+1}=D$.


% \anastasis{place model here}

% We consider an attention-type feature encoding which modifies the \textit{attention mechanism} of \cite{bahdanau2016neural} and in GNNs \cite{TBD} to the context of continuous-time path inputs and like those attention mechanisms, allows us to adaptively encode any newly observed path in terms of its similarity scores to ``know/previously generated paths''.  


% \begin{definition}[Similarity Score]
% \label{defn:Sim_Score}
% Fix positive integers $N$, $N_1$, $d$, and a ``time horizon'' $t> 0$.  
% Given a set of $N$ distinct paths $\{y^{(n)}\}_{n=1}^N$ in $C([0,1],\mathbb{R}^d)$, a $B$ is an $N_1\times N$-matrix, $b\in \mathbb{R}^{N_1}$, $A$ is an $N_1\times N_1$-matrix, and $a\in \mathbb{R}^{N_1}$.  Denote $\theta_0\eqdef (A,B,a,b,\{y^{(n)}\}_{n=1}^N)$.\\
% \noindent The \textit{similarity score}, is a map $\operatorname{sim}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$ by
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{sim}_t^{\theta_0}:
%         y_{\cdot} 
%     \mapsto 
%             \operatorname{Softmax}
%         \circ
%             \biggl(
%                 A\operatorname{ReLU}\bullet 
%             \Big(
%                     B
%                     \big(\|y_{\cdot}-y^{(n)}_{\cdot}\|_t\big)_{n=1}^N
%                 +
%                     b
%             \Big)
%                 +
%                     a
%         \biggr)
%     ,
% \end{equation}
% where $\operatorname{ReLU}(u)=\max\{0,u\}$ for all $u\in \mathbb{R}$, $\bullet$ denotes component-wise composition,  and $\operatorname{Softmax}$ takes any vector $u\in \mathbb{R}^n$ for any $n\in \mathbb{N}_+$ and returns $\operatorname{softmax}(u)\eqdef \big(e^{u_n}/\sum_{j=1}^N\,e^{u_j}\big)_{n=1}^N$.
% \end{definition}

% \begin{definition}[Positional Encoding]
% \label{defn:PositionalEncoding}
% In the notation of Definition~\ref{defn:Sim_Score}, fix a positive integer $N_2$, and set of query times $0\le t_1<\dots< t_N\le t$, an $N_2\times d$ matrix $V$, and a $N_2\times N$ matrix $U$.  Set $\theta_1\eqdef (V,U,\{t_n\}_{n=1}^N)$.
% \noindent The \textit{positional encoding}, is a map $\operatorname{pos}_t^{\theta_0}:C([0,1],\mathbb{R}^d)\rightarrow\mathbb{R}^N$, defined by 
% \begin{equation}
% \label{eq:featuremap}
%     \operatorname{pos}_t^{\theta_1}:
%         y_{\cdot} 
%     \mapsto 
%            U \,(x_{t_n})_{n=1}^N + V
%     ,
% \end{equation}
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$.
% \end{definition}

% \begin{definition}[Pathwise Attention]
% \label{defn:PathAttention}
% In the notation of Definitions~\ref{defn:Sim_Score} and~\ref{defn:PositionalEncoding}.  The \textit{pathwise attention}, with parameter $\theta\eqdef (\theta_0,\theta_1)$, is the map $\operatorname{attn}_t^{\theta}:C([0,1],\mathbb{R}^d)\rightarrow \mathbb{R}^{d\times N}$ given by
% \[
%         \operatorname{attn}_t^{\theta}(y_{\cdot})
%     \eqdef 
%             \operatorname{sim}_t^{\theta_0}(y_{\cdot}) 
%         \odot
%             \operatorname{pos}_t^{\theta_1}(y_{\cdot})
% \]
% for any $y_{\cdot}\in C([0,1],\mathbb{R}^d)$, where $v\odot X\eqdef (v_i\,X_{i,j})_{i=1,\dots,N,\,j=1,\dots,d}$ for any $N\times d$ matrix $X$ and $v\in \mathbb{R}^N$.
% \end{definition}

% % \[
% %     \hat{\phi}:
% %         u
% %     \mapsto 
% %         A\operatorname{ReLU}\bullet (Bu+ b)
% %     ,
% % \]  
% % where 

% % $D\in \mathbb{N}_+$, and each of the $W^{(d)}:\mathbb{R}^{F_{d-1}}\rightarrow \mathbb{R}^{F_d}$ (for $d=1,\dots,D$) is an ``invertible'' affine map defined for every $v\in \mathbb{R}^{F_{d-1}}$ by
% % \[
% %         W^{(d)}(v) 
% %     = 
% %         (A^{(d:1)},e^{A^{(d:0)}})v + b^{(d)}
% %     ,
% % \]
% % where $F_d>F_{d-1}$, $b\in \mathbb{R}^{F_d}$, $A^{(d:1)}$ is a $(F_d-F_{d-1})\times F_{d-1}$ matrix, and $e^{A^{(d:0)}}$ is the matrix exponential of a $F_{d-1}\times F_{d-1}$-matrix $A^{(d:0)}$.  Furthermore, $F_0\eqdef N$, and $F\eqdef F_d$.

% % \anastasis{We can perhaps sample these from some ``prior model we believe on the process $Y_{\cdot}$''?} \yannick{Is there any indicator in \Cref{lem:Good_Feature_Map} that yields what properties the paths $x_\cdot^{(1)}, x_\cdot^{(2)}, ...$ should have? Or to put it another way, if the paths are sampled from the actual distribution, they would do the job? }

% % \anastasis{Explain good feature map, Comment @Yannick the easiest explanation is found in ``Non-Euclidean Universal Approximation''.} \yannick{TODO.} 


% % \anastasis{The idea is to train $\operatorname{attn}_T$ on a set in a centralized manner, then update $\varphi$ in a decentralized way.}

% % Let us fix $(\operatorname{attn}_t)_{t\ge 0}$ using as in Lemma~\ref{lem:Good_Feature_Map}.  This allows us to reduce our deep-learning model class to a smaller hypothesis class $\mathcal{H}$ of non-Euclidean kernel regressors mapping paths in $C([0:T],\mathbb{R}_d)$ to non-singular Gaussian measures $\mathcal{N}_{d_X}$
% % %\yannick{its bijective characterization in $\mathbb{R}^{d_X+d_X(d_X+1)/2}$, right?}\anastasis{yes}
% % .  

% % At any given time $0\le t\le T$ and for each path $y_{\cdot}\in C([0:t],\mathbb{R}^d)$, each kernel regressor $f_{\theta_{\cdot}}\in \mathcal{H}$ is determined by a $\mathcal{Y}_{\cdot}$-predictable process $\theta_{\cdot}\eqdef (\theta_t)_{0\le t\le T}$ via
% % \[
% %         f_{\theta_{\cdot}}
% %             (t,y_{[0:t]})
% %         \eqdef
% %             \psi\big(
% %                 \theta_t
% %                 \operatorname{attn}_t(y_{[0:t]})
% %             \big)
% %     ,
% % \]
% % where $\theta_t$ is a ${d_X+d_X(d_X+1)/2}\times F$-dimensional matrix.  NB, that $\psi$ is a homeomorphism between $\mathcal{N}_{d_X}$ and $\mathbb{R}^{d_X+d_X(d_X+1)/2}$. 




% % \subsection{The Objective Function}

% % Fix a set of realizations/sample paths from the process $Y_{\cdot}$, which we denote by $y_{[0:T]}^{(1)},\dots,y_{[0:T]}^{(N)}$ for some positive integer $N$.
% % We wish to select an optimal (dynamic) kernel regressor by minimizing the \textit{penalized regret functional}
% % \begin{equation}
% %         \mathcal{R}(\theta_{\cdot})
% %     \eqdef 
% %         \underbrace{
% %             \int_0^T\, 
% %                 \frac1{N}
% %                 \sum_{n=1}^N\,
% %                 \mathcal{W}_2^2\big(
% %                     f_t(y_{[0:t]}^{(n)})
% %                 ,   
% %                     \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})
% %                 \big)
% %                 -
% %                 \mathcal{R}^{\star}
% %             \,dt
% %             }_{
% %                 \mbox{$W_2$-Regret}
% %             }
% %         +
% %             \underbrace{
% %             \int_0^T
% %                 \lambda \,\|
% %                     \theta_t
% %                 \|_2^2
% %                 \,
% %             dt
% %             }_{
% %                 \mbox{Running Regularizer}
% %             }
% %     ,
% % \end{equation}
% % and $\lambda >0$ is a regularizing hyperparameter and where $\mathcal{R}^{\star}$ represents the minimal possible value which the running $\mathcal{W}_2^2$-SSEs loss can achieve
% % \[
% %     \mathcal{R}^{\star} 
% % \eqdef 
% %     \inf_{\theta_{\cdot}\in ...}
% %         \int_0^T\, 
% %             \frac1{N}
% %             \sum_{n=1}^N\,
% %             \mathcal{W}_2^2\big(
% %                 f_t(y_{[0:t]}^{(n)})
% %             ,   
% %                 \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})
% %         \big)
% %     dt
% % \]
% % \anastasis{Describe the set of controls...which determins our hypothesis class}\hfill\\
% % Minimizing the regret functional $\mathcal{R}$ is equivalent to minimizing the following energy/loss function, in the sense that their set of minimizers coincide.   
% % \anastasis{I'll add the details in this, and the diagonal, cass (this will be a proposition)}
% % \begin{equation}
% %         L(\theta_{\cdot})
% %     \eqdef 
% %         \int_0^T\, 
% %                 \frac1{N}
% %                 \sum_{n=1}^N\,
% %                     \| \mu_{n:t} - \hat{\mu}_{n:t} \|_2^2 
% %                         + 
% %                     \operatorname{tr}\big(
% %                         \Sigma_{n:t} + \hat{\Sigma}_{n:t}
% %                         -2
% %                         (
% %                             \hat{\Sigma}_{n:t}^{1/2}
% %                             \Sigma_{n:t} 
% %                             \hat{\Sigma}_{n:t}^{1/2}
% %                         )^{1/2}
% %                     \big)
% %         +
% %                 \|
% %                     \theta_t
% %                 \|_2^2
% %         \,
% %         dt
% %     ,\label{id:LossFunction}
% % \end{equation}
% % where we have made the abbreviations $\mathcal{N}(\byyan{\hat{\mu}_{n:t}}, \hat{\Sigma}_{n:t})\eqdef \hat{f}_{\theta_{\cdot}}(t,y_{[0:t]}^{(n)})$ and 
% % $\mathcal{N}(\byyan{\mu_{n:t}}, \Sigma_{n:t})\eqdef f_t(y_{[0:t]}^{(n)})$ for each $0\le t\le T$ and each $n\in \{1,\dots,N\}$.  
% % \anastasis{With Xuwei, we will identify when things are diagonal and derive the optimal control; i.e.\ optimal dynamic non-Euclidean kernel model.}
% % \yannick{(For next discussion:) How can we minimize \eqref{id:LossFunction}, as $f_t(y_{[0:t]}^{(n)}) [= \mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)]$ is not observable? $\rightarrow$ we have closed form expressions for $\mu$, $\Sigma$ given by \eqref{id:ClosedFormMu}, \eqref{id:ClosedFormSigma}.} \yannick{I think $\lambda$ will occur in \eqref{id:LossFunction}?}



% % \newpage
% % \begin{definition}\label{defn:BV_Paths}
% % Fix a positive integer $d$.  A continuous path $x:[0:1]\rightarrow \mathbb{R}^d$ with $x(0)=0$ is said to be of bounded variation if $\|x\|_{BV}\eqdef \sup_{\pi}\, \sum_{i=1}^{l-1}\, \|h(t_{i+1})-h(t_i)\|_{\mathbb{R}^D}$ is finite, where the supremum is taken over all finite partitions $\pi=\{(t_i)_{i=1}^l:\, 0=t_1<\dots<t_l=1\}$ of $[0:1]$.  The set of all such paths denoted by $C^1_0([0:1],\mathbb{R}^d)$.
% % \end{definition}
% % Let $x_{\cdot}$ and $y_{\cdot}$ be paths in $C^1_0([0:1],\mathbb{R}^d)$, their we the component-wise Riemann-Stieltjes integral of $y_{\cdot}$ against $x_{\cdot}$ by $\int_0^1\,y(t)\,dx(t)\eqdef \big(\int_0^1\,y(t)_i\,dx_i(t)\big)_{i=1}^d$.  The Riemann-Stieltjes integrals are a type of ``polynomial features'' for paths in $C^1_0([0:1],\mathbb{R}^d)$ and their associated feature maps are the signatures of \cite{???}, defined as follows.
% % \begin{definition}[Signature of a BV-Path]\label{defn:Signatures}
% % Let $x_{\cdot}\in C^1_0([0:1],\mathbb{R}^$
% % \end{definition}



% \section{Main Result}
% \label{s:Main_Results}



















% \paragraph{The Feature Map}
% \anastasis{Explain why no sig, discrete/trivial topology analogy; and note that one could consider a variant of the model using sig if they needed the stronger p-variation topology.  But since we don't then its more efficient to consider approximators depending on fewer parameters.}


% \newpage
% \section{Applications}

% In this section, we will discuss exemplary applications that leverage the possibility to approximate a Kalman filter setting with our suggested framework. 

% \subsection{(Conditional) simulation of the observation process}

% Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation} and are known by the agent. For a fixed time $t \in [0:T]$, the objective is now to simulate the process $Y$ at times $t \leq s \leq T$. If both, $X, Y$ are observable, then a typical Euler-scheme for $Y_{[t:T]}$ is usually given by fixing a time-discretization $t := t_0 < t_1  < \cdots < t_N := T$ with $N \in \N$ and approximating
% \begin{align*}
%     X_{t_{n+1}} & \approx X_{t_{n}} + [a_0(t,Y_{[0:t_n]}) + a_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, b_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)} \\
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)}
% \end{align*}
% where $(Z_n^{(1)})_{n \in \myset{1}{N}}, (Z_n^{(2)})_{n \in \myset{1}{N}}$ are standard normal distributed random variables. Note that we have a slight abuse of notation, as $a_0, a_1, b_1, b_2, A_0, A_1, B_1, B_2$ are now approximations from discretized paths instead of the continuous counterparts.

% In our setting, however, the component $X$ is not observable. To overcome this, we have to rely on standalone simulations of $Y_{[t:T]}$, while inferring $X$ conditional on $Y$. This means, 
% \begin{align*}
%     Y_{t_{n+1}} & \approx Y_{t_{n}} + [A_0(t,Y_{[0:t_n]}) + A_1(t,Y_{[0:t_n]}) X_{t_n} \vert  Y_{[0:t_n]}](t_{n+1}-t_n) + \sum_{i=1}^2\, B_i(t,Y_{[0:t_n]})\sqrt{t_{n+1}-t_n}Z_n^{(i)},
% \end{align*}
% where $X_{t_n} \vert Y_{[0:t_n]}$ refers to the conditional law described by \eqref{id:ConditionalDistribution}.

% \yannick{If we want to do these simulations fast and efficient, we are reliant on fast access to $X_{t_n} \vert Y_{[0:t_n]}$.}


% \subsection{Optimal control and BSDEs in finance}

% Suppose that the dynamics of $X, Y$ are given as in \eqref{eq:filtering_dynamics__signal}, \eqref{eq:filtering_dynamics__observation}. While there are numerous settings where this structure is applicable, the reader may regard the observation process $Y$ as an asset price process and assume that the signal process $X$ constitutes a stochastic drift model that is generally not observable. 

% We now consider an optimal control problem of the form 
% \begin{align}
%     J(u) \eqdef \mathbb{E}\left[\int_0^T r(t, Y_t, (u \bdot Y)_t, u_t) dt + g(Y_T, (u \bdot Y)_T) \right] \label{id:OptimalControl}
% \end{align}
% for a measurable function $r: \R_+ \times \R^{d_Y} \times \R^{d_Y} \times \R^{d_Y}$, a concave function $g: \R^{d_Y} \times \R^{d_Y} \to \R$, and $u$ being a predictable control process with values in $\R^{d_Y}$. We write 
% \begin{align*}
%     (u \bdot Y)_t := \int_0^t u_s dY_s \quad \forall t \in [0:T], 
% \end{align*}
% which is interpreted as trading with rate $u$ on the asset $Y$. Furthermore, $r$ refers to the running reward that accumulates over all times $s \in [0,T]$ and $g$ is interpreted as the terminal reward which is received at maturity. 

% \begin{example}[Optimal control problems in finance]
% \begin{enumerate}[wide]
%     \item \emph{Hedging European options.} In the following, let $h: \R^{d_Y} \to \R$ denote the payoff of a European contingent claim, and set $r \equiv 0$, $g(y, z) := - (z - h(y))^2$. \yannick{Concave?} Then, the optimization task reads as 
%     \begin{align*}
%         J(u) \eqdef - \mathbb{E}\left[  \left(h(Y_T) - (u \bdot Y)_T) \right)^2 \right],
%     \end{align*}
%     which is tantamount to minimizing the $L^2$-distance of the wealth process at terminal time to the option's payoff.
%     \item \emph{Optimal Liquidation.} Assume $d_Y \eqdef 2$ with the first component of $Y$ representing the asset price and let the second component of $Y$ constitute the constant process, i.e. $(Y)_{2} \eqdef 1$, therefore $d((u)_{2} \cdot (Y)_{2})_t = u_t dt$ corresponds to the inventory if we require $(u)_1 \equiv (u)_2$. Now, define $alpha: \R \to \R$ as a (concave) utility function and $\beta: \R \to \R$ as a (convex) inventory penalty. If we set $g(y, z) \eqdef \alpha((y)_1) - \beta((y)_1)$ and define by $r(t, y, z, u) \eqdef \Tilde{r}(t, (y)_1, (u)_1)$ the trading cost of $u$ at time $t$ and asset price $(y)_1$, we arrive at a classical optimal liquidation task.
%     \item ...
% \end{enumerate}
% \end{example}

% In order to solve \eqref{id:OptimalControl}, we assume conditions XXX. Then we can define the generalized Hamiltonian
% \begin{align*}
%     H:
%     \begin{array}{ccc}
%         \R_+ \times (\R^{d_Y})^{\times 3} \times \R^{d_Y} & \longrightarrow & \\
%          & \longmapsto &
%     \end{array}
% \end{align*}

% \subsection{Model ambiguity}
% Let $x_{[0:T]} \in XXX$ and assume the dynamics of $Y$ are given by \eqref{eq:filtering_dynamics__observation}. Then,  $Y \vert \lbrace X = x \rbrace$ which is defined via $(Y \vert \lbrace X = x \rbrace)_t \eqdef Y_t \vert \lbrace X_t = x_{t} \rbrace$ for all $t \in [0:T]$ represents an ordinary SDE with full observability. 
% \begin{example}\label{exa:UncertaintyHeston}
%     For any $t \in [0:T]$ and $y_{[0:t]} \in XXX$ consider $A_0(t, y_{[0:t]}) \eqdef (\mu, - \kappa y_t^2)$, $A_1(t, y_{[0:t]}) \eqdef (0, \kappa)$, $B_1(t, y_{[0:t]}) \eqdef 0$, $B_2(t, y_{[0:t]})^1 \eqdef (y_t^1\sqrt{y_t^2}, 0)$, and $B_2(t, y_{[0:t]})^1 \eqdef (\sigma \rho \sqrt{y_t^2}, \sigma \sqrt{1-\rho^2} \sqrt{y_t^2})$, where $\mu \in \R$, $\kappa, \sigma > 0$, and $\rho \in [-1:1]$. This corresponds to the Heston model with (stochastic) mean-reversion parameter $X_t$,
%     \begin{align*}
%             d 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \\
%                     Y_t^2
%                 \end{matrix}
%             \right)
%         = 
%             \left(
%                 \begin{matrix}
%                     \mu \\
%                     \kappa X_t - \kappa Y_t^2
%                 \end{matrix}
%             \right)
%             dt
%         + 
%             \left(
%                 \begin{matrix}
%                     Y_t^1 \sqrt{Y_t^2}  \\
%                     \sigma \sqrt{Y_t^2} 
%                 \end{matrix}
%             \right)
%             \left(
%                 \begin{matrix}
%                     1 & \rho \\
%                     \rho & 1
%                 \end{matrix}
%             \right)^{1/2}
%             dW^{(2)}_t, \quad  \forall t \in [0:T],
%     \end{align*}
%     and $Y \vert \lbrace X \equiv \theta \rbrace$, $\theta > 0$ represents the Heston model with deterministic (and constant) mean-reversion parameter $\theta$.
% \end{example}

% In the following, let $g: A \times XXX \mapsto \R$, define a control problem, where the control $a \in A$ acts on the path $y \in XXX$ to obtain the payoff $g(a, y)$. Further, let $u: \R \to \R$ denote a utility (concave) function. Then, under the model assumption $X = x$, the (ambiguity-unaware) control problem reads as follows,
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}} \mathbb{E}\left[
%         u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)
%     \right].
% \end{align*}
% In terms of \Cref{exa:UncertaintyHeston}, one could for instance consider the hedging task $g(a, y) := (a \bdot y^1)_T - h(y_T^1)$ of the European option with payoff structure $h: \R \to \R$, where $\mathcal{A}$ is the set of previsible trading strategies on $Y^1$.

% In \cite{KlibanoffMarinacciMukerji05}, the authors suggest considering not only one choice of model (as we did above with $X = x$) but instead a distribution of models, which are evaluated with a second expected utility. Let $r: \R \to \R$ denote a second (concave) utility function and since 
% \begin{align*}
%         \mathbb{E}\left[u \circ g(\alpha, Y \vert \lbrace X = x \rbrace)\right]    
%     =
%         \mathbb{E}\left[u \circ g(\alpha, Y) \mid \lbrace X = x \rbrace \right],
% \end{align*}
% ambiguity-aware control problem reads as follows, 
% \begin{align*}
%     \argmax_{\alpha \in \mathcal{A}}
%         \mathbb{E}\left[
%             r \left(
%             \mathbb{E}\left[
%                 u \circ g(\alpha, Y)
%             \mid
%                 X
%             \right]
%             \right)
%         \right].
% \end{align*}
% \yannick{TODO. Explain how a DKF setting applies as the model-process is unobservable.}




% \section{Theoretical Analysis}
% \label{s:Theoretical_Analysis}

% \subsection{The Structure of the Target Function: The Optimal Filter}

% In this section, we employ results of \cite{LipShiryaev_II_2001} to show that  $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, and, denote an explicit formulation of the resulting distribution. For this, assume that
% \begin{align*}
%     \int_0^T \vert \process{a_0}{t, y_{[0:t]}}{i} \vert + \vert \process{a_1}{t, y_{[0:t]}}{i,j}\vert + (\process{b_1}{t, y_{[0:t]}}{i, j})^2 dt &< \infty, \,\, \forall i  \in \myset{1}{d_X}\, \forall j \in  \myset{1}{d_X} \\
%     \int_0^T (\process{b_2}{t, y_{[0:t]}}{i, j})^2 + (\process{A_1}{t, y_{[0:t]}}{j, i})^2 + (\process{B_1}{t, y_{[0:t]}}{j, i})^2 dt &< \infty, \,\, \forall i \in  \myset{1}{d_X}  \,\forall j \in  \myset{1}{d_Y}\\
%     \int_0^T (\process{A_0}{t, y_{[0:t]}}{i})^2 + (\process{B_2}{t, y_{[0:t]}}{i, j})^2 dt &< \infty, \,\, \forall i \in \myset{1}{d_Y}\, \forall j \in \myset{1}{d_Y} 
% \end{align*}
% for all $y_{[0:T]} \in C([0:T], \R^{d_Y})$; the matrix $B \circ \process{B}{t,x}{} := \process{B_1}{t,x}{} \process{B_1}{t,x}{}^\intercal + \process{B_2}{t,x}{} \process{B_2}{t,x}{}^\intercal$ is uniformly non-singular, that is, its inverse is uniformly bounded; there are constants $L_1, L_2 \in \R$ as well as a non-decreasing right-continuous function $K: [0:T] \to [0:1]$ such that for every $x, y \in C([0:T], \R^{d_Y})$ and every $k=1,2$, and $i,j=1,\dots,d$ it holds for all $0 \leq t\leq T$ that 
% % entry $g$ in $B_1, B_2$ holds
% \begin{align*}
%         \vert (B_k)_{i,j}(t, x) - (B_k)_{i,j}(t, y) \vert^2 
%     & \leq
%         L_1 \int_0^{t} \vert x_s - y_s \vert^2 dK(s) + L_2 \vert x_t - y_t \vert^2, 
%     \\
%         (B_k)_{i,j}(t, x)^2  
%     & \leq 
%         L_1 \int_0^t \vert (1 + \vert x_s \vert^2 ) dK(s) + L_2 (1 +\vert x_t \vert^2) 
% \end{align*}
% where $\vert \cdot \vert$ is the Euclidean distance on $\R^{d_Y}$; and we have
% \begin{align*}
%     \int_0^T \bE[\vert \process{A_1}{(t, Y_{[0:t]})}{i, j}(X_t)_j \vert] dt & < \infty; \\
%     \bE[\vert (X_t)_j \vert] & < \infty, \quad \forall t \in [0:T]; \\
%     \bP\left( \int_0^T (\process{A_1}{t, Y_{[0:t]}}{i, j} \bE[(X_t)_j \vert \cY_t])^2dt  < \infty \right) & = 1;
% \end{align*}
% for indices $i \in \myset{1}{d_Y}, j\in \myset{1}{d_X}$.

% This allows us to apply \citep[Theorem 12.6]{LipShiryaev_II_2001} and we deduce that $\mathbb{P}(X_t\in \cdot|\mathcal{Y}_t)$ is conditionally Gaussian, meaning that for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$ the probability measure $f_t(y_{[0:t]})$ is a $d_X$-dimensional Gaussian measure.  We denote the mean and covariance of this measure by $\mu(y_{[0:t]})$ and $\Sigma(y_{[0:t]})$.  Thus, 
% \begin{align}
%         \mathcal{N}(\mu(y_{[0:t]}),\Sigma(y_{[0:t]})) 
%     \sim 
%         \mathbb{P}(X_t\in \cdot|y_{[0:t]})
%     \eqdef 
%         f_t(y_{[0:t]})
%     , \label{id:LipsterShiryaevRepresentation}
% \end{align}
% for each $0\le t\le T$ and each path $y_{[0:t]}\in C([0:t], \R^{d_Y})$.

% We assume further
% \begin{align*}
% \begin{array}{cc}
%     \vert \process{a_1}{t, x}{i, j}\vert \leq L, &\quad \forall i \in \myset{1}{d_X}, \\
%     \vert \process{A_1}{t, x}{i, j}\vert \leq L, &\quad \forall i \in \myset{1}{d_Y},
% \end{array} \quad \forall j \in \myset{1}{d_X},
% \end{align*}
% for $x \in C([0:t], \R^{d_Y})$, $t \in [0:T]$; as well as
% \begin{align*}
%     \begin{array}{cc}
%     \int_0^T \bE[\process{a_0}{t, Y_{[0:t]}}{i}^4 + \process{b_1}{t, Y_{[0:t]}}{ij}^4 + \process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty, &\quad \forall j \in \myset{1}{d_X}, \\
%     \int_0^T \bE[\process{b_2}{t, Y_{[0:t]}}{ij}^4] dt < \infty, &\quad \forall j \in \myset{1}{d_Y}, \\
%     \end{array} \quad \forall i \in \myset{1}{d_X},
% \end{align*}
% and eventually
% \begin{align*}
%     \bE\bigg[\sum_{j = 1}^{d_X}(X_0)_j^4\bigg] < \infty.
% \end{align*}
% Then, \citep[Theorem 12.7]{LipShiryaev_II_2001} implies that $\mu_t\eqdef \mu(y_{[0:t]})$ and $\Sigma_t\eqdef \Sigma(y_{[0:t]})$ are
% \allowdisplaybreaks
% \begin{align}
% \notag
%     d\mu_t 
%         =&[a_0(t,y_{[0:t]}) + a_1(t,y_{[0:t]}) \mu_t]dt +[(b\circ B)(t,y_{[0:t]})+\Sigma_t A_1^{\intercal}(t,y_{[0:t]})](B\circ B)^{-1}(t,y_{[0:t]})\\
%         &\times [dy_t - (A_0(t,y_{[0:t]}) + A_1(t,y_{[0:t]}))\mu_t dt] \label{id:ClosedFormMu}
%     \\
% \notag
%     \partial_t\Sigma_t =& a_1(t,y_{[0:t]}) \Sigma_t + \Sigma_t a_1^{\intercal}(t,y_{[0:t]}) + (b\circ b)(t,y_{[0:t]}) - [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]}) ]
%         \\
%         & \times (B\circ B)^{-1} (t,y_{[0:t]}) [(b\circ B)(t,y_{[0:t]}) + \Sigma_t A_1^{\intercal}(t,y_{[0:t]})]^{\intercal} \label{id:ClosedFormSigma}
% \end{align}
% with initial conditions $\mu_0=\mathbb{E}[X_0|Y_0]$ and $\Sigma_0\eqdef \mathbb{E}[(X_0-\mu_0)(X_0-\mu_0)^{\intercal}|Y_0]$. Note that we used the notation 
% \begin{align*}
%     B \circ B \eqdef B_1B_1^\intercal + B_2B_2^\intercal, \quad 
%     b \circ B \eqdef b_1B_1^\intercal + b_2B_2^\intercal, \quad 
%     b \circ b \eqdef b_1b_1^\intercal + b_2b_2^\intercal.
% \end{align*}
% Eventually (again \cite{LipShiryaev_II_2001}, Theorem 12.7), we have that $\Sigma_t$ is positive definite for all $t \in [0,T]$ if $\Sigma_0$ is positive definite. 
% \anastasis{argue (as in page 34) that we may consider $B_0=0$ and $B\eqdef B_1$ and likewise for $b_i$ where $i=0,1$.}
% \anastasis{(which we assume to be known or tuneable?)}.

% \anastasis{@Xuwei, let's check conditions under which $\Sigma_t$ remains positive definite for all $t$ and all $y_{[0:t]}$.} 

% \begin{lemma}[Local Lipschitz-Continuity of the Optimal Filter]
%     Fix $t \in [0, T]$. Under the assumptions of \Cref{lem:LipschitzSigma} and \Cref{lem:LipschitzMu}, $f_t$ from \eqref{id:ConditionalDistribution} is locally Lipschitz-continuous. In particular, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%     \begin{align*}
%         \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]})) \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t 
%     \end{align*}
% \end{lemma}



% \subsection{Proof of Lipschitz Continuity}
% \begin{proof}
%     By \eqref{id:LipsterShiryaevRepresentation}, \Cref{lem:LoewnerBound}, and \Cref{lem:LipschitzManifold_Nd} there exists a constant $\bar{K} < \infty$ s.t.
%     \begin{align*}
%     \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         &\leq 
%             \bar{K}
%                 \,
%             \sqrt{\| \mu(y_{[0:t]}^{(1)}) - \mu(y_{[0:t]}^{(2)}) \|_2^2 + \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2}.
%     \end{align*}
%     We see from \Cref{lem:LipschitzMu} and \Cref{lem:LipschitzSigma} that there exists a constant $K < \infty$, s.t.
%     \begin{align*}
%             \|\Sigma(y_{[0:t]}^{(1)})-\Sigma(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%             \quad 
%             \|\mu(y_{[0:t]}^{(1)})-\mu(y_{[0:t]}^{(2)})\|_2^2
%         \leq
%             K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2, 
%     \end{align*}
%     so we obtain 
%     \begin{align*}
%             \mathcal{W}_2(\mathbb{P}(X_t \in \cdot \vert y^{(1)}_{[0:t]}), \mathbb{P}(X_t \in \cdot \vert y^{(2)}_{[0:t]}))
%         \leq
%             \sqrt{2} K \bar{K}\Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%     \end{align*}
%     and the statement follows. 
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\mu$ in the path]\label{lem:LipschitzMu}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:TimeLipschitzMu}, $\mu_\cdot$ from \eqref{id:ClosedFormMu} is locally Lipschitz-continuous. This means that for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 
%  \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%  \end{align*} 
% \end{lemma}
% \begin{proof}
% Define 
% \allowdisplaybreaks
% \begin{align} 
%   \Phi_1(s, y_{[0:s]}) & \eqdef a_1(s, y_{[0:s]}) \notag \\
%   & \quad \quad - [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) [A_0(s, y_{[0:s]}) + A_1(s, y_{[0:s]})], \label{id:Phi1} \\
%   \Phi_2(s, y_{[0:s]}) & \eqdef a_0(s, y_{[0:s]}) + [(b\circ B)(s, y_{[0:s]}) + \Sigma_t A_1^{{\intercal}}(s, y_{[0:s]}) ] (B\circ B)^{-1}(s, y_{[0:s]}) \label{id:Phi2}. 
% \end{align}
% Note that conditions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} are satisfied, therefore, $\Phi_1$ and $\Phi_2$ are globally Lipschitz w.r.t. time and locally Lipschitz w.r.t. the path. 

% By \eqref{id:ClosedFormMu}, $\mu_t$ can be written as 
% \begin{align} 
%  \mu_t = & \mu_0 + \int_0^t a_0(s, y_{[0:s]}) ds  + \int_0^t \Phi_2(s, y_{[0, s]}) d y_{[0, s]} 
%  + \int_0^t \Phi_1(s, y_{[0:s]}) \mu_s ds .   \notag 
% \end{align}
% We further have that  
% \begin{align} 
%  & \mu^{(1)}_t - \mu^{(2)}_t \notag \\
%  & =   \mu_0^{(1)} - \mu_0^{(2)} 
%   + \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds 
%   + \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \notag \\ 
%  & \quad + \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \notag  
%   + \int_0^t  \Phi_1(s, y^{(1)}_{[0 : s]})\,
% (\mu^{(1)}_s - \mu^{(2)}_s ) ds .  \notag
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2 \leq & \gamma(t) + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 \cdot 
%  \big\| \mu^{(1)}_s - \mu^{(2)}_s \big\|_2 ds ,\notag 
% \end{align} 
% %\anastasis{this rhs is Jensen + Cauchy Schwartz}
% where 
% \begin{align*} 
% \gamma(t) \eqdef & \big\| \mu_0^{(1)} - \mu_0^{(2)} \big\|_2 
%   + \underbrace{\Big\| \int_0^t a_0(s, y_{[0:s]}^{(1)}) -  a_0(s, y_{[0:s]}^{(2)} )  ds \Big\|_2}_{\term{t:gammaA}} \\  
% & + \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0: s]}) d y^{(1)}_{[0, s]}
%   - \int_0^t \Phi_2(s, y^{(2)}_{[0 : s]})  d  y^{(2)}_{[0 : s]} \Big\|_2 }_{\term{t:gammaB}} 
%   + \underbrace{\Big\| \int_0^t \Phi_1(s, y^{(1)}_{[0 : s]}) -   \Phi_1(s, y^{(2)}_{[0 : s]}) \mu^{(2)}_s ds \Big\|_2}_{\term{t:gammaC}} .
% \end{align*} 
% For an application of Gr\"onwalls inequality, it is sufficient to show $\Vert \gamma(t) \Vert_2 < \infty$. We have due to $a_0$ being Lipschitz,
% \begin{align*}
%     \eqref{t:gammaA} 
%     \leq \int_0^t \Vert a_0(s, y_{[0:s]}^{(1)}) - a_0(s, y_{[0:s]}^{(2)}) \Vert_2 ds  
%     \leq \int_0^t K \Vert y_{[0:s]}^{(1)} - y_{[0:s]}^{(2)} \Vert_s ds  
%     \leq t K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t.
% \end{align*}
% Further, we see that 
% \begin{align} 
%  \eqref{t:gammaB}
%  \leq & 
%   \underbrace{\Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2}_{\term{t:gammaE}}
%   + 
%   \underbrace{ \Big\| \int_0^t \Phi_2(s, y^{(1)}_{[0:s]}) 
%    d ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \Big\|_2 }_{\term{t:gammaD}} . \notag 
% \end{align} 
% % \byyan{By the use of integration by parts,
% % \begin{align*}
% %     \eqref{t:gammaE}  
% %     & = 
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     \\
% %     &\qquad   - \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 \\
% %     & \leq 
% %     \underbrace{
% %     \Big\| 
% %           (\Phi_2(t, y^{(2)}_{[0:t]}) - \Phi_2(t, y^{(1)}_{[0:t]})) y^{(2)}_{[0:t]} 
% %         - (\Phi_2(0, y^{(2)}_0) - \Phi_2(0, y^{(1)}_0)) y^{(2)}_0     
% %     \Big\|_2
% %     }_{\term{t:gammaE1}}\\
% %     &\qquad   +
% %     \underbrace{
% %     \Big\|
% %         \int_0^t y^{(2)}_{[0:s]} \, d (\Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}))
% %     \Big\|_2 
% %     }_{\term{t:gammaE2}}.
% % \end{align*}
% % We see that $\eqref{t:gammaE1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to \textcolor{red}{(path-)Lipschitz continuity of $\Phi_2$} and 
% % \begin{align*}
% %     \eqref{t:gammaE2} 
% %     & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y^{(2)}_{[0:s_i]} \Vert_2  \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     & \leq \epsilon_I + \Vert y^{(1)}_{[0:t]} \Vert_t \sum_{i = 1}^I \big\| \Phi_2(s_i, y^{(2)}_{[0:s_i]})  - \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \big(\Phi_2(s_{i-1}, y^{(2)}_{[0:s_{i-1}]}) + \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big) \big\|_2 \\
% %     %& \leq \epsilon_I + K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \cdot \sum_{i = 1}^I \Vert y^{(2)}_{[0:s_i]} - y^{(2)}_{[0:s_{i-1}]} \Vert_2  \\
% %     %& \leq \epsilon_I + K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t ,
% % \end{align*}
% % }
% Using It\^{o}'s isometry, we have 
% \allowdisplaybreaks 
% \begin{align*} 
%     \eqref{t:gammaE}^2 
%     & =  \int_0^t 
%         \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
%     d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \\
%     & \leq 
%         K^2 \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert^2_t
%         \int_0^t d \, (B\circ B)(s, y^{(2)}_{[0:s]})
% \end{align*} 
% where the last inequality holds due to (path-)Lipschitz continuity of $\Phi_2$. As a next step, let $\mySet{[s_{i-1}:s_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[0:t]$, we see due to the (time-) Lipschitz continuity of $B \circ B$ together with the definition of the Riemann-Stieltjes integral that 
% \begin{align*}
%     \eqref{t:gammaE}^2 
%     & \leq \epsilon_I + K^2 \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert^2_t \cdot \sum_{i = 1}^I \Vert (B\circ B)(y^{(2)}_{[0:s_i]}) - (B\circ B)(y^{(2)}_{[0:s_{i-1}]}) \Vert_2  \\
%     & \leq \epsilon_I + K^2 T \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t^2.
% \end{align*}
% As $\epsilon_I \to 0$ for $I \to \infty$, we obtain $\eqref{t:gammaE} \leq K\sqrt{T} \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.

% % \xuwei{As $I\to \infty$, we have 
% % \begin{align} 
% % \sum_{i=1}^I \big\| y^{(2)}_{[0:s_i]} 
% %  - y^{(2)}_{[0:s_{i-1}]} \big\|_2^2
% % \rightarrow \int_0^t B\circ B(s, y^{(2)}_{[0:s]}) ds . \notag 
% % \end{align} 
% % } 
% % 
% % \xuwei{ Using It\^{o}'s isometry, we have 
% % \allowdisplaybreaks 
% % \begin{align} 
% %   (IV)^2 = & 
% %   \Big\| \int_0^t \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]}) d y^{(2)}_{[0:s]} \Big\|_2^2 \notag \\ 
% %   = & \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \notag 
% % \end{align} 
% % \begin{align} 
% %   (IV) 
% %   = & \Big[ \int_0^t \big\| \Phi_2(s, y^{(2)}_{[0:s]}) - \Phi_2(s, y^{(1)}_{[0:s]})\big\|_2^2 
% %   d \, (B\circ B)(s, y^{(2)}_{[0:s]}) \Big]^{1/2} \notag 
% % \end{align} 
% % }

% Moreover, by the use of integration by parts, we have
% \begin{align} 
%     \eqref{t:gammaD}  
%     & = \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0)    
%         - \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq \Big\| \Phi_2(t, y^{(1)}_{[0:t]}) (y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]}) 
%         - \Phi_2(0, y^{(1)}_0) (y^{(2)}_0 - y^{(1)}_0) \Big\|_2 
%         + \Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2 \notag \\ 
%     & \leq 2 \max_{0 \leq s \leq t} \Big\| \Phi_2(s, y^{(1)}_{[0:s]}) \Big\|_2 
%         \cdot \Big\|  y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} \Big\|_t 
%         + \underbrace{\Big\|  \int_0^t ( y^{(2)}_{[0:s]} - y^{(1)}_{[0:s]} ) \, d \Phi_2(s, y^{(1)}_{[0:s]})  \Big\|_2}_{\term{t:gammaF}}. \notag 
% \end{align} 
% (Time-)Lipschitz continuity of $\Phi_2$, implying $\max_{s \in [0:t]} \| \Phi_2(s, y^{(1)}_{[0:s]}) \|_2 < \infty$, together with (path-) Lipschitz continuity of $\Phi_2$ yields
% \begin{align*}
%     \eqref{t:gammaF} 
%     & \leq \epsilon_I + \sum_{i = 1}^I \big\| y^{(2)}_{[0:s_i]} - y^{(1)}_{[0:s_i]} \big\|_2  \big\Vert \Phi_2(s_i, y^{(1)}_{[0:s_i]}) - \Phi_2(s_{i-1}, y^{(1)}_{[0:s_{i-1}]}) \big\Vert_2 
%       \leq \epsilon_I + K t \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t ,
% \end{align*}
% which holds for $\epsilon_I \to 0$ for $I \to \infty$; we conclude that $\eqref{t:gammaB} \leq K \Vert y^{(2)}_{[0:t]} - y^{(1)}_{[0:t]} \Vert_t$. Eventually, consider
% \begin{align*}
%     \eqref{t:gammaC} 
%     \leq \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) - \Phi_1(s, y^{(2)}_{[0 : s]}) \big\|_2 \big\|\mu^{(2)}_s \big\|_2 ds 
%     \leq  K t \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t \max_{s \in [0:t]} \big\|\mu^{(2)}_s \big\|_2
% \end{align*}
% what holds due to Lipschitz continuity of $\Phi_1$. We conclude, since $\max_{s \in [0:t]} \|\mu^{(2)}_s \|_2 < \infty$ due to \Cref{lem:TimeLipschitzMu}, that $\eqref{t:gammaC} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$, and therefore $\gamma(t)\leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$.
% \medskip

% With that, we are able to apply Gr\"{o}nwall's inequality and obtain
% \begin{align} 
% \big\| \mu^{(1)}_t - \mu^{(2)}_t \big\|_2  
%     & \leq \gamma(t) + \int_0^t \gamma(s) \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%     \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds  
%     \notag   \\
%     & \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t
%         \left( 
%             1
%             + \int_0^t \big\| \Phi_1(s, y^{(1)}_{[0 : s]}) \big\|_2 
%               \exp\Big( \int_s^t \big\| \Phi_1(r, y^{(1)}_{[0 : r]}) \big\|_2 d r \Big) ds   
%         \right)
%      \notag  
% \end{align} 
% As $\Phi_1$ is (time-)Lipschitz continuous, implying $\max_{s \in [0:t]} \| \Phi_1(s, y^{(1)}_{[0:s]}) \|_2 < \infty$ we conclude the proof. 
% \end{proof}\setcounter{termcounter}{0}

% \begin{lemma}[Global Lipschitz-continuity of $\mu$ in time]\label{lem:TimeLipschitzMu}
%     Let the assumptions of \Cref{lem:LipschitzPhi1} and \Cref{lem:LipschitzPhi2} be fulfilled. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \mu_t - \mu_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\mu$ is defined as in \eqref{id:ClosedFormMu}.
% \end{lemma}
% \begin{proof}
%     With the notation of \Cref{lem:LipschitzMu}, we have
%     \begin{align*}
%             \| \mu_t - \mu_s \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_s^t a_0(u, y_{[0, u]})du \Big\Vert_2}_{\term{t:muA}}
%           + \underbrace{\Big\Vert\int_s^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{\term{t:muB}}
%           + \underbrace{\Big\Vert \int_s^t \Phi_1(u, y_{[0, u]})\mu_u du \Big \Vert_2}_{\term{t:muC}}.
%     \end{align*}
    
%     We see that $\eqref{t:muA} \leq K \vert t - s \vert$ as $\max_{u \in [0:T]}\Vert a_0(u, y_{[0:u]}) \Vert_2 < \infty$ due to (time-)Lipschitz-continuity of $a_0$.

%     By the use of integration by parts,
%     \begin{align*}
%         \eqref{t:muB}  
%         & = 
%         \Big\| 
%               \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%             - \Phi_2(s, y_{[0:s]}) y_{[0:s]} 
%             - \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%         \Big\|_2 \\
%         & \leq 
%             \underbrace{
%             \Big\| 
%                   \Phi_2(t, y_{[0:t]}) y_{[0:t]} 
%                 - \Phi_2(0, y_0) y_0 
%             \Big\|_2
%             }_{\term{t:muB1}}
%         +
%             \underbrace{
%             \Big\|
%                 \int_0^t y_{[0:u]} \, d \Phi_2(u, y_{[0:u]})
%             \Big\|_2 
%             }_{\term{t:muB2}},
%     \end{align*}
%     we see that $\eqref{t:muB1} \leq K \Vert y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \Vert_t$ due to (path-)Lipschitz continuity of $\Phi_2$. 
%     Moreover, let $\mySet{[u_{i-1}:u_{i}]}{i \in \myset{1}{I}}, I \in \N$ be a fine enough partition of $[s:t]$, then we see due to global (time-)Lipschitz continuity of $\Phi_2$ and the definition of the Riemann-Stieltjes integral that 
%     \begin{align*}
%         \eqref{t:muB2} 
%         & \leq \epsilon_I + \sum_{i = 1}^I   \Vert y_{[0:u_i]} \Vert_2  \big\| \Phi_2(u_i, y_{[0:u_i]}) - \Phi_2(u_{i-1}, y_{[0:u_{i-1}]})  \big\|_2 
%         \leq \epsilon_I + \Vert y_{[0:t]} \Vert_t \sum_{i = 1}^I K \vert u_i - u_{i-1} \vert
%     \end{align*}
%     and, since $\epsilon_I \to 0$ for $I \to \infty$, it follows $\eqref{t:muB} \leq K \vert t - s \vert$.

%     Due to $\eqref{t:muA} < \infty$ and $\eqref{t:muB} < \infty$, we can apply Gr\"onwalls inequality to 
%     \begin{align*}
%             \| \mu_t \|_2 
%         \leq 
%             \underbrace{\Big\Vert \int_0^t a_0(u, y_{[0, u]})du \Big\Vert_2
%           + \Big\Vert\int_0^t \Phi_2(u, y_{[0, u]})dy_{[0, u]} \Big\Vert_2}_{:= \alpha(t)}
%           + \int_0^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big\Vert_2 du,
%     \end{align*}
%     which yields
%     \begin{align*}
%             \| \mu_t \|_2 
%         & \leq 
%             \alpha(t) + \int_0^t \alpha(s)\big\Vert \Phi_1(s, y_{[0, s]}) \big \Vert_2
%             \exp\left(
%                 \int_s^t \big\Vert \Phi_1(u, y_{[0, u]}) \big \Vert_2 du 
%             \right) ds 
%         \leq 
%             K t 
%     \end{align*}
%     where the last equality holds due to $\alpha(s) \leq K s$ for all $s \in [0:T]$ and (time-)Lipschitz continuity of $\Phi_1$, implying $\max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 < \infty$. 

%     With that, we have
%     \begin{align*}
%         \eqref{t:muC} \leq  \int_s^t \big\Vert \Phi_1(u, y_{[0, u]})\big\Vert_2 \big\Vert \mu_u \big \Vert_2du   \leq \max_{u \in [0:t]}\Vert \Phi_1(u, y_{[0:u]}) \Vert_2 K T \vert t - s \vert
%     \end{align*}
%     what proves the claim.
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi1}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_1$, $ (b \circ B)$, $(B\circ B)^{-1}$, $ A_0$, and $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_1(t, y_{[0:t]}) - \Phi_1(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_1$ is defined as in \eqref{id:Phi1}.
%         \item Also, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_1(t, y^{(1)}_{[0:t]}) - \Phi_1(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
% \begin{enumerate}[wide]
%     \item The statement holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are globally Lipschitz continuous w.r.t. the time component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%     \item The assertion holds if $a_1$, $ (b\circ B)(B\circ B)^{-1}A_0$, $ (b\circ B)(B\circ B)^{-1}A_1$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_0$, $ \Sigma_\cdot A_1(B\circ B)^{-1}A_1$ are locally Lipschitz continuous w.r.t. the path component. As $a_1$, $ (b \circ B)$, $ \Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_0$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
% \end{enumerate}
% \end{proof}

% \begin{lemma}\label{lem:LipschitzPhi2}
%     In the notation of \Cref{lem:LipschitzMu}, assume $a_0$, $(b \circ B)$, $(B\circ B)^{-1}$, $ A_1$ are globally Lipschitz continuous in the time component and locally Lipschitz continuous in the path component. Further, let the assumptions of \Cref{lem:LipschitzSigma} as well as \Cref{lem:TimeLipschitzSigma} be fulfilled. Then,
%     \begin{enumerate}
%         \item for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%         \begin{align*}
%             \| \Phi_2(t, y_{[0:t]}) - \Phi_2(s, y_{[0:s]}) \|_2 \leq K \vert t-s \vert. 
%         \end{align*}
%         where $\Phi_2$ is defined as in \eqref{id:Phi2}.
%         \item Additionally, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
%         \begin{align*}  
%             \big\| \Phi_2(t, y^{(1)}_{[0:t]}) - \Phi_2(t, y^{(2)}_{[0:t]}) \big\|_2 
%             \leq K \big\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \big\|_t.
%         \end{align*} 
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}[wide]
%         \item The assertion holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are globally Lipschitz continuous w.r.t. the time component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ satisfy this already (see \Cref{lem:TimeLipschitzSigma}) and with this are also bounded on the interval $[0:T]$, their product is globally Lipschitz continuous w.r.t. time as well. 
%         \item The statement holds if $a_0$, $(b \circ B)(B\circ B)^{-1}$, $\Sigma_\cdot A_1(B\circ B)^{-1}$ are locally Lipschitz continuous w.r.t. the path component. As $a_0$, $(b \circ B)$, $\Sigma_\cdot$, $ (B\circ B)^{-1}$, $ A_1$ are locally Lipschitz continuous w.r.t. the path component (see \Cref{lem:LipschitzSigma}) this also follows for their product. 
%     \end{enumerate}
% \end{proof}

% \begin{lemma}[Local Lipschitz-continuity of $\Sigma$]\label{lem:LipschitzSigma}
%  Fix $t \in [0, T]$. Under assumptions of \Cref{lem:LipschitzA1}, $\Sigma_\cdot$ from \eqref{id:ClosedFormSigma} is locally Lipschitz-continuous. This means, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\epsilon > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$ holds
% \begin{align*}  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq K \big\| y^{1}_{[0:t]} - y^{2}_{[0:t]} \big\|_t ,
%  \end{align*} 
%  where $\Vert \cdot \Vert_2$ on the left hand side refers to the Forbenius norm.
% \end{lemma} 
% \begin{proof} 
% From \eqref{id:ClosedFormSigma}, we obtain the integral representation of $\Sigma_t$
% \allowdisplaybreaks
% \begin{align} 
% \Sigma_t = & \Sigma_0 + \int_0^t
% a_1(t,y_{[0:s]}) \Sigma_s + \Sigma_s a_1^{\intercal}(s,y_{[0:s]}) + (b\circ b)(s,y_{[0:s]}) - [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]}) ]
%    \notag      \\
%         & \hspace{3cm} \times (B\circ B)^{-1} (s,y_{[0:s]}) [(b\circ B)(s,y_{[0:s]}) + \Sigma_s A_1^{\intercal}(s,y_{[0:s]})]^{\intercal} ds . \notag  
% \end{align} 
% Let $\Sigma^{(1)}_t$, $\Sigma^{(2)}_t$ be the covariance matrices corresponding to paths $y^{(1)}_\cdot, y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ where $y^{(1)}_\cdot$ is arbitrary and $y^{(2)}_\cdot$ s.t. $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \epsilon$. The difference $\Sigma^{(1)}_t - \Sigma^{(2)}_t$ satisfies the integral representation
% \allowdisplaybreaks 
% \begin{align*} 
% & \Sigma^{(1)}_t - \Sigma^{(2)}_t \\
% & = \Sigma^{(1)}_0 - \Sigma^{(2)}_0 
%   + \int_0^t 
%  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  d s 
% \\ 
% & \quad + \int_0^t (\Sigma^{(1)}_s - \Sigma^{(2)}_s) 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) + 
% \Xi_2^\intercal (s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  (\Sigma^{(1)}_s - \Sigma^{(2)}_s) ds , 
% \end{align*} 
% where we denote 
% \allowdisplaybreaks
% \begin{align} 
%         & \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)\notag \\ 
%     & \quad\quad\quad \eqdef  
%             (a_1(s, y^{(1)}_{[0:s]}) - a_1(s, y^{(2)}_{[0:s]}) ) \Sigma^{(1)}_s
%         +
%             \Sigma^{(1)}_s (a_1^\intercal(s, y^{(1)}_{[0:s]}) - a_1^\intercal(s, y^{(2)}_{[0:s]})) \notag \\
%         & \quad\quad\quad\quad +
%             (b\circ b)(s, y^{(1)}_{[0:s]}) - (b\circ b) (s, y^{(2)}_{[0:s]}) \notag\\ 
%         & \quad\quad\quad\quad -
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(1)}_{[0:s]}) 
%                 - 
%                     A_1^\intercal (B\circ B)^{-1} (b\circ B)(s, y^{(2)}_{[0:s]})
%             ] \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(1)}_{[0:s]}) 
%                 -
%                     (b\circ B) (B\circ B)^{-1} A_1(s, y^{(2)}_{[0:s]}) 
%              ] \Sigma^{(2)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             \Sigma^{(2)}_s [
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(1)}_{[0:s]}) 
%                 -
%                     A_1^\intercal (B\circ B)^{-1} A_1(s,y^{(2)}_{[0:s]})
%             ] \Sigma^{(1)}_s \notag\\ 
%         & \quad\quad\quad\quad - 
%             [
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(1)}_{[0:s]})
%                 -
%                     (b\circ B) (B\circ B)^{-1} (b\circ B)^\intercal(s, y^{(2)}_{[0:s]}) 
%             ] \label{Xi1}
% \end{align} 
% and 
% \allowdisplaybreaks 
% \begin{align} 
% \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \eqdef & \big[ a_1^\intercal(s, y^{(2)}_s) 
%  + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) (b\circ B) (s, y^{(1)}_{[0:s]}) \notag \\ 
% &\quad + A_1^\intercal(s, y^{(1)}_{[0:s]}) 
%  (B\circ B)^{-1}(s, y^{(1)}_{[0:s]}) A_1(s, y^{(1)}_{[0:s]}) \Sigma^{(1)}_s
% \big] .   \label{Xi2} 
% \end{align} 
% By the triangular inequality, Jensen's inequality, and Cauchy-Schwarz inequality, we have 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 
%  \leq & \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 
%   + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds \notag \\ 
%   & + 2 \int_0^t \big\| \Sigma^{(1)}_s - \Sigma^{(2)}_s \big\|_2 \cdot \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%    ds . \notag 
% \end{align}  
% By Gr\"{o}nwall's inequality, it holds that 
% \begin{align} 
%  &\big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\
% & \leq  
% \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^t \big\| \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 ds 
%  \notag \\ 
%  & \quad  + \int_0^t 
%  \Big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \int_0^s \big\| \Xi_1(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 d r 
%  \Big)  \cdot \notag \\ 
%  & \quad \qquad \cdot 2 \big\|  \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big\|_2 \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s . \label{Gronwall:Sigma1-Sigma2} 
% \end{align}  
% From \Cref{lem:LipschitzA1}, we have that 
% \begin{align} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
%   \label{Xi1Lip}
% \end{align} 
% Combining \eqref{Gronwall:Sigma1-Sigma2} and \eqref{Xi1Lip}, we obtain
% \allowdisplaybreaks 
% \begin{align} 
%  & \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  \notag \\ 
% &\quad \leq  
% \big( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2  + KT \big\| y^{(1)} - y^{(2)} \big\|_T \big) 
% \cdot \notag \\ 
% &\quad  \cdot \Big[ 1+  \int_0^t 2 \big\| \Xi_2(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
% \exp \Big( 2 \int_s^t \big\|  \Xi_2(r, y^{(1)}_{[0:r]}, y^{(2)}_{[0:r]}, \Sigma^{(1)}_r, \Sigma^{(2)}_r) \big\|_2 
%  d r  \Big) d s \Big] .  
%  \label{Sigma1-2bddXi2}
% \end{align} 
% Since $a_1$, $A_1$, $(B\circ B)^{-1}$
%  and $b\circ B$ are globally (time-) Lipschitz continuous, $\Xi_2$ is also uniformly bounded, according to \eqref{Xi2}. 
%  Therefore, from \eqref{Sigma1-2bddXi2} we obtain that 
% \begin{align} 
%  \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2  
% \leq 
% K ( \big\| \Sigma^{(1)}_0 - \Sigma^{(2)}_0 \big\|_2 + \big\| y^{(1)} - y^{(2)} \big\|_T ) .  \notag  
% \end{align}

% \end{proof} 

% \begin{lemma}\label{lem:LipschitzA1}
% Let $\Xi_1$ be defined as in \eqref{Xi1}, and assume local Lipschitz continuity in the path component as well as time-continuity of $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$.
% Then, for every path $y^{(1)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ there exists constant $K \in \R$, $\delta > 0$ such that for all paths $y^{(2)}_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ with $\| y^{(1)}_{[0:t]} - y^{(2)}_{[0:t]} \|_t < \delta$ holds
% \begin{align*} 
%  \big\|  \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s)  \big\|_2 
%   \leq K \big\| y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\|_s . 
% \end{align*} 
% \end{lemma}
% \begin{proof}
%     Since $a_1$, $b \circ b$, $b \circ B$, $A_1$, $(B \circ B)^{-1}$ are locally Lipschitz continuous in the path component, we conclude that $a_1$, $b \circ b$, $A_1^\intercal(B \circ B)^{-1}(b \circ B)$, $(b \circ B)(B \circ B)^{-1}A_1$, $A_1^\intercal (B \circ B)^{-1}A_1$, and $(b \circ B)(B \circ B)^{-1}(b \circ B)^\intercal$ have the same property. By this, together with the triangular inequality, 
%     \begin{align*}
% \big\Vert \Xi_1(s, y^{(1)}_{[0:s]}, y^{(2)}_{[0:s]}, \Sigma^{(1)}_s, \Sigma^{(2)}_s) \big \Vert  & \leq  
%  2K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(\big\Vert\Sigma^{(1)}_s\big\Vert_2 + \big\Vert\Sigma^{(2)}_s \big\Vert_2\Big) + \\
% & \qquad + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \big\Vert\Sigma^{(1)}_s\big\Vert_2\big\Vert\Sigma^{(2)}_s\big\Vert_2 + 
%  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \\
% & =  K \big\Vert y^{(1)}_{[0:s]} - y^{(2)}_{[0:s]}  \big\Vert_s \Big(1+ \Vert\Sigma^{(1)}_s \big\Vert_2 + \Vert\Sigma^{(2)}_s \big\Vert_2 + \big\Vert\Sigma^{(1)}_s\big\Vert_2 \big\Vert\Sigma^{(2)}_s \big\Vert_2 \Big).
% \end{align*}
% With that, it is left to show that $\Vert\Sigma^{(1)}_s \Vert_2 < \infty$ and $\Vert\Sigma^{(2)}_s \Vert_2 < \bar{K} \in \R$. The former is trivially fulfilled due to the continuity of $a_1, b \circ b, b \circ B, A_1, (B \circ B)^{-1}$. 
% Since $\Sigma_t$ is continuous in $y_{[0:t]}$, for any $\epsilon>0$, there exists $\delta>0$ such that 
% when 
% $\| y^{(1)}_t - y^{(2)}_t \|_2 < \delta$,  
% $\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \|_2 < \epsilon$, and therefore 
% \begin{align*} 
% \big\| \Sigma^{(2)}_t \big\|_2 \leq \big\| \Sigma^{(1)}_t - \Sigma^{(2)}_t \big\|_2 + \big\| \Sigma^{(1)}_t \big\|_2 
% \leq \epsilon + K . %\label{Sigma2bdd} 
% \end{align*} 
% \end{proof}

% \begin{lemma}[Global Lipschitz-continuity of $\Sigma$ in time]\label{lem:TimeLipschitzSigma}
%     Let $a_1, b \circ b, b \circ B, (B \circ B)^{-1}, b \circ B, A_1$ be continuous. Then, for any path $y \in C([0:T]), \R^d)$ there is a constant $K \in \R$ s.t. for all $t > s \in [0:T]$ holds
%     \begin{align*}
%         \| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert. 
%     \end{align*}
%     where $\Sigma$ is defined as in \eqref{id:ClosedFormSigma}.
% \end{lemma}
% \begin{proof}
%     Note that $\Sigma_\cdot$ is continuous in time. From \eqref{id:ClosedFormSigma}, we obtain
% \allowdisplaybreaks
% \begin{align*} 
% \Vert \Sigma_t  - \Sigma_s \Vert_2 
%     = & \int_s^t
%           \Vert a_1(t,y_{[0:u]}) \Sigma_u \Vert_2
%         + \Vert \Sigma_u a_1^{\intercal}(u,y_{[0:u]}) \Vert_2
%         + \Vert (b\circ b)(u,y_{[0:u]}) \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  (b\circ B)(u,y_{[0:u]})
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  (b\circ B)(u,y_{[0:u]})^{\intercal} \Vert_2 \\
%       & \quad \quad
%         + \Vert  \Sigma_u A_1^{\intercal}(u,y_{[0:u]}) 
%                  (B\circ B)^{-1} (u,y_{[0:u]})
%                  \Sigma_u A_1^{\intercal}(u,y_{[0:u]})^{\intercal} \Vert_2
%     du .
% \end{align*} 
% As all components are continuous, we can bound them by their maximal value on $[0:T]$. With this, we conclude $\| \Sigma_t - \Sigma_s \|_2 \leq K \vert t-s \vert$.
% \end{proof}


% \begin{lemma}[Lower Loewner order bound]\label{lem:LoewnerBound}
%     Let $\Sigma$ be defined as in \Cref{id:ClosedFormSigma}, then there exists an $r > 0$, s.t. for all times $t \in [0,T]$ and paths  $y_\cdot \in C^{\color{blue} 1}([0, T], \R^{d_Y})$ holds that 
%     \begin{align*}
%         \Sigma_t - r \cdot I_{d_X}
%     \end{align*}
%     is positive semi-definite.
% \end{lemma}
% \yannick{TODO. Assumptions are highlighted below.}
% \begin{proof}
%     By the Courant-Fisher Theorem, see \cite{hornjohnson2012}, the statement is equivalent to finding a lower bound on the eigenvalues of $\Sigma$, which we will show by finding an upper bound on the Eigenvalues of $\Sigma^{-1}$, which exists as it is positive definite.
    
%     Following the proof of \cite[Theorem 12.7]{LipShiryaev_II_2001}, we note that 
%     \begin{align*}
%             \partial_t\Sigma_t^{-1} 
%         = &
%             - \Tilde{a}_1^\intercal(t, y_{[0:t]})\Sigma_t^{-1}
%             - \Sigma_t^{-1}\Tilde{a}_1(t, y_{[0:t]})
%             + A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]}) \\
%         &   - \Sigma_t^{-1}\left[
%                   (b \circ b)(t, y_{[0:t]})
%                 - (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})
%             \right]\Sigma_t^{-1}
%     \end{align*}
%     with 
%     \begin{align*}
%         \Tilde{a}_1^\intercal(t, y_{[0:t]}) \eqdef a_1(t, y_{[0:t]}) - (b \circ B)(B \circ B)A_1(t, y_{[0:t]}).
%     \end{align*}
%     Now, let $G_t(y_{[0:t]})$ be a solution of $\partial_tG_t(y_{[0:t]}) = \Tilde{a}_1(t, y_{[0:t]})G_t(y_{[0:t]})$ with $G_0(y_{[0:t]}) = I_{d_X}$. 
%     Then, as pointed out in \cite[Theorem 12.7]{LipShiryaev_II_2001}, we arrive due to \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ being positive semi-definite} at 
%     \begin{align*}
%             \tr( G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal )
%         \leq 
%                 \tr(\Sigma_0^{-1})
%             +
%                 \int_0^T
%                     \tr\left(
%                         G_s(y_{[0:s]})
%                         A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                         G_s(y_{[0:s]})^\intercal
%                     \right)
%                 ds.
%     \end{align*}
%     As \byyan{$G_t(y_{[0:t]})$ is positive definite}, we conclude by submultiplicativity of positive semi-definite matrices that 
%     \begin{align*}
%             \tr(\Sigma_t^{-1})
%         &\leq
%             \tr(
%                 G_t(y_{[0:t]})^{-1}
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%                 (G_t(y_{[0:t]})^{-1})^\intercal
%             ) \\
%         &\leq 
%             \tr(G_t(y_{[0:t]})^{-1})^2
%             \tr(
%                 G_t(y_{[0:t]}) \Sigma_t^{-1} G_t(y_{[0:t]})^\intercal
%             )
%     \end{align*}
%     and 
%     \begin{align*}
%             \tr\left(
%                 G_s(y_{[0:s]})
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%                 G_s(y_{[0:s]})^\intercal
%             \right)
%         \leq 
%             \tr\left(
%                 G_s(y_{[0:s]})
%             \right)^2
%             \tr\left(
%                 A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]})
%             \right).
%     \end{align*}
%     As we \byyan{assumed that there exist constants $K_1, K_2 > 0$ s.t. uniformly $K_1 \leq \tr(G_t(y_{[0:t]})) \leq K_2$} as well as \byyan{$K_3 > 0$ s.t. $\tr(A_1^\intercal(B \circ B)^{-1}A_1(t, y_{[0:t]})) \leq K_3$} we conclude $\tr(\Sigma_t^{-1}) < K$ uniformly for some constant $K > 0$. As the trace is the sum of all Eigenvalues, this proves the claim.
%     % As \byyan{$(b \circ b)(t, y_{[0:t]})- (b \circ B)(B \circ B)(b \circ B)^\intercal(t, y_{[0:t]})$ is positive semi-definite} we conclude that 
%     % \begin{align*}
%     %         \tr( \Sigma_t^{-1} )
%     %     \leq &
%     %         \int_0^t
%     %             - 2\tr(\Tilde{a}_1^\intercal(s, y_{[0:s]})\Sigma_t^{-1})
%     %             + \tr(A_1^\intercal(B \circ B)^{-1}A_1(s, y_{[0:s]}))
%     %         ds
%     % \end{align*}.
%     % \yannick{I don't see a nice way of controlling the first term in here. WE could follow the argumentation in \cite{LipShiryaev_II_2001}, but I don't fully understand how they get rid of the term there... If that is the case, we need some assumptions on this fundamental matrix $G$ that they are using.}
% \end{proof}


% % \subsection{The Non-Euclidean Kernel Regressor}
% % Let $\mathcal{N}$ denote the space of $d_X$-dimensional Gaussian measures $\mathcal{N}(\mu,\Sigma)$ with mean $\mu\in \mathbb{R}^{d_{X}}$ and non-singular covariance matrix $\Sigma$.  
% % Following \citep[Section 4.4.2]{kratsios2021universal}, we note that $\mathcal{N}$ can be bijectively parameterized by $\mathbb{R}^{d_X+d_X(d_X+1)/2}$ via
% % \begin{equation}
% % \label{eq:parameterization}
% % \begin{aligned}
% %     \psi:\mathbb{R}^{d_X(d_X+3)/2} & \rightarrow \mathcal{N}\\
% %         \psi(\mu,\sigma) 
% %     & \eqdef 
% %         \mathcal{N}
% %         \left(
% %                 \mu
% %             ,
% %                 \exp\circ \operatorname{sym}(\sigma)
% %         \right)
% % \end{aligned}
% % \end{equation}
% % where $\exp$ is the matrix exponential and $\operatorname{sym}$ is the \textit{symmetrized vectorization operation} defined \byyan{as in \cite{herrera2023Denise_TMLR}} for any $\sigma\in \mathbb{R}^{d_X(d_X+1)/2)}$ by
% % \[ 
% %         \operatorname{sym}(\sigma)
% %     \eqdef
% %         \begin{pmatrix}
% %         \sigma_1 & \sigma_2 & \dots & \sigma_{d_X} \\
% %         \sigma_2 & \sigma_3 & \dots & \sigma_{2d_X -1 } \\
% %         \vdots & \vdots& \ddots & \vdots \\
% %         \sigma_{d_X}& \sigma_{2d_X-1}& \dots & \sigma_{2d_X}
% %     .
% %         \end{pmatrix}
% % \]


% \section{Proof of Approximation Theorem}
% \label{s:Proof}
% This section contains the derivations of our paper's main results.

% \subsection{ The Attention Layer Implements Good Feature Maps}
% \begin{proof}[{Proof of Proposition~\ref{prop:Non_Vaccousness}}]
% Since $(\mathcal{X},d_{\mathcal{X}})$ is compact then the Kuratowksi embedding $\phi_1:\,x\mapsto d_{\mathcal{X}}(\cdot,x)$ is an isometric embedding of $\mathcal{X}$ into the Banach space $C(\mathcal{X})$ with its uniform norm (since $\mathcal{X}$ is compact); where $d_{\mathcal{X}}$ denotes the metric on $\mathcal{X}$.  By the Banach-Mazur theorem, there exists an isometric embedding of $\phi_2:C(\mathcal{X})\rightarrow C([0,1])$.  
% Since the map $\psi_3:C([0:1])\rightarrow C([0:T],\mathbb{R}^d)$, given by $f\mapsto \big(f(\cdot /T),0,\dots,0\big)$, is an isometric embedding; then $\phi\eqdef \phi_3\circ\phi_2\circ \phi_1$ is an isometric embedding of $\mathcal{X}$ into $C([0:T],\mathbb{R}^d)$.
% \end{proof}


% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Qualitative Version]
% \label{lem:Good_Feature_Map_Qualitative}
% Under Assumption~\ref{ass:reg_compact} (i).  There exist $y^{(1)},\dots,y^{(N)}\in \psi(M)\subset C([0:T],\mathbb{R}^d)$ and matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a continuous injective map.  
% Here, $N=D_K+1$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map_Qualitative}}]
% \anastasis{Add details:}
% Since $(M,g)$ is a connected, homogeneous, geodesically complete Riemannian manifold of dimension $D_K$ then, \citep[Corollary 3.7]{HeydarpourMaghsoudi_2015_MetricDimension_GeometricSpaces} implies that there exist $p^{(1)},\dots,p^{(N)}$, with $N=D_K+1$, such that the map $p\mapsto \big(d_g(p,p_n)\big)_{n=1}^N$ is injective.  Clearly, the map $\big(d_g(p,p_n)\big)_{n=1}^N$ is continuous since the metric $d_g$ is a continuous function.  
% \end{proof}


% In the case where the ``latent geometry'' of $K$ has additional structure, we may guarantee that the attention mechanism $\operatorname{attn}_T$ is linearly-stable with linearly-stable inverse, how to generate the reference paths $y^{(1)}$, $\dots$, $y^{(N)}$ in $C([0:T],\mathbb{R}^d)$, and quantitative estimates on how many paths must be generated.  

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Quantitative Version]
% \label{lem:Good_Feature_Map}
% Under Assumption~\ref{ass:reg_compact} (ii).  
% There exists a constant $C_{D_K}>0$ depending only on $D_K$ such that for and $\delta$-packing $\{y^{(n)}\}_{n=1}^N$ of $K$, and matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a bi-Lipschitz embedding
% of $K$ into $(\mathbb{R}^{N+1},\|\cdot\|_2)$ provided that
% \[
%         \delta 
%     \lesssim 
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \]
% where $\lesssim$ hides a constant $C_{D_K}>0$ depending only on $D_K$.  Furthermore\footnote{\anastasis{Define $\|\cdot\|_0$-notation.}}, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$, and $C_{D_K}< (3/5)\, (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any sampling distribution $\mathbb{P}_{in}$ with support $K$.\anastasis{define in intro.}
% \hfill\\
% Moreover, if $K$ is not aspherical then the conclusion holds without a quantitative upper-bound on $\delta$, and therefore on $N$.
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Good_Feature_Map}}]
% \noindent\textbf{Step 1 - Estimating $N$ on the Riemannian Manifold $(M,g)$}
% \hfill\\
% %%
% Since $(K,\|\cdot\|_T)$ be isometric to $(M,d_g)$ where $d_g$ is the geodesic distance on an aspherical compact $D_K$-dimensional Riemannian manifold $(M,g)$, then Gromov's systolic inequality \citep[Theorem 0.1.A]{gromov1983filling} implies that the systole of $M$ denoted by $\operatorname{sys}(M)$ satisfies
% \begin{equation}
% \label{eq:Systolic}
%         \operatorname{sys}(M) 
%     \le
%     \,\tilde{C}_{D_K}
%     \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     ,
% \end{equation}
% where $\operatorname{Vol}(M,g)$ denotes the Riemannian volume of $(M,g)$ and $\lesssim$ hides a constant depending only on the dimension $D_K$, for a universal constant $\tilde{C}_{D_K}>0$ satisfying
% \[
%         0
%     <
%         \tilde{C}_{D_K}
%     <
%         6 (D_K+1)D_K^{D_K}\,\sqrt{(D_K+1)!}
% \,
% .
% \]
% In the proof of \cite[Theorem 1]{katz2011bi} (circa \cite[Equation (1.1)]{katz2011bi}) we see that if $\delta = \operatorname{Sys}(M)/10$ then the given any $\delta$-net $\widetilde{\mathbb{X}}$ in $(M,g)$, the map $\varphi_2:(M,d_g)\mapsto (\mathbb{R}^{\#\widetilde{\mathbb{X}}},\|\cdot\|_2)$ given for any $p\in M$ by
% \[
%     \varphi_2:p\mapsto \big(d_g(p,u)\big)_{u\in \widetilde{\mathbb{X}}}
% \]
% is a bi-Lipschitz embedding.  Set $C_{D_K}\eqdef \tilde{C}_{D_K}/10$, $N\eqdef \#\widetilde{\mathbb{X}}$, and enumerate $\widetilde{\mathbb{X}}\eqdef \{u_n\}_{n=1}^N$.  Therefore,
% \[
%         \delta 
%     \le
%         C_{D_N}
%         \,
%         \operatorname{Vol}(M,g)^{1/D_K}
%     .
% \]
% We note that, if $K$ is not aspherical, then but it is only closed, then the conclusion still holds however, without the quantitative upper-bound on $\delta$.
% \hfill\\
% \noindent\textbf{Step 2 - Building the Feature Map with Well-posed Inverse}
% \hfill\\
% %%
% Let $\varphi_1:(M,d_g)\rightarrow (K,\|\cdot\|_T)$ by an any isometry, which we have assumed to exist.  Set $\mathbb{X}\eqdef \{\varphi(u):\,u\in \widetilde{\mathbb{X}}\}=\{y^{(n)}\}_{n=1}^N$ where, for $n=1,\dots,N$ we set $y^{(n)}\eqdef \phi_1(u_n)$.  
% Define $\varphi: C([0,T],\mathbb{R}^d)\rightarrow \mathbb{R}^N$ by $y_{\cdot}\mapsto (\|y_{\cdot}-y^{(n)}_{\cdot}\|_{T})_{n=1}^N$.  Observe that, for every path $y\in K$, the following holds
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         \varphi(y_{\cdot})
%     \eqdef &
%         \Big(
%             \|y_{\cdot}-y^{(n)}_{\cdot}\|_{T}
%         \Big)_{n=1}^N
% \\
% \nonumber
% = &
%         \Big(
%             \big\|
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                 -
%                 \varphi_1\circ \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big\|_T
%         \Big)_{n=1}^N
% \\
% \label{proofFeatureMap_isometry_assumption}
% = &
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 \varphi_1|_{\phi(K)}^{-1}(y^{(n)}_{\cdot})
%             \big)
%         \Big)_{n=1}^N
% \\
% = &
% \label{proofFeatureMap_injectivity}
%         \Big(
%             d_g\big(
%                 \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
%                     , 
%                 u^n
%             \big)
%         \Big)_{n=1}^N
% \\
% \nonumber
% = & 
%     \varphi_2\circ \varphi_1|_{\phi(K)}^{-1}(y_{\cdot})
% ,
% \end{align}
% where~\eqref{proofFeatureMap_isometry_assumption} holds since $\varphi_2$ is an isometry and~\eqref{proofFeatureMap_injectivity} holds unambiguously since $\varphi_1$ is a bijection from $M$ to $K$.  Since every isometry is a bi-Lipschitz map, the compositions of bi-Lipschitz maps is again bi-Lipschitz, and since we have just shown that $\varphi|_{K}=\varphi_2\circ \varphi_1|_{\phi(K)}^{-1}$ then, $\phi|_{K}$ is a bi-Lipschitz embedding of $K$ into the $N$-dimensional Euclidean space.
% \hfill\\
% \noindent\textbf{Step 3 - Aligning to a Hyperplane in $\mathbb{R}^{N+1}$ with a Shallow ReLU Neural Network}
% \hfill\\
% Set $N_1\eqdef N+1$.  Let $b$ be the zero vector in $\mathbb{R}^N$.
% A mild variation of the example on~\citep[page 3]{cheridito2021efficient}, the respective $N\times 2N$ and $2N\times N$ block-matrices $A_1$ and $B$
% \[
%         A_1
%     =
%         \begin{pmatrix}
%             I_N & \vert & -I_N
%         \end{pmatrix}
%     \mbox{ and }
%         B
%     =
%         \begin{pmatrix}
%             I_N \\
%             \-- \\
%             -I_N
%         \end{pmatrix}
% \]
% are such that the ReLU neural network $\tilde{\psi}:\mathbb{R}^N\rightarrow \mathbb{R}^N$ defined by $\tilde{\psi}(u)\eqdef A_1\operatorname{ReLU}\bullet(Bu+b)$ satisfies $\tilde{\psi}(u)=u$, for each $u\in \mathbb{R}^N$.  Consider the $N_1\times N$ block-matrix $A_2$ and the vector $a\in \mathbb{R}^{N_1}$ given by
% \[
%         A_2
%     =
%         \begin{pmatrix}
%             I_N & 0 \\
%             0 & 0 \\
%         \end{pmatrix}
%     \mbox{ and }
%         a_i 
%     =
%         \begin{cases}
%             0 & \mbox{ if } i=1,\dots,N\\
%             1 & \mbox{ if } i=N_1
%     .
%         \end{cases}
% \]
% Set $A\eqdef A_2A_1$, $\psi\eqdef A\operatorname{ReLU}\bullet(Bu+b)+a$, and note that $\psi$ is a ReLU neural network.  A direct computation shows that, $\|A\|_0=2N$, $\|B\|_0=2N$, $\|a\|_0=1$, and $\|b\|_0=0$.  
% \hfill\\
% \noindent\textbf{Step 4 - Injectivity of Softmax Function on Hyperplane}
% \hfill\\
% Note that, for each $u\in \mathbb{R}^N$
% \[
%     \psi(u) = (u_1,\dots,u_N,1)^{\top}
% ,
% \]
% therefore bijectively $\psi$ maps $\mathbb{R}^N$ onto the $N$-dimensional hyperplane $H\eqdef \{(u,1):\,u\in \mathbb{R}^N\}$ in $\mathbb{R}^{N_1}$.  Observe that the Softmax function $\operatorname{Softmax}:u\mapsto (e^{u_j}/\sum_{k=1}^N\,e^{u_k})_{j=1}^N$ maps $H$ surjectively and continuously onto the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})\subset \operatorname{int}(\Delta_N)\eqdef \{v\in [0,1]^{N_1}:\,\sum_{i=1}^{N_1}\,v_i=1\}$; i.e.\ of the interior of the $N_1$-simplex.  Since, 
% \begin{equation}
% \label{eq:inverse_softmax_interior}
%         v
%     \mapsto
%         \big(\ln(v_i)-\ln(v_{N_1}) + 1\big)_{i=1}^{N}
% \end{equation}
% is a continuous right-inverse of $\operatorname{Softmax}$ on the interior of the image set $\operatorname{Softmax}(\mathbb{R}^{N_1})$ then, the softmax function $\operatorname{Softmax}$ defines a continuous bijection from $H$ onto $\operatorname{Softmax}(\mathbb{R}^{N_1})$.  

% Therefore, the map $\Psi\eqdef \operatorname{Softmax}\circ \psi\circ \phi$ is a continuous and injective when restricted to $K$.  Since, $\Psi$ was constructed to be an instance of $\operatorname{attn}_T$.  
% %%%
% Since $K$ is compact and $\Psi$ is continuous then $\Psi(K)$ is a compact subset of the interior $\operatorname{int}(\Delta_N)$ of the $N_1$-simplex then, $C^{\star}\eqdef \max_{u\in \Phi(K)}\,\min_{v\in \Delta_{N_1}\setminus \operatorname{int}(\Delta_{N_1})}\,\|u-v\|>0$.  Therefore, $\Psi(K)$ is contained in the set
% \[
%         \Delta_{N_1}^{\star}
%     \eqdef 
%         \{
%             t^{\star}(u-\bar{\Delta}_{N_1})
%             +
%             \bar{\Delta}_{N_1}
%         \}
% \]
% where $\bar{\Delta}_{N_1}\eqdef (1/N_1,\dots,1/N_1)$ is the barycenter of the $N_1$-simplex $\Delta_{N_1}$ for some $t^{\star}\in [0,1)$ such that $\Psi(K)\subseteq \Delta_{N_1}^{\star}$ (which is possible since $C^{\star}>0$).  Since the map~\eqref{eq:inverse_softmax_interior} is Lipschitz\footnote{\anastasis{Add details about Lipschitzness? or Obvious?}} on $\Delta_{N_1}^{\star}$ then $\Psi$ has a Lipschitz inverse on its image, since it is the composition of Lipschitz functions with Lipschitz inverses.  This completes the proof.  

% \end{proof}

% \begin{lemma}[$\operatorname{attn}_T$ is a Good Feature Map - Finite Version]
% \label{lem:Good_Feature_Map__FiniteVariant}
% Under Assumption~\ref{ass:reg_compact} (i) and let $k\eqdef \#K$.  
% Set $N=48\lceil\log(k)\rceil$ and $\{y_i\}_{i=1}^k$ enumerate $K$.  
% There exists a matrices matrices $A,B,b$ such that
% the map $\operatorname{attn}_T$ defined by~\eqref{eq:featuremap} is a $(2^{-1/2},(3N/6)^{1/2})$-bi-Lipschitz embedding
% of $K$ into $(\mathbb{R}^{48\lceil \log(k)\rceil},\|\cdot\|_2)$.
% \hfill\\
% In particular, $\operatorname{attn}_T$ satisfies \citep[Setting 3.6 (i)]{kratsios2023transfer} for any sampling distribution $\mathbb{P}_{in}$ with support $K$.\anastasis{define in intro.}
% \end{lemma}
% \begin{proof}
% We argue similarly to the proof of Lemma~\ref{lem:Good_Feature_Map}, with only Steps $1$ and $2$ of its proof being replaced with the following argument.  
% \hfill\\
% \noindent\textbf{Step 1 and 2 - Modified- Building the Feature Map}
% \hfill\\
% Enumerate $K=\{x_n\}_{n=1}^N$.  The map $\phi_1:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^N,\|\cdot\|_{\infty})$ given by $x\mapsto \big(\|x-x_n\|_t\big)_{n=1}^N$ is an isometric embedding, called the \textit{Kuratowski embedding} (see \cite[page 99]{Heinonen_2001_BookAnalMetSpace}).  The optimal constants for the equivalence of the Euclidean $\|\cdot\|_2$ and max $\|\cdot\|_{\infty}$ norms are given by
% \begin{equation}
% \label{eq:equivalence_2infty_norms}
%     \|u\|_{\infty} \le \|u\|_2
%     \quad\mbox{ and }\quad
%     \|u\|_2\le N^{1/2}\,\|u\|_{\infty}
% \end{equation}
% for each $u\in\mathbb{R}^N$.  Therefore, the ``set theoretic identity map'' $\phi_2:(\mathbb{R}^N,\|\cdot\|_{\infty})\rightarrow (\mathbb{R}^N,\|\cdot\|_2)$ is bi-Lipschitz with optimal (shrinking and expansion) constants given by~\eqref{eq:equivalence_2infty_norms}.  
% By the Johnson-Lindenstrauss Lemma, as derived in \citep[Theorem 2.1]{DubhashiPanconesi_2009_Concentration}%%
% \footnote{We use this formulation since the constant in $48$ as opposed to $200$ in the standard derivation; found for example in \cite{JohnsonLindenstrauss_1984_originalpaper}.}%%%
% , there is a linear map $\phi_3:(\mathbb{R}^N,\|\cdot\|_2)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$, i.e.\ $\varphi_3(u)=A_0\,u$ for some $(\lceil48\,\ln(N)\rceil)\times N$-matrix $A_0$, satisfying: for every $u,v\in \mathbb{R}^N$
% \[
%     2^{-1/2}
%     \,
%     \|u-v\|_2
%     \le 
%         \|A_0\,u-A_0\,v\|_2
%     \le 
%     (3/2)^{1/2}
%     \,
%     \|u-v\|_2
%     .
% \]
% Consequentially, $\varphi:(K,\|\cdot\|_t)\rightarrow (\mathbb{R}^{\lceil48\,\ln(N)\rceil},\|\cdot\|_2)$ given by $\varphi\eqdef \varphi_3\circ \varphi_2\circ \varphi_1$ is $(2^{-1/2},(3N/2)^{1/2})$-bi-Lipschitz, since the Kuratowksi embedding $\varphi_1$ is an isometry and $\varphi_2$ satisfies~\eqref{eq:equivalence_2infty_norms}; this is because for each $x,\tilde{x}\in K$ we have
% \allowdisplaybreaks
% \begin{align*}
%     2^{-1/2}
%     \,
%         \|x-\tilde{x}\|_{t}
%     = &
%         2^{-1/2}
%     \,
%         \|\varphi_1(x)-\varphi_1(\tilde{x})\|_{\infty}
% \\
%     \le & 
%         2^{-1/2}
%     \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \eqdef &
%         \|\varphi(x)-\varphi(\tilde{x})\|_2  
% \\
%     \eqdef &
%         \|\varphi_3\circ \varphi_2\circ \varphi_1(x)-\varphi_3\circ \varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le &
%         (3/2)^{1/2}
%         \,
%         \|\varphi_2\circ \varphi_1(x)-\varphi_2\circ \varphi_1(\tilde{x})\|_2
% \\
%     \le & 
%         (3/2)^{1/2}
%         \,
%         N^{1/2}\,
%         \| \varphi_1(x)-\varphi_1(\tilde{x}) \|_{\infty} 
% \\
%     = & 
%         (3N/2)^{1/2}
%         \,
%         \| x-\tilde{x} \|_t 
% .
% \end{align*}
% \noindent\textbf{Remaining Steps:}
% \hfill\\
% The rest of the proof is identical to the proof of Lemma~\ref{lem:Good_Feature_Map} but with $B$ defined instead as $B\eqdef B_1A_0$, where $B_1=  (I_N\,\vert \,I_N)^{\top}$.
% \end{proof}

% \anastasis{Update Theorems to also include this case.}

% \subsection{Polish QAS Space Structure on the space of Positive Semi-Definite Matrices}
% \label{s:Proof__ss:Universality___sss:Outputs}
% Let $d\in \mathbb{N}_+$, and $\operatorname{Sym}_{0,d}$ denote the set of $d\times d$ symmetric positive semi-definite matrices and let $\|\cdot\|_F$ denote the Frobenius norm on the set of $d\times d$ matrices.  Here the $0$ emphasizes that there is no rank-restriction on the matrices in $\operatorname{Sym}_{0,d}$ unlike, for example, in \cite{herrera2023Denise_TMLR,neuman2023restricted}.  Consider the $2$-product metric on $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ defined for any $(m^{(1)},A),(m^{(2)},B)$ by
% \begin{equation}
% \label{eq:Quantization}
%         \operatorname{d}_{2,F}\big(
%             (m^{(1)},A),(m^{(2)},B)
%         \big)^2
%     \eqdef 
%         \|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2
% .
% \end{equation}

% We show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ satisfies the conditions of \citep[Theorem 3.7]{kratsios2023transfer}; namely \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% %
% This requires defining a few maps first.  
% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ by sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \] 
% The family $\mathcal{Q}\eqdef (\mathcal{Q}_q)_{q\in \mathbb{N}_+}$ will serve to quantize $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$, in the sense of \citep[Definition 3.2]{Acciaio2022_GHT}.

% Next, we consider the so-called \textit{mixing function }$\eta:\cup_{N\in \mathbb{N}_+}\,\Delta_N\times (\mathbb{R}^d\times \operatorname{Sym}_{0,d})^{N} \rightarrow 
% \mathbb{R}^d\times \operatorname{Sym}_{0,d}$, where $N\in\mathbb{N}_+$ and $\Delta_N$ is the $N$-simplex, defined for any $N\in\mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:MixingFunction}
%     \eta\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 w_n
%                 \cdot
%                 (m^{(n)},A^{(n)})
% .
% \end{equation}
% Note that by the convexity of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and the fact that each $w\in \Delta_N$, for some $N\in \mathbb{N}_+$, then $\eta$ does indeed take values in $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$.  The mixing function $\eta$ will be used to inscribe ``abstract geodesic simplices'' in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\operatorname{d}_{2,F})$ thereby endowing it with the structure of an approximately simplicial space, in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.


% \begin{lemma}
% \label{lem:QAS_Space_Sym0d}
% $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space, in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  In particular, it satisfies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.
% \end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lem:QAS_Space_Sym0d}]  
% We first show that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is a QAS space, as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  We also show that it is barycentric, meaning that it admits a $1$-barycenter map as defined, for example, in \citep[Section 3.2]{basso2018fixed}.
% \hfill\\
% \textbf{QAS Space Structure}
% \hfill\\
% Since $\operatorname{Sym}_{0,d}$ is a closed convex subset of space $(\mathbb{R}^{d\times d},\|\cdot\|_F)$.  Since the Cartesian product of closed subsets is a closed subset of $(\mathbb{R}^{d^2+d},d_{2,F})$ and since the product of convex sets is again convex by \citep[Proposition 3.6]{CombettesBauschke_Book_ConvexAnalysisMonotonOperators_2017} then, $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the normed space $(\mathbb{R}^{d+d^2},d_{2,F})$.  


% For $q\in \mathbb{N}$ define the map $\mathcal{Q}_q:\mathbb{R}^{d+d^2}\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ as sending any $(m,A)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ to
% \[
%         \mathcal{Q}_q((m,A)) 
%     \eqdef 
%         (m,A^{\top}A)
%     .
% \]
% The map $\mathcal{Q}_q$ is a surjection since every symmetric matrix is the square of some $d\times d$ matrix \cite{TBD}.  
% Therefore, $\mathcal{Q}_{\cdot}=(\mathcal{Q}_q)_{q\in\mathbb{N}_+}$ trivially satisfies \citep[Definition 3.2]{Acciaio2022_GHT} with modulus of quantizability, defined on \citep[page 12]{Acciaio2022_GHT}, given by $\mathcal{Q}_{K}(\varepsilon)=D_1\eqdef d(d+1)$ for every compact subset $K$ of $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and for every $\varepsilon>0$.  

% Observe that, for any $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d\times d}$ we have
% \allowdisplaybreaks
% \begin{align}
% \nonumber
%         d_{2,F}\Big(
%             \eta\big(
%                 w
%             ,
%                 \{(m^{(n)},A^{(n)}\}_{n=1}^N
%             \big)
%             ,
%                 y_i
%         \Big)
%     = &
%     \Big(
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,m^{(n)}\big) - m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 \big(\sum_{n=1}^N\,w_n\,A^{(n)}\big) - A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
%     \label{eq:Because_Simplex}
%     = &
%     \Big(
%             \big\|
%                 \sum_{n=1}^N\,w_n\,m^{(n)} 
%                     - 
%                 \sum_{n=1}^N\,w_n\,m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad
%         +
%             \big\|
%                 \sum_{n=1}^N\,w_n\,A^{(n)}
%                 - 
%                 \sum_{n=1}^N\,w_n\,A^{(i)}
%             \big\|_F^2
%     \big)^{1/2}
%     \\
% \nonumber
%     \le &
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
% \\
% \nonumber
% &\qquad            
%         +
%         \Big(\sum_{n=1}^N\,w_n\Big)^2\,
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     \le &
%     \sum_{n=1}^N\,w_n
%     \,
%     \Big(
%             \big\|
%                 m^{(n)} 
%                     - 
%                 m^{(i)}
%             \big\|^2
%         +
%             \big\|
%                 A^{(n)}) 
%                 - 
%                 A^{(i)}) 
%             \big\|_F^2
%     \big)^{1/2}
% \\
% \nonumber
%     = &
%     1\cdot
%     \sum_{n=1}^N\,w_n
%     \,
%         d_{2,F}\big(
%             (m^{(n)},A^{(n)})
%             ,
%             (m^{(i)},A^{(i)})
%             \big)^1
% ,
% \end{align}
% for $i=1,\dots,N$,
% where~\eqref{eq:Because_Simplex} holds since $\sum_{n=1}^N\,w_n=1$ since $w\in \Delta_N$.  Thus, $\eta$ is a mixing function and therefore $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is approximately simplicial, as defined in \citep[Definition 3.1]{Acciaio2022_GHT}.
% Consequentially, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\mathcal{Q},\eta)$ is a QAS space; as defined in \citep[Definition 3.4]{Acciaio2022_GHT}.  
% \hfill\\
% \textbf{Barycentricity}
% \hfill\\
% Consider the map $\sigma:(\mathbb{R}^d\times \operatorname{Sym}_{0,d})^2\times [0,1]$ given for any $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ and $t\in [0,1]$ by
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),t
%         \big)
%     \eqdef 
%         \eta\big(
%             (m,A),(\tilde{m},B),(t,1-t)
%         \big)
%     .
% \]
% Since geodesics in $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ are line segments, since $\mathbb{R}^d\times \operatorname{Sym}_{0,d}$ is a closed and convex subset of the inner-product space $(\mathbb{R}^d\times \operatorname{Sym}_d)$, with inner-product given by the product of the Euclidean and Frobenius inner-products, then clearly for each $(m,A),(\tilde{m},B)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ the map $t\mapsto \sigma\big((m,A),(\tilde{m},B),t\big)$ is a geodesic in the global NPC space, as defined in \citep[Definition 2.1]{Sturm_2003}, $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$.  Thus, $\sigma$ is a \textit{geodesic bicombing} in the sense of \citep[page 1]{basso2018fixed}.  Since 
% \[
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
%     =
%         \sigma\big(
%             (m,A),(\tilde{m},B),1/2
%         \big)
% \]
% then \citep[Theorem 3.4]{basso2018fixed} applies; whence $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is barycentric with $1$-Lipschitz barycenter map explicitly given therein.  

% Since is a barycentric QAS space then, \citep[Setting 3.6]{kratsios2023transfer} (iii) is satisfied.
% \end{proof}

% Having established the barycentricity and the QAS space structure of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F},\eta,\mathcal{Q}_{\cdot})$, we are now ready to prove the following result.
% \anastasis{Here in transcription}
% \begin{lemma}
% \label{lem:approximation_Sym}
% Fix an activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition}.
% For every $K\subset C([0:T],\mathbb{R}^d)$ satisfying Assumption~\ref{ass:reg_compact}, each $0<\delta,\alpha\le 1$, $0 \le L$, and every $(L,\alpha)$-H\"{o}lder%%
% \footnote{That is, $f$ is $\alpha$ H\"{o}lder with optimal H\"{o}lder coefficient $L$.} %%
% function $f:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ there is a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ satisfying
% \begin{equation}
% \label{lem:approximation_Sym__approximation}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x_{\cdot}),f(x_{\cdot})) < \delta
% \end{equation}
% with representation
% \begin{equation}
% \label{lem:approximation_Sym__approximation___representation}
%         \hat{t}(x_{\cdot}) 
%     % = 
%     %     \hat{\eta}(\hat{f}\circ \phi(x_{\cdot}),Z_n)
%     =
%         \sum_{i=1}^M\,
%                 P_{\Delta_M}(\hat{f}\circ \operatorname{attn}_T(x_{\cdot}))_i
%                 \cdot
%                 (m^{(i)},(A^{(i)})^{\top}A^{(i)})
% ,
% \end{equation}
% where $M\in \mathbb{N}_+$, $m^{(1)},\dots,m^{(M)}\in \mathbb{R}^d$, $A^{(1)},\dots,A^{(M)}\in \mathbb{R}^{d\times d}$, $P_{\Delta_M}:\mathbb{R}^M\rightarrow\Delta_M$ is the Euclidean (orthogonal) projection onto the $M$-simplex, and an MLP $\hat{f}:\mathbb{R}^N\rightarrow \mathbb{R}^M$ with activation function $\sigma$.  The depth, width, encoding dimension (N), and decoding dimension (M) are recorded in Table~\ref{tab:approximationrates}.
% % and 
% % \[
% % \begin{aligned}
% %         N
% %     =
% %         \mathcal{N}_{\operatorname{pack}}(K,C_{D_K}\operatorname{Vol}(M,g)^{1/D_K})
% % \mbox{ and }
% %         M
% %     \in
% %         \mathcal{O}\Big(
% %             \varepsilon^{-1}\,L
% %         \Big)
% % \end{aligned}
% % \]
% % where $\mathcal{N}_{\operatorname{pack}}(A,\delta)$ is the $\delta$-packing number of a compact subset $A$ of $C([0:T],\|\cdot\|_T)$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:approximation_Sym}.}}
%     \label{tab:approximationrates}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:approximation_Sym}}]
% \anastasis{Relabel $N$ (index) as $M$}
% \hfill\\
% We work in the notation of \citep[Theorem 3.7]{kratsios2023transfer}, or rather, its quantitative version \citep[Lemma 5.10]{kratsios2023transfer}.  
% We will apply \citep[Theorem 3.7]{kratsios2023transfer}, which requires us to verify each of the conditions of \citep[Setting 3.6]{kratsios2023transfer}.

% \paragraph{Step 1 - Implementing a Bi-Lipschitz Feature Map with the Attention Layer}
% \hfill\\
% \textbf{Remark:} \textit{We first show that the conditions of {\citep[Setting 3.6 (i)]{kratsios2023transfer}} are met, by verifying that the parameters of the attention layer~\eqref{eq:featuremap} can be chosen such that $\operatorname{attn}_T$ is a suitable feature map}.
% \hfill\\
% \begin{comment}
% \paragraph{Case (i) - The Continuous and Injective Case} 
% \anastasis{come back to this shortly...}
% \paragraph{Case (ii) - The Bi-Lipschitz Case} 
% \noindent 
% \end{comment}
% Let $N$ denote the $C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(\mathcal{M},d_g)$.  Since $(K,\|\cdot\|_T)$ and $(\mathcal{M},d_g)$ are isometric, then $N$ is the $C_{D_K} \operatorname{Vol}(M,g)^{1/D_K}$-packing number of $(K,\|\cdot\|_T)$.  
% By Lemma~\ref{lem:Good_Feature_Map}, there are matrices $A,B$, $a$, and $b$ with $\|A\|_0=2N=\|B_0\|$, $\|a\|_0=1$, and $\|b\|_0=0$ such that $\varphi\eqdef \operatorname{attn}_T$, as defined in~\eqref{lem:Good_Feature_Map}, is a bi-Lipschitz embedding of $(K,\|\cdot\|_{T})$ to $(\mathbb{R}^N,\|\cdot\|_2)$.  Set $\{(K,\varphi)\}$, let $\nu$ denote the normalized (uniform) Volume probability measure on $(\mathcal{M},g)$, and let $\mu\eqdef \varphi_{\#}\nu$ be its pushforward to $(K,\|\cdot\|_T)$.  Since every bi-Lipschitz map is a quasi-symmetry\footnote{See \citep[page 78]{Heinonen_2001_BookAnalMetSpace}.}, as defined on \citep[page 78]{Heinonen_2001_BookAnalMetSpace}, then \citep[Theorem 12.1]{Heinonen_2001_BookAnalMetSpace} implies that $(M,d_g)$ is a doubling metric space, as defined on \citep[10.13; page 81]{Heinonen_2001_BookAnalMetSpace}.  Since $(\mathcal{M},d_g)$ and $(K,\|\cdot\|_T)$ since both are isometric then $(K,\|\cdot\|_T)$ is also a doubling metric space (see \citep[Lemma 9.6 (v)]{RobinsonDimEmbAt_2011Book}).  This verifies \citep[Setting 3.6 (i)]{kratsios2023transfer}.




% \paragraph{Step 2 - Feature Space Geometry}\hfill\\
% Since the codomain of $\phi$ is simply a Euclidean space, then the constant sequence of identity maps $\{T^i\eqdef 1_{\mathbb{R}^N}\}_{i=1}^{\infty}$ are trivially finite-rank linear operators realizing the bounded approximation property on any compact subset of $\mathbb{R}^N$.  That is, for each non-empty compact $A\subseteq\mathbb{R}^N$, 
% \[
%     \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-T^i(u)\|_2 = \lim\limits_{i\mapsto \infty}\,\max_{u\in A}\,\|u-1_{\mathbb{R}^N}(u)\|_2 = 0
% \]
% and the operator norm $\|1_{\mathbb{R}^N}\|_{op}$ of $1_{\mathbb{R}^N}$, thus of $T^i$ for every $i\in \mathbb{N}_+$, is uniformly bounded above by $1$.  
% Therefore, \citep[Setting 3.6 (ii)]{kratsios2023transfer} is holds.

% \paragraph{Step 3 - Geometry of $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$}
% \hfill\\
% By Lemma~\ref{lem:QAS_Space_Sym0d} shows that $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},\mathcal{Q},\eta)$ is barycentric and a QAS space with quantized mixing function, see \citep[page 7]{kratsios2023transfer}, given for any $N\in\mathbb{N}_+$, $u\in \mathbb{R}^N$, and $(m^{(1)},A^{(1)}),\dots,(m^{(N)},A^{(N)})\in \mathbb{R}^d\times \mathbb{R}^{d^2}$ by
% \begin{equation}
% \label{eq:QMF}
%     \hat{\eta}\big(
%             w
%         ,
%             \{(m^{(n)},A^{(n)}\}_{n=1}^N
%     \big)
%         \eqdef 
%             \sum_{n=1}^N\,
%                 P_{\Delta_N}(w_n)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% .
% \end{equation}
% This verifies \citep[Setting 3.6 (iii)]{kratsios2023transfer}.


% \paragraph{Step 4 - Determining The Euclidean Universal Approximator}
% \hfill\\
% \textbf{Remark:} \textit{We now verify that the class of all MLPs with activation function $\sigma$ satisfying Assumption~\ref{ass:KLCondition} satisfies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.  The case where $\sigma=\operatorname{ReLU}$ and $\sigma\neq \operatorname{ReLU}$ are treated separately.}\\
% First, consider the case where $\sigma\neq \operatorname{ReLU}$.
% Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:GeneralSigma_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le d+D+3
% .
% \end{equation}
% Since $\sigma$ was assumed to satisfy Assumption~\ref{ass:KLCondition} then, \citep[Theorem 9]{kratsios2022universal}, as formulated in \citep[Proposition 53]{kratsios2022universal}, implies that $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is recorded in \citep[Proposition 53]{kratsios2022universal}.  Therefore, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:GeneralSigma_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% Next, suppose that $\sigma=\operatorname{ReLU}$.  Then, for each $d,D,c\in \mathbb{N}_+$ let $\mathcal{F}_{d,D,c}$ denote the family of maps $f:\mathbb{R}^d\rightarrow \mathbb{R}^D$ with representation~\eqref{eq:MLP} and satisfying
% \begin{equation}
% \label{eq:ReLU_Version}
%         J \le c
%     \mbox{ and }
%         \max_{j=0,\dots,J}\,
%             d_{j} 
%         \le c
% .
% \end{equation}
% By \citep[Theorem 1.1]{pmlr-v125-kidger20a}, $\mathcal{F}_{\cdot}$ is a universal approximator in the sense of \citep[Definition 2.11]{kratsios2023transfer}.  Moreover, its rate function is given in \citep[Theorem 1]{galimberti2022designing}, as recorded in \citep[Table 1]{galimberti2022designing}.  In either case, $\mathcal{F}_{\cdot}$, as defined in~\eqref{eq:ReLU_Version}, verifies \citep[Setting 3.6 (iv)]{kratsios2023transfer}.

% \paragraph{Step 5 - Applying~{\citep[Theorem 3.7]{kratsios2023transfer}}}
% Steps $1$ though $5$ verify that the conditions of Theorem~\citep[Theorem 3.7]{kratsios2023transfer} are indeed met.  Furthermore, we have just shown that we are in the special case where the Feature Decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$, as defined in \citep[Definition 3.4]{kratsios2023transfer}, is a singleton.  
% Therefore, Theorem~\citep[Theorem 3.7]{kratsios2023transfer} implies, thus for every $\varepsilon>0$ there is a map $\hat{t}:K\rightarrow \mathbb{R}^d\times \operatorname{Sym}_{0,d}$ with representation%%
% \footnote{Since the barycentric decomposition $\{(K,\varphi)\}$ of $(K,\|\cdot\|_T,\mu)$ has exactly one part then the partition of unity \citep[Setting 3.7]{kratsios2023transfer} is trivial and $\psi_1(x_{\cdot})=1$ for each $x_{\cdot}\in K$.}%%
% \begin{align}
% \label{eq:transformer_pre_mapped_BEGIN}
%         \hat{t}(x_{\cdot})
%     = &
%         \beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}
%         \big(
%             \delta_{\hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)}
%         \big)
%     \\
% \label{eq:transformer_barycentercancellation}
%     = & 
%         \hat{\eta}(P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot}),(Z_n)_{n=1}^N)
%     \\
% \label{eq:transformer_pre_mapped_END}
%         = & 
%             \sum_{n=1}^N
%             \,
%                 \big(
%                     P_{\Delta_N}\circ \hat{f}_n\circ \phi(x_{\cdot})
%                 \big)
%                 \cdot
%                 (m^{(n)},(A^{(n)})^{\top}A^{(n)})
% \end{align}
% for each $x_{\cdot}\in K$ satisfying 
% \[
%     \sup_{x_{\cdot}\in K}\,
%         d_{2,F}\big(
%             \hat{t}(x_{\cdot})
%         ,
%             f(x_{\cdot})
%         \big)
%     <
%         \varepsilon_A + \varepsilon_Q + \varepsilon_E = \varepsilon
% ,
% \]
% where $\varepsilon_E=0$ and $\varepsilon_A\eqdef \varepsilon_Q\eqdef \varepsilon/2$ and where $\hat{f}\in \mathcal{F}_{d_n,N_n,c_n}$, $Z_n\in \mathbb{R}^{N_n\times D_n}$, for some positive integers $d_n,c_n,D_n$, and $N_1,\dots,N_N\in \mathbb{N}_+$ recorded in \citep[Table 3]{kratsios2023transfer}, and $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a $1$-Lipschitz barycenter map on $(\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ (which exists by Lemma~\ref{lem:QAS_Space_Sym0d}).  We observe that that~\eqref{eq:transformer_barycentercancellation} follows from the fact that the barycenter map $\beta_{\mathbb{R}^d\times \operatorname{Sym}_{0,d}}$ is a right-inverse of the map $\mathbb{R}^d\times \operatorname{Sym}_{0,d}\ni (m,B)\mapsto \delta_{(m,B)}\in \mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$, where $\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d})$ denotes the $1$-Wasserstein space on $(\mathcal{P}_1(\mathbb{R}^d\times \operatorname{Sym}_{0,d}),d_{2,F})$ and~\eqref{eq:transformer_pre_mapped_END} follows from the expression for $\hat{\eta}$ given in~\eqref{eq:QMF}.  Consequentially,~\eqref{eq:transformer_pre_mapped_BEGIN}-~\ref{eq:transformer_pre_mapped_END} reduces to~\eqref{lem:approximation_Sym__approximation___representation}.  


% \paragraph{Step 6 - Tallying Parameters}
% Since the quantitative version of \citep[Theorem 3.7]{kratsios2023transfer} held, namely \citep[Lemma 5.10]{kratsios2023transfer}, then we obtain the following parameter estimates
% \begin{enumerate}
%     \item $N=\mathcal{N}_{\operatorname{pack}}\big(K,C_{D_K}\,\operatorname{Vol}(M,g)^{1/D_K}\big) \in \mathcal{O}(1)$,
%     \item $c$ is recorded in Table~\ref{tab:approximationrates} as the depth of the network $\hat{f}$,
%     \item The expression of $N$ is recorded, in detail, atop \citep[page 46]{kratsios2023transfer} and is
%     \[
%             N
%         \le 
%             \big(
%                 C_{K,1}^{\lceil \frac1{4\alpha}\rceil}
%             \big)^{
%                 \log_2(\operatorname{diam}(K)) - \frac1{\alpha}\log_2(\epsilon_A/(2L C_{K:2}))
%             }
%         \in 
%         \mathcal{O}_{K}\big(
%             L/\varepsilon
%         \big)
%         .
%     \]
%     for constants $C_{K,1},C_{K,2},C_K>0$ depending only on the compact set $K$ and on the mixing function $\eta$, $\alpha=1$ as $f$ is $1$-H\"{o}lder, and where $\mathcal{O}$ suppresses a constant depending only on $K$ and on the mixing function $\eta$ in~\eqref{eq:MixingFunction}.
% \end{enumerate}
% \end{proof}

% \subsection{Proof of the Main Approximation Lemma}
% \label{s:Proof__ss:Universality___sss:Theorem}
% In what follows, for any $d\in \mathbb{N}_+$, let $\overline{\mathcal{N}_d}$ denotes the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  

% The Lemmata in the previous sections together with the main results of \cite{kratsios2021universal} and \cite{kratsios2023transfer} to deduce our main approximation theoretic tool.  The proof method is summarized visually in Figure~\ref{fig:Approximation_Theorem}.


% \anastasis{t and t hat}
% \begin{figure}[H]
%     \centering
%     \begin{tikzcd}
%     \big(C([0:T],\mathbb{R}^d),\|\cdot\|_{\infty}\big) & (\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2) \\
%     (K,\|\cdot\|_{\infty}) 
%     \arrow[hookrightarrow]{u}{\iota} 
%     \arrow{r}{f} 
%     % \arrow[swap]{d}{\varphi} 
%     \arrow{dr}{\varrho\circ f}
%     & ({\mathcal{N}}_d,\mathcal{W}_2) 
%     \arrow[hookrightarrow]{u}{i}
%     \arrow{d}{\varrho} \\%
%     % (\mathbb{R}^F,\|\cdot\|) 
%     % \arrow{r}{\bar{f}}
%     & (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
%     \end{tikzcd}
%     \caption{Summary of Proof Strategy for Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd} \anastasis{details}.}
%     \label{fig:Approximation_Theorem}
% \end{figure}

% \begin{lemma}
% \label{lem:Universal_Approximation_Theorem__PathToNd}
% Let $d\in \mathbb{N}_+$, $L>0$, and $K\subset C([0:T],\mathbb{R}^d)$ be non-empty and regular compact set in the topology of uniform convergence.  For every $0<\varepsilon< 1/2$ and every $L$-Lipschitz function $f:(K,\|\cdot\|_{\infty})\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ there exists a map $\hat{t}:C([0,T],\|\cdot\|_T)\rightarrow (\mathcal{N}_d,\mathcal{W}_2)$ with representation 
% \[
%         \hat{t}(x)
%     \eqdef
%         \mathcal{N}_d\Biggl(
%                 \sum_{n=1}^N\,
%                     P_{\Delta_q}(\mathcal{NN}(x))_n
%                     \cdot
%                     m^{(n)}
%             ,
%                 \sum_{n=1}^N\,
%                     P_{\Delta_q}(\mathcal{NN}(x))_n
%                     \cdot
%                     (A^{(n)})^{\top}A^{(n)})
%         \Biggr)
% \]
% \anastasis{Update representation/simplify ofc + explain notation} 
% such that
% \[
%     \max_{u\in K}\,
%         \mathcal{W}_p\big(
%                 f(x)
%             ,
%                 \hat{t}(x)
%         \big)
%     < 
%         \varepsilon
%     ,
% \]
% for every $1\le p\le 2$.  Furthermore, the depth, width, encoding dimension $(N)$ and Decoding dimension $(M)$ are all recorded in Table~\ref{tab:approximationrates__nonFlatVersion} depending on the the choice of activation function $\sigma$.
% \end{lemma}

% \begin{table}[!ht]
%     \centering
%     \caption{{Complexity Estimates for transformer-type model $\hat{t}$ in Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd}.}}
%     \label{tab:approximationrates__nonFlatVersion}
%     \begin{tabular}{lllll}
%     \toprule
%         $\sigma$ Regularity & Depth & Width & Encode (N) & Decode (M)\\
%     \midrule
%         $\operatorname{ReLU}$ & 
%         $
%             \mathcal{O}\big(
%                 (LV( L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & 
%         $
%             \mathcal{O}\big(
%                 (LV(L))^{-m}\,\varepsilon^{-m}
%             \big)
%         $
%         & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%         \\
%         Smooth $\&$ Non-poly.
%          & 
%          $
%          %%% GENERAL FORM
%         %  \mathcal{O}\left(
%         % \frac{
%         %     m (2\operatorname{diam}(K))^{2p} 
%         %     }{
%         %     \left(C_0\omega^{-1} \left(
%         %         f 
%         % , \frac{C \, \epsilon}{(1+\frac{p}{4})m} \right)\right)^{2p} }
%         % \right)
%          %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\left(
%             L^{4m+1}\, \varepsilon^{-4m-1}
%         \right)
%          $
%          &
%          $ m + N +2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          Poly. $\&$ Non-affine
%          & 
%          $
%         %%% GENERAL FORM
%     %      \mathcal{O}\left(
%     % \frac{
%     %     m(m+p)(2\operatorname{diam}(K))^{4p+2}
%     %     }{
%     %     \left(C_0\,\omega^{-1} \left(
%     %     f 
%     %     , \frac{C\,\epsilon}{(1+\frac{p}{4})m} \right)\right)^{4p+2}
%     %     }
%     %     \right)
%         %%% Simplified FORM for Lipschitz Maps
%         \mathcal{O}\big(
%             L^{8m+6}\, \varepsilon^{-8m-6}
%         \big)
%          $
%          & 
%          $m+N+3$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%          $C(\rr)$ $\&$ Non-poly.
%             &
%          % $
%          %%% GENERAL FORM (Too Complicated IMo)
%     %     \mathcal{O}\left( 
%     % \frac{
%     %     m (2\operatorname{diam}(K))^{2p}
%     % }{
%     %     C_0^{2p}\,\omega^{-1}\left(
%     %         f 
%     %             , 
%     %         \frac{C\,\epsilon}{2m(1+\frac{p}{4})}    
%     %     \right)^{2p} 
%     %     \left(C_0\,\omega^{-1} \left( \sigma, \frac{C\,\epsilon}{2Bm(2^{(2\operatorname{diam}(K))^{2}[C_0\,\omega^{-1}(
%     %     f 
%     %     , \frac{C\,\epsilon}{2m(1+\frac{p}{4})})]^{-2}+1} -1)} \right) \right)
%     % }
%     %     \right)
%          % $
%         %%% Readable Form
%         Finite
%         &
%         $m+N+2$
%          & $\mathcal{O}(1)$ & $\mathcal{O}\big(L\varepsilon^{-1}\big)$
%          \\
%     \bottomrule
%     \end{tabular}
%     \caption*{Where $V(t)$ is the inverse of $s\mapsto s^4\,\log_3(t+2)$ on $[0,\infty)$ evaluated at $131 t$.}
%     % Where $C,C_0>0$ are constant depending only on the modulus of continuity $\omega$ of the target function $f^{\star}$ and on the compact set $K$.
% \end{table}

% \begin{proof}[{Proof of Lemma~\ref{lem:Universal_Approximation_Theorem__PathToNd}}]
% \hfill\\
% \textbf{Step 1 - Bounded The Local Lipschitz Stability of $\rho$ on $f(K)$}
% By Lemma~\ref{lem:LipschitzManifold_Nd} the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is continuous.  By definition of the product topology, see \citep[page 114]{MunkresTopology_2000}, the projection map $\pi:(\mathbb{R}^d,\operatorname{Sym}_{0,d},d_{2,F})\ni (\mu,\Sigma)\rightarrow \Sigma \in (\operatorname{Sym}_{0,d},\|\cdot\|_F)$ is continuous.  
% Since the composition of continuous functions is again continuous then the map
% \[
%     g: (K,\|\cdot\|_T)\ni x \mapsto 
%     \pi\circ \varrho\circ f(x)
%     \in (\mathbb{R},|\cdot|)
% \]
% is continuous.  By \citep[Theorem 26.5]{MunkresTopology_2000}, $\tilde{K}\eqdef g(K)$ is a compact subset of $(\mathbb{R},|\cdot|)$.  


% By \citep[Theorem 9.2.6 - page 130]{LaxBookLinearAlgebra_2007} the map $\lambda_{\text{min}}:(\operatorname{Sym}_{0,d},\|\cdot\|_F)\rightarrow (\mathbb{R},|\cdot|)$ which sends any $d\times d$ square matrix $\Sigma$ to its minimal eigenvalue $\lambda_{\text{min}}(\Sigma)$ is continuous.  Since every continuous function with compact domain is achieves its minimum on its domain then, there exists some $\Sigma_0\in \tilde{K}$ minimizing $\lambda_{\text{min}}$; i.e.
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved}
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% Since $f$ takes values in $\mathcal{N}_d$ then $\pi\circ \varrho(f(x))$ is positive definite, for each $x\in K$.  In particular, $\lambda_{\text{min}}(\Sigma_0)>0$.  Consequentially,~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalueachieved} implies that
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___minimaleigenvalue}
%         0
%     <
%         r
%     \eqdef 
%         \lambda_{\text{min}}(\Sigma_0)
%     =
%         \min_{\Sigma\in g(K)}\,\lambda_{\text{min}}(\Sigma)
%     <
%         \infty
% .
% \end{equation}
% \anastasis{Add reference to Lemma~\ref{lem:LoewnerBound} here.}
% Consequentially, Lemma~\ref{lem:LipschitzManifold_Nd} implies that the map $\varrho:(\mathcal{N}_d,\mathcal{W}_2)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ is Lipschitz on $\tilde{K}$ with Lipschitz constant bounded-above by $\operatorname{Lip}\big(\varrho|f(K)\big)$.  Consequentially, we have that
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}
%         \operatorname{Lip}\big(\varrho\circ f | K\big)
%     \le 
%         \operatorname{Lip}\big(\varrho|f(K)\big)
%         \,
%         \operatorname{Lip}\big(f|K\big)
%     \le 
%         \max\big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\big\}
%         \,
%         L
% .
% \end{equation}
% \hfill\\
% \textbf{Step 2 - Approximating $\varrho \circ f$ on $K$}
% \hfill\\
% Fix $\varepsilon>0$ and fix the ``perturbed approximation error''
% \begin{equation}
% \label{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}
%         \delta
%     \eqdef 
%         \min\biggl\{
%                 1
%             ,
%                 \frac{\varepsilon
%                 }{
%                 \sqrt{d}2\sqrt{
%                     L
%                     \,\operatorname{diam}(K) + 1
%                 }
%                 }
%         \biggr\}
% .
% \end{equation}
% We many now apply Lemma~\ref{lem:approximation_Sym} to deduce that there exists a map $\hat{t}:(K,\|\cdot\|_T)\rightarrow (\mathbb{R}^d\times \operatorname{Sym}_{0,d},d_{2,F})$ with representation~\eqref{lem:approximation_Sym__approximation___representation} satisfying the uniform estimate\begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate}
%     \max_{x\in K}\,
%         d_{2,F}(\hat{t}(x),\varrho\circ f(x))
%     <
%         \delta
% .
% \end{equation}
% Since Lemma~\ref{lem:LipschitzManifold_Nd} showed that $\varrho$ has a locally bi-Lipschitz homeomorphism then, in particular, $\varrho^{-1}$ exists and it is Lipschitz continuous.  Set $t\eqdef \varrho^{-1}\circ \hat{t}$ and 
% denote the $1$-thickening of $\varrho\circ f(K)$ by 
% \[
%         \bar{B}_1
%     \eqdef 
%         \{(m,\Sigma)\in \mathbb{R}^d\times \operatorname{Sym}_{0,d}:\,(\exists x\in K)\, d_{2,F}(f(x),(m,\Sigma))\le 1\}
% .
% \]
% Since $\delta$ was defined, in~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta}, to be at-most $1$, then~\eqref{eq:prop:Universal_Approximation_Theorem__VALUEOFDelta} implies that 
% \begin{equation}
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___CONTAINEMENTAPPROXIMATION}
%     \hat{t}(K)\subseteq \bar{B}_1
%     .
% \end{equation}
% From~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate} and Lemma~\ref{lem:LipschitzManifold_Nd} we deduce the uniform estimate
% \allowdisplaybreaks
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% = & 
%     \max_{x\in K}\,
%         \mathcal{W}_2\big(
%                 \varrho^{-1}\circ \hat{t}(x)
%             ,
%                 \varrho^{-1}\circ \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \max_{x\in K}\,
%         d_{2,F}\big(
%                 \hat{t}(x)
%             ,
%                 \varrho\circ f(x)
%         \big)
% \\
% \nonumber
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1}
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \delta
% \\
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_A}
% \le &
%     \operatorname{Lip}\big(
%             \varrho^{-1} 
%         |
%             \bar{B}_1
%     \big)
%     \,
%     \frac{\varepsilon
%     }{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \label{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_B}
% \le &
%     \sqrt{d}2\sqrt{
%             L
%             \,\operatorname{diam}(K) + 1
%         }
%     \,
%     \varepsilon
%     \,
%     \frac1{
%     \sqrt{d}2\sqrt{
%         L
%         \,\operatorname{diam}(K) + 1
%     }
%     }
% \\
% \nonumber
% \label{eq:Approxim_LEMMA__END}
% = & 
%     \varepsilon
% ,
% \end{align}
% where~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_A} followed from Lemma~\ref{lem:LipschitzManifold_Nd} and the definition of $\bar{B}_1$ 
% and bound~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___BOUND_B} followed from the estimate~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___Lipschitzvarrho}.  Since $\mathcal{W}_p\le \mathcal{W}_2$ for all $1\le p\le 2$, see \citep[Remark 6.6]{VillaniBook_2009}, then estimates in~\eqref{eq:Approxim_LEMMA__BEGIN}-~\eqref{eq:Approxim_LEMMA__END} imply that
% \begin{align}
% \label{eq:Approxim_LEMMA__BEGIN}
%     \max_{x\in K}\,
%         \mathcal{W}_p\big(
%                 t(x)
%             ,
%                 f(x)
%         \big)
% \le & 
%     \varepsilon
% ,
% \end{align}
% \hfill\\
% for all $1\le p\le 2$; as claimed.  
% \textbf{Step 3 - Counting Parameters}
% Using $\delta$, as defined in~\eqref{eq:lem:Universal_Approximation_Theorem__PathToNd___uniformestimate}, in the place of $\varepsilon$ in Table~\ref{tab:approximationrates} and noting that $\delta^{-1} \in \mathcal{O}(\varepsilon^{-1})$ yields the conclusion.  
% \anastasis{Add computations tomorrow}
% \end{proof}



% \begin{comment}
%     \subsubsection{Polish QAS Space Structure on $d$-dimensional Gaussian Measures - OLD Construction}
%     \label{s:Proof__ss:Universality___sss:Outputs_OLD}
%     \anastasis{package this nicely...}\hfill\\
%     Let $\overline{\mathcal{N}_d}$ denote the set of Gaussian measure on $\mathbb{R}^d$ equipped with the $2$-Wasserstein metric $\mathcal{W}_2$.  
%     We now show that $\overline{\mathcal{N}_d}$ is a QAS space and we exhibit one such QAS structure; in the sense of \citep[Definition 3.4]{Acciaio2022_GHT}.  
%     \anastasis{Show that $\overline{\mathcal{N}_d}$ can be identified with \textit{all} $d$-dimensional Guassian measures (using geodesic completeness)...}
%     \begin{lemma}
%     \label{lem:QAS_Nd}
%     $(\overline{\mathcal{N}_d},\mathcal{W}_2,\hat{\eta})$ is a barycenteric, Polish QAS space with quantized mixing function $\hat{\eta}:\cup_{N=1}^{\infty}\, [\Delta_N\times \mathbb{R}^{d(d+3)/2}]\rightarrow \overline{\mathcal{N}_d}$ defined for every $N\in \mathbb{N}_+$, each $w\in \Delta_N$, and every $(m_1,A_1)$, $\dots$, $(m_N,A_N)$ we have
%     \[
%             \hat{\eta}(w,(m_n,A_n)_{n=1}^N)
%         \eqdef 
%             \eta\big(w,
%                 \mathcal{N}(m_n,\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n))
%             \big)
%         .
%     \]
%     Moreover, \anastasis{details...}
%     \end{lemma}
%     \begin{proof}[{Proof of Lemma~\ref{lem:QAS_Nd}}]
%     \anastasis{polish details}\hfill\\
%     For every $q\in \mathbb{N}_+$, define the map $\mathcal{Q}_q:\mathbb{R}^{d(d+3)/2}\rightarrow \overline{\mathcal{N}_d}$ sending any $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}\cong \mathbb{R}^{d(d+3)/2}$ to the measure
%     \begin{equation}
%     \label{eq:quantization}
%             \mathcal{Q}(m,A)
%         \eqdef 
%             \mathcal{N}(m,\operatorname{sym}(A)^{\top}\operatorname{sym}(A))
%     .
%     \end{equation}
%     Note that, $\mathcal{Q}_1=\mathcal{Q}_q$ for every $q\in \mathbb{N}_+$.  Furthermore, if $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ then $\Sigma$ is symmetric and positive semi-definite.  Thus, \anastasis{citation} there is some symmetric matrix $B$ such that $\Sigma=B^2$; where $B^2\eqdef B^{\top}B$.  Since $\operatorname{sym}$ is a linear isometry between the Euclidean spaces $(\mathbb{R}^{d(d-1)/2},\|\cdot\|_2)$ and the Hilbert space of $d\times d$ symmetric matrices with Frobenius inner product \anastasis{citation} then, for every $\mathcal{N}(m,\Sigma)\in \overline{\mathcal{N}_d}$ there exists some $(m,A)\in \mathbb{R}^d\times \mathbb{R}^{d(d+1)/2}$ such that 
%     \[
%             \mathcal{Q}(m,A) 
%         = 
%             \mathcal{N}(m,\Sigma)
%         .
%     \]
%     Therefore, for any compact subset $K\subset \overline{\mathcal{N}_d}$ and any $\varepsilon>0$ the \textit{modulus of quantizability}, denoted by $q_{K,\varepsilon}$ and defined in \citep[Definition 3.3]{Acciaio2022_GHT}, is identically $d(d+3)/2$.  In particular, $\overline{\mathcal{N}_d}$ is \textit{quantizable} by the ``constant quantization'' $\mathcal{Q}_{\cdot}\eqdef \{\mathcal{Q}_q\}_{q=1}^{\infty}$.  
    
    
%     Let us now show that $\overline{\mathcal{N}_d}$ is \textit{approximately simplicial}; in the sense of \citep[Definition 3.1]{Acciaio2022_GHT}.
%     For any $N\in \mathbb{N}_+$, denote the $N$-simplex by $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n=1\}$.
%     Define the map $\eta:\cup_{N=1}^{\infty}\,[\Delta_N\times \mathcal{P}_2(\mathbb{R}^d)]\rightarrow\mathcal{P}_2(\mathbb{R}^d)$ as follows: for any $N\in \mathbb{N}_+$ and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ we define $\Delta_N\ni w\mapsto 
%     \eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ as a measurable selection of the set of optimizers of
%     \[
%         V(w) \eqdef \inf_{\nu \in \mathcal{P}_2(\mathbb{R}^d)}\,
%             \sum_{n=1}^N\, w_n \mathcal{W}_2\big(\nu,\mathcal{N}(m_n,\Sigma_n)\big)^2
%     .
%     \]
%     As shown \citep[Example 5.6]{Acciaio2022_GHT}, such an $\eta$ is well-defined as satisfies \citep[Definition 3.1]{Acciaio2022_GHT}.  Therefore, $\big(\overline{\mathcal{N}_d},\mathcal{W}_2,\eta,\mathcal{Q}_{\cdot}\big)$ is a QAS space.  Moreover, since $\overline{\mathcal{N}_d}$ is, by definition, a closed subset of $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ and $(\mathcal{P}_2(\mathbb{R}^d),\mathcal{W}_2)$ is a Polish space, by \citep[Theorem 6.18]{VillaniBook_2009}, since $\mathbb{R}^d$ is Polish; then, $\overline{\mathcal{N}_d}$ is a Polish space.
    
%     Furthermore, by \citep[Theorem 2.4]{AlvarezEstebanDelBarrioCusestaAlbertosMatran_WBartycenters_JMAA_2016} if $N\in \mathbb{N}_+$, $w\in \Delta_N$, and $\mathcal{N}(m_1,\Sigma_1)$, $\dots$, $\mathcal{N}(m_N,\Sigma_N)$ are such that $\Sigma_1$, $\dots$, $\Sigma_N$ are all non-singular then $\eta \big(
%                 w
%                 ,
%                 (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%             \big)
%     $ is uniquely determined by
%     \begin{equation}
%     \label{eq:simplified_quantization}
%     \eta \big(
%             w
%             ,
%             (\mathcal{N}(m_n,\Sigma_n))_{n=1}^N
%         \big)
%         =
%         \mathcal{N}\Biggl(
%                 \sum_{n=1}^N\,w_n\,m_n
%             ,
%                 S_w
%         \Biggr)
%     \end{equation}
%     where $S_w$ is the \textit{unique} solution to the matrix equation $S =\sum_{n=1}^N\, w_n\, (S^{1/2}\Sigma_nS^{1/2})^{1/2}$.
    
%     Thus, $\hat{\eta}$ is a quantized mixing map $\hat{\eta}$.  Moreover, the expression for $\eta$ can be simplified using~\eqref{eq:simplified_quantization}, in the obvious way, when $\operatorname{sym}(A_n)^{\top}\operatorname{sym}(A_n)$ is positive-definite for $n=1,\dots,N$.\anastasis{details}
    
%     \anastasis{I wonder if I can leverage quantization to ensure this nice expression always holds by adding $1/q\cdot I_d$ at quantization level $\mathcal{Q}_q$...then the uniform quantization rate (modulus oQ) must be verified and is not fully trivial.}
%     \end{proof}
% \end{comment}



% \appendix
% \section{Auxiliary Lemmata}
% \label{s:AuxLemmata}
% This section records auxiliary lemmata used in our proofs but proven elsewhere.
% \begin{lemma}[\cite{LocalLipschitz_Pinelis}]
% \label{lem:LipschitzManifold_Nd}
% Fix $d\in \mathbb{N}_+$ and $R,r>0$.  For every every $m^{(1)},m^{(2)}\in \mathbb{R}^d$ and each $d\times d$ symmetric positive semi-definite matrix $A,B$ satisfying: $\|A\|_F,\|B\|_F\le R$ and $A-r\cdot I_d$ and $B-r\cdot I_d$ are positive semi-definite%%
% \footnote{%%
%     I.e. $A,B\ge r\cdot I_d$ where $\ge $ is the partial ordering on the set of $d\times d$-dimensional symmetric positive-definite matrices given by $A\ge B$ if and only if $A-B$ is positive semi-definite.
% } %% 
% it holds that
% \[
% \begin{aligned}
%     % Lipschitz Inverse 
%             \frac1{
%                 \min\{1,\sqrt{d}(2\sqrt{R})\}
%             }
%             \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
%         \le &
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%     \\
%             \mathcal{W}_2\big(
%                 \mathcal{N}(m^{(1)},A)
%             ,
%                 \mathcal{N}(m^{(2)},B)
%             \big)
%         \le &
%             \max\Big\{1,\frac{\sqrt{d}}{2\sqrt{r}}\Big\}
%                 \,
%             \sqrt{\|m^{(1)}-m^{(2)}\|^2+\|A-B\|_F^2}
% .
% \end{aligned}
% \]
% In particular, the map $\varrho:(\overline{\mathcal{N}}_d,\mathcal{W}_2)
% \rightarrow
% (\mathbb{R}^d\times \operatorname{Sym}_{0,d},\|\cdot\|\times \|\cdot\|_F)
% $ is locally-Lipschitz; where $\|\cdot\|\times \|\cdot\|_F$ denotes the product of the Euclidean norm on $\mathbb{R}^d$ and the Fr\"{o}benius norm on the space of $d\times d$-dimensional symmetric positive semi-definite matrices $\operatorname{Sym}_{0,d}$.
% \end{lemma}
% \begin{proof}[{Proof of Lemma~\ref{lem:LipschitzManifold_Nd}}]
% The proof is due to Iosif Pinelis, and is given in \cite{LocalLipschitz_Pinelis}.  We only note that, $\|\cdot\|_{\lambda:2}\le \|\cdot\|_F\le \sqrt{d}\|\cdot\|_{\lambda:2}$ where $\|A\|_{\lambda:2}\eqdef \sqrt{\max_{i=1,\dots,d}\,\lambda_{\text{max}}(C^{\top}C})$ denotes the spectral norm on the set of $d\times d$ matrices and where $\lambda_{\text{max}}(C^{\top}C)$ denotes the largest eigenvalue $C^{\top}C$ for a given $d\times d$ matrix $C$. 
% \end{proof}

% \section{Background: Riemannian Geometry and Algebraic Topology}
% \label{s:Background_Geo}



% \bibliographystyle{abbrvnat}
% \bibliography{Bookkeaping/2_References}


% \newpage
% \section{Algorithms}
% \input{Sections/Practical_Approach}

% \end{document}


==> OLD/Old_notes.tex <==
\newpage
\newpage
\anastasis{Please ignore this bit for now friends :)}
Let $X_{\cdot}\eqdef (X_t)_{t=0}^{\infty}$ be a discrete-time stochastic process defined on a filtered probability space $(\Omega,\mathcal{F},\mathbb{F}\eqdef (\mathcal{F}_t)_{t=0}^{\infty},\mathbb{P})$ taking values in $\mathbb{R}^d$.  Suppose that for $\P$-a.s.\ each $x_{\cdot}\in (\mathbb{R}^d)^{\mathbb{N}}$ the conditional law
\[
        \mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \eqdef 
        \mathbb{P}(X_{t+1}\in \cdot \vert x_{[0:t]})
    ,
\]
is absolutely continuous with respect to the $d$-dimensional Lebesgue measure and has finite moments.  This happens, for example in continuous time, for SDEs with sufficiently smooth drift and diffusion coefficients \cite{aida1993support,kusuoka2010existence,de2011smoothness}, possibly with jumps \cite{cass2009smooth}, driven by Gaussian processes with continuous paths of $p$-variations \cite{baudoin2014upper} such as fractional Brownian motions with Hurst parameter even in $[1/4,1/2]$ \cite{inahama2022positivity}, or even certain strong solutions to SDEs with H\"{o}lder drift \cite{olivera2019density}.  The discrete-time analogues of these results are immediately obtained by discretizing time
\anastasis{Provide a concrete example of a non-Markovian ``discrete-time" SDE.}


The conditional law of such a general process $X_{\cdot}$ can be a complicated high-dimensional object, which can make approximation of it computationally much more challenging \cite{kratsios2021universal} compared to approximation of functions in Euclidean spaces \cite{...} or smooth Riemannian manifolds \cite{kratsios2022universal}.  Since we will be interested in computationally tractable estimates of the conditional law of $X_{\cdot}$, then the starting point for our analysis is a low-dimensional non-degenerate Gaussian surrogate for $\mathcal{L}(X_{t+1} |x_{[0:t]})$ which preserves the maximum information possible of $\mathcal{L}(X_{t+1} |x_{[0:t]})$.

One possible surrogate function is formalized using the \textit{information projection}, or \textit{$I$-projection}.  More specifically, under the aforementioned conditions, \citep[Theorem 1]{CsiszarInfoProjRevisited2003IEEE} guarantees that there exists a unique Gaussian measure with non-singular covariance, which we denote by $\mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]})$, which best represents the conditional law $\mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]})$ 
\anastasis{Relate to dimension-reduction/regularization and capacity control :)}
\[
\operatorname{KL}\biggl(
        \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})
        ,
        \mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \biggr)
    =
    \min_{\mathbb{Q}}\,
    \operatorname{KL}\big(
    \mathbb{Q},\mathcal{L}(X_{t+1}\vert x_{[0:t]})
    \big)
\]
where the minimum is taken over a suitable space of probability measures $\mathcal{Q}$ to be described below.

\subsection{Case 1 - $\mathcal{Q}$}
Suppose that $\mathcal{Q}\subseteq \mathcal{P}_1(\mathbb{R}^d)$ consists of all Gaussian measures on $\mathbb{R}^d$ with covariance of the form $\otimes_{i=1}^d\, \sigma_i$ for some $\sigma_1,\dots,\sigma_d>0$.
% That is, is the \textit{information projection} of the conditional law $\mathcal{L}(X_{t+1}\vert x_{[0:t]})$ onto the space $\otimes_{i=1}^d\,\mathcal{N}_1$ of $d$-dimensional Gaussian measures with non-singular diagonal covariance matrices; denoted by $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$.  
% \cite{Takatsu2011}
The measures in $\mathcal{Q}$ can be parameterized bijectively and continuously by
\[
\begin{aligned}
\psi:\mathbb{R}^{2d}& \rightarrow \otimes_{i=1}^d\,\mathcal{N}_1
\\
(\mu,\varsigma)& \mapsto \mathcal{N}_d\left(\mu,
\begin{pmatrix}
e^{\varsigma_1} & 0 & \dots & 0 \\
0 & e^{\varsigma_2} & \dots & 0 \\
0 & 0& \ddots & 0 \\
0 & 0& \dots & e^{\varsigma_d}
\end{pmatrix}
\right)
.
\end{aligned}
\]
If we were to fix a time $t\in \mathbb{N}_+$, a feature map $\varphi:\mathbb{R}^{t(d+1)}\rightarrow \mathbb{R}^F$, and consider the hypothesis class $\mathcal{F}$ of \textit{non-Euclidean kernel learners} $f_{\theta}:\mathbb{R}^{t(d+1)}\rightarrow \otimes_{i=1}^d\,\mathcal{N}_1$
\[
    \hat{f}_{\theta_{\cdot}}(x_{[0:t]})
    \eqdef 
    \psi\big(
        \theta_t^{\top}
        \varphi(x_{[0:t]})
    \big)
,
\]
where $\theta$ belongs to the parameter space $\Theta\eqdef \mathbb{R}^{d\times F}$ of $d\times F$-dimensional real-matrices.  \anastasis{Given examples of such $\varphi$, e.g.\ random NNs and discuss their properties$\dots$}.  
Then, given a set of i.i.d.\ sample paths $\{x^{(n)}_{[0:t]}\}_{n=1}^N$ from the process $X_{\cdot}$ up to time $t$, for some positive integer $N$, we can train the non-Euclidean kernel regressor to approximate the function $\mathcal{L}(X_{t+1} \vert x_{[0:t]})$ by optimizing the empirical risk functional
\begin{equation}
\tag{Static}
\label{eq:static_objective}
\min_{\theta}\,
    \frac1{N}\sum_{n=1}^N\,
        \mathcal{W}_2^2\big(
            \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}^{(n)})
            ,
            f_{\theta}(x_{[0:t]}^{(n)})
        \big)
,
\end{equation}
associated to the $2$-Wasserstein distance on $\mathcal{P}_2(\mathbb{R}^d)$. 

We are interested in optimizing the dynamic version of~\eqref{eq:static_objective} where our learners are of the form 
\[
\{f_{\theta_{\cdot}} :\, \theta_{\cdot}\in (\mathbb{R}^F)^{\mathbb{N}}\}
\]
and each $\hat{f}_{\theta_{\cdot}}$ is as above.  Our goal is to optimize the following regret functional
\begin{equation}
\tag{Regret}
\label{eq:dynamic_objective}
        \mathcal{R}(\theta_{[0:T]})
    \eqdef 
        \frac1{T N}\,
            \sum_{t=0}^{T-1}\,
                % \frac1{N}
                \sum_{n=1}^N\,
                \big(
                        \mathcal{W}_2^2\big(
                            \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}^{(n)})
                            ,
                            f_{\theta}(x_{[0:t]}^{(n)})
                        \big)
                +
                    \lambda\|\Delta_t\theta_t\|_2^2
            \big)
,
\end{equation}
where $\lambda>0$ is a regularizing hyperparameter and the minimization is performed $\mathcal{F}_T$ by optimizing over the set of controls in~\eqref{eq:control}.  Using coincidence results with the Wasserstein-$2$ distance, we can show that the regret functional~\eqref{eq:dynamic_objective} can be rewritten as
\begin{equation}
\label{eq:dynamic_objective__simplified}
        \mathcal{R}(\theta_{[0:T]})
    \eqdef 
        \frac1{T N}\,
            \sum_{t=0}^{T-1}\,
                % \frac1{N}
                \sum_{n=1}^N\,
                \Big(
                        \big(
                                \|\mathbb{E}(X_{t+1} \vert x_{[0:t]}^{(n)}) - \mu(\theta_t)\|_2^2
                            +
                                \|
                                    (\sqrt{\exp(\varsigma_i)}
                                    -
                                    \sqrt{\sigma_i})_{i=1}^d
                                \|_2^2
                        \big)
                +
                    \lambda\|\Delta_t\theta_t\|_2^2
            \Big)
,
\end{equation}

% \anastasis{%if we solve this, then perhaps we can extend to the mean-field N-player version where each player controls a mixture component...  Show that
% I will show this:
% \[
%         \mathcal{W}_2^2\big(
%             \mathcal{L}_{\pi}(X_{t+1} \vert x_{[0:t]}^{(n)})
%             ,
%             f_{\theta}(x_{[0:t]}^{(n)})
%         \big)
%     =
%         \|\mathbb{E}(X_{t+1} \vert x_{[0:t]}^{(n)}) - \mu(\theta_t)\|_2^2
%         +
%         \|
%             (\sqrt{\exp(\varsigma_i)}
%             -
%             \sqrt{\sigma_i})_{i=1}^d
%         \|_2^2
% \]
% explain the notation later...\hfill\\
% @Xuwei, Note that this is now a linear-quadratic problem.  We can possibly optimize the weights like last time also.
% \hfill\\
% @Xuwei I wonder if we can introduce symmetry into the problem and view this as several agents controlling $\theta_{\cdot}$ then use our decentralization technique.
% \hfill\\
% @AK: I wonder if we can use a VMP-type estimate here to reduce the complexity of computing the OC, up to some error ofc.
% }

% \anastasis{Possibly extend to fancier exponential families later.}

% \anastasis{I'd suggest replacing the class of general controls in~\eqref{eq:control} with a class which is ``designed to look forward''; namely,
% \[
% \theta_t = f(\theta_{t-1},\nabla_{\theta} R(\theta_{t-1})
% \]
% We can use \citep[Theorem 3.18]{KrieglMichor_ConvenientBook_1997_AMS} to get a critical point of the regret functional $\mathcal{R}$:
% \begin{enumerate}
%     \item First compute the Gateau derivative of the regret functional (see \citep[Theorems 5 and 6]{pmlr-v134-casgrain21a}),
%     \item Then input the derivative of f into the chain-rule
%     \item Solve.
% \end{enumerate}
% }


% \subsection{Case 2 - $\mathcal{Q}$ Maximum Entropy Family}
% Let $\mathcal{Q}$

% Since $\otimes_{i=1}^d\mathcal{N}_1$ is an exponential family, then \citep[Theorem 1]{CsiszarInfoProjRevisited2003IEEE} guarantees that $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ exists. for each $x_{[0:t]}\in \mathbb{R}^{(1+t)d}$.  Since any such $\nu\eqdef \mathcal{N}(\mu,\otimes_{i=1}^d\,\sigma_i)$ is characterized by the moment constraints
% \[
% \mathbb{E}_{X\sim \nu}[X_i] = \mu_i \mbox{ and } \mathbb{E}_{X\sim \nu}[(X_i)^2] = \mu_i^2 + \sigma_i,
% \]
% for $i=1,\dots,d$, then \citep[Theorem 3.1]{csiszar1975divergence} implies that $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ is of the form
% \begin{equation}
% \label{eq:IprojForm}
% \mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]}) 
% \propto
% \exp\Big(\sum_{i=1}^d\,\beta_i\,u_i + \beta_{d+i}\,u_i^2\Big)
% d\lambda(u),
% \end{equation}
% where $\lambda$ is the $d$-dimensional Lebesgue measure, $\beta\in \mathbb{R}^{2d}$, and $\propto$ hides the unique constant ensuring that the measure on the right-hand side of~\eqref{eq:IprojForm} integrates to $1$.  Whence, $\mathcal{L}_{\pi}(X_{t+1}\vert x_{[0:t]})$ belongs to $\otimes_{i=1}^d\,\mathcal{N}_1$. \anastasis{redundant.}

==> OLD/Working_Introduction/Intro.tex <==
\begin{abstract}
% GPT
% Inspired by the Kalman filter, Deep Kalman Filters (DKFs) have lacked strong theoretical ties to the stochastic filtering problem, limiting their trustworthy applicability, in areas where traditional stochastic filtering has been applied mathematical finance. We present a class of continuous-time DKFs designed to approximate the conditional law of various non-Markovian, conditionally Gaussian signal processes using noisy measurements. Our approach quantifies approximation quality through worst-case 2-Wasserstein distance, computed uniformly computed over regular compact path spaces. Unlike other infinite-dimensional deep learning models, our DKF adapts to path space geometry and does not require a Schauder basis, enhancing its versatility for filtering tasks.
% ME - 1
% Deep Kalman filters (DKFs) are neural network models that generate Gaussian input probability measures.  However, beyond their inspiration from the Kalman filter, there are still weak theoretical ties between DKFs and the stochastic filtering problem where one tries best to reconstruct a partially observed signal from noisy measurements.  Nevertheless, without stronger clear ties to the filtering problem, the use of DKFs to numerically solve problems where stochastic filtering has traditionally deployed, e.g.\ XXX finance, is questionable.   We address this issue by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  Unlike other deep learning models defined on infinite-dimensional spaces, our DKF does not rely on a Schauder basis for the path space.  Rather, it adapts to the geometry of the compact set of paths on which it approximates the optimal filter.  
% Me -2 
Deep Kalman filters (DKFs) are a class of neural network models that generate Gaussian probability measures from sequential data.  Though DKFs are inspired by the Kalman filter, they lack concrete theoretical ties to the stochastic filtering problem, thus limiting their applicability to areas where traditional model-based filters have been used, e.g.\ model calibration for bond and option prices in mathematical finance.  We address this issue in the mathematical foundations of deep learning by exhibiting a class of continuous-time DKFs which can approximately implement the conditional law of a broad class of non-Markovian and conditionally Gaussian signal processes given noisy continuous-times measurements.  Our approximation results hold uniformly over sufficiently regular compact subsets of paths, where the approximation error is quantified by the worst-case 2-Wasserstein distance computed uniformly over the given compact set of paths.  
% Unlike most deep learning models defined on the infinite-dimensional domains, our DKF does not rely on a particular Schauder basis, and instead, it adapts to the geometry of a given path space.  
\end{abstract}


\section{Introduction}
\label{s:Algorithm}
%\fbox{\begin{minipage}{0.8\textwidth}
%    \textbf{Structure of introduction.}
%    \begin{enumerate}
%        \item Opening
%        \item What are Kalman filters and what are traditional use cases of Kalman filters in finance (and beyond)
%        \item What are Deep Kalman Filters (when/how) and why did they become popular and what (were) limitations of Kalman Filters that can be resolved by Deep Kalman Filters?
%        \item What is the main result in this paper and why is it useful? Universality: Limitations of existing results and extensions.
%        \item This is what we don't do (re: training) but "this is why it is ok"...
%        \item Structure of the article.
%    \end{enumerate}
%\end{minipage}
%}
%\bigskip

\byyan{Opening.}\hfill\\
In several scientific problems, especially in mathematical finance, one is typically interested in predicting an unobservable \textit{signal} process $X_{\cdot}$ given the information available in noisy \textit{observations} $Y_{\cdot}$; both of which have continuous paths and are defined on a filtered probability space $(\Omega,\mathcal{F},(\mathcal{F}_t)_{t\in [0,T]},\mathbb{P})$.  For example, market sentiment impacts market prices, however, only the latter of these two can be reliably measured.  
% Filtering
% Consequentially, an accurate estimation of the unobservable signal process implies reliable forecasts of all affected quantities.  The objective of the \textit{stochastic filtering problem}, is to recursively estimate the conditional law of the unobserved signal process $X_{\cdot}$, at any time given $t>0$, given the information contained in the $\sigma$-algebra generated by the observation process $Y_{\cdot}$ up to time $t$.
% Robust Filtering
The objective of the \textit{robust stochastic filtering problem}, studied by \cite{clark1978design,Kushner_1979_RobustDiscreteSTate,Davis_1980MultiplicativeFunctionalNonLinearFiltering,DavisFiltering,clark2005robust,CrisanDielhFrizOberhauser_2013_AAP}, is for any time $t>0$ to identify a continuous function $f_t:C([0,t],\mathbb{R}^d)\rightarrow \mathcal{P}(\mathbb{R}^D)$ satisfying 
\begin{align}
    \label{goal:Robust_Filtering}
        f_t(y_{[0:t]})
    =
        \mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)%y_{[0:t]})
    ,
\end{align}
conditioned on any continuous path $y_{[0:t]}$ realized the $d$-dimensional observable process $Y_{\cdot}$ up time $t>0$; where $\mathbb{P}(X_t\in \cdot|\mathcal{F}_t^Y)$ is the conditional law of the $D$-dimensional signal process $X_t$ given the $\sigma$-algebra generated by $(Y_s)_{s\in [0,t]}$.  The continuity of $f_t$ is qualified by equipping the set of Borel probability measures on $\mathbb{R}^D$, denoted by $\mathcal{P}(\mathbb{R}^D)$, with the weak topology and by equipping the set of continuous paths from $[0:t]$ to $\mathbb{R}^d$, denoted by $C([0,t],\mathbb{R}^d)$, with the uniform norm. 

\byyan{Applications of Robust Filtering in Finance (high-level).}\hfill\\
When one has access to a \textit{robust representation}~\eqref{goal:Robust_Filtering}, then they can reliably predict the conditional law of $X_t$ even subject to imperfections on the observed historical data in $y_{[0:t]}\in C([0:t],\mathbb{R}^d)$.  These robust representations are particularly 
% day2016deep,mishev2020evaluation
% Filtering problems, integral to the realm of stochastic systems, involve the challenging task of estimating the state of a dynamic system from observations contaminated by noise. These problems find widespread applications in diverse domains such as finance, control systems, and environmental monitoring, where accurate state estimation is paramount. At the heart of the filtering paradigm lies the concept of filter distribution—the conditional distribution describing the state of a stochastic system conditional on the noisy observations up to a given time. In this work, we demonstrate that in the case of a continuous-time conditionally Gaussian filter, this filtering distribution can be approximated universally by a transformer-like machine learning model uniformly in time.
% \medskip
% \byyan{Kalman filters.} \hfill\\
% The simplest form of a conditionally Gaussian filter is the well-known Kalman-Bucy filter, which is the case when the underlying system follows linear dynamics, observations are linear, and noise terms are Gaussian. Rudolf Kalman's work introduced the discrete-time Kalman filter \cite{Kalman60}, which later found a continuous-time counterpart in \cite{KalmanBucy61}. These filters provide finite-dimensional representations of the filter distribution, summarizing the first two conditional moments of the system's state based on observations. In the linear Gaussian scenario, the filter distribution is fully characterized by these first two moments, specifically, the mean vector and variance-covariance matrix of the resulting Gaussian distribution. The Kalman filter's elegance and utility have made it a staple in various fields, particularly when dealing with linear dynamics and Gaussian noise assumptions.
% Stochastic filters have proven to be 
invaluable in mathematical finance where continuous streams of data are often noisy.  More broadly, stochastic filters are indispensable in situations where latent parameters influence or obscure market factors.  Applications include the computation of optimal investment under partial information \cite{lakner1998optimal, BjorkDavis}, the estimation of volatility from observed intra-day stock prices \cite{Barndorff-NielsenShephard02}, estimation of interest rates \cite{chen1993maximum,duan1999estimating,BabbsNowman99,JavaheriLautierGalli03}, estimation of spot price estimation for commodity futures \cite{schwartz1997stochastic,schwartz2000short,ManoliuTompaidis02,LautierGalli04,Cody2007parameter}, hedging of credit derivatives \cite{frey2010pricing,FreySchmidt_2012_PricingHedging}, estimation of equilibria under asymmetric information \cite{ccetin2018financial}, and calibration of option pricing models \cite{LindstroemStroejbyBrodenWiktorssonHolst08,LindstroemWiktorsson14}.  Pathwise, or so-called robust, formulations were later derived in \cite{clark2005robust,crisan2013robust}.  Indeed, the abilities of stochastic filters to estimate unobservable variables, track market dynamics, and improve the precision of financial models have made them a staple tool in the quantitative finance toolbox, with several books treating the role of stochastic filtering in finance \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear,remillard2013statistical}.  

\byyan{Do Optimal Filters Exist?.}\hfill\\
In its general form, the stochastic filtering problem is a well-understood mathematical problem.   Many of the fundamental questions in stochastic filtering, such as existence and dynamics for the evolution of the conditional law of signal process $X_t$ given the realizations of the measurement process $Y_{\cdot}$, were solved in a series of papers \cite{stratonovich1959optimum,stratonovich1960application,Sirjaev1965Filtering,zakai1969optimal,Sirjaev1965Filtering,Sirjaev_1978Filtering}.  Nevertheless, the infinite-dimensionality of general stochastic filters, being measure-valued processes, make the problem computationally intractable.  

\byyan{Computational Challenges}\hfill\\
The exception to this rule is so-called finite-dimensional filters, which are rare situations in which the dynamics of $X_{\cdot}$ and $Y_{\cdot}$ give way to optimal filters that are finitely parameterized.  Examples include the \textit{Kalman-Bucy filters} \cite{Kalman60,KalmanBucy61} where closed-forms are derived under the assumption of Markovian Gaussian noise and affine OU-type dynamics of $X_{\cdot}$ and $Y_{\cdot}$, the \cite{wonham1964some} filter where all involved quantitative are finite-state Markov processes, and the Be\v{n}es filter \cite{benevs1970existence} which relies a particular set of one-dimensional dynamics.

\byyan{Numerical Approaches.}\hfill\\
The intractability of the computational general filtering problem has the use of approximately optimal filters.  These approaches include particle filters which aim at dynamically approximating optimal filters using an evolving interacting particle system \cite{del1997nonlinear,djuric2003particle,DelMoralBook_2013}, linear relaxations of the optimal filtering functional for affine processes which can be numerically computed by solving specific stochastic Riccati equations \cite{LukasJosef_LinearizedFiltering}, or by projection of the optimal filter onto finite-dimensional manifolds of exponential families \cite{brigo1998differential,brigo1999approximate,armstrong2023optimal} when it admits a square-integrable density.  The latter two instances work well if the coupled system $(X_{\cdot},Y_{\cdot})$ genuinely follows the postulated dynamics, and the former particle-filtering approach is effective for low-dimensional state space systems.  

\byyan{Why Deep Learning?.}\hfill\\
The ability of deep neural networks to efficiently solve a variety of problems has inspired the use of deep learning approaches to the numerical stochastic filtering problem; e.g.~\cite{Balint_FinalPaper_2023,Ariel_2023Filtering}, and example of deep neural network approximations to measure-valued processes; e.g.~\cite{Acciaio2022_GHT}.  In particular, the need for a more generic approximate stochastic filtering toolbox has motivated the deep learning community to introduce deep Kalman filters (DKFs) \cite{KrishnanShalitSontag15}, which is the primary object of study in this paper.  Broadly speaking, a DKF is a deep neural network model which maps historical data to Gaussian measures.  Though these deep learning-powered model, are inspired by Kalman filters, there is still little connection between them and the stochastic filtering problem.  

This paper confirms the ability of deep Kalman filters to map $f_t$ in the robust representation~\eqref{goal:Robust_Filtering} for any pair of $\mathbb{F}\eqdef (\mathcal{F}_s)_{s\in [0,T]}$-adapted processes governed by the coupled dynamics
\begin{align}
\label{eq:filtering_dynamics__signal}
% \tag{Sig}
dX_t & = [a_0(t,Y_{[0:t]}) + a_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, b_i(t,Y_{[0:t]})dW^{(i)}_t \\
\label{eq:filtering_dynamics__observation}
% \tag{Obs}
dY_t & = [A_0(t,Y_{[0:t]}) + A_1(t,Y_{[0:t]}) X_t]dt + \sum_{i=1}^2\, B_i(t,Y_{[0:t]})dW^{(i)}_t
\end{align}
where $a_0$ and $A_0$ respectively take values in $\mathbb{R}^{d_X}$ and $\mathbb{R}^{d_Y}$, and where $a_1,A_1,b_1,b_2,B_1,B_2$ are matrix-valued of respective dimensions $d_X\times d_X$, $d_Y\times d_X$, $d_X\times d_X$, $d_X\times d_Y$, $d_Y\times d_X$, and $d_Y\times d_Y$, and the entries of $a_0, a_1, b_0, b_1, A_0, A_1, B_0, B_1$ are measurable nonanticipative functionals on the measurable space $([0:T] \times C([0:T], \R^{d_Y}), \cB_{[0:T]} \times \cB_T^{d_Y})$, and where $\cB_t^d  \eqdef  \sigma(C([0: t], \R^d))$ denotes the $\sigma$-algebra generated by continuous paths on $[0: t]$ to $\R^d$.   
We will always assume that the filtration $\mathbb{F}$ is right-continuous and that the probability space $(\Omega,\mathcal{F},\mathbb{F},\mathbb{P})$ supports independent $\mathbb{F}$-adapted Brownian motions, $W^{(1)}_{\cdot}\eqdef (W_t^{(1)})_{0\le t\le T}$ and $W^{(2)}_{\cdot}\eqdef (W^{(2)}_t)_{0\le t\le T}$, of respective dimensions $d_X$ and $d_X$, for positive integers $d_X$ and $d_Y$.  


% HERE!

% \begin{enumerate}
%     \item Optimal investment under partial information \cite{lakner1998optimal,BjorkDavis}
%     \item \textit{Volatility Estimation from Intra-day Stock Prices.}
%    \cite{Barndorff-NielsenShephard02} introduced the use of Kalman filters to estimate underlying volatility from observed intra-day stock prices. Volatility estimation is crucial in risk management, options pricing, and trading strategy development. By incorporating high-frequency price data into the Kalman filter framework, this approach provides more accurate and timely volatility estimates, enhancing decision-making in financial markets.
%    \item \textit{Fixed Income and Interest Rate Estimation Modeling} 
%    \cite{chen1993maximum,duan1999estimating}
%    \textit{Instantaneous Interest Rate Estimation from Bond Yields.}
%    Further research, including \cite{BabbsNowman99}, have applied Kalman filters to estimate underlying instantaneous interest rates, also known as short rates, from observed bond yields. This estimation is fundamental in fixed income markets, aiding in bond pricing, yield curve modelling, and interest rate risk analysis. The Kalman filter's ability to handle noisy and irregularly sampled bond yield data makes it an ideal choice for this application.
%    \item \textit{Spot Price Estimation from Futures Prices for Commodities.} Approaches as for instance \cite{Schwartz97}, \cite{ManoliuTompaidis02}, and \cite{LautierGalli04} employ Kalman filters to tackle this problem. By modelling the relationship between spot and futures prices, Kalman filters provide a dynamic framework for spot price estimation, allowing market participants to make informed decisions.
%    \item \textit{Estimation of Latent Factors Affecting Pricing.}
%    Kalman filters are also utilized to estimate latent factors that influence asset pricing, e.g.\ in commodity market model \cite{schwartz1997stochastic,schwartz2000short,Cody2007parameter}, energy future pricing \cite{manoliu2002energy}, and . These factors could include macroeconomic variables, market sentiment, or other unobservable drivers. By integrating observed asset prices and a dynamic state-space model, researchers can extract these latent factors, enhancing our understanding of market dynamics and improving pricing models.
%    \item \textit{Updating Estimates of Uncertain Drift Parameters.}
%    In the context of hedging strategies in incomplete markets, as explored by \cite{Monoyios07}, Kalman filters are employed to update estimates of uncertain drift parameters in the price process. This adaptation allows market participants to dynamically manage risk by adjusting their hedging positions as market conditions evolve.
%    \item Books \cite{harvey1990forecasting,wells1995kalman,bhar2010stochastic,date2011linear}
% \end{enumerate}


% In these financial applications, the Kalman filter's adaptability to handle noisy, irregular, and dynamic data has proven to be a significant advantage. Its ability to estimate unobservable variables, track market dynamics, and improve the precision of financial models has made it a staple tool in quantitative finance. However, it's important to acknowledge that the financial markets often present challenges that extend beyond the simplistic filtering dynamics of the Kalman-Bucy filter.

\byyan{Applications outside of Finance (high-level).}
The Kalman filter's versatility and effectiveness in dealing with linear dynamics and Gaussian noise assumptions have also led to its widespread use across various fields outside of finance: In aerospace and navigation, it plays a pivotal role in spacecraft navigation and autonomous vehicle positioning, providing accurate state estimates despite inherent uncertainties. In geophysics and seismology, it contributes to ground motion and structural response monitoring during seismic events, enhancing early warning systems and structural health assessments. Control engineering relies on the Kalman filter for state estimation in feedback control systems, benefiting industries such as manufacturing, robotics, and aerospace, where precise control is essential. In the realm of medical imaging, it improves image quality by reducing noise, leading to advancements in disease diagnosis and treatment planning. Environmental monitoring applications leverage the Kalman filter to estimate and predict environmental parameters, including pollutant concentrations, weather conditions, and ocean currents, supporting climate studies and disaster management. Additionally, robotics equipped with sensors use the Kalman filter to estimate their positions and orientations in unfamiliar environments.

\medskip
\byyan{More complex conditionally Gaussian filters.}
Many real-world situations deviate from these idealized assumptions, featuring nonlinear or non-Markovian dynamics. In such cases, the simplicity of the Bucy-Kalman filter may not suffice, prompting the need for more sophisticated filtering methods.

\yannick{Generalizations include
\begin{itemize}
    \item Non-linear, non-Markovian signal dynamics
    \item Non-linear, non-Markovian dependence of hidden state on signal dynamics
    \item Opening the door for learning procedures, where dynamics are (mostly model-freely) learned from data
\end{itemize}
}
    


\paragraph{The main result in this paper}

\paragraph{Structure of the article}

~\\ 
\bigskip

Literature surrounding applications of filtering in Mathematical Finance: \\
For a general motivation for the geometric (also: information geometric) idea behind Filtering problems in typical applications in mathematical finance, see the excellent overview presented in the the recent work \href{https://arxiv.org/pdf/2205.01594.pdf}{Brigo (2022)} and the expose in \href{https://arxiv.org/pdf/1303.6236.pdf}{Armstrong and Brigo (2013)} as well as well-known early works \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}. A gentle introduction to typical linear and nonlinear filtering problems in mathamatical finance can be found in the review article \href{ura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{Date and Ponomareva (2010)} and for a comprehensive introduction to stochastic filtering we direct to the eteemed monograph \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)} as the reference literature.\\


\anastasis{I would mention that there are at-least two sources of ``complexity'' to the general filtering problem: 1) The infinite-dimensionality of the set of all probability measures (complexity of representing conditional densities/measures) and 2) The complexity of the dynamics governing the solution of the signal, observation, and conditional dynamics.  \\
I would then say some like Kalman filters simplify both, the general conditional Gaussian filters studied in \cite{LipShiryaev_II_2001} provide a theoretical foundations for filtering when (1) is resolved by considering conditionally Gaussian filters.  Then somehow relate that we work in (1), by developing a universal model class, in the conditionally-Gaussian framework based on the ideas of deep Kalman filtering.}

\paragraph{Historical development:} 
The filtering problem consists in estimating the state of a stochastic differential system
from noisy observations. \\ 
The general solution of the filtering problem at a given time is given by the probability density
of the unperturbed state of the system at that time, conditional on the perturbed observations
up to the given time. When the unobserved signal and the observed signal evolve in continuous
time, the filter density follows a stochastic partial differential equation (SPDE), see \href{https://link.springer.com/book/10.1007/978-0-387-76896-0}{Bain and Crisan (2009)}. 
If the dynamic evolution of the unobserved
system is linear, the observations are linear, the noise terms are Gaussian\footnote{The initial condition of the
unperturbed signal are also assumed to be Gaussian or deterministic.}, then this is a setting that leads to the celebrated \emph{Kalman-Bucy filter}:
\\
Indeed, in the linear Gaussian case the problem was solved in discrete-time by Rudolf Kalman, and later in continuous time in \cite{TBD}\anastasis{(Bucy Paper)},
who introduced what is known today as the \emph{Kalman filter} (see next paragraph), a finite dimensional system of equations
for the first two conditional moments of the state of the stochastic system, given the observations:
In such a case, the filter is Gaussian and its density can
be characterized by a finite dimensional set of parameters, namely the mean vector and variance-covariance matrix of the resulting Gaussian distribution,
%\\In classical Kalman Filters, the evolution of this system (both observable and unobservable parts) are modelled as linear functions
%perturbed by Gaussian noise.
%In a linear setting 
these equations determine the whole conditional density of the state of the system given the observations,
as this (Gaussian) density is fully characterized by the first two moments. \\
 For real world applications the assumption of a linear evolution of this system\footnote{I.e. transition and emission distributions.}
limits the capacity to model complex phenomena, and modifications to the functional form of Kalman Filters
have been proposed.
\\
As indicated above, 
in the  general nonlinear case, the filtering problem is far more complex as it consists in computing the conditional density of the
state given the observations. This density is the solution of a stochastic partial differential
equation which is referred to as the \emph{Kushner-Stratonovich equation} and the resulting nonlinear filter is in general not finite dimensional\footnote{I.e. it does not evolve in a finite dimensional
statistical manifold.}. A well
known approximation method is the extended Kalman filter (EKF), in which one linearizes around
the current estimate obtaining a locally linear system, and then applies the Kalman filter
equations in this (linearised) neighbourhood. Traditionally, this procedure was usually justified by heuristic considerations.  
Though more recent linear approximations have also been considered, e.g.\ in \cite{LukasJosef_LinearizedFiltering}.
Another choice in the nonlinear case is the Gaussian assumed density filter (GADF),
obtained by assuming the conditional density to be Gaussian\footnote{This is dangerous, because by assuming a false hypothesis one can deduce anything as well as its opposite.}, which yields a finite dimensional filter. %However, this approach depends heavily on conditional Gaussianity, which is not necessarily fulfilled in many real-life applications.\\
We are universal in the conditional Gaussian class.\\
Contrast it with neural SDEs (no hidden suff (ANASTASISSSS)

Hanzon suggested to project the SPDE equation in Stratonovich form for the evolution of the filter density onto a finite dimensional statistical manifold, using the Fisher metric/Hellinger distance. We call this “Stratonovich projection” and it consists in projecting the separate vector
fields of the SPDE corresponding to the drift and diffusion part of the Stratonovich version. The projected equation would describe a finite dimensional density evolution, called projection filter, approximating the full filter evolution associated with the optimal filter.\\
In 1987, Hanzon (BH: reference missing) introduced the projection filter (PF), which is a finite dimensional nonlinear filter based on a differential geometric approach: The projection filter is obtained by projecting the Kushner-Stratonovich equation onto the tangent space
of a finite dimensional manifold of probability densities, according to the Fisher information metric.\\
Hanzon and Hut (1991) (BH: add ref) showed that if one projects onto the
tangent space of the finite dimensional manifold of Gaussian densities, the resulting projection filter
coincides with an assumed density filter which is obtained as follows: one computes the first two conditional moments equations in McShane-Fisk-Stratonovich (MFS) form, and then assumes the conditional density to be Gaussian, closing in this way the equations for the first two moments.   
It was also proven in Hanzon and Hut (1991) that what we described above is in general not the same as assuming a Gaussian density in the It\^{o} equations for the first two moments and then transforming the obtained filter in MFS form.
The equivalence between the MFS-based GADF and the Gaussian Projection Filter is very important when generalized to
exponential families (see \href{https://inria.hal.science/hal-02101519/document}{Brigo et al. (1998)}), because it gives a simple characterization of the exponential projection
filter (EPF) which is independent of geometric concepts. \\

For a comprehensive but introductory review of linear and non-linear filterin applications in mathematical finance see: \href{https://bura.brunel.ac.uk/bitstream/2438/8540/1/Fulltext.pdf}{P. Date and K. Ponomareva (2010)} among which we will highlight some simple but heavily used (Gaussian or near-Gaussian) use cases
\begin{itemize}
    \item In stochatic volatility modelling Kalman Filters have traditionally been used to estimate (and forecast) spot and realised volatility.
    \item Monoyios in \href{https://people.maths.ox.ac.uk/monoyios/docs/ima_final.pdf}{Monoyios (2007)} develops a filtering approach with applications to (optimal) hedging, in which the hedger updates her parameter estimates from
observations of the asset prices, and where he finds an analytic solution to the hedger’s combined filtering and
control problem in the case that the drift of the traded asset is known with certainty.
\item Filtering has been traditionally heavily used in linear Gaussian interest rate models. 
    \end{itemize}
    

\paragraph{Kalman filters} At a high level, a Kalman filter operates by combining a model of a system with partial state-observations to estimate the current overall state of the system. The filter uses two primary steps to make these estimates: a prediction step and an update step.
\begin{itemize}
    \item In the prediction step, the Kalman filter uses the model of the system to predict the state of the system at the next time step. This prediction is based on the current estimate of the system state, as well as any known inputs or disturbances in the system. The Kalman filter uses a probabilistic approach to estimate the state of the system, this means the prediction includes both the expected value of the state as well as an estimate of the uncertainty or error in the prediction.
    \item In the update step, the Kalman filter uses the actual observation to correct the predicted state estimate. The filter compares the distribution of the predicted state to the actual observed state (which acknowledges uncertainty and is perceived as a distribution itself). The filter then adjusts the state estimate based on this difference.
\end{itemize}

\paragraph{Deep Kalman filters} The term, ``deep Kalman filter'' (DKF) refers to deep learning models, that bolster the capacity of traditional Kalman filter by leveraging a neural network component. The neural network component is used to learn the probabilistic model of the underlying system dynamics, thus allowing DKFs to generically adapt to any situation in which the conditional evolution of the signal process is Gaussian.  This generic flexibility, of DKFs is what has lead to their empirical predictive edge over traditional Kalman filters \cite{TBD}.

The neural network component in a DKF is typically used to model the transition function of the system, which describes how the state of the system evolves over time. The neural network takes as input the current state of the system, as well as any control inputs or disturbances, and outputs a probability distribution over the possible next states of the system. This distribution is then used to make a prediction of the next state, as well as an estimate of the uncertainty or error in the prediction. 

The traditional Kalman filter components are then used to combine the neural network predictions with actual observations in order to update the state estimate. The neural network component in a DKF can be trained using a variety of techniques, such as maximum likelihood or Bayesian inference. The training process involves minimizing the error between the predicted state and the actual state, as well as minimizing the uncertainty in the predictions.

\paragraph{Exemplary (existing) applications of (D)KF in finance}
\begin{enumerate}
    \item Sequential calibration of options
    \begin{itemize}
        \item Problem: The parameter estimates are noisy and old data are typically discarded, as only the most recent data are used.
        \item As a solution, the calibration is formulated as a filtering problem.
        \item The observable process consists of market option prices, spot, strike, interest, and maturity.
        \item The unobservable process consists of the difference between the modelled option price and the denoted option price, as well as the difference of the model's parameters to the day before.
        \item See \cite{LindstroemStroejbyBrodenWiktorssonHolst08}, extensions \cite{LindstroemWiktorsson14}
    \end{itemize}
    \item Computing VaR in a stochastic volatility model, see \cite{LindstroemMadsenNielsen16}
    \item Filtering with bond prices, see \cite{LindstroemMadsenNielsen16}
    \begin{itemize}
        \item The observable process constitutes the prices obtained from solving the ``bond pricing equation''
        \item The unobservable variables are the parameters of the estimated model and the implied interest rate (by bond prices, not quoted)
    \end{itemize}
    \item Calibration of term structure models of commodity prices \cite{JavaheriLautierGalli03}
    \item Dynamic pricing (this is probably more economics than finance), see \cite{CohenTreetanthiploet22}
    \item Besides state estimation in control systems, Kalman filters have found applications in financial markets for constructing trading strategies. Two common approaches involve using Kalman filters to:
    \begin{itemize}
        \item Identify Mean-Reverting Patterns: Kalman filters can be utilized to detect instances where asset prices deviate from their long-term average, indicating potential mean-reverting behaviour. Traders can then develop strategies that take advantage of these deviations, expecting prices to eventually return to their mean.
        \item Identify Momentum-Based Trends: Kalman filters can also be employed to identify momentum-based trends in asset prices, indicating sustained movements in a particular direction. Traders can develop strategies to follow and capitalize on these trends.
        \item \yannick{References missing.}
    \end{itemize}
    \item Portfolio Optimization with Kalman Filters and Multi-Asset Models:
    \begin{itemize}
        \item Kalman filters applied to optimize asset portfolios by considering individual asset dynamics and correlations.
        \item Particularly beneficial for multi-asset portfolios.
        \item Estimation of assets' covariance matrix using Kalman filters.
        \item Portfolio optimization based on the covariance matrix while adhering to specified constraints.
        \item \yannick{References missing.}
    \end{itemize}
    \item  Risk Management and Stress Testing with Kalman Filters:
    \begin{itemize}
        \item Utilization of Kalman filters for risk management and stress testing purposes.
        \item Estimation of portfolio risk and identification of potential risk sources.
        \item Modelling asset behaviour under various market scenarios using Kalman filters.
        \item Assessment of the portfolio's vulnerability to the impact of these scenarios.
        \item \yannick{References missing.}
    \end{itemize}
\end{enumerate}


\begin{comment}
\paragraph{Limitations and contribution} The results \cite{kratsios2021universal, Acciaio2022_GHT} show that, while it is possible to universally approximate the function used above with a class of transformer models, the required number of parameters to approximate the function at each state in time can depend highly non-favourably on the dimensions of the (observable and unobservable) state. In this work, we suggest to best approximate the function at all times by a class of non-Euclidean kernel regressors, trained on a finite set of observations. 
\end{comment}
